Enhancing Interpretability and Generalizability in Extended Isolation Forests

Anomaly Detection (AD) focuses on identifying unusual behaviors in complex datasets. Machine Learning (ML) algorithms and Decision Support Systems (DSSs) provide effective solutions for AD, but detecting anomalies alone may not be enough, especially in engineering, where diagnostics and maintenance are crucial. Users need clear explanations to support root cause analysis and build trust in the model. The unsupervised nature of AD, however, makes interpretability a challenge. This paper introduces Extended Isolation Forest Feature Importance (ExIFFI), a method that explains predictions made by Extended Isolation Forest (EIF) models, which split data using hyperplanes. ExIFFI provides explanations at both global and local levels by leveraging feature importance. We also present an improved version, Enhanced Extended Isolation Forest (EIF+), designed to enhance the model's ability to detect unseen anomalies through a revised splitting strategy. Using five synthetic and eleven real-world datasets, we conduct a comparative analysis, evaluating unsupervised AD methods with the Average Precision metric. EIF+ consistently outperforms EIF across all datasets when trained without anomalies, demonstrating better generalization. To assess ExIFFI's interpretability, we introduce the Area Under the Curve of Feature Selection (AUC\_FS), a novel metric using feature selection as a proxy task. ExIFFI outperforms other unsupervised interpretability methods on 8 of 11 real-world datasets and successfully identifies anomalous features in synthetic datasets. When trained only on inliers, ExIFFI also outperforms competing models on real-world data and accurately detects anomalous features in synthetic datasets. We provide open-source code to encourage further research and reproducibility.

==> sections/Experimental_results_old.tex <==

\section{Evaluation of interpretation algorithms}\label{Evaluation}
%In this Section we will try to provide basis to affirm that our explanation algorithm works well \jacopo{non mi convince molto questa frase}, and it is a valid alternative to provide interpretations of the results made by the Extended Isolation Forest.\\
One significant challenge in the evaluation of ML interpretability approaches is that it is difficult to determine the quality of an explanation. Indeed, there is no objective metric for comparing the performance of different algorithms in terms of their ability to provide good explanations. Since the popular book written by Molnar \cite{molnar2020interpretable}, many papers tried to set up an objective theory on what is an explanation and how to evaluate it \cite{confalonieri2021historical, doshi2017towards, linardatos2020explainable, sejr2021explainable, zhou2021evaluating}. 
To evaluate the XAI algorithm, we first assess its effectiveness on synthetic benchmark datasets. Such datasets are designed to analyze if the algorithm is able to detect the dimensions along which the anomalies are distributed, both with Local and Global Feature Importance scores. We will then make experiments on "real datasets" where the distributions are not defined ad-hoc for our purposes.

As discussed in \cite{molnar2020interpretable}, assessing the effectiveness of XAI approaches in real world problems is not straightforward. One way to provide an evaluation is through a 'proxy task', i.e. a related problem which can be instead easily assessed in a quantitative way: we then exploit the evaluation on the proxy task as a surrogate for the evaluation of the original task, the XAI problem. As done in \cite{diffi} we will exploit feature selection as a proxy task: we will use the indication of \approach and competitor methods for guiding the feature selection, i.e. by keeping the $k$ features (for different values of $k$) that are globally considered as the most important by the XAI approach. While feature selection in anomaly detection is not the focus of this work, we will implicitly show the effectiveness of exploiting \approach also in this task.

Moreover, we will resort to an additional test for assessing the quality of the  \approach interpretation, which is a comparison with the interpretation provided by Random Forest (RF). RF is a popular supervised algorithm, which is also  an ensemble approach based on trees, with the main difference that in RF we are resorting to decision trees, not isolation trees as in the IF/EIF. RF is equipped with a procedure for providing feature rankings, that is widely used by the scientific community and by practitioners: we will compare the feature rankings provided by RF, when considering the AD problem as a binary classification one (with inliers and outliers being the two classes), with the ones provided by \approach. While the rankings provided by RF are not to be considered a ground truth and RF may not be effective with unbalanced classification problems, RF has the advantage of exploiting labels for both solving the classification and the XAI task: in light of this, we consider such test as a relevant one for the purpose of evaluation \approach capabilities.  
\todo[inline]{Non mi è chiara una cosa: qui si intended che RF è addestrato sulle label vere del dataset oppure che è un modello surrogato addestrato a riprodurre le predizioni del metodo di AD? il significato della feature importance di RF cambia parecchio nei due casi, \ale{addestrato sulle label vere}}

%the interpretation provided by a model similar to the unsupervised Isolation Forest, but that has access to the ground truth labels. The idea is to evaluate the interpretation made by the Isolation Forest using the interpretation provided by the Random Forest (RF), that has the adva
% which is a widely used supervised model that has a similar structure with respect to Isolation Forest. 
%The assumption is that the best possible interpretation an Isolation could give is the one made by the RF. 

%Usually a good way to evaluate an interpretation is establishing a proxy able to compare the results with other interpretation methods.  \ale{The term "proxy" typically refers to something that serves as a substitute or representation of something else. For example, proxy data or proxy variables are often used in research to represent or stand in for a concept or phenomenon that is difficult to directly measure or observe. In this context, a proxy is a surrogate or indirect measure of a particular concept or variable of interest.} \gian{Secondo me aiuta parlare di 'proxy task' anzichè di 'proxy'.} 
%\tom{\cite{molnar2020interpretable} parla di proxy task quando parla di evaluation of interpretability }
%\gian{contributo su feature selection}
%\aledel{With proxy we mean a variable that is not in itself directly relevant, but that serves in place of an immeasurable variable. In order for a variable to be a good proxy, it must have a close correlation with the variable of interest}.
%\todo[inline, color=purple]{Non sono sicura di aver capito bene la frase precedente. Si puà semplificare o esemplificare? }

% QUESTA REF NON MI PARE UTILE citare Proxy Tasks and Subjective Measures Can Be Misleading in
%Evaluating Explainable AI Systems %\cite{buccinca2020proxy}}


%\tom{Towards Quantification of Explainability in Explainable Artificial Intelligence Methods \cite{islam2020towards}}

 %the anomalies are specifically set up to evaluate the effectiveness of the algorithm.


\subsection{Synthetic datasets}
\input{sections/toy_examples}


\subsection{Real data examples}
\input{sections/real_datasets_results}


==> sections/Experimental_results_old_old.tex <==

\section{Experimental results}
In this section we will try to provide basis to affirm that our explanation algorithm works well, and it is a valid alternative to analyze the results made by the Extended Isolation Forest.\\
One of the biggest problem is that evaluating the goodness of an explanation is an opaque task because there is not an objective metric that can show if our algorithm is better or not than other algorithms.  \\
Since the book written by Molnar \cite{molnar2020interpretable} many papers tried to set up an objective theory on what is an explanation and how to evaluate it \cite{linardatos2020explainable}\cite{doshi2017towards}\cite{zhou2021evaluating}\cite{confalonieri2021historical}\cite{sejr2021explainable}. Usually a good way to evaluate an interpretation is establishing a proxy able to compare the results with other interpretation methods \ale{ci torneremo}. With proxy we mean a variable that is not in itself directly relevant, but that serves in place of an immeasurable variable. In order for a variable to be a good proxy, it must have a close correlation with the variable of interest. \boh{in our case the correlation is not quantifiable but it is a correlation of meanings.}



The experiments done to evaluate in which extent the Extended-DIFFI interpretation is a good explanation of the features are of two kind. 
\begin{itemize}
    \item {\bfseries Consistency}: Since the EIF model is a stochastic model it can provide slightly different results at each run of the algorithm. It is necessary that even if the trees are different, the knowledge of the feature acquired by the explanation remains consistent, it means the features that contains the most information on the outliers have to be more or less the same at each iteration. It is noticeable the correlation between the consistency of the importance of the features and the accuracy of the model, in fact if the model has a good precision it encodes well the outlier position, thus which are the feature that discriminate the most a sample as an outlier or not.
    \item {\bfseries Feature Selection}: In the anomaly detection task a feature can be considered more important than another one if it is able to discriminate better if a sample is an outlier or not. The feature selection is a good proxy to evaluate the goodness of the interpretation because by contracting the number of features, maintaining more and more the most important ones, it is expected that the precision of the model remains high instead of decreasing with the loss of information of the sample features.
\end{itemize}  
\subsection{Robustness and similarity with ACME and DIFFI}
Keeping the attention on the precision of the model in recognizing anomalies, the previously discussed feature ranking algorithms will compared on multiple datasets. The focus will be devoted in particular to the robustness and consistency across different algorithms and datasets.


\subsubsection{Results}
The robustness results are analyzed compared to the robustness of DIFFI \ref{DIFFI} algorithm and AcME algorithm.
AcME is an algorithm written by Dandolo et al.\cite{dandolo2021acme} which give an unsupervised explanation of the features by calculating the variance of the result modifying a single feature and maintaining the other features at the mean value. It is very similar to a variance selection but more correlated to the output rather than to the features themselves. AcME here is proposed as an alternative of SHAP because it is too low to be feasible doing the experiments with it.

Here we show some results of the interpretation algorithm, the key to understand the graphs is: the more the barplots colours are ordered, the more the algorithm is robust. In fact what they represent is the times in which the algorithm classifies the feature in a particular position, each feature have its specific colour.  
The graphs show how the precision change dropping one feature per time, maintaining always the most important ones with regards to the algorithm chosen. Its important to underline that once the dataset dimension is contracted to a small number of feature there are points that are equivalent, then we had to drop casually the duplicates, as a result we will see big change in precision when the number of feature is low.
%\newpage
%\begin{description}
%    \input{figures/annthyroid/annthyroid.tex}
%\newpage
%    \input{figures/breastw/breastw.tex}
%\newpage
%    \input{figures/cardio/cardio.tex}
%\newpage
%    \input{figures/ionosphere/ionosphere.tex}
%\newpage
%    \input{figures/lympho/lympho.tex}
%\newpage
%    \input{figures/mammography/mammography.tex}
%\newpage
%    \input{figures/pendigits/pendigits.tex}
%\newpage
%    \input{figures/pima/pima.tex}
%\newpage
%    \input{figures/shuttle/shuttle.tex}
%\newpage
%    \input{figures/thyroid/thyroid.tex}
%\newpage
%    \input{figures/vowels/vowels.tex}
%\newpage
%    \input{figures/wine/wine.tex}






%\newpage
%    \input{figures/wbc/wbc.tex}

%\newpage
%    \input{figures/satimage/satimage.tex}
%\newpage
%\end{description}

\newpage
\input{tables/BigTable.tex}



\input{figures/RFfeature_importance/RF}

==> sections/extended_diffi.tex <==

\section{Extended Isolation Forest Feature Importance}
As DIFFI does with the IF (Section \ref{DIFFI}), with the Depth-based Extended Isolation Forest Feature Importance (\approach) we will try to rank and evaluate the importance of the features in deciding whether a data is an anomaly or not for EIF, so which are the features that most generate an anomaly.

As seen in Section \ref{ExtendedIF} a tree is built in a way that an hyperplane $\mathcal{H}^{t}_{k}$, that splits the subsample $X_k^t \subseteq X^t \subseteq X$, is associated to each node $k \in \mathcal{K}_t$ of the tree $t \in \mathcal{T}$. The hyperplane is well defined by a vector orthogonal to its direction and a point that belongs to it $\{\pmb{v}^{t}_{k},\mathbf{p}^{t}_{k}\}$ with $\pmb{v}^{t}_{k}\sim\frac{\pmb{Z}}{\|\pmb{Z}\|_2}$ where $\pmb{Z}=(Z_1,\dots,Z_{d})^{\top}$ with $Z_i\sim\mathcal{N}(0,1) \, \forall i \in \{1,\dots,d\}$ and  $\mathbf{p}^{t}_{k}  = \alpha^{t}_{k} \pmb{v}^{t}_{k}$ with $\alpha^{t}_{k} \in [\min{\{\mathbf{x}\cdot\pmb{v}^{t}_{k} \,\,\forall x \in X_k^t\}},\max{\{\mathbf{x}\cdot\pmb{v}^{t}_{k} \,\,\forall x \in X_k^t\}}]$ using the Lesouple et al. \cite{LESOUPLE2021109} correction of the EIF.\\

The hyperplane $\mathcal{H}^{t}_{k}$ separates the points in a set of elements on the left side of the hyperplane and a set of elements on the right side of the hyperplane. 
\begin{align}
\begin{split}
 L^{t}_{k}&=\{\mathbf{x}|\mathbf{x} \in X^{t}_{k},\mathbf{v}^{t}_{k} \cdot x>\mathbf{v}^{t}_{k} \cdot p^{t}_{k}\} ,
\\
 R^{t}_{k}&=X^{t}_{k} \setminus L^{t}_{k} .
\end{split}
\end{align}

We want to know which are the features for a sample $x$ that the most influenced its isolation. 
The \approach assign an importance vector to each node of the tree, based on 2 paradigms: 
\begin{itemize}
    \item The importance of the node for an point $x$ is higher when it creates a greater inequality between the number of elements in each side of the hyperplane and $x$ is in the smaller subset. Because greater inequality means a higher grade of isolation for the points in the smaller set.
    \item In each node the importance of each single feature is proportional to the projection along every dimension of the space of the vector normal to the splitting hyperplane.
\end{itemize}

Then we assign an importance value function to every node of the trees that is the projection on the normal vector of the splitting hyperplane of the quotient between the cardinality of the sample before a particular node and after it based following the path of a sample $x$.
Thus, knowing that the splitting hyperplane $\mathcal{H}^t_k$ of that node is determined by the pair $\{\mathbf{v}^{t}_{k},\mathbf{p}^{t}_{k}\}$:
\begin{equation}
\pmb{\lambda}^{t}_{k}(x) = \begin{cases} \left(\frac{|X^{t}_{k}|}{|L^{t}_{k}|}\right) |\mathbf{v}^{t}_{k}|, & \mbox{if } \mathbf{v}^{t}_{k} \cdot x>\mathbf{v}^{t}_{k} \cdot \mathbf{p}^{t}_{k}\\
\left(\frac{|X^{t}_{k}|}{|R^{t}_{k}|}\right) |\mathbf{v}^{t}_{k}|,& \mbox{otherwise} \end{cases}
\end{equation}

Then the vector of importances evaluated in the tree $t$ for an point $x$ is the sum of all the importance vectors of all the nodes that the element $x$ passed through on its path to the leaf node in the tree $t$ defined in Eq(\ref{setnodesx}):
\begin{equation}
\pmb{I}_{t}(x)=\sum_{k \in \mathcal{P}^{t}_x} \pmb{\lambda}_{t,k}(x).
\end{equation}

Then when we calculate the sum of the importance vector of the point $x$ for all the trees in $\mathcal{T}$
\begin{equation}\label{equaimport}
\pmb{I}(x) = \sum_{t \in T} \pmb{I}_{t}(x)
\end{equation}

$\pmb{V}(x)$ is the sum of the vectors orthogonal to the hyperplanes of the nodes that an element $x$ passes in a tree, then we calculate the sum of the values in all the trees:
\begin{equation}
\pmb{V}(x) = \sum_{t \in T}\sum_{k \in \mathcal{P}^{t}_x} \pmb{v}_k^t
\end{equation}

\subsection{Global and Local interpretation}
On one hand the interpretation of the results made by the EIF can be a global, referred to the whole model, an interpretation that gives an order of which are the features that globally create more outliers. On the other hand it can be local, when you want to know which are the features for a particular sample that make it deviate from the distribution.

\subsubsection{Global Feature Importance}
\label{sec:GFI}
To globally evaluate the importance of the features, as DIFFI does with the IF interpretation, we divide $X$ into the subset of predicted inliers $\mathcal{Q}_I=\{x_i \in X|\hat{y}_i=0\}$  and the one of predicted outliers $\mathcal{Q}_O=\{x_i \in X|\hat{y}_i=1\}$ where $\hat{y}_i \in \{0,1\}$ is the binary label produced by the thresholding operation indicating whether the corresponding data point $\mathbf{x}_i$ is anomalous $(\hat{y}_i =1)$ or not $(\hat{y}_i =0)$. 

We define the global importance vectors for the inliers and for the outliers by summing out the importance values introduced in Eq(\ref{equaimport}):
\begin{align}
\begin{split}
    \pmb{I}_I&=\sum_{x\in \mathcal{Q}_I} \pmb{I}(x),\\
    \pmb{I}_O&=\sum_{x\in \mathcal{Q}_O} \pmb{I}(x).
\end{split}
\end{align}
Likewise the sum of the orthogonal vectors
\begin{align}
\begin{split}
    \pmb{V}_I&=\sum_{x\in \mathcal{Q}_I} \pmb{V}(x),\\
    \pmb{V}_O&=\sum_{x\in \mathcal{Q}_O} \pmb{V}(x).
\end{split}
\end{align}
 \\

Due to stochastic sampling of hyperplanes, in order to avoid the bias generated by the fact that it is possible that some dimensions are sampled more often than others, the vectors of importance have to be divided by the sum of the orthogonal vectors.\\
\begin{align}\label{impvectfinal}
\begin{split}
    \hat{\pmb{I}}_I&=\frac{\pmb{I}_I}{\pmb{V}_I},\\
    \hat{\pmb{I}}_O&=\frac{\pmb{I}_O}{\pmb{V}_O}.
\end{split}
\end{align}

To evaluate which are the most important features to discriminate a data as an outlier we divide the importance vector unbiased of the inliers by the one of the outliers Equation (\ref{impvectfinal}), and we obtain the global feature importance vector as the DIFFI algorithm \cite{diffi}.
\begin{equation}
    \pmb{GFI}=\frac{\hat{\pmb{I}}_I}{\hat{\pmb{I}}_O}
\end{equation}

\subsubsection{Local Feature Importance}
Let's take into account an element $x$, the equation Eq(\ref{equaimport}) gives a vector of importances $\pmb{I}(x)$ of the sample $x$ for each feature. Then the vector $\pmb{V}(x)$ is the normalization factor of the feature importance.
Then the Local Feature Importance ($\pmb{LFI}$) of an element $x$ is the quotient 
\begin{equation}
    \pmb{LFI}(x) = \frac{\pmb{I}(x)}{\pmb{V}(x)}
\end{equation}


==> sections/introduction_v0.tex <==

\section{Introduction}
%Machine Learning and Artificial intelligence are playing a central role in today's socio-economic change, revolutionising many sectors, including the industry, giving rise to what is called the fourth industrial revolution, the industry 4.0 \cite{krafft2020challenges}\cite{xu2018fourth}.\\

Machine Learning (ML) and Artificial intelligence are playing a central role in today's socio-economic change, revolutionising many sectors, like manufacturing \cite{krafft2020challenges, xu2018fourth}, medicine \cite{houssein2021deep} and Internet of Things \cite{klaib2021eye}. Together with the increasing deployment of intelligent systems in every substrata of the economy, new problems arise due to the widespread applications of these systems that   are \tom{however often} opaque and complex to decode. \jacopo{In particular, we are observing the paradigm shift of the final users that moves towards a variety of people with different background, mostly not related with data-driven methods. For this reason, it is needed to find explanation algorithms that allows deeper understanding of the backbone behind predicting models.} \jadel{( This characteristic is widely recognized as an obstacle on their adoption in many fields).}

Many scientific works identify explanability\footnote{While authors in the literature use the term 'interpretability' and 'explainability' associated with slighty different concepts when associated to Machine Learning/Artificial Intelligence as presented in \cite{gilpin2018explaining}, in this work we will use both terms interchangeably.} as a key factor to overcome the problem of machine learning-based systems adoption \cite{confalonieri2021historical, doshi2017towards, linardatos2020explainable}. \ale{The current relevance of the adoption of Machine Learning-based technologies is paramount, as users are being asked to accept their integration into everyday decisions, particularly in critical areas such as medical diagnosis, insurance, and financial services. Given the significant influence of these technologies, institutions are making considerable efforts to regulate them, typically by ensuring that interpretability traits are available.}

%The matter of adoption is nowadays of key importance when dealing with Machine Learning-based technologies: users are asked to accept the integration of such tools in everyday decisions, especially in critical contexts like medical diagnosis, insurance or financial services. Given the huge impact that ML-based technologies, institutions are providing important effort to regulate such technologies, typically ensuring that interpretability traits are available.
%This is relevant not only for social reason, but also for legal reasons, as underlined in \cite{confalonieri2021historical}; for example,
In recent years the European Union's General Data Protection Regulation (GDPR) \cite{EUdataregulations2018} stipulates a right to obtain “\emph{meaningful information about the logic involved}” for consumers affected by an automatic decision.% (Parliament and Council of the European Union, 2016), and 

In the common case of tabular data, interpretability \jacopo{hints can be formulated in different ways} \cite{molnar2020interpretable}\jacopo{. However a popular approach is to associate the concept of interpretability computing an index of the \tom{feature importance}  considering the influence that they have both on the single prediction (\emph{local importance}) and the on the overall dataset took as a whole.} \textbf{AL posto di [However a popular approach is to provide an indication of the importance of an input feature in affecting the output in general (so-called \emph{global importance}) or in single predictions (\emph{local importance})]}. This \jacopo{metric} %\textbf{al posto di: type of information} 
was widely \jacopo{exploited} \jadel{popularized} in the past \jacopo{years} thanks to \jacopo{the} Random Forest \jacopo{algorithm, a method}, that has many built-in approaches to provide a ranking of the most important features \cite{kursa2010feature}. Moreover, thanks to the rise of many post-hoc method, like permutation importance \cite{altmann2010permutation} or SHAP \cite{NIPS2017_7062}, such type of intepretability information through feature rankings has been extended also \jacopo{to} models that are not tree-based.

Even in presence of such advancements in recent years by the eXplainable Artificial Intelligence (XAI), most approaches in this area are designed for supervised tasks, leaving unsupervised tasks, like Anomaly Detection (AD), rarely discussed in the literature. 

Anomaly Detection (AD), also referred as Outlier Detection\footnote{In this paper, we will refer to 'Outlier Detection' and 'Anomaly Detection' alternatively, always referring to the same unsupervised task of finding anomalous data points.}, is a field of Machine Learning (ML) %\jacopo{è giusto? se penso a modelli statistici come AR, ARMA, sono modelli statistici utilizzati per il riconoscimento anomalie in time series, però sono modelli statistici non di machine learning. Esempio https://dl.acm.org/doi/pdf/10.1145/1541880.1541882}
that focuses on the identification of outlying elements that live outside %\jacopo{rimosso: from} 
the standard "normal" behaviour observed in the majority of the dataset \cite{hawkins1980identification}.
\tom{non stiamo cambiando il significato?}
\jacopo{It is worth noticing that inside this framework, the knowledge embeeded inside the interpretability model directly came out from the distribution of the samples inside the dataset and on the belief that an anomaly corresponds to samples that lie far from what is recognized to be a "normal" distribution of the data}
\textbf{al posto di: If in the Supervised anomaly detection models we refer to Interpretation as a knowledge on the input features that rises from the interaction of them with the corresponding label, in the case of the Unsupervised scenario the information arises by the model itself without the need of labelled data, by analysing the merely distribution of the sample, on the belief that an anomaly is a sample that lie far from the normal distribution of the data.}


One of the most popular approach in the context of AD is the Isolation Forest (IF) \cite{4781136}, for its high accuracy, low computational costs and relatively simple inner mechanisms. For the IF, an approach has been presented in the literature,  able to provide global and local interpretability information: such approach is called Depth-based Isolation Forest Feature Importance (DIFFI) \cite{diffi}. 

In this paper, we will contribute to the research area of interpretabilty in AD, by providing, to the best of our knowledge, the first model-specific\footnote{Model-specific interpretation tools are limited to specific model classes. Instead Model-agnostic tools can be used on any machine learning model and are applied after the model has been trained \cite{molnar2020interpretable}} approach, called \emph{\approach}, \jacopo{able to provide an} \textbf{al posto di: for providing} interpretabilty \jacopo{attribute} to the Extended Isolation Forest (EIF), a \jacopo{state of the art(?) method inspierd by IF algorithm} \textbf{more sophisticate and derivative approach of IF}.

\jacopo{The main innovation brought by EIF consists into a new conceptual formalization of the isolation tree, different from that one described inside the IF method for the lack of bias. L'idea sarebbe quello di stare un pò generico qui}
\textbf{al posto di: EIF aims at overcoming one of the main limitation of IF that is the introduction of wrong bias in favour of the hyperplanes orthogonal to the feature space principal directions.}
\gpt{We will apply analogous reasoning to that used for deriving DIFFI to a more intricate situation where attributing the contribution to the task resolution to a single feature is problematic. Additionally, we will conduct an extensive comparison of IF and EIF to assist scientists and practitioners in deciding when to use one or the other algorithm.} \gian{verificare alla fine}

%This paper will address the problem of explainable Anomaly Detection, providing an explainability algorithm conceived ad-hoc for a particular AD algorithm named Extended Isolation Forest (EIF) that proved to be very effective in the detection task but unfortunately miss the ability to explain its outcome.

The rest of the paper is organized as follows. First, \jacopo{ a general introduction of the Isolation Forest (IF) algorithm is provided in Section \ref{IF}} \textbf{we will introduce the
Isolation Forest (IF) original in Section \ref{IF}}.
 Then, in Section \ref{ExtendedIF}, we will present the results obtained in \cite{8888179},  \jacopo{ in particular focusing on the improvements brought by this method regarding the structural problems that are hidden in the IF implementation. } \textbf{al posto di: where we highlight the structural problems of the Isolation Forest algorithm and present a way to overcome them by their EIF model.} 
\jacopo{rimosso  then (ripetizione)} In Section \ref{IFvsEIF}, we will present a comparison of the two methods, IF and EIF, with the intention \jacopo{ of providing a deeper understanding of their different inner mechanisms used for the anomaly predictions and how this difference is also reflected on the precision achieved. } \textbf{al posto di: of understanding the structural differences of the two algorithms and how far they differ in terms of precision.} Next, after introducing DIFFI in Section \ref{DIFFI}, we provide the theory behind \approach in Section \ref{DEIFFI}. 
Finally, we validate our model-specific feature importance algorithm on 12 datasets, 4 synthetic and 8 real, comparing it with DIFFI and Random Forest feature importance.
We then evaluate the {\itshape global importance} of features using feature selection as a proxy and the {\itshape local importance} of features by analyzing the importance scoremaps of the \approach algorithm compared to those of the DIFFI algorithm.

 
%Both these models thanks to their characteristics are extensively used in many fields. As a direct consequence of their use, the need to provide a meaningful explanation has become an must. Provide an explaination  usually means providing a sort of explanation showing the most important features that lead the algorithm to take a particular decision.
%Then, starting from the idea of an interpretation algorithm of the Isolation Forest presented by Carletti et al. in \cite{diffi} called Depth-based Isolation Forest Feature Importance (DIFFI), we will develop an an interpretation algorithm conceived model-specific to provide an interpretation of the Extended Isolation Forest model, thus, as a consequence, the explanation algorithm is named Depth-based Extended Isolation Forest Feature Importance (\approach).


==> sections/real_dataset_results_v0.tex <==

We used 8 widely used real datasets benchmark for anomaly detection introduced in Section \ref{datasets} and listed in the Table \ref{tab:dataset_used}.
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% RANDOM FOREST
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
Obtaining a gold standard reference for evaluating explanations in the context of explainability can be challenging, as it often requires either a large group of people to assess the quality of a set of explanations or a domain expert to provide expert explanations of anomalies. 
As an alternative, we use feature importances provided by a supervised method, specifically Random Forest (RF), as a proxy measure of the performance of our unsupervised approach. The use of RF feature importances is motivated by the belief that they provide good explanations because it is a supervised algorithm and the similarity between RF and EIF, both based on a decision tree structure. We compare the ranking of features produced by our unsupervised approach with those produced by RF to understand how much \approach is close to RF in terms of feature selection. This allows us to assess the efficacy of our unsupervised approach.

\tom{non so se piazzare prima sto paragrafo}\ale{per me sta meglio qua dato che prima introduciamo RF come nostro termine massimo di paragone e poi spieghiamo l'esperimento}
The feature selection experiments have been repeated $10$ times: the detection model has been trained on the full set of features, and the least important feature has been removed at each step, retraining the model and recording the detection performances. At the end of the procedure,  the model is allowed to observe only the most important feature. The same procedure has been computed using the feature importance provided by different approaches: the random approach (baseline), the DIFFI (old approach), the \approach (proposed approach) and the RF one that is the only allowed to see the labels of the points. \tom{CITARE LAVORI}\ale{QUALI LAVORI? DIFFI MI SEMBRA RIDONDANTE MA LO POSSO METTERE E DI RF NON SO CHE METTERE CONSIGLI?} \ale{ho tolto via la variance selection e ACME perche troppo out of context}

%We decided to take into account also alternative models mainly based on the variance of the dataset in order to have an all-round comparison with other unsupervised Anomaly Detection Feature Importance algorithms.
%ACME is an algorithm written by Dandolo et al.\cite{dandolo2021acme} which gives an unsupervised explanation of the features by calculating the variance of the result modifying a single feature and maintaining the other features at the mean value. 
%The variance selection is a simple way to do feature selection based on the variance of each feature, with the simple assumption that the more a feature contains information the more a feature is important, the higher its variance.
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% ANNTHYROID :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::

The first real dataset where \approach was tested is Annthyroid, a medical dataset showing patients with thyroid diseases. The results of the repeated feature importance for DIFFI and \approach (\tom{Figures \ref{fig:annthyroid-diffi} and \ref{fig:annthyroid-ediffi}}) concerning the most important feature are in accordance with the one shown in Figure \tom{\ref{fig:annthyroid_RFordered_features}},  however DIFFI tends to give a high rank to feature 2 and 4 that are the least important according to RF. 

In Figure \ref{fig:annthyroid} it is interesting to observe the behaviour of the feature selection provided by DIFFI and \approach on Annthyroid: removing the unnecessary features, the detection model is able to perform much better than with the full set of features. On the contrary, removing a random feature (\tom{red line}), the model is not able to improve. It's important to notice that this dataset is the only dataset \tom{that in previous study (Figure \ref{fig:IF vs EIF} in Section \ref{dof}) had} an increase in terms of precision \tomdel{when the more the splitting hyperplanes have less degrees of freedom,} \tom{when the degrees of freedom of the hyperplane are reduced,} suggesting that it is easier to discriminate between outliers and inliers observing one dimension per time. Moreover Figure \ref{fig:annthyroid_score} shows explicitly that the outliers, shown in the shape of a star, are easily detected using the feature 1 alone, without being mislead by considering distributions along other features. \tom{GLI SCORE MAP SONO STATI ANTICIPATI?}
    
\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/annthyroid/diffi_annthyroid.pdf}
      \caption{DIFFI}
      \label{fig:annthyroid-diffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/annthyroid/DEIFFI_annthyroid.pdf}
      \caption{\approach}
      \label{fig:annthyroid-ediffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/rfbarplots/rfannthyroid.pdf}
      \caption{Random Forest}
      \label{fig:annthyroid_RFordered_features}
    \end{subfigure}\hfil % <-- added
        \begin{subfigure}{0.48\textwidth}
      \includegraphics[width=\linewidth]{figures/annthyroid/annthyroid_2.pdf}
      \caption{annthyroid}
      \label{fig:annthyroid}
    \end{subfigure}\hfil % <-- added
\caption{comparison of the consistency of the feature importance on annthyroid dataset}\label{fig:annthyroid-consistency}
\end{figure}


% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% PIMA :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::

Pima is also a medical dataset showing diabetic patients. Here it seems DIFFI and \approach capture different aspects of the problem, indeed  DIFFI and \approach quite disagree (Figure \ref{fig:pima-consistency}): DIFFI is more consistent in highlighting feature 2 and 5 while \approach 1 and 2. However RF consistently prefers feature 1 and feature 5 while discards common feature 2. 

\tomdel{The confusion about the most important features reflects in Figure} \ref{fig:pima}: \tomdel{on one hand DIFFI rapidly deteriorates its detection performances but on the other hand there is not a clear winner between} \approach \tomdel{and Random Forest probably because there are no features that clearly help to discriminate between inliers and outliers.}
\tom{That said, Figure \ref{fig:pima} shows that with many features DIFFI and \approach perform quite the same, but selecting the three most important features \approach starts to perform much better with respect to DIFFI, with performances similar to RF. However in this dataset it is possible to see that for some combinations of the features, the random feature selection can achieve even better results. This might indicate that RF is a good reference, but might not be the best possible option.}
\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/pima/diffi_pima.pdf}
      \caption{DIFFI}
      \label{fig:pima-diffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/pima/DEIFFI_pima.pdf}
      \caption{\approach}
      \label{fig:pima-ediffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/rfbarplots/rfpima.pdf}
      \caption{Random Forest}
      \label{fig:pima_RFordered_features}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.48\textwidth}
      \includegraphics[width=\linewidth]{figures/pima/pima_2.pdf}
      \caption{pima}
      \label{fig:pima}
    \end{subfigure}\hfil % <-- added
\caption{comparison of the consistency of the feature importance on pima dataset}
\label{fig:pima-consistency}
\end{figure}

% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% SHUTTLE :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::

Shuttle, \tomdel{probably the hardest dataset,} is shown in Figure \ref{fig:shuttle-consistency}. It is interesting to note DIFFI consistently ranks feature 3 in the first position while RF never suggests it as a relevant feature. On the contrary, \approach gives more similar results, highlighting feature 8 and feature 0. 
Similarly to "Pima" feature selection in Figure \ref{fig:shuttle} we can observe that DIFFI algorithm have a drop down in precision \tomdel{but it is impossible to assert without any doubt that there is an algorithm that selects the features better than others.} \tom{while RF achieves the best possible results. However, despite the good explanation results,  \approach performs on average as the random feature selection.}

\begin{figure}[ht!] 
    \centering % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/shuttle/diffi_shuttle.pdf}
      \caption{DIFFI}
      \label{fig:shuttlDEIFFI}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/shuttle/DEIFFI_shuttle.pdf}
      \caption{\approach}
      \label{fig:shuttle-ediffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/rfbarplots/rfshuttle.pdf}
      \caption{Random Forest}
      \label{fig:shuttle_RFordered_features}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.48\textwidth}
      \includegraphics[width=\linewidth]{figures/shuttle/shuttle_2.pdf}
      \caption{shuttle}
      \label{fig:shuttle}
    \end{subfigure}\hfil % <-- added
\caption{comparison of the consistency of the feature importance on shuttle dataset}\label{fig:shuttle-consistency}
\end{figure}

% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% WINE :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::

\tom{A very different result is obtained in}
"Wine", the smallest dataset with $129$ elements and $13$ dimensions, has only 10 anomalies.  In this context DIFFI and \approach strongly disagree, but only \approach is able to detect the most important feature, the number 12 (Figure \ref{fig:wine-consistency}).
\tom{This directly reflects in} Figure \ref{fig:wine}, where \approach performs much better than DIFFI as it is able to select quite easily the most important feature for the detection. 

%In this case \approach seems to be even faster than supervised and semi-supervised methods like RF and ACME. 

\begin{figure}[ht!] 
    \centering % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/wine/diffi_wine.pdf}
      \caption{DIFFI}
      \label{fig:winDEIFFI}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/wine/DEIFFI_wine.pdf}
      \caption{\approach}
      \label{fig:wine-ediffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/rfbarplots/rfwine.pdf}
      \caption{Random Forest}
      \label{fig:wine_RFordered_features}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.48\textwidth}
      \includegraphics[width=\linewidth]{figures/wine/wine_2.pdf}
      \caption{wine}
      \label{fig:wine}
    \end{subfigure}\hfil % <-- added
\caption{comparison of the consistency of the feature importance on wine dataset}\label{fig:wine-consistency}
\end{figure}

% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% BREASTW :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
In the case of "Breastw" dataset both algorithms DIFFI and \approach agree on which are the most important features to detect the anomalies, on the contrary, Random Forest feature importance have completely different results.
Then taking a look to the Figure \ref{fig:breastw} we can observe that RF has a very low performance compared to the first two feature selection algorithms, moreover \approach has higher performances than DIFFI algorithm so we can state that in this case \approach is the best algorithm.

\begin{figure}[ht!] 
    \centering % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/breastw/diffi_breastw.pdf}
      \caption{DIFFI}
      \label{fig:breastw-diffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/breastw/DEIFFI_breastw.pdf}
      \caption{\approach}
      \label{fig:breastw-ediffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/rfbarplots/rfbreastw.pdf}
      \caption{Random Forest}
      \label{fig:breastw_RFordered_features}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.48\textwidth}
      \includegraphics[width=\linewidth]{figures/breastw/breastw_2.pdf}
      \caption{Feature Selection}
      \label{fig:breastw}
    \end{subfigure}\hfil % <-- added
\caption{comparison of the consistency of the feature importance on breastw dataset}\label{fig:breastw-consistency}
\end{figure}

% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% IONOSPHERE :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::

"Ionosphere" is a very complex dataset due to its high dimensionality (33 features).
We can observe in Figure \ref{fig:ionosphere-diffi} that the feature 0 is consistently selected by DIFFI as the most important feature. %\tomdel{ than starting from the second position it is impossible to infer any sort of feature ranking. } 
On the contrary in Figure \ref{fig:ionosphere-ediffi} \approach does not show to have any preferences on the most important feature.
Instead for the RF we have that the features $2$,$3$ and $25$ are considered very important, but this is not depicted in the feature selection (Figure \ref{fig:ionosphere})  \tom{CORREGGERE} \tomdel{where, not only we can observe that none of the algorithm is consistently better than the others but also the algorithm that has the highest precision score with the less number of feature is surprisingly} \approach algorithm. This fact underlines that as far as the "Ionosphere"  dataset is concerned, there are not real preferences among the features. %\tomdel{, thus it is pretentious determine a robust feature ranking.}
\begin{figure}[ht!] 
    \centering % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/ionosphere/diffi_ionosphere.pdf}
      \caption{DIFFI}
      \label{fig:ionosphere-diffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/ionosphere/DEIFFI_ionosphere.pdf}
      \caption{\approach}
      \label{fig:ionosphere-ediffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/rfbarplots/rfionosphere.pdf}
      \caption{Random Forest}
      \label{fig:ionosphere_RFordered_features}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.48\textwidth}
      \includegraphics[width=\linewidth]{figures/ionosphere/ionosphere_2.pdf}
      \caption{ionosphere}
      \label{fig:ionosphere}
    \end{subfigure}\hfil % <-- added
\caption{comparison of the consistency of the feature importance on ionosphere dataset}\label{fig:ionosphere-consistency}
\end{figure}
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% CARDIO :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::

In the case of the dataset named "Cardio" we can observe that DIFFI and \approach algorithm agree that the feature $6$ and the feature $2$ play a central role to detect anomalies, moreover the DIFFI observe the feature $5$ as the most important one very consistently.
The only feature that the unsupervised feature ranking algorithm have in common with Random Forest feature importance is the feature number $6$. 

What it is possible to infer from the feature selection in Figure \ref{fig:cardio} is that the most performing feature selection is the one based on the ranking given by random forest, even if DIFFI is very close. The \approach in this case does not have good performances but is consistently above the random feature selection.
\begin{figure}[ht!] 
    \centering % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/cardio/diffi_cardio.pdf}
      \caption{DIFFI}
      \label{fig:cardio-diffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/cardio/DEIFFI_cardio.pdf}
      \caption{\approach}
      \label{fig:cardio-ediffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/rfbarplots/rfcardio.pdf}
      \caption{Random Forest}
      \label{fig:cardio_RFordered_features}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.48\textwidth}
      \includegraphics[width=\linewidth]{figures/cardio/cardio_2.pdf}
      \caption{cardio}
      \label{fig:cardio}
    \end{subfigure}\hfil % <-- added
\caption{comparison of the consistency of the feature importance on cardio dataset}\label{fig:cardio-consistency}
\end{figure}
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% PENDIGITS :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
The last dataset taken in consideration is called "Pendigit", in this case we can observe that, even if DIFFI and \approach consistently agree on the two most important features, RF strongly disagrees. It is important to mention that both \approach and Random forest give to the feature number $5$ some high importance.
%It is possible to observe in the feature selection that \approach  %\tomdel{ feature selection shares the first position as the most performing feature selection until the feature are more than 7.}
In the feature selection plot it is possible to observe that \approach improves and reaches its maximum at 9 features. Then the precision of \approach drops, while RF and ACME keep good performances with even less features. 
\begin{figure}[ht!] 
    \centering % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/pendigits/diffi_pendigits.pdf}
      \caption{DIFFI}
      \label{fig:pendigits-diffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/pendigits/DEIFFI_pendigits.pdf}
      \caption{\approach}
      \label{fig:pendigits-ediffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/rfbarplots/rfpendigits.pdf}
      \caption{Random Forest}
      \label{fig:pendigits_RFordered_features}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.48\textwidth}
      \includegraphics[width=\linewidth]{figures/pendigits/pendigits_2.pdf}
      \caption{pendigits}
      \label{fig:pendigits}
    \end{subfigure}\hfil % <-- added
\caption{comparison of the consistency of the feature importance on pendigits dataset}\label{fig:pendigits-consistency}
\end{figure}


In almost all feature selection Figures we have previously discusses, we can observe that the feature selection made using the ranking made by the \approach algorithm are consistently above the "casual" feature ranking, stressing the fact that it is able to detect consistently the feature that contribute the most in defining if a sample is an outlier or not. Moreover we can observe that in datasets like "Annthyroid","Wine","Breastw" and "Ionosphere"  \approach is one of the best feature selection strategies.



% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% FEATURE SELECTION :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
\subsection{Scoremap}
As in the results on synthetic dataset presented at the beginning of this Section, also on in the case of real datasets shown in Figure \ref{fig:score_map} the score map of \approach has much less artifacts with respect to DIFFI. This is particularly evident in Figure \ref{fig:wine_score} where we present the scoremaps of 4 different datasets showing the two most important features highlighted by DIFFI and \approach. As in Section \ref{lfi} we can observe how much the \approach is able to generalize the importance in each point of the space, instead the DIFFI method is very biased both on the specific dataset of training and on the direction orthogonal to the principal dimensions.

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}{0.87\textwidth}
      \includegraphics[width=\linewidth]{figures/annthyroid/annthyroid_score.pdf}
      \caption{annthyroid}
      \label{fig:annthyroid_score}
    \end{subfigure} % <-- added
    \begin{subfigure}{0.87\textwidth}
      \includegraphics[width=\linewidth]{figures/pima/pima_score.pdf}
      \caption{pima}
      \label{fig:pima_score}
    \end{subfigure} % <-- added
\end{figure}

\begin{figure}\ContinuedFloat
    \begin{subfigure}{0.87\textwidth}
      \includegraphics[width=\linewidth]{figures/shuttle/shuttle_score.pdf}
      \caption{shuttle}
      \label{fig:shuttle_score}
    \end{subfigure} % <-- added
    \begin{subfigure}{0.87\textwidth}
      \includegraphics[width=\linewidth]{figures/wine/wine_score.pdf}
      \caption{wine}
      \label{fig:wine_score}
    \end{subfigure} % <-- added
\caption{Scoremaps}\label{fig:score_map}
\end{figure}









==> sections/real_datasets_results.tex <==

\subsubsection{Experimental Setup}
We used eight well-known real datasets benchmark for anomaly detection introduced in Section \ref{datasets} and listed in Table \ref{tab:dataset_used}.
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% RANDOM FOREST
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
Obtaining a gold standard reference for evaluating explanations in the context of explainability can be challenging, as it often requires either a large group of people to assess the quality of a set of explanations or a domain expert to provide expert explanations of anomalies. 

One of the most common method to provide the importance of the features is using an algorithm named SHAP \cite{NIPS2017_7062}, SHAP (SHapley Additive exPlanations) is a post-hoc method used to explain the output of any machine learning model. The technique is based on the concept of Shapley values from cooperative game theory.
In practice, SHAP values are computed by averaging the difference in a model's output caused by the presence or absence of each feature. Intuitively, this tells us how much a particular feature contributes to a given prediction. 
SHAP is nowadays the most used explanation algorithm first because it is based on solid theoretical foundations in cooperative game theory. Second, it provide a unified measure of feature importance that can be used with any model and any type of data. 
Even if it may seem the solution for the explanation of the models in practice often it is unfeasible to use it, one of the main issues with SHAP is that it has a high computational complexity $O(2^d)$, where $d$ is the number of features. This means that as the number of features increases, the computation time increases exponentially. \todo[inline]{Va messa la reference ad un articolo in cui si dice che quella è la complessità di SHAP, ma se non c'è evitiamo di dirla esplicitamente e citiamo paper in cui si argomenta la lentezza di SHAP}, \ale{Nel molnar ad un certo punto dice  "How much faster is TreeSHAP? Compared to exact KernelSHAP, it reduces the computational complexity from $O(TL2^M)$  to $O(TLD^2)$" dove $M$ è il numero di features, $T$ number of trees $L$ maximum number of leaves and $D$ maximum depth of the tree} 

The complexity of the computations for large datasets, as well as the computational cost of the algorithm, pose limitations on its applicability. Therefore, this study employed SHAP, with the EIF model's anomaly score as label, applied to datasets with "Low" or "Middle" dimensionality, as reported in Table \ref{tab:dataset_used}.To mitigate the computational costs, a subset of the data consisting of only 100 samples was selected through random sampling without replacement, which was then used to compute the SHAP values. 
\todo[inline]{Forse andrebbe anticipate che il sampling può avere effetti molto negativi, come analizzato in AcME}
By this approach, we were able to apply the algorithm to five datasets \texttt{annthyroid}, \texttt{breastw}, \texttt{pima}, \texttt{shuttle} and \texttt{wine} limiting the computational resources necessary.

As an alternative, in order to have a proxy measure of the feature importances for all the dataset used, we use a supervised model, specifically Random Forest (RF). The use of RF feature importances is motivated by the assumption that they provide good explanations because it is a supervised algorithm and the similarity between RF and EIF, both based on a decision tree structure. We compare the ranking of features produced by our unsupervised approach with those produced by RF to understand how much \approach is close to RF in terms of feature selection. This allows us to assess the efficacy of our unsupervised approach.
\todo[inline]{Possiamo già dire qui che la RF è addestrata sulle label vere del dataset, cosa che adesso è scritta più in basso.}

%\tom{non so se piazzare prima sto paragrafo}\ale{per me sta meglio qua dato che prima introduciamo RF come nostro termine massimo di paragone e poi spieghiamo l'esperimento}
The feature selection experiments have been repeated $10$ times: the detection model has been trained on the full set of features, and the least important feature has been removed at each step, retraining the model and recording the detection performances. At the end of the procedure,  the model is allowed to observe only the most important feature. The same procedure has been computed using the feature importance provided by different approaches: the random approach (baseline), the DIFFI (old approach), the \approach (proposed approach) and the RF one that is the only allowed to see the labels of the points. %\tom{CITARE LAVORI}
%\ale{QUALI LAVORI? DIFFI MI SEMBRA RIDONDANTE MA LO POSSO METTERE E DI RF NON SO CHE METTERE CONSIGLI?} 
%\ale{ho tolto via la variance selection e ACME perche troppo out of context} \gian{Possono essere menzionati nei future works?} \ale{sicuramente come possibili feature importance ???unsupervised??? anche se ACME non lo è veramente. Forse se si vogliono menzionare si potrebbe parlare di analisi delle feature più importanti tenendo conto della varianza}\ale{non menzionare l'acme}

%We decided to take into account also alternative models mainly based on the variance of the dataset in order to have an all-round comparison with other unsupervised Anomaly Detection Feature Importance algorithms.
%ACME is an algorithm written by Dandolo et al.\cite{dandolo2021acme} which gives an unsupervised explanation of the features by calculating the variance of the result modifying a single feature and maintaining the other features at the mean value. 
%The variance selection is a simple way to do feature selection based on the variance of each feature, with the simple assumption that the more a feature contains information the more a feature is important, the higher its variance.
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% ANNTHYROID :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
\subsubsection{Results}
The first real dataset where \approach was tested is \texttt{annthyroid}, a medical dataset related to patients with thyroid diseases. The results of the repeated feature importance for DIFFI and \approach are shown respectively in Figures \ref{fig:annthyroid-diffi} and \ref{fig:annthyroid-ediffi}: in such panels statistics concerning the most important feature are reported; it can be seen that such statistics are in accordance with the ones obtained with the RF shown in Figure \ref{fig:annthyroid_RFordered_features}; however, it can be seen how DIFFI tends to give a high rank to feature 2 and 4 that are the least important according to RF. 
In Figure \ref{fig:annthyroid} it is interesting to observe the behaviour of the feature selection provided by DIFFI and \approach on \texttt{annthyroid}: removing the unnecessary features, the detection model is able to perform much better than with the full set of features. On the contrary, removing a random feature (red line), the model is not able to improve. It is important to notice that this dataset is the only dataset that in previous study (Figure \ref{fig:IF vs EIF} in Section \ref{dof}) has an increase in terms of precision when the degrees of freedom of the hyperplane are reduced, suggesting that it is easier to discriminate between outliers and inliers observing one dimension per time.
Moreover looking at the dataset distribution in Figure \ref{fig:annthyroid_score} it is possible to observe that the outliers, shown in the shape of a star, are easily detected using the feature 1 alone. 
    
\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/annthyroid/diffi_annthyroid.pdf}
      \caption{DIFFI}
      \label{fig:annthyroid-diffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/annthyroid/ExIFFI_annthyroid.pdf}
      \caption{\approach}
      \label{fig:annthyroid-ediffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/rfbarplots/rfannthyroid.pdf}
      \caption{RF}
      \label{fig:annthyroid_RFordered_features}
    \end{subfigure}\hfil % <-- added
        \begin{subfigure}{0.48\textwidth}
      \includegraphics[width=\linewidth]{figures/annthyroid/annthyroid_2.pdf}
      \caption{Feature selection}
      \label{fig:annthyroid}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.48\textwidth}
      \includegraphics[width=\linewidth]{figures/annthyroid/shap_annthyroid.png}
      \caption{SHAP importance scores}
      \label{fig:shap_annthyroid}
    \end{subfigure}\hfil % <-- added
\caption{Consistency of the feature importance and feature selection applied to the \texttt{annthyroid} dataset.}\label{fig:annthyroid-consistency}
\end{figure}


% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% BREASTW :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
In the case of \texttt{breastw} dataset while both DIFFI and \approach agree on which are the most important features to detect the anomalies, Random Forest feature importance have completely different outcomes.
By analyzing Figure \ref{fig:breastw}, we can observe that RF has lower performances compared to the unsupervised feature selection algorithms, while \approach has consistently the highest performances. \tom{This supports the idea that it is meaningful to perform unsupervised feature selection.}
\chiara{Non sono sicurissima che in questo caso sia utile considerare la RF addestrata sulle label vere... mi convincete?}\ale{quando l'abbiamo pensata ci serviva come gold standard di riferimento, se l'alleno a rispecchiare il modello fatto con EIF poi l'interpretazione che tira fuori non mi sta dando una verità di riferimento al di là del mio modello}\chiara{ok, in questo modo assumiamo che la RF sappia perfettamente modellare la realtà. Se le performance di classificazione sono ottime, ci potrebbe stare...  }


\begin{figure}[ht!] 
    \centering % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/breastw/diffi_breastw.pdf}
      \caption{DIFFI}
      \label{fig:breastw-diffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/breastw/ExIFFI_breastw.pdf}
      \caption{\approach}
      \label{fig:breastw-ediffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/rfbarplots/rfbreastw.pdf}
      \caption{RF}
      \label{fig:breastw_RFordered_features}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.48\textwidth}
      \includegraphics[width=\linewidth]{figures/breastw/breastw_2.pdf}
      \caption{Feature Selection}
      \label{fig:breastw}
    \end{subfigure}\hfil % <-- added
\caption{Consistency of the feature importance and feature selection applied to the \texttt{breastw} dataset }\label{fig:breastw-consistency}
\end{figure}


% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% CARDIO :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::

In the case of the dataset named \texttt{cardio} we can observe that DIFFI and \approach algorithm agree that the feature $6$ and the feature $2$ play a central role to detect anomalies, moreover the DIFFI observes the feature $5$ as the most important one very consistently.
The only feature that the unsupervised feature ranking algorithm have in common with Random Forest feature importance is the feature number $6$. 

What it is possible to infer from the feature selection in Figure \ref{fig:cardio} is that the best feature selection is the one based on the ranking given by RF. In this case DIFFI performs better than \approach. %\tomdel{in this case does not have good performances but is consistently above the random feature selection, instead DIFFI algorithm average precision is between the RF performance and} \approach \tomdel{performance.}
\begin{figure}[ht!] 
    \centering % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/cardio/diffi_cardio.pdf}
      \caption{DIFFI}
      \label{fig:cardio-diffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/cardio/ExIFFI_cardio.pdf}
      \caption{\approach}
      \label{fig:cardio-ediffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/rfbarplots/rfcardio.pdf}
      \caption{RF}
      \label{fig:cardio_RFordered_features}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.48\textwidth}
      \includegraphics[width=\linewidth]{figures/cardio/cardio_2.pdf}
      \caption{Feature Selection}
      \label{fig:cardio}
    \end{subfigure}\hfil % <-- added
\caption{ Consistency of the feature importance and feature selection applied to the \texttt{cardio} dataset}\label{fig:cardio-consistency}
\end{figure}
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% IONOSPHERE :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::

\texttt{ionosphere} is a very complex dataset due to its high dimensionality (33 features),  and this complexity reflects in the different behaviour of the models.
We can observe in Figure \ref{fig:ionosphere-diffi} that the feature 0 is consistently selected by DIFFI as the most important feature while in Figure \ref{fig:ionosphere-ediffi} \approach does not show to have any preferences on the most important feature.
RF on the contrary highlights the features $2$,$3$ and $25$. What we can observe looking to the feature selection graph is that DIFFI is only slightly better than the other algorithms.
%\tomdel{none of the algorithm is consistently better than }
This fact underlines that as far as the \texttt{ionosphere}  dataset is concerned, there are not real preferences among the features.  %\tomdel{, thus it is pretentious determine a robust feature ranking.}
\begin{figure}[ht!] 
    \centering % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/ionosphere/diffi_ionosphere.pdf}
      \caption{DIFFI}
      \label{fig:ionosphere-diffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/ionosphere/ExIFFI_ionosphere.pdf}
      \caption{\approach}
      \label{fig:ionosphere-ediffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/rfbarplots/rfionosphere.pdf}
      \caption{RF}
      \label{fig:ionosphere_RFordered_features}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.48\textwidth}
      \includegraphics[width=\linewidth]{figures/ionosphere/ionosphere_2.pdf}
      \caption{Feature selection}
      \label{fig:ionosphere}
    \end{subfigure}\hfil % <-- added
\caption{ Consistency of the feature importance and feature selection applied to the \texttt{ionosphere} dataset}\label{fig:ionosphere-consistency}
\end{figure}


% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% PENDIGITS :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
Considering the case of the dataset named \texttt{pendigit} we can observe that, even if DIFFI and \approach consistently agree on the two most important features, RF strongly disagrees sharing with them only feature 5. %\tomdel{It is important to mention that both ExIFFI and Random forest give to the feature number $5$ some high importance}.
\approach initially follows the  performances of RF, while DIFFI has the same performances of the casual feature selection.
%\tomdel{In the feature selection plot it is possible to observe that ExIFFI improves and reaches its maximum at 9 features. }
%Then the precision of \approach drops, while RF and ACME keep good performances with even less features. 
\begin{figure}[ht!] 
    \centering % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/pendigits/diffi_pendigits.pdf}
      \caption{DIFFI}
      \label{fig:pendigits-diffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/pendigits/ExIFFI_pendigits.pdf}
      \caption{\approach}
      \label{fig:pendigits-ediffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/rfbarplots/rfpendigits.pdf}
      \caption{RF}
      \label{fig:pendigits_RFordered_features}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.48\textwidth}
      \includegraphics[width=\linewidth]{figures/pendigits/pendigits_2.pdf}
      \caption{Feature selection}
      \label{fig:pendigits}
    \end{subfigure}\hfil % <-- added
\caption{ Consistency of the feature importance and feature selection applied to the \texttt{pendigits} dataset}\label{fig:pendigits-consistency}
\end{figure}



% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% PIMA :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::

\texttt{pima} is a medical dataset as \texttt{annthyroid}, showing diabetic patients. Here it seems DIFFI and \approach capture different aspects of the problem, indeed in Figure \ref{fig:pima-consistency} DIFFI is more consistent in highlighting feature 2 and 5 while \approach 1 and 2. However RF consistently prefers feature 1 and feature 5 while discards common feature 2. 

%\tomdel{The confusion about the most important features reflects in Figure} \ref{fig:pima}: \tomdel{on one hand DIFFI rapidly deteriorates its detection performances but on the other hand there is not a clear winner between} \approach \tomdel{and Random Forest probably because there are no features that clearly help to discriminate between inliers and outliers.}

That said, Figure \ref{fig:pima} shows that with many features DIFFI and \approach perform quite the same, but selecting the three most important \approach starts to perform much better with respect to DIFFI, with performances similar to RF. However in this dataset it is possible to observe that for some combinations of the features, the random feature selection can achieve even better results. This indicates that RF is a good reference, but might not be the best possible option.
\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/pima/diffi_pima.pdf}
      \caption{DIFFI}
      \label{fig:pima-diffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/pima/ExIFFI_pima.pdf}
      \caption{\approach}
      \label{fig:pima-ediffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/rfbarplots/rfpima.pdf}
      \caption{RF}
      \label{fig:pima_RFordered_features}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.48\textwidth}
      \includegraphics[width=\linewidth]{figures/pima/pima_2.pdf}
      \caption{Feature selection}
      \label{fig:pima}
    \end{subfigure}\hfil % <-- added
        \begin{subfigure}{0.48\textwidth}
      \includegraphics[width=\linewidth]{figures/pima/shap_pima.png}
      \caption{SHAP importance scores}
      \label{fig:shap_pima}
    \end{subfigure}\hfil % <-- added
\caption{Consistency of the feature importance and feature selection applied to the \texttt{pima} dataset}
\label{fig:pima-consistency}
\end{figure}

% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% SHUTTLE :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::

\texttt{shuttle}  is shown in Figure \ref{fig:shuttle-consistency}. It is interesting to note DIFFI consistently ranks feature 3 in the first position while RF never suggests it as a relevant feature. On the contrary, \approach gives results more similar to RF, highlighting feature 8 and feature 0. 
Similarly to \texttt{pima} feature selection in Figure \ref{fig:shuttle} we can observe that DIFFI algorithm have a drop down in precision. %\tomdel{but it is impossible to assert without any doubt that there is an algorithm that selects the features better than others.} 
Unfortunately, while RF achieves the best possible results and despite the good explanation results,  \approach performs on average as the random feature selection.

\begin{figure}[ht!] 
    \centering % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/shuttle/diffi_shuttle.pdf}
      \caption{DIFFI}
      \label{fig:shuttlDEIFFI}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/shuttle/ExIFFI_shuttle.pdf}
      \caption{\approach}
      \label{fig:shuttle-ediffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/rfbarplots/rfshuttle.pdf}
      \caption{RF}
      \label{fig:shuttle_RFordered_features}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.48\textwidth}
      \includegraphics[width=\linewidth]{figures/shuttle/shuttle_2.pdf}
      \caption{Feature Selection}
      \label{fig:shuttle}
    \end{subfigure}\hfil % <-- added
\caption{Consistency of the feature importance and feature selection applied to the \texttt{shuttle} dataset}\label{fig:shuttle-consistency}
\end{figure}

% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% WINE :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::

A very different result is obtained in
\texttt{wine}, the smallest dataset with $129$ elements and $13$ dimensions with only 10 anomalies.  In this context DIFFI and \approach strongly disagree, but only \approach is able to detect the most important feature, the number 12 (Figure \ref{fig:wine-consistency}).
This directly reflects in Figure \ref{fig:wine}, where \approach performs much better than DIFFI as it is able to select quite easily the most important feature for the detection. 

%In this case \approach seems to be even faster than supervised and semi-supervised methods like RF and ACME. 

\begin{figure}[ht!] 
    \centering % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/wine/diffi_wine.pdf}
      \caption{DIFFI}
      \label{fig:winDEIFFI}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/wine/ExIFFI_wine.pdf}
      \caption{\approach}
      \label{fig:wine-ediffi}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/rfbarplots/rfwine.pdf}
      \caption{RF}
      \label{fig:wine_RFordered_features}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.48\textwidth}
      \includegraphics[width=\linewidth]{figures/wine/wine_2.pdf}
      \caption{Feature selection}
      \label{fig:wine}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.48\textwidth}
      \includegraphics[width=\linewidth]{figures/wine/shap_wine.png}
      \caption{SHAP importance scores}
      \label{fig:shap_wine}
    \end{subfigure}
\caption{ Consistency of the feature importance and feature selection applied to the \texttt{wine} dataset}\label{fig:wine-consistency}
\end{figure}

In almost all feature selection Figures we have previously discusses, we can observe that the feature selection made using the ranking made by the \approach algorithm are often above the "casual" feature ranking, stressing the fact that it is able to detect consistently the feature that contribute the most in defining if a sample is an outlier or not. Moreover we can observe that in datasets like \texttt{annthyroid},   \texttt{wine},    \texttt{breastw} and \texttt{pendigits}  \approach is one of the best feature selection strategies. 

% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% FEATURE SELECTION :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::
\subsection{Scoremap}
As in the results on synthetic dataset presented at the beginning of this Section, also on in the case of real datasets shown in Figure \ref{fig:score_map} the score map of \approach has much less artifacts with respect to DIFFI. This is particularly evident in Figure \ref{fig:wine_score} where we present the scoremaps of 4 different datasets showing the two most important features highlighted by DIFFI and \approach. As in Section \ref{lfi} we can observe how much the \approach is able to generalize the importance in each point of the space, instead the DIFFI method is very biased both on the specific dataset of training and on the direction orthogonal to the principal dimensions.

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}{0.65\textwidth}
      \includegraphics[width=\linewidth]{figures/annthyroid/annthyroid_score.png}
      \caption{\texttt{annthyroid}}
      \label{fig:annthyroid_score}
    \end{subfigure} % <-- added
    \begin{subfigure}{0.65\textwidth}
      \includegraphics[width=\linewidth]{figures/pima/pima_score.png}
      \caption{\texttt{pima}}
      \label{fig:pima_score}
    \end{subfigure} % <-- added
    \begin{subfigure}{0.65\textwidth}
      \includegraphics[width=\linewidth]{figures/shuttle/shuttle_score.png}
      \caption{\texttt{shuttle}}
      \label{fig:shuttle_score}
    \end{subfigure} % <-- added
    \begin{subfigure}{0.65\textwidth}
      \includegraphics[width=\linewidth]{figures/wine/wine_score.png}
      \caption{\texttt{wine}}
      \label{fig:wine_score}
    \end{subfigure} % <-- added
\caption{Scoremaps of the importance value of the two most important features, according the RF feature ranking, in the space that surrounds the data distribution. 
Representation of the data with the inliers in form of a circle and the outliers in form of a star.}\label{fig:score_map}
\end{figure}









==> sections/sections_synthetic_datasets/Bisec3D.tex <==
\subsubsection*{{\ttfamily Bisec3D}}
In the dataset labeled as {\ttfamily Bisec3D}, detailed in Appendix \ref{sec:appendix-synthetic-data} and already used to show the \approach results visualization in Section \ref{sec:viz-explanations}, the anomalous data points are artificially positioned along the bisector of the subspace engendered by the initial three features. Outliers in this setting manifest as data points with anomaly values along the first three directions, namely Feature 0, Feature 1 and Feature 2. This hypothesis is confirmed by the observations presented in at Figure \ref{fig:GFI-Bisect-3d} where the top three rankings are nearly evenly distributed between the features on which the 3-dimensional bisector is defined. 

The importance is shared between Feature 0 and 1 but also Feature 2. This attribution is depicted in \ref{fig:Feat-imp-Bisect-3d}, where Feature 2 has a relevant Feature Importance Score. 
 
As stated in Section \ref{sec:viz-explanations},  Figure \ref{fig:Feat-imp-Bisect-3d} showcases the Scoremap, providing a visual representation of anomaly locations. It is evident that the anomalies associated with the first two features coincide with areas where the color changes within the map. This observation implies that identifying a distinct feature within which these anomalies reside is not possible, consistent with the overall assessment of global feature importance. A similar pattern emerges when examining Feature 2.

Regarding the model's performances in terms of Average Precision, as illustrated in Table \ref{tab:avg-prec-table}, the results demonstrate a notable improvement in the performance of the IF model when compared to the precedent \texttt{Xaxis} dataset. Furthermore, the EIF and \EIFplus models consistently maintain their high performance levels, and as a consequence confidence in the reliability of the interpretation results is provided. 


==> sections/sections_synthetic_datasets/Bisec3D_new.tex <==
\subsection*{{\ttfamily Bisect 3D}} \label{sec:Bisec3D-exp}

\subsubsection{Performance}
\ale{From the analysis presented in plot \ref{fig:Bisec3D_contamination_full}, we note that the DIF model struggles with accurately identifying the correct anomalies within the {\ttfamily Bisect3D} dataset (described in \ref{sec:appendix-synthetic-data}).  Conversely, all other models demonstrate the capability to detect perfectly anomalies once the contamination level dips below 0.06, while still maintaining high performance across all the levels of contamination. This observation underscores the robustness of these models in handling anomaly detection in datasets with low contamination rates.}
 \begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.49\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Bisec3D/Contamination/18-03-2024_14-29-02_bisect_3d_contamination_full_plot.pdf}
      \caption{Models evaluation, varying the contamination levels}
      \label{fig:Bisec3D_contamination_full}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.44\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Bisec3D/Contamination/19-03-2024_09-16-28_bisect_3d_EIF+_minus_EIF_precision_over_contamination.pdf}
      \caption{Difference between \EIFplus and EIF average precision}
      \label{fig:Bisec3D_contaminationEIFvsEIF+}
    \end{subfigure}\hfil % <-- added
\caption{Figure \ref{fig:Bisec3D_contamination_full} illustrates the average precision as the contamination level in the training set increases. Figure \ref{fig:Bisec3D_contaminationEIFvsEIF+} compares the performance graphs of EIF and \EIFplus, using the difference of their scores in various contamination levels.}
\label{fig:Bisec3D_contamination}

\end{figure}

\begin{table}[htbp]
\centering
%\caption{{\ttfamily Bisec3D} Precision Report}
\caption{Performances of 5 different Anomaly Detection models over {\ttfamily Bisec3D} are compared using classical Classification metrics. Moreover, the last two columns contain the average time for a fit and predict operation. The highest metric values and the lowest execution times are highlighted in bold}\label{tab:Bisec3D-perf}
\begin{tabular}{|c||ccc|ccc||cc|}
\toprule
\hline
& \multicolumn{3}{c|}{Scenario I} & \multicolumn{3}{c||}{Scenario II} & \multicolumn{2}{c|}{Time} \\
\hline
AD Model & Avg & Prec & ROC & Avg & Prec & ROC & fit & pred \\
& Prec &  & AUC & Prec &  & AUC & fit & pred \\
\hline
IF          & 0.95 & 0.85 & 0.91    & \textbf{1.00}& \textbf{1.00}& \textbf{1.00}& \textbf{0.08}& \textbf{0.008}\\
EIF         & \textbf{0.96}& \textbf{0.89}& \textbf{0.93}& 0.99& \textbf{1.00}& \textbf{1.00}& 0.09 & 0.02 \\
EIF+        & 0.93 & 0.71 & 0.84    & 0.99 & 0.99 & 0.99     & 0.097 & 0.01\\
DIF         & 0.30& 0.28& 0.60& 0.79& 0.72& 0.84& 1.84 & 1.44 \\
AE & 0.97 & 0.92& 0.95& \textbf{1.00}& \textbf{1.00}& \textbf{1.00} & 3.86 & 0.07 \\
\hline
\end{tabular}
\end{table}

\ale{From the analysis presented in Table \ref{tab:Bisec3D-perf}, it's evident that the IF, EIF, and \EIFplus models exhibit robust performance across both scenarios, effectively identifying anomalies within the {\ttfamily Bisect3D} dataset, as detailed in Appendix \ref{sec:appendix-synthetic-data}. In contrast, the DIF model encounters significant challenges in Scenario I, struggling to accurately detect anomalies. Moving to Scenario II, even if it increased its Average Precision score, it remains remarkably lower than the other models. Instead, the Anomaly AutoEncoder displays a perfect anomaly detection as the IF model.}


\subsubsection{Importance Plots}

\ale{The division of the dataset into two distinct scenarios does not significantly alter the relative importance of features, except for variations in the absolute scores of these importances. The results depicted in Figures \ref{fig:Bar-plot-Bisec3D-EXIFFI+-1}, \ref{fig:Score-plot-Bisec3D-EXIFFI+-1}, \ref{fig:Bar-plot-Bisec3D-EXIFFI+-2}, and \ref{fig:Score-plot-Bisec3D-EXIFFI+-2} align with the expected structure of the dataset, identifying features 0, 1, and 2 as the most crucial, each holding similar importance scores. Notably, the presence of multiple features contributing equally to the deviation of points from the dataset's normal distribution results in a smaller gap between scores of significant and less significant features. This contrast is evident when compared to observations from the {\ttfamily Xaxis} dataset shown in Figures \ref{fig:Score-plot-Xaxis-EXIFFI+-1} and \ref{fig:Score-plot-Xaxis-EXIFFI+-2}, where the disparity in importance scores between important and non important features is more pronounced.}

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Bisec3D/Importance_plots/12-03-2024_21-16-25_GFI_Bar_plot_bisect_3d_EXIFFI+_1.pdf}
      \caption{Score Plot {\ttfamily Bisec3D} Scenario I}
      \label{fig:Bar-plot-Bisec3D-EXIFFI+-1}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.27\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Bisec3D/Importance_plots/12-03-2024_21-16-26_GFI_Score_plot_bisect_3d_EXIFFI+_1.pdf}
      \caption{Bar Plot {\ttfamily Bisec3D} Scenario I}
      \label{fig:Score-plot-Bisec3D-EXIFFI+-1}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Bisec3D/Local_Scoremap/13-03-2024_09-44-04_importance_map_bisect_3d_EXIFFI+_1_feat_0_1.pdf}
      \caption{Scoremap {\ttfamily Bisec3D} Scenario I}
      \label{fig:Local-Bisec3D-EXIFFI+-1}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Bisec3D/Importance_plots/12-03-2024_21-15-59_GFI_Bar_plot_bisect_3d_EXIFFI+_2.pdf}
      \caption{Score Plot {\ttfamily Bisec3D} Scenario I}
      \label{fig:Bar-plot-Bisec3D-EXIFFI+-2}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.27\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Bisec3D/Importance_plots/12-03-2024_21-15-59_GFI_Score_plot_bisect_3d_EXIFFI+_2.pdf}
      \caption{Bar Plot {\ttfamily Bisec3D} Scenario II}
      \label{fig:Score-plot-Bisec3D-EXIFFI+-2}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Bisec3D/Local_Scoremap/13-03-2024_09-43-26_importance_map_bisect_3d_EXIFFI+_2_feat_0_1.pdf}
      \caption{Scoremap {\ttfamily Bisec3D} Scenario II}
      \label{fig:Local-Bisec3D-EXIFFI+-2}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot and Scoremap of the dataset {\ttfamily Bisect3D} in the two different Scenarios, using the ExIFFI algorithm applied to the \EIFplus model.}\label{fig:interpretation-Bisec3D}
\end{figure}

\subsubsection{Feature Selection}
\ale{In the Figures \ref{fig:interpretation-Bisec3D}  we can observe that the important features are preserved until the latter stages of feature selection, in fact the average precision remains high, underscoring the importance of these features in maintaining model accuracy. Conversely, when we consider the case in which we removed important features in the early phases of Feature Selection, there's a noticeable decrement in average precision with each step. In particular as soon as the three most relevant features are omitted (i.e. when the model considers 3 features or less) the Average Precision is very close to 0, highlighting the pivotal role that the selected important features play in the model's ability to predict anomalies.}

\begin{figure}[!ht] 
    \centering
    \hspace{0.05\textwidth}\textbf{IF} \hspace{0.29\textwidth} \textbf{EIF} \hspace{0.29\textwidth} \textbf{EIF+}
    % First row with vertical caption on the left
    \begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Ad-Hoc}}} % Adjust the parbox width as necessary for your caption text
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
              \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Bisec3D/Feature_Selection/08-05-2024_14-07-19_bisect_3d_EIF+_IF_EXIFFI_feature_selection_2.pdf}
              \caption{\approach applied to IF}
              \label{fig:Feat-Sel_Bisec3D_valEIF+_DIFFI_2}
            \end{subfigure}\hfil % <-- added
            \begin{subfigure}[t]{0.30\textwidth}
            \centering
              \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Bisec3D/Feature_Selection/08-05-2024_14-06-57_bisect_3d_EIF+_EXIFFI_feature_selection_2.pdf}
              \caption{\approach applied to EIF}
              \label{fig:Feat-Sel_Bisec3D_valEIF+_EXIFFI_2}
            \end{subfigure}\hfil % <-- added
            \begin{subfigure}[t]{0.30\textwidth}
            \centering
              \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Bisec3D/Feature_Selection/08-05-2024_14-02-06_bisect_3d_EIF+_EXIFFI+_feature_selection_2.pdf}
              \caption{\approach applied to \EIFplus}
              \label{fig:Feat-Sel_Bisec3D_valEIF+_EXIFFI+_2}
      \end{subfigure}
    \end{minipage}
\end{minipage}

% Second row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Post-Hoc}}} % Adjust as necessary
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
              \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Bisec3D/Feature_Selection/08-05-2024_14-07-41_bisect_3d_EIF+_IF_RandomForest_feature_selection_2.pdf}
              \caption{RandomForest fitted to IF}
              \label{fig:Feat-Sel_Bisec3D_valEIF+_IF_RandomForest_2}
            \end{subfigure}\hfil % <-- added
            \begin{subfigure}[t]{0.30\textwidth}
            \centering
              \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Bisec3D/Feature_Selection/08-05-2024_14-08-04_bisect_3d_EIF+_EIF_RandomForest_feature_selection_2.pdf}
              \caption{RandomForest fitted to EIF}
              \label{fig:Feat-Sel_Bisec3D_valEIF+_EIF_RandomForest_2}
            \end{subfigure}\hfil % <-- added
            \begin{subfigure}[t]{0.30\textwidth}
            \centering
              \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Bisec3D/Feature_Selection/08-05-2024_14-08-26_bisect_3d_EIF+_EIF+_RandomForest_feature_selection_2.pdf}
              \caption{RandomForest fitted to \EIFplus}
              \label{fig:Feat-Sel_Bisec3D_valEIF+_EIF+_RandomForest_2}
                   \end{subfigure}
            \end{minipage}
        \end{minipage}
      \caption{Feature Selection of the different Ad-Hoc and Post-Hoc methods applied to the 3 Isolation Forest models: IF, EIF and \EIFplus. The blue line is the values of average precision, calculated with the \EIFplus model in the Scenario II, dropping the most important feature at each step, the red line is the values of average precision dropping the least important feature at each step and the green line is the value of the feature selection dropping a random feature at each step.}\label{fig:feature_selections-Bisec3D}
\end{figure}



\ale{The Table \ref{tab:fs-tab-Bisec3D} shows consistent performance across interpretation algorithms and Scenarios, except for DIFFI and IF\_\approach in Scenario II, likely due to not selecting all key features, as seen in Figure \ref{fig:Feat-Sel_Bisec3D_valEIF+_DIFFI_2}. This highlights the importance of comprehensive Feature Selection for model accuracy. For what concerns the time performances the EIF and \EIFplus models are almost 10 times faster than the other methods considered in the analysis, proving again their computational efficiency.}

\begin{table}[htbp]
\centering
%\caption{Feature Selection Scores  {\ttfamily Bisec3D}}
\caption{Quantitative evaluation of the effectiveness of 6 different interpretation algorithms on {\ttfamily Bisec3D} through the $AUC_{FS}$ metric, introduced in \ref{sec:interpr_evaluat}. In the last column the average time taken by the different models to produce the importance scores is reported. The highest $AUC_{FS}$ and lowest Importance time values are highlighted in bold.}\label{tab:fs-tab-Bisec3D}
\begin{tabular}{|c||c|c|c|c||c|}
\toprule
\hline
&\multicolumn{2}{c|}{Evaluation with EIF}&\multicolumn{2}{c||}{Evaluation with \EIFplus}&\\
\hline
& Scenario I & Scenario II & Scenario I & Scenario II & Time\\

 Algorithm & $AUC_{FS}$  & $AUC_{FS}$ & $AUC_{FS}$  & $AUC_{FS}$ &  \\
\hline
DIFFI         & 3.424      & 2.79   & 3.327     & 2.834    &       0.56 \\
IF\_\approach         & \textbf{3.452}& 3.011& 3.466& 3.011  &       0.18 \\
EIF\_\approach        & 3.397& 3.011& 3.382& 3.028&         \textbf{0.07}\\
\EIFplus\_\approach      & 3.421& 3.021& \textbf{3.486}& 3.032&       \textbf{0.07}\\
IF\_RF        & 3.411& \textbf{3.054}& 3.444& \textbf{3.034}&    0.68 \\
EIF\_RF       &  3.445& 3.034& 3.432& 3.016&                0.68 \\
\EIFplus\_RF      & 3.393& 3.047& 3.408& 3.016&         0.68 \\
\hline
\end{tabular}
\end{table}



==> sections/sections_synthetic_datasets/Bisec3D_prop_new.tex <==
\subsection*{{\ttfamily Bisect 3D prop}} \label{sec:Bisec3D-prop-exp}

\davide{Subsection describing the {\ttfamily Bisect 3D Prop} synthetic dataset.}

\subsubsection{Performance}

 \begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.49\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Bisect3D_prop/Contamination/02-09-2024_11-18-19_bisect_3d_prop_contamination_full_plot.pdf}
      \caption{Models evaluation, varying the contamination levels}
      \label{fig:Bisec3D_prop_contamination_full}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.44\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Bisect3D_prop/Contamination/02-09-2024_18-01-16_bisect_3d_prop_EIF+_minus_EIF_precision_over_contamination.pdf}
      \caption{Difference between \EIFplus and EIF average precision}
      \label{fig:Bisec3D_prop_contaminationEIFvsEIF+}
    \end{subfigure}\hfil % <-- added
\caption{Figure \ref{fig:Bisec3D_prop_contamination_full} illustrates the average precision as the contamination level in the training set increases. Figure \ref{fig:Bisec3D_prop_contaminationEIFvsEIF+} compares the performance graphs of EIF and \EIFplus, using the difference of their scores in various contamination levels.}
\label{fig:Bisec3D_prop_contamination}
\end{figure}

\begin{comment}
To update with the bisect_3d_prop metric values 
\end{comment}

\begin{table}[htbp]
\centering
%\caption{{\ttfamily Bisec3D} Precision Report}
\caption{Performances of 5 different Anomaly Detection models over {\ttfamily Bisec3D} are compared using classical Classification metrics. Moreover, the last two columns contain the average time for a fit and predict operation. The highest metric values and the lowest execution times are highlighted in bold}\label{tab:Bisec3D-perf}
\begin{tabular}{|c||ccc|ccc||cc|}
\toprule
\hline
& \multicolumn{3}{c|}{Scenario I} & \multicolumn{3}{c||}{Scenario II} & \multicolumn{2}{c|}{Time} \\
\hline
AD Model & Avg & Prec & ROC & Avg & Prec & ROC & fit & pred \\
& Prec &  & AUC & Prec &  & AUC & fit & pred \\
\hline
IF          & 0.95 & 0.85 & 0.91    & \textbf{1.00}& \textbf{1.00}& \textbf{1.00}& \textbf{0.08}& \textbf{0.008}\\
EIF         & \textbf{0.96}& \textbf{0.89}& \textbf{0.93}& 0.99& \textbf{1.00}& \textbf{1.00}& 0.09 & 0.02 \\
EIF+        & 0.93 & 0.71 & 0.84    & 0.99 & 0.99 & 0.99     & 0.097 & 0.01\\
DIF         & 0.30& 0.28& 0.60& 0.79& 0.72& 0.84& 1.84 & 1.44 \\
AE & 0.97 & 0.92& 0.95& \textbf{1.00}& \textbf{1.00}& \textbf{1.00} & 3.86 & 0.07 \\
\hline
\end{tabular}
\end{table}

\subsubsection{Importance Plots}

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Bisect3D_prop/Importance_plots/02-09-2024_09-12-37_GFI_Bar_plot_bisect_3d_prop_EXIFFI+_1.pdf}
      \caption{Score Plot {\ttfamily Bisec3D Prop} Scenario I}
      \label{fig:Bar-plot-Bisec3D-prop-EXIFFI+-1}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.27\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Bisect3D_prop/Importance_plots/02-09-2024_09-12-38_GFI_Score_plot_bisect_3d_prop_EXIFFI+_1.pdf}
      \caption{Bar Plot {\ttfamily Bisec3D Prop} Scenario I}
      \label{fig:Score-plot-Bisec3D-prop-EXIFFI+-1}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Bisect3D_prop/Local_Scoremap/02-09-2024_09-18-38_importance_map_bisect_3d_prop_EIF+_EXIFFI+_1_feat_0_1.pdf}
      \caption{Scoremap {\ttfamily Bisec3D Prop} Scenario I}
      \label{fig:Local-Bisec3D-prop-EXIFFI+-1}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Bisect3D_prop/Importance_plots/02-09-2024_08-57-49_GFI_Score_plot_bisect_3d_prop_EXIFFI+_2.pdf}
      \caption{Score Plot {\ttfamily Bisec3D Prop} Scenario I}
      \label{fig:Bar-plot-Bisec3D-prop-EXIFFI+-2}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.27\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Bisec3D/Importance_plots/12-03-2024_21-15-59_GFI_Score_plot_bisect_3d_EXIFFI+_2.pdf}
      \caption{Bar Plot {\ttfamily Bisec3D Prop} Scenario II}
      \label{fig:Score-plot-Bisec3D-prop-EXIFFI+-2}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Bisec3D/Local_Scoremap/13-03-2024_09-43-26_importance_map_bisect_3d_EXIFFI+_2_feat_0_1.pdf}
      \caption{Scoremap {\ttfamily Bisec3D Prop} Scenario II}
      \label{fig:Local-Bisec3D-prop-EXIFFI+-2}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot and Scoremap of the dataset {\ttfamily Bisect3D} in the two different Scenarios, using the ExIFFI algorithm applied to the \EIFplus model.}\label{fig:interpretation-Bisec3D-prop}
\end{figure}

\subsubsection{Feature Selection}

==> sections/sections_synthetic_datasets/Bisec6D.tex <==
\subsubsection*{{\ttfamily Bisec6D}}
\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}{0.52\textwidth}
      \includegraphics[width=\linewidth]{figures/global_synthetic_new/GFI_Bisect_6d_synt.pdf}
      \caption{Bar Plot {\ttfamily Bisec6d}}
      \label{fig:GFI-Bisect-6d}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.40\textwidth}
      \includegraphics[width=\linewidth]{figures/global_synthetic_new/Feat_bar_plot_Bisect_6d.pdf}
      \caption{Score Plot {\ttfamily Bisec6d}}
      \label{fig:Feat-imp-Bisect-6d}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]        {figures/scoremaps_synthetic/Local_Importance_Scoremap_Bisect_6d_no_scaled.png}
        \caption{Scoremap {\ttfamily Bisec66d}}
        \label{fig:Imp-scoremap-Bisect-6d}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot, and Scoremap {\ttfamily Bisec6d}}
\label{fig:Bisect-6d}
\end{figure}

Within the dataset denoted as {\ttfamily Bisec6D}, detailed in Appendix \ref{sec:appendix-synthetic-data}, anomalies are strategically positioned along the bisector line encompassing the entire feature space. This spatial arrangement makes it possible to have outliers with atypical values along every direction.  Moreover, this scenario is characterized by the absence of normal features meaning that each feature is potentially informative and their composition determine the direction of the anomalies. This intricate configuration engenders considerable complexity for the model, rendering the identification of a singular globally preeminent feature a complex task.

The outcome is perceptible in Figure \ref{fig:GFI-Bisect-6d}, wherein the absence of a dominant feature is observed. Instead, all features have been positioned in the topmost rank throughout the experimental runs. Upon an examination of the Score Plot featured in Figure \ref{fig:Feat-imp-Bisect-6d}, Feature 1 emerges as the most salient attribute across the diverse iterations. However it is noteworthy that Importance scores are very close among all attributes. The ranking shown here will likely change if a new instance of the model is used to perform the experiment. 

The Figure \ref{fig:Imp-scoremap-Bisect-6d} illustrates the Scoremap of the {\ttfamily Bisec6d} dataset, depicting the importance score distribution within the Feature 0 and 1 subspace. This representation closely resembles what we've observed in the {\ttfamily Bisec} and {\ttfamily Bisec3d} datasets, where anomalies are consistently located in regions where the most important feature transitions from 0 to 1. Consequently, the importance scores tend to be evenly distributed between these two features.

Given that the dataset projection into every possible pair of 2-feature subspace remains consistent, it's evident that anomalies don't exhibit a preference for specific features. Instead, the global importance scores appear to be relatively uniform across all features.


In the context of the model's performances presented in Table \ref{tab:avg-prec-table}, the observed results exhibit consistently high values. This increase in performance can be attributed to the multidimensional nature of the anomalies. In such scenarios, the Isolation Forest (IF) algorithm excels in segregating anomalies from the normal data points, achieving multiple instances of successful separations within the generated trees as described in Section \ref{performance}.

Notably, the exceptionally high Average Precision values indicate the reliability of the algorithm's classifications.

==> sections/sections_synthetic_datasets/Bisec6D_new.tex <==
\subsection*{{\ttfamily Bisect 6D}} \label{sec:Bisect6D-exp}

\subsubsection{Performance}
\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.49\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Bisec6D/Contamination/18-03-2024_15-09-29_bisect_6d_contamination_full_plot.pdf}
      \caption{Models evaluation, varying the contamination levels}
      \label{fig:Bisec6D_contamination_full}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.44\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Bisec6D/Contamination/19-03-2024_09-16-36_bisect_6d_EIF+_minus_EIF_precision_over_contamination.pdf}
      \caption{Difference between \EIFplus and EIF average precision}
      \label{fig:Bisec6D_contaminationEIFvsEIF+}
    \end{subfigure}\hfil % <-- added
\caption{Figure \ref{fig:Bisec6D_contamination_full} illustrates the average precision as the contamination level in the training set increases. Figure \ref{fig:Bisec6D_contaminationEIFvsEIF+} compares the performance graphs of EIF and \EIFplus, using the difference of their scores in various contamination levels.}
\label{fig:Bisec6D_contamination}
\end{figure}

\ale{The contamination plot in Figure \ref{fig:Bisec6D_contamination_full} reveals that all algorithms, except for DIF, have impressive performances. As the contamination level decreases, both EIF and \EIFplus models exhibit a slight improvement in their ability to detect anomalies, ultimately achieving near-perfect anomaly detection.}

\ale{Table \ref{tab:Bisec6D-perf} shows observations from the contamination plots, indicating that, across both Scenarios, all algorithms exhibit high performance levels, with the notable exception of DIF. Specifically, the IF model and the Autoencoder stand out as the most effective across both scenarios, demonstrating their superior anomaly detection capabilities within the {\ttfamily Bisec6D} dataset context. Observing the execution time for a single fit and predict operation IF, EIF and \EIFplus showcase the most efficient performances.}

\begin{table}[htbp]
\centering
%\caption{{\ttfamily Bisec6D} Precision Report}
\caption{Performances of 5 different Anomaly Detection models over {\ttfamily Bisec6D} are compared using classical Classification metrics. Moreover, the last two columns contain the average time for a fit and predict operation. The highest metric values and the lowest execution times are highlighted in bold}\label{tab:Bisec6D-perf}
\begin{tabular}{|c||ccc|ccc||cc|}
\toprule
\hline
& \multicolumn{3}{c|}{Scenario I} & \multicolumn{3}{c||}{Scenario II} & \multicolumn{2}{c|}{Time} \\
\hline
AD Model & Avg & Prec & ROC & Avg & Prec & ROC & fit & pred \\
& Prec &  & AUC & Prec &  & AUC & fit & pred \\
\hline
IF          & \textbf{0.99} & \textbf{0.98} & 0.98    & \textbf{1.00} & \textbf{1.00} & \textbf{1.00}    & \textbf{0.08} & \textbf{0.008} \\
EIF         & 0.96 & 0.92 & 0.95    & 0.99 & 0.99 & 0.99     & 0.09 & 0.01 \\
\EIFplus        & 0.93 & 0.81 & 0.89    & 0.99 & \textbf{1.00} & \textbf{1.00}     & 0.1 & 0.01 \\
DIF         & 0.19 & 0.16& 0.53       & 0.36& 0.32& 0.62& 1.62 & 1.29 \\
AE & 0.97& 0.95& 0.97& \textbf{1.00}& \textbf{1.00}& \textbf{1.00}& 3.89 & 0.09 \\
\hline
\end{tabular}
\end{table}


\subsubsection{Importance Plots} \label{sec:imp-bisect6d}

\ale{Since the {\ttfamily Bisect6D} is crafted in such a way that the anomalies deviate along all the directions. As a result the Bar Plot, in Figure \ref{fig:Bar-plot-Bisec6D-EXIFFI+-2} and \ref{fig:Bar-plot-Bisec6D-EXIFFI+-1}, shows as most important feature a blend of the six different features and the scores are very similar, as observable in Figures \ref{fig:Score-plot-Bisec6D-EXIFFI+-1} and \ref{fig:Score-plot-Bisec3D-EXIFFI+-2}, underlying the characteristics of the dataset.}

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Bisec6D/Importance_plots/13-03-2024_14-10-21_GFI_Bar_plot_bisect_6d_EXIFFI+_1.pdf}
      \caption{Score Plot {\ttfamily Bisec6D} Scenario I}
      \label{fig:Bar-plot-Bisec6D-EXIFFI+-1}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.27\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Bisec6D/Importance_plots/13-03-2024_14-09-59_GFI_Score_plot_bisect_6d_EXIFFI+_2.pdf}
      \caption{Bar Plot {\ttfamily Bisec6D} Scenario I}
      \label{fig:Score-plot-Bisec6D-EXIFFI+-1}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Bisec6D/Local_Scoremap/13-03-2024_14-56-19_importance_map_bisect_6d_EXIFFI+_1_feat_0_1.pdf}
      \caption{Scoremap {\ttfamily Bisec6D} Scenario I}
      \label{fig:Local-Bisec6D-EXIFFI+-1}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Bisec6D/Importance_plots/13-03-2024_14-09-59_GFI_Bar_plot_bisect_6d_EXIFFI+_2.pdf}
      \caption{Score Plot {\ttfamily Bisec6D} Scenario II}
      \label{fig:Bar-plot-Bisec6D-EXIFFI+-2}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.27\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Bisec6D/Importance_plots/13-03-2024_14-09-59_GFI_Score_plot_bisect_6d_EXIFFI+_2.pdf}
      \caption{Bar Plot {\ttfamily Bisec6D} Scenario II}
      \label{fig:Score-plot-Bisec6D-EXIFFI+-2}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Bisec6D/Local_Scoremap/13-03-2024_14-56-03_importance_map_bisect_6d_EXIFFI+_2_feat_0_1.pdf}
      \caption{Scoremap {\ttfamily Bisec6D} Scenario II}
      \label{fig:Local-Bisec6D-EXIFFI+-2}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot and Scoremap for {\ttfamily Bisect6D}  in the two different Scenarios, using the ExIFFI algorithm applied to the \EIFplus model.}\label{fig:interpretation-Bisec6D}
\end{figure}

\subsubsection{Feature Selection}

\ale{The Feature Selection plots reveal a consistent decrease in average precision, irrespective of the feature selection strategy employed: least important first (red line), most important first (blue line), or selected randomly (green line). This is a consequence of the fact that, as outlined in Section \ref{sec:imp-bisect6d}, the relevance in detecting anomalies is evenly shared across all features thus all possible importance ranking will produce the same outcomes. In this peculiar situation the decreasing trend of the Average Precision metric can be justified by the fact that, as features are removed, the model is equipped with less information to identify anomalous points from normal ones leading to a degradation of its performances.}

\begin{figure}[!ht] 
    \centering
    \hspace{0.05\textwidth}\textbf{IF} \hspace{0.29\textwidth} \textbf{EIF} \hspace{0.29\textwidth} \textbf{EIF+}
    % First row with vertical caption on the left
    \begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Ad-Hoc}}} % Adjust the parbox width as necessary for your caption text
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
    \centering
          \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Bisec6D/Feature_Selection/08-05-2024_14-37-46_bisect_6d_EIF+_IF_EXIFFI_feature_selection_2.pdf}
          \caption{\approach applied to IF}
          \label{fig:Feat-Sel_Bisec6D_valEIF+_DIFFI_2}
        \end{subfigure}\hfil % <-- added
        \begin{subfigure}[t]{0.30\textwidth}
        \centering
          \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Bisec6D/Feature_Selection/08-05-2024_14-37-24_bisect_6d_EIF+_EXIFFI_feature_selection_2.pdf}
          \caption{\approach applied to EIF}
          \label{fig:Feat-Sel_Bisec6D_valEIF+_EXIFFI_2}
        \end{subfigure}\hfil % <-- added
        \begin{subfigure}[t]{0.30\textwidth}
        \centering
          \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Bisec6D/Feature_Selection/08-05-2024_14-37-01_bisect_6d_EIF+_EXIFFI+_feature_selection_2.pdf}
          \caption{\approach applied to \EIFplus}
          \label{fig:Feat-Sel_Bisec6D_valEIF+_EXIFFI+_2}
          \end{subfigure}
        \end{minipage}
    \end{minipage}
    
% Second row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Post-Hoc}}} % Adjust as necessary
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
        \centering
          \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Bisec6D/Feature_Selection/08-05-2024_14-38-08_bisect_6d_EIF+_IF_RandomForest_feature_selection_2.pdf}
          \caption{RandomForest fitted to IF}
          \label{fig:Feat-Sel_Bisec6D_valEIF+_IF_RandomForest_2}
        \end{subfigure}\hfil % <-- added
        \begin{subfigure}[t]{0.30\textwidth}
        \centering
          \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Bisec6D/Feature_Selection/08-05-2024_14-38-31_bisect_6d_EIF+_EIF_RandomForest_feature_selection_2.pdf}
          \caption{RandomForest fitted to EIF}
          \label{fig:Feat-Sel_Bisec6D_valEIF+_EIF_RandomForest_2}
        \end{subfigure}\hfil % <-- added
        \begin{subfigure}[t]{0.30\textwidth}
        \centering
          \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Bisec6D/Feature_Selection/08-05-2024_14-38-53_bisect_6d_EIF+_EIF+_RandomForest_feature_selection_2.pdf}
          \caption{RandomForest fitted to \EIFplus}
          \label{fig:Feat-Sel_Bisec6D_valEIF+_EIF+_RandomForest_2}
            \end{subfigure}
        \end{minipage}
    \end{minipage}
  \caption{Feature Selection of the different Ad-Hoc and Post-Hoc methods applied to the 3 Isolation Forest models: IF, EIF and \EIFplus. The blue line is the values of average precision, calculated with the \EIFplus model in the Scenario II, dropping the most important feature at each step, the red line is the values of average precision dropping the least important feature at each step and the green line is the value of the feature selection dropping a random feature at each step.}\label{fig:feature_selections-Bisec6D}
\end{figure}

In Table \ref{tab:fs-tab-Bisec6D}  the $AUC_{FS}$ metric values obtained by the different interpretation approaches tested are reported. As already easily noticeable from the plots contained in Figure \ref{fig:feature_selections-Bisec6D}  the quantitative results of the Feature Selection proxy task obtained by the different methods are comparable and none of them stands out as significantly better then the others. 

Notably the proposed approach \approach showcases the smaller execution times for the computation of the importance scores being almost 10 times faster than post-hoc approached like RandomForest or ad-hoc approaches like DIFFI, making it a good choice for the application of Explainable Anomaly Detection in a practical setting. 

\begin{table}[htbp]
\centering
\caption{Quantitative evaluation of the effectiveness of 6 different interpretation algorithms on {\ttfamily Bisec6D} through the $AUC_{FS}$ metric, introduced in \ref{sec:interpr_evaluat}. In the last column the average time taken by the different models to produce the importance scores is reported. The highest $AUC_{FS}$ and lowest Importance time values are highlighted in bold.}\label{tab:fs-tab-Bisec6D}
\begin{tabular}{|c||c|c|c|c||c|}
\toprule
\hline
&\multicolumn{2}{c|}{Evaluation with EIF}&\multicolumn{2}{c||}{Evaluation with \EIFplus}&\\
\hline
& Scenario I & Scenario II & Scenario I & Scenario II & Time\\

 Algorithm & $AUC_{FS}$  & $AUC_{FS}$ & $AUC_{FS}$  & $AUC_{FS}$ &  \\
\hline
DIFFI         & 0.026      & -0.045   & -0.027     & -0.128    &       0.55 \\
IF\_\approach        & 0.181& 0.067& \textbf{0.189}& 0.095&         0.16 \\
EIF\_\approach        & 0.088& \textbf{0.118}& 0.057& 0.13&         \textbf{0.07} \\
\EIFplus\_\approach       & 0.167& 0.078& 0.004& 0.081&       \textbf{0.07} \\
IF\_RF        & \textbf{0.198}& 0.107& 0.078& \textbf{0.119}&    0.67 \\
EIF\_RF       &  0.162& 0.067& 0.057& 0.064&                0.67 \\
\EIFplus\_RF      & 0.167& 0.044& 0.081& 0.077&         0.67 \\
\hline
\end{tabular}
\end{table}

\ale{Table \ref{tab:fs-tab-Bisec6D} displays $AUC_{FS}$ scores, indicating similar outcomes across different feature importance methods, except for DIFFI, which slightly underperforms compared to the others.}





==> sections/sections_synthetic_datasets/Bisec_new.tex <==
\subsection*{{\ttfamily Bisec}}

\subsubsection{Performance}

\ale{Figure \ref{fig:Bisec_contamination_full} reports the Average Precision of various AD models in relation to different percentages of outliers inserted in the training set and taking part to the fitting process. Similarly to what can be observed in the {\ttfamily Bisec3D} dataset, described in \ref{sec:Bisec3D-exp}, the entirety of the models shows comparable results except for DIF where the Average Precision suffers a significant drop as outliers are progressively included as training samples. The EIF and \EIFplus models emerge as the ones with the highest metric values and their performances are comparable as shown in Figure \ref{fig:Bisec_contaminationEIFvsEIF+}.}

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.49\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Bisec/Contamination/25-03-2024_10-46-56_bisect_contamination_full_plot.pdf}
      \caption{Models evaluation, varying the contamination levels}
      \label{fig:Bisec_contamination_full}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.44\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Bisec/Contamination/25-03-2024_10-47-12_bisect_EIF+_minus_EIF_precision_over_contamination.pdf}
      \caption{Difference between \EIFplus and EIF average precision}
      \label{fig:Bisec_contaminationEIFvsEIF+}
    \end{subfigure}\hfil % <-- added
\caption{Figure \ref{fig:Bisec_contamination_full} illustrates the average precision as the contamination level in the training set increases. Figure \ref{fig:Bisec_contaminationEIFvsEIF+} compares the performance graphs of EIF and \EIFplus, using the difference of their scores in various contamination levels.}
\label{fig:Bisec_contamination}
\end{figure}

\ale{Table \ref{tab:Bisec_perf}  offers a more detailed overview of the performances of the Anomaly Detection models considered focusing on the comparison between Scenario I (i.e. all the outliers inserted in the training set) and Scenario II (i.e. training set composed of only inliers). After a careful analysis of the values reported on the table it is possible to conclude about the superiority of the EIF and \EIFplus models, that achieve excellent results both in terms of precision in detecting anomalies and time efficiency. }

\begin{table}[htbp]
\begin{minipage}[t]{0.46\textwidth}
\strut\vspace*{-\baselineskip}\newline
\resizebox{\textwidth}{!}{
\begin{tabular}{|c||ccc|ccc||cc|}
\toprule
\hline
&\multicolumn{3}{c|}{Scenario I}&\multicolumn{3}{c||}{Scenario II}&\multicolumn{2}{c|}{Time}\\
\hline
AD Model& Avg & Prec & ROC & Avg & Prec & ROC & fit & pred \\
 & Prec &  & AUC & Prec &  & AUC &  &  \\
\hline
IF          & 0.75& 0.74& 0.85& 0.99& 0.95& 0.97& \textbf{0.05}& \textbf{0.006}\\
EIF         & 0.97& 0.91& 0.95& 0.99& 1.0& 1.0& \textbf{0.05}& 0.06\\
EIF+        & 0.94& 0.83& 0.9& \textbf{1.0}& \textbf{1.0}& \textbf{1.0}& \textbf{0.05}& 0.07\\
DIF         & 0.16& 0.2& 0.56& 0.85& 0.78& 0.87& 1.54& 1.21\\
AE & 0.89& 0.82& 0.9& 1.0& 1.0& 1.0& 3.77& 0.06\\
\hline
\end{tabular}}
\vspace{0.41cm}
\caption{Performances of 5 different Anomaly Detection models over {\ttfamily Bisec} are compared using classical Classification metrics. Moreover the last two columns contain the average time for a fit and predict operation. The highest metric values and the lowest execution times are highlighted in bold}\label{tab:Bisec_perf}
\end{minipage}
\hfill
\begin{minipage}[t]{0.46\textwidth}
\strut\vspace*{-\baselineskip}\newline
\resizebox{\textwidth}{!}{
\begin{tabular}{|c||c|c|c|c||c|}
\toprule
\hline
&\multicolumn{2}{c|}{Evaluation with EIF}&\multicolumn{2}{c||}{Evaluation with \EIFplus}&\\
\hline
& Scenario I & Scenario II & Scenario I & Scenario II & Time\\

 Algorithm & $AUC_{FS}$  & $AUC_{FS}$ & $AUC_{FS}$  & $AUC_{FS}$ &  \\
\hline
DIFFI                & 4.121& 2.925& \textbf{4.166}& 2.924& 0.34\\
IF\_\approach        & 4.137& \textbf{3.842}& 4.12& 3.828& \textbf{0.16}\\
EIF\_\approach       & \textbf{4.152}& 3.844& 4.042& 3.833& \textbf{0.16}\\
\EIFplus\_\approach  & 4.077& 3.827& 4.052& 3.833& \textbf{0.16}\\
IF\_RF               & 4.019& 3.828& 3.93& 3.83& 0.66\\
EIF\_RF              & 4.057& 3.834& 3.957& \textbf{3.841}& 0.66\\
EIF+\_RF             & 4.029& 3.832& 4.012& 3.832& 0.66\\
\hline
\end{tabular}}
\caption{Quantitative evaluation of the effectiveness of 6 different interpretation algorithms on {\ttfamily Bisec} through the $AUC_{FS}$ metric, introduced in \ref{sec:interpr_evaluat}. In the last column the average time taken by the different models to produce the importance scores is reported. The highest $AUC_{FS}$ and lowest Importance time values are highlighted in bold.}\label{tab:fs-tab-Bisec}
\end{minipage}
\end{table}

\subsubsection{Importance Plots}

\ale{The newly introduced \approach+ interpretation model is evaluated through the plots presented in Figure \ref{fig:interpretation-Bisec}. As expected, considering how this synthetic dataset was constructed, it is possible to select two relevant features (i.e. Feature 0 and 1) with similar importance scores that stand out with the respect to the ones of other variables contained in the dataset, as represented in Figures \ref{fig:Feat-imp-Bisec} and \ref{fig:Feat-imp-Bisec-split}. The Local Scoremaps, displayed in Figures \ref{fig:Local-Bisec} and \ref{fig:Local-Bisec-split}, provides a better visual explanation on how the anomalies and importance scores are distributed in the feature space.}

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Bisec/Importance_plots/25-03-2024_11-17-00_GFI_Bar_plot_bisect_EXIFFI+_1.pdf}
      \caption{Bar Plot {\ttfamily Bisec} Scenario I}
      \label{fig:GFI-Bisec}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.27\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Bisec/Importance_plots/25-03-2024_11-17-00_GFI_Score_plot_bisect_EXIFFI+_1.pdf}
      \caption{Score Plot {\ttfamily Bisec} Scenario I}
      \label{fig:Feat-imp-Bisec}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Bisec/Local_Scoremap/07-03-2024_16-36-58_importance_map_bisect_EXIFFI+_1.pdf}
      \caption{Scoremap {\ttfamily Bisec} Scenario I}
      \label{fig:Local-Bisec}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Bisec/Importance_plots/25-03-2024_11-17-00_GFI_Bar_plot_bisect_EXIFFI+_1.pdf}
      \caption{Bar Plot {\ttfamily Bisec} Scenario II}
      \label{fig:GFI-Bisec-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.27\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Bisec/Importance_plots/25-03-2024_11-19-21_GFI_Score_plot_bisect_EXIFFI+_2.pdf}
      \caption{Score Plot {\ttfamily Bisec} Scenario II}
      \label{fig:Feat-imp-Bisec-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Bisec/Local_Scoremap/07-03-2024_16-36-41_importance_map_bisect_EXIFFI+_2.pdf}
      \caption{Scoremap {\ttfamily Bisec} Scenario II}
      \label{fig:Local-Bisec-split}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot and Scoremap for {\ttfamily Bisec} in the two different Scenarios, using the ExIFFI algorithm applied to the \EIFplus model.}\label{fig:interpretation-Bisec}
\end{figure}

\subsubsection{Feature Selection} \label{sec:Bisec-fs}

\ale{The plots obtained as a result of the application of the Unsupervised Feature Selection proxy task, represented in Figure \ref{fig:fs-interpretation-Bisec}, present a similar behavior. For what concerns the Feature Selection approach in which at every step the least important feature is excluded (i.e. red line) the Average Precision obtains constantly a perfect score of 1. On the the other hand, if attributes are removed starting from the most relevant one the precision drops significantly after both Feature 0 and Feature 1 are excluded, testifying the importance of these attributes, without which the model performances experience a dramatic degradation.}

\begin{figure}[!ht] 
\centering
\hspace{0.05\textwidth}\textbf{IF} \hspace{0.29\textwidth} \textbf{EIF} \hspace{0.29\textwidth} \textbf{EIF+}
% First row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Ad-Hoc}}} % Adjust the parbox width as necessary for your caption text
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Bisec/Feature_Selection/08-05-2024_14-53-54_bisect_EIF+_IF_EXIFFI_feature_selection_2.pdf}
            \caption{\approach applied to IF}
            \label{fig:Feat-Sel_Bisec_valEIF+_DIFFI_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Bisec/Feature_Selection/08-05-2024_14-53-32_bisect_EIF+_EXIFFI_feature_selection_2.pdf}
            \caption{\approach applied to EIF}
            \label{fig:Feat-Sel_Bisec_valEIF+_EXIFFI_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Bisec/Feature_Selection/08-05-2024_14-53-10_bisect_EIF+_EXIFFI+_feature_selection_2.pdf}
            \caption{\approach applied to \EIFplus}
            \label{fig:Feat-Sel_Bisec_valEIF+_EXIFFI+_2}
        \end{subfigure}
    \end{minipage}
\end{minipage}

\vspace{5mm} % Space between rows

% Second row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Post-Hoc}}} % Adjust as necessary
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Bisec/Feature_Selection/08-05-2024_14-54-16_bisect_EIF+_IF_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to IF}
            \label{fig:Feat-Sel_Bisec_valEIF+_IF_RandomForest_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Bisec/Feature_Selection/08-05-2024_14-54-38_bisect_EIF+_EIF_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to EIF}
            \label{fig:Feat-Sel_Bisec_valEIF+_EIF_RandomForest_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Bisec/Feature_Selection/08-05-2024_14-55-00_bisect_EIF+_EIF+_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to \EIFplus}
            \label{fig:Feat-Sel_Bisec_valEIF+_EIF+_RandomForest_2}
        \end{subfigure}
    \end{minipage}
\end{minipage}

\caption{Feature Selection of the different Ad-Hoc and Post-Hoc methods applied to the 3 Isolation Forest models: IF, EIF and \EIFplus. The blue line is the values of average precision, calculated with the \EIFplus model in the Scenario II, dropping the most important feature at each step, the red line is the values of average precision dropping the least important feature at each step and the green line is the value of the feature selection dropping a random feature at each step.}\label{fig:fs-interpretation-Bisec}
\end{figure}

\ale{Various interpretation algorithms are quantitatively compared through the usage of the $AUC_{FS}$ metric, whose values are reported in Table \ref{tab:fs-tab-Bisec} . Because of the similarity across the plots observed in \ref{sec:Bisec-fs} the values of  $AUC_{FS}$ are comparable, thus all the models are valid choices. If a selection has to be made in order to use one of the cited models in a practical application the choice would fall on the proposed \approach and \approach+ that achieve a significant speed up in the computation of the importance scores with the respect to the other models.} 




==> sections/sections_synthetic_datasets/Xaxis.tex <==
\subsubsection*{{\ttfamily Xaxis}}

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/global_synthetic_new/GFI_Xaxis_synt.pdf}
      \caption{Bar Plot {\ttfamily Xaxis}}
      \label{fig:GFI-Xaxis}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.40\textwidth}
      \includegraphics[width=\linewidth]{figures/global_synthetic_new/Feat_bar_plot_Xaxis.pdf}
      \caption{Score Plot {\ttfamily Xaxis}}
      \label{fig:Feat-imp-Xaxis}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/scoremaps_synthetic/Local_Importance_Scoremap_Xaxis_no_scaled.png}
        \caption{Scoremap {\ttfamily Xaxis}}
        \label{fig:Imp-scoremap-Xaxis}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot and Scoremap {\ttfamily Xaxis}}
\label{fig:Xaxis}
\end{figure}

The first dataset considered is {\ttfamily Xaxis}. As described in Appendix \ref{sec:appendix-synthetic-data}, the name comes from the fact that anomalous data points are exclusively along the x-axis, corresponding to Feature 0.

As expected, the model can select Feature 0 as the most relevant across all iterations, as evidenced in Figure \ref{fig:GFI-Xaxis}.  Conversely, there is not a certain and robust result of other features selected in the rankings. Moreover, looking at the Score Plot in Figure \ref{fig:Feat-imp-Xaxis} it can be seen that the Importance Score of Feature 0 is much higher than all the others confirming the dominance of the feature in this configuration.

As shown in Figure \ref{fig:Imp-scoremap-Xaxis}, the orange star points denoting the anomalies are dispersed along Feature 0, displaying a distinct separation from the central cluster comprising the blue dots, which are the inlier observations. This observation serves as graphical and geometrical evidence of the anomalous nature of the dataset distributed along Feature 0.
The points on the scoremap of the space exhibit a clear pattern: as we consider the points more closely to a normal distribution, the pixels have a lighter color. The greater the deviation of Feature 1 from the conter of the distribution, the more intense the red color becomes. Conversely, when Feature 1 follows a normal distribution and Feature 0 deviates from it, the colors shift toward red.
What can be deduced from this map is that anomalous data points predominantly cluster in regions where the color appears blue, indicating a higher anomaly score for Feature 0. Therefore, on average, Feature 0 appears to be the most significant factor in order to identify anomalies.

In Table \ref{tab:avg-prec-table} the Average Precision values for the {\ttfamily Xaxis} dataset can be found. As discussed in Section \ref{performance}, it is evident that overall the scores are notably low in the case of the IF model. This phenomenon can be attributed to the presence of anomalies solely along one specific feature. Consequently, the IF model encounters significant challenges in detecting these anomalies, given their proximity to the anomaly score artifacts mentioned in Section \ref{sec:IFvsEIF}.

In contrast, both EIF and \EIFplus models demonstrate exceptional performance, effectively addressing the limitations observed in the IF models. The notably high Average Precision scores further enhance the reliability and robustness of the interpretation results, enabling accurate detection of the most crucial feature.


==> sections/sections_synthetic_datasets/Xaxis_new.tex <==
\subsection*{{\ttfamily Xaxis}} \label{sec:Xaxis-exp}
\subsubsection{Performance}
\ale{In Figure \ref{fig:Xaxis_contamination}, we observe the changes in average precision across various models as we adjust the number of anomalies that contaminate the train set. The dataset, which is described in the Appendix \ref{sec:appendix-synthetic-data} , is specifically designed to expose the limitations of the Isolation Forest (IF) model. It does this by distributing anomalies along a singular direction, knowing that in that bundle the anomalies are artificially influenced by the IF model's bias in its decision boundaries as presented in Appendix \ref{sec:IFvsEIF}.}

\ale{
Contrastingly, the EIF and its improved version, \EIFplus, demonstrate high performance. Their effectiveness is not diminished by the anomalies' structured distribution, thus the enhanced generalization capabilities of \EIFplus are not distinctly observable since both models achieve perfect precision (a score of 1) when there is no contamination.}

\ale{
Additionally, we note that the DIF model struggles to detect anomalies as effectively as IF when anomalies are present in the dataset used to fit the model. Yet, when trained exclusively on inliers, its performance increase, aligning with that of EIF and \EIFplus.}

\ale{
Finally, the AutoEncoder Avg Prec is below 0.5 when the training set is contaminated by anomalies. On the other hand the performances of the model are similar to the ones of the EIF and \EIFplusspace when the contamination factor is close (or equal) to 0.}

\ale{
Figure \ref{fig:Xaxis_contaminationEIFvsEIF+} showcases the performance delta between \EIFplusspace and EIF, highlighting their distinct characteristics. In this analysis, we note that \EIFplusspace similar performance to the EIF, with a small difference when \EIFplusspace is fitted by a contaminated dataset. }
\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.49\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Xaxis/Contamination/18-03-2024_13-51-54_Xaxis_contamination_full_plot.pdf}
      \caption{Models evaluation, varying the contamination levels}
      \label{fig:Xaxis_contamination_full}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.44\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Xaxis/Contamination/19-03-2024_09-16-18_Xaxis_EIF+_minus_EIF_precision_over_contamination.pdf}
      \caption{Difference between \EIFplus and EIF average precision}
      \label{fig:Xaxis_contaminationEIFvsEIF+}
    \end{subfigure}\hfil % <-- added
\caption{Figure \ref{fig:Xaxis_contamination_full} illustrates the average precision as the contamination level in the training set increases. Figure \ref{fig:Xaxis_contaminationEIFvsEIF+} compares the performance graphs of EIF and \EIFplus, using the difference of their scores in various contamination levels.}
\label{fig:Xaxis_contamination}
\end{figure}

\ale{In the Table \ref{tab:xaxis_performance}, we detail the performance metrics of various models under the two Scenarios outlined in Section \ref{sec:performance_evaluation}. This comparison reveals that in Scenario I, the EIF and \EIFplusspace models surpass the performance of their counterparts, showcasing superior ability to discern the dataset's structure. Conversely, in Scenario 2, where the training dataset is made of inliers, the AE model exhibits comparable effectiveness to the EIF and \EIFplusspace models. A critical aspect of our analysis also includes the evaluation of fitting and prediction times. This highlights that the IF, EIF, and \EIFplusspace models significantly outpace the DIF model, being over 20 times quicker in model fitting and 200 times faster in making predictions. Finally, the AutoEncoder is 2 times slower than the DIF model fitting the dataset but its prediction times are comparable with the ones of IF, EIF and \EIFplus.}
\begin{table}[htbp]
\begin{minipage}[t]{0.47\textwidth}
\strut\vspace*{-\baselineskip}\newline
\resizebox{\textwidth}{!}{
\begin{tabular}{|c||ccc|ccc||cc|}
\toprule
\hline
& \multicolumn{3}{c|}{Scenario I} & \multicolumn{3}{c||}{Scenario II} & \multicolumn{2}{c|}{Time} \\
\hline
AD Model & Avg & Prec & ROC & Avg & Prec & ROC & fit & pred \\
& Prec &  & AUC & Prec &  & AUC & fit & pred \\
\hline
IF          & 0.09 & 0.11 & 0.51 & 0.10 & 0.0 & 0.45 & \textbf{0.07} & \textbf{0.007} \\
EIF         & \textbf{0.97} & \textbf{0.89} & \textbf{0.93} & \textbf{0.99} & \textbf{1.0} & \textbf{1.0} & \textbf{0.07} & \textbf{0.004} \\
\EIFplus        & 0.91& \textbf{0.89} & \textbf{0.93} & \textbf{0.99} & \textbf{1.0} & \textbf{1.0} & \textbf{0.07} & {0.005} \\
DIF         & 0.06 & 0.06& 0.48& 0.97& 0.9& 0.94& 1.57 & 1.25 \\
AE & 0.52& 0.46& 0.7& \textbf{1.0}& \textbf{1.0}& \textbf{1.0}& 3.74 & 0.07 \\
\hline
\end{tabular}
}
\vspace{0.41cm}
\caption{Performances of 5 different Anomaly Detection models over {\ttfamily Xaxis} are compared using classical Classification metrics. Moreover, the last two columns contain the average time for a fit and predict operation. The highest metric values and the lowest execution times are highlighted in bold}\label{tab:xaxis_performance}
\end{minipage}
\hfill
\begin{minipage}[t]{0.47\textwidth}
\strut\vspace*{-\baselineskip}\newline
\resizebox{\textwidth}{!}{

\begin{tabular}{|c||c|c|c|c||c|}
\toprule
\hline
&\multicolumn{2}{c|}{Evaluation with EIF}&\multicolumn{2}{c||}{Evaluation with \EIFplus}&\\
\hline
& Scenario I & Scenario II & Scenario I & Scenario II & Time\\

 Algorithm & $AUC_{FS}$  & $AUC_{FS}$ & $AUC_{FS}$  & $AUC_{FS}$ &  \\
\hline
DIFFI         & \textbf{4.739}       & 2.838     & 4.548     &  2.728    &           0.55 \\
IF\_\approach  & -4.724& -4.73& -4.491&  -4.747    &           0.18 \\
EIF\_\approach        & 4.715&  4.727& 4.554&  4.742&  \textbf{0.07} \\
\EIFplus\_\approach       & 4.714&  \textbf{4.741}& 4.524&  \textbf{4.746}&  \textbf{0.07} \\
IF\_RF        & -2.824&  -2.858& -2.683&  -2.856&           0.67 \\
EIF\_RF       & 4.724&  4.735& 4.561&  \textbf{4.746}&           0.67 \\
\EIFplus\_RF      & 4.729&  4.74& \textbf{4.577}&  4.745&           0.67 \\
\hline
\end{tabular}
}
\caption{Quantitative evaluation of the effectiveness of 6 different interpretation algorithms on {\ttfamily Xaxis} through the $AUC_{FS}$ metric, introduced in \ref{sec:interpr_evaluat}. In the last column the average time taken by the different models to produce the importance scores is reported. The highest $AUC_{FS}$ and lowest Importance time values are highlighted in bold.}\label{tab:fs-tab-Xaxis}
\end{minipage}
\end{table}

\begin{comment}
\begin{table}[htbp]
\centering
%\caption{{\ttfamily Xaxis} Precision Report}
\caption{Performances of 5 different Anomaly Detection models over {\ttfamily Xaxis} are compared using classical Classification metrics. Moreover, the last two columns contain the average time for a fit and predict operation. The highest metric values and the lowest execution times are highlighted in bold}\label{tab:xaxis_performance}
\begin{tabular}{|c||ccc|ccc||cc|}
\toprule
\hline
& \multicolumn{3}{c|}{Scenario I} & \multicolumn{3}{c||}{Scenario II} & \multicolumn{2}{c|}{Time} \\
\hline
AD Model & Avg & Prec & ROC & Avg & Prec & ROC & fit & pred \\
& Prec &  & AUC & Prec &  & AUC & fit & pred \\
\hline
IF          & 0.09 & 0.11 & 0.51 & 0.10 & 0.0 & 0.45 & \textbf{0.07} & \textbf{0.007} \\
EIF         & \textbf{0.97} & \textbf{0.89} & \textbf{0.93} & \textbf{0.99} & \textbf{1.0} & \textbf{1.0} & \textbf{0.07} & \textbf{0.004} \\
\EIFplus        & 0.91& \textbf{0.89} & \textbf{0.93} & \textbf{0.99} & \textbf{1.0} & \textbf{1.0} & \textbf{0.07} & {0.005} \\
DIF         & 0.06 & 0.06& 0.48& 0.97& 0.9& 0.94& 1.57 & 1.25 \\
AE & 0.52& 0.46& 0.7& \textbf{1.0}& \textbf{1.0}& \textbf{1.0}& 3.74 & 0.07 \\
\hline
\end{tabular}
\end{table}
\end{comment}



\subsubsection{Importance Plots}

\ale{The interpretation results of the \EIFplus model across both scenarios are showcased in Figures \ref{fig:interpretation-Xaxis}. Across 40 algorithm iterations, feature 0 consistently emerges as the most significant, as depicted in Figures \ref{fig:Bar-plot-Xaxis-EXIFFI+-1} and \ref{fig:Bar-plot-Xaxis-EXIFFI+-2}. The primary distinction between the scenarios is observed in the importance scores; in the second scenario, these scores present an increased gap between the importance score of feature 0 and the one of the other features, indicating a clearer differentiation in feature importance.}

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
    \includegraphics[width=\linewidth]{Newfigures/Xaxis/Importance_plots/12-03-2024_08-51-24_GFI_Bar_plot_Xaxis_EXIFFI+_1.pdf}
      \caption{Bar Plot {\ttfamily Xaxis} Scenario I}
      \label{fig:Bar-plot-Xaxis-EXIFFI+-1}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.27\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Xaxis/Importance_plots/12-03-2024_08-51-24_GFI_Score_plot_Xaxis_EXIFFI+_1.pdf}
      \caption{Score Plot {\ttfamily Xaxis} Scenario I}
      \label{fig:Score-plot-Xaxis-EXIFFI+-1}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]
      {Newfigures/Xaxis/Local_Scoremap/12-03-2024_15-30-25_importance_map_Xaxis_EXIFFI+_1_feat_0_1.pdf}
      \caption{Scoremap {\ttfamily Xaxis} Scenario I}
      \label{fig:Local-Xaxis-EXIFFI+-1}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
      \includegraphics[width=\linewidth,valign=t]{Newfigures/Xaxis/Importance_plots/12-03-2024_08-49-30_GFI_Bar_plot_Xaxis_EXIFFI+_2.pdf}
      \caption{Bar Plot {\ttfamily Xaxis} Scenario II}
      \label{fig:Bar-plot-Xaxis-EXIFFI+-2}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.27\textwidth}
    \centering
      \includegraphics[width=\linewidth,valign=t]{Newfigures/Xaxis/Importance_plots/12-03-2024_08-49-31_GFI_Score_plot_Xaxis_EXIFFI+_2.pdf}
      \caption{Score Plot {\ttfamily Xaxis} Scenario II}
      \label{fig:Score-plot-Xaxis-EXIFFI+-2}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth,valign=t]{Newfigures/Xaxis/Local_Scoremap/12-03-2024_15-30-10_importance_map_Xaxis_EXIFFI+_2_feat_0_1.pdf}
      \caption{Scoremap {\ttfamily Xaxis} Scenario II}
      \label{fig:Local-Xaxis-EXIFFI+-2}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot and Scoremap of the dataset {\ttfamily Xaxis} in the two different Scenarios, using the ExIFFI algorithm applied to the \EIFplus model.}\label{fig:interpretation-Xaxis}
\end{figure}


\subsubsection{Feature Selection} \label{sec:feat-sel-Xaxis}

\begin{figure}[htbp] 
    \centering
    \hspace{0.05\textwidth}\textbf{IF} \hspace{0.29\textwidth} \textbf{EIF} \hspace{0.29\textwidth} \textbf{EIF+}
    % First row with vertical caption on the left
    \begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Ad-Hoc}}} % Adjust the parbox width as necessary for your caption text
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
      \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Xaxis/Feature_Selection/08-05-2024_15-26-53_Xaxis_EIF+_IF_EXIFFI_feature_selection_2.pdf}
      \caption{\approach applied to IF}
      \label{fig:Feat-Sel_Xaxis_valEIF+_IF_EXIFFI_2}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.30\textwidth}
    \centering
      \includegraphics[trim={0 0 3.5cm 0}, clip,width=\linewidth]{Newfigures/Xaxis/Feature_Selection/08-05-2024_15-26-31_Xaxis_EIF+_EXIFFI_feature_selection_2.pdf}
      \caption{\approach applied to EIF}
      \label{fig:Feat-Sel_Xaxis_valEIF+_EIF_EXIFFI_2}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.30\textwidth}
    \centering
      \includegraphics[trim={0 0 3.5cm 0}, clip,width=\linewidth]{Newfigures/Xaxis/Feature_Selection/08-05-2024_15-26-08_Xaxis_EIF+_EXIFFI+_feature_selection_2.pdf}
      \caption{\approach applied to \EIFplus}
      \label{fig:Feat-Sel_Xaxis_valEIF+_EIF+_EXIFFI_2}
      \end{subfigure}
    \end{minipage}
\end{minipage}

% Second row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Post-Hoc}}} % Adjust as necessary
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
              \includegraphics[trim={0 0 3.5cm 0}, clip,width=\linewidth]{Newfigures/Xaxis/Feature_Selection/08-05-2024_15-27-15_Xaxis_EIF+_IF_RandomForest_feature_selection_2.pdf}
              \caption{RandomForest fitted to IF}
              \label{fig:Feat-Sel_Xaxis_valEIF+_IF_RandomForest_2}
            \end{subfigure}\hfil % <-- added
            \begin{subfigure}[t]{0.30\textwidth}
            \centering
              \includegraphics[trim={0 0 3.5cm 0}, clip,width=\linewidth]{Newfigures/Xaxis/Feature_Selection/08-05-2024_15-27-37_Xaxis_EIF+_EIF_RandomForest_feature_selection_2.pdf}
              \caption{RandomForest fitted to EIF}
              \label{fig:Feat-Sel_Xaxis_valEIF+_EIF_RandomForest_2}
            \end{subfigure}\hfil % <-- added
            \begin{subfigure}[t]{0.30\textwidth}
            \centering
              \includegraphics[trim={0 0 3.5cm 0}, clip,width=\linewidth]{Newfigures/Xaxis/Feature_Selection/08-05-2024_15-27-59_Xaxis_EIF+_EIF+_RandomForest_feature_selection_2.pdf}
              \caption{RandomForest fitted to \EIFplus}
              \label{fig:Feat-Sel_Xaxis_valEIF+_EIF+_RandomForest_2}
                    \end{subfigure}
            \end{minipage}
        \end{minipage}
      \caption{Feature Selection of the different Ad-Hoc and Post-Hoc methods applied to the 3 Isolation Forest models: IF, EIF and \EIFplus. The blue line is the values of average precision, calculated with the \EIFplus model in the Scenario II, dropping the most important feature at each step, the red line is the values of average precision dropping the least important feature at each step and the green line is the value of the feature selection dropping a random feature at each step.}\label{fig:fs-interpretation-Xaxis}
\end{figure}

\ale{Figure \ref{fig:Feat-Sel_Xaxis_valEIF+_EIF+_EXIFFI_2} presents Feature Selection in Scenario II, comparing various interpretation algorithms across different isolation models. Since the IF model has very low performances both the ad-hoc and post-hoc interpretation reveal a significant Feature Selection performance impact. Notably, both Figures \ref{fig:Feat-Sel_Xaxis_valEIF+_IF_EXIFFI_2} \ref{fig:Feat-Sel_Xaxis_valEIF+_IF_RandomForest_2}  demonstrates that prioritizing the removal of features deemed most important by the RandomForest and IF (blue line) surprisingly enhances feature selection, indicating a reversal in the expected feature importance order. This phenomenon suggests the more the model has low performances, the more its interpretation is not reliable.}

\ale{Looking at the remaining plots, a significant decline in performance is observed once feature 0, the feature used to craft the anomalies in this dataset, is removed. 
For both EIF models, Feature Selection guided by the importance scores from \approach and the Random Forest exhibits strong performance, acknowledging Feature 0 as the most crucial, underscoring its significance in accurate anomaly detection and interpretation within this context.}

% \ale{Scrivere sulla feature selection fatta in questo modo}
% \ale{Scriovere dell' $AUC_{FS}$ come score valutativo della feature selection citando il paper di nature}


\ale{In the Table \ref{tab:fs-tab-Xaxis}, we showcase the $AUC_{FS}$ scores for Feature Selection across both scenarios, evaluated through the EIF and \EIFplus models and considering various interpretation algorithms. In Scenario I, the performance across different interpretation algorithms is largely comparable, except in the case of feature importance derived from the Random Forest model fitted on the IF model's results or the feature importance derived from the \approach applied to the IF model. This exception is attributed to the IF model's under-performance. Moreover in the Scenario II we observe a drop in performances even in the case of the DIFFI.
It's important to highlight the efficiency aspect in our analysis: the \approach algorithm demonstrates a notably quicker computation time for evaluating importance scores. This observation emphasizes the speed advantage of our proposed ad-hoc interpretation method over alternative approaches, illustrating not only its effectiveness in interpretation but also its operational efficiency.}


\begin{table}[htbp]
\centering
%\caption{Feature Selection Scores {\ttfamily Xaxis}}
\caption{Quantitative evaluation of the effectiveness of 6 different interpretation algorithms on {\ttfamily Xaxis} through the $AUC_{FS}$ metric, introduced in \ref{sec:interpr_evaluat}. In the last column the average time taken by the different models to produce the importance scores is reported. The highest $AUC_{FS}$ and lowest Importance time values are highlighted in bold.}\label{tab:fs-tab-Xaxis}

\begin{tabular}{|c||c|c|c|c||c|}
\toprule
\hline
&\multicolumn{2}{c|}{Evaluation with EIF}&\multicolumn{2}{c||}{Evaluation with \EIFplus}&\\
\hline
& Scenario I & Scenario II & Scenario I & Scenario II & Time\\

 Algorithm & $AUC_{FS}$  & $AUC_{FS}$ & $AUC_{FS}$  & $AUC_{FS}$ &  \\
\hline
DIFFI         & \textbf{4.739}       & 2.838     & 4.548     &  2.728    &           0.55 \\
IF\_\approach  & -4.724& -4.73& -4.491&  -4.747    &           0.18 \\
EIF\_\approach        & 4.715&  4.727& 4.554&  4.742&  \textbf{0.07} \\
\EIFplus\_\approach       & 4.714&  \textbf{4.741}& 4.524&  \textbf{4.746}&  \textbf{0.07} \\
IF\_RF        & -2.824&  -2.858& -2.683&  -2.856&           0.67 \\
EIF\_RF       & 4.724&  4.735& 4.561&  \textbf{4.746}&           0.67 \\
\EIFplus\_RF      & 4.729&  4.74& \textbf{4.577}&  4.745&           0.67 \\
\hline
\end{tabular}
\end{table}


==> sections/sections_synthetic_datasets/Yaxis_new.tex <==
\subsection*{{\ttfamily Yaxis}}\label{sec:Yaxis}

\ale{Prior to the analysis of the experiment results on the {\ttfamily Yaxis} dataset it is worth noticing how this dataset was produced with the same process used to obtain the {\ttfamily Xaxis} dataset with the only difference that anomalies were distributed along Feature 1 instead of Feature 0. As a consequence the outocomes of the experiments are expected to be very similar, if not coincident, with the ones obtained on {\ttfamily Xaxis} and described in \ref{sec:Xaxis-exp} except for the Importance plots, that will be illustrated in \ref{sec:Yaxis-imp-plots}, where the most relevant feature is expected to be Feature 1, instead of Feature 0. }

\subsubsection{Performance}
 
\ale{Similarly to what was observed for the {\ttfamily Xaxis} dataset in Figure \ref{fig:Yaxis_contamination_full} it is possible to notice how EIF and \EIFplus obtain a perfect Average Precision score of 1 for almost all the contamination values considered and their performances are corresponding as depicted in Figure \ref{fig:Yaxis_contaminationEIFvsEIF+}. Additionally the IF model struggles to detect anomalies in a dataset were the drawbacks of the Isolation Forest model are exposed and the deep learning based approaches considered (i.e. DIF and Autoencoder) are able to achieve similar performances to EIF and \EIFplus only for minimal values of the contamination level. }

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.49\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Yaxis/Contamination/25-03-2024_10-18-22_Yaxis_contamination_full_plot.pdf}
      \caption{Models evaluation, varying the contamination levels}
      \label{fig:Yaxis_contamination_full}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.44\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Yaxis/Contamination/25-03-2024_10-20-20_Yaxis_EIF+_minus_EIF_precision_over_contamination.pdf}
      \caption{Difference between \EIFplus and EIF average precision}
      \label{fig:Yaxis_contaminationEIFvsEIF+}
    \end{subfigure}\hfil % <-- added
\caption{Figure \ref{fig:Yaxis_contamination_full} illustrates the average precision as the contamination level in the training set increases. Figure \ref{fig:Yaxis_contaminationEIFvsEIF+} compares the performance graphs of EIF and \EIFplus, using the difference of their scores in various contamination levels.}
\label{fig:Yaxis_contamination}
\end{figure}

\ale{A Performance Report of the various AD models explored in this study is reported in Table \ref{tab:Yaxis_perf}  highlighting the difference between Scenario I and Scenario II. The results are very close to the ones presented in \ref{sec:Xaxis-exp} with EIF and \EIFplus being clearly the optimal models both in terms of evaluation metrics and time efficiency. }
\begin{table}[htbp]
\begin{minipage}[t]{0.47\textwidth}
\strut\vspace*{-\baselineskip}\newline
\resizebox{\textwidth}{!}{
\begin{tabular}{|c||ccc|ccc||cc|}
\toprule
\hline
& \multicolumn{3}{c|}{Scenario I} & \multicolumn{3}{c||}{Scenario II} & \multicolumn{2}{c|}{Time} \\
\hline
AD Model& Avg & Prec & ROC & Avg & Prec & ROC & fit & pred \\
 & Prec &  & AUC & Prec &  & AUC &  &  \\
\hline
IF          & 0.1& 0.07& 0.48& 0.12& 0.1&0.5& 0.06& \textbf{0.006}\\
EIF         & \textbf{0.97} & \textbf{0.85}& \textbf{0.91}& \textbf{0.99} & \textbf{1.0} & \textbf{1.0} & \textbf{0.05}& 0.07\\
\EIFplus        & \textbf{0.94}& \textbf{0.9}& \textbf{0.94}& \textbf{0.99} & \textbf{0.99}& \textbf{0.99}& \textbf{0.05}& 0.07\\
DIF         & 0.05& 0.01&0.45& 0.99& 0.97&0.98& 1.65& 1.33\\
AE         & 0.54& 0.49&0.71& 1.0 & 1.0&1.0& 4.07& 0.07 \\
\hline
\end{tabular}
}
\vspace{0.41cm}
\caption{Performances of 5 different Anomaly Detection models over {\ttfamily Yaxis} are compared using classical Classification metrics. Moreover the last two columns contain the average time for a fit and predict operation. The highest metric values and the lowest execution times are highlighted in bold}\label{tab:Yaxis_perf}
\end{minipage}
\hfill
\begin{minipage}[t]{0.47\textwidth}
\strut\vspace*{-\baselineskip}\newline
\resizebox{\textwidth}{!}{
\begin{tabular}{|c||c|c|c|c||c|}
\toprule
\hline
&\multicolumn{2}{c|}{Evaluation with EIF}&\multicolumn{2}{c||}{Evaluation with \EIFplus}&\\
\hline
& Scenario I & Scenario II & Scenario I & Scenario II & Time\\

 Algorithm & $AUC_{FS}$  & $AUC_{FS}$ & $AUC_{FS}$  & $AUC_{FS}$ &  \\
\hline
DIFFI         & 4.726& \textbf{4.740}& \textbf{4.567}& 4.743& 0.36\\
IF\_\approach        & -4.714& 0.952& -4.536& 0.955& \textbf{0.16}\\
EIF\_\approach        & 4.73& 4.729& 4.484& 4.744& \textbf{0.16}\\
\EIFplus\_\approach       & 4.733& 4.73& 4.508& 4.745& \textbf{0.16}\\
IF\_RF        & -2.843& -0.95& -2.669& -0.946& 0.67\\
EIF\_RF       & \textbf{4.734}& 4.733& 4.537& 4.74& 0.67\\
EIF+\_RF      & 4.705& 4.729& 4.506& \textbf{4.746}& 0.67\\
\hline
\end{tabular}
}
\caption{Quantitative evaluation of the effectiveness of 6 different interpretation algorithms on {\ttfamily Yaxis} through the $AUC_{FS}$ metric, introduced in \ref{sec:interpr_evaluat}. In the last column the average time taken by the different models to produce the importance scores is reported. The highest $AUC_{FS}$ and lowest Importance time values are highlighted in bold.}\label{tab:fs-tab-Yaxis}
\end{minipage}
\end{table}

\subsubsection{Importance Plots} \label{sec:Yaxis-imp-plots}

\ale{An evaluation of the proposed interpretation model \approach+ is presented in Figure \ref{fig:interpretation-Yaxis}. As expected the results are symmetrical to the ones obtained in {\ttfamily Xaxis} with Feature 1 being the most relevant feature in both Scenario I and II and the dominance of this variable can also be observed in the Local Scoremaps depicted in Figures \ref{fig:Local-Yaxis-EXIFFI+-1} and \ref{fig:Local-Yaxis-EXIFFI+-2}. }

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Yaxis/Importance_plots/25-03-2024_10-55-00_GFI_Bar_plot_Yaxis_EXIFFI+_1.pdf}
      \caption{Bar Plot {\ttfamily Yaxis} Scenario I}
      \label{fig:Bar-plot-Yaxis-EXIFFI+-1}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.27\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Yaxis/Importance_plots/25-03-2024_10-55-00_GFI_Score_plot_Yaxis_EXIFFI+_1.pdf}
      \caption{Score Plot {\ttfamily Yaxis} Scenario I}
      \label{fig:Score-plot-Yaxis-EXIFFI+-1}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Yaxis/Local_Scoremap/07-03-2024_16-07-27_importance_map_Yaxis_EXIFFI+_1.pdf}
      \caption{Scoremap {\ttfamily Yaxis} Scenario I}
      \label{fig:Local-Yaxis-EXIFFI+-1}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Yaxis/Importance_plots/25-03-2024_10-57-23_GFI_Bar_plot_Yaxis_EXIFFI+_2.pdf}
      \caption{Bar Plot {\ttfamily Yaxis} Scenario II}
      \label{fig:Bar-plot-Yaxis-EXIFFI+-2}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.27\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Yaxis/Importance_plots/25-03-2024_10-57-24_GFI_Score_plot_Yaxis_EXIFFI+_2.pdf}
      \caption{Score Plot {\ttfamily Yaxis} Scenario II}
      \label{fig:Score-plot-Yaxis-EXIFFI+-2}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Yaxis/Local_Scoremap/07-03-2024_16-06-53_importance_map_Yaxis_EXIFFI+_2.pdf}
      \caption{Scoremap {\ttfamily Yaxis} Scenario II}
      \label{fig:Local-Yaxis-EXIFFI+-2}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot and Scoremap of the dataset {\ttfamily Yaxis} in the two different Scenarios, using the ExIFFI algorithm applied to the \EIFplus model.}\label{fig:interpretation-Yaxis}
\end{figure}

\subsubsection{Feature Selection}

\ale{Also in the Feature Selection Plots, portrayed in Figure \ref{fig:fs-interpretation-Yaxis},  a clear resemblance with the plots displayed in Figure \ref{fig:fs-interpretation-Xaxis} can be observed, except for the peculiar behavior associated to the interpretation of the IF model predictions, shown in Figures \ref{fig:Feat-Sel_Yaxis_valEIF+_DIFFI_2} and \ref{fig:Feat-Sel_Yaxis_valEIF+_IF_RandomForest_2}. As it happens in the {\ttfamily Xaxis} dataset the anomaly score artifacts of IF are exposed in this dataset leading to poor performances of the IF model. However differently from the outcomes described in \ref{sec:feat-sel-Xaxis} the features ranking produced by IF\_\approach and IF\_RandomForest , place Feature 1 (i.e. the most relevant feature for {\ttfamily Yaxis}) in the middle of the ranking, in particular in position 4 and 3 respectively leading to a peculiar parallelogram shape in the Feature Selection plots.}

\begin{comment}
Also for {\ttfamily Yaxis} the newly introduced ad-hoc interpretability methods \approach and \approach+ produce better looking plots than the ones produced by the IF model (\ref{fig:Feat-Sel_Yaxis_valEIF+_DIFFI_2}, \ref{fig:Feat-Sel_Yaxis_valEIF+_IF_RandomForest_2}), in particular, by post-hoc interpretability methods based on the Random Forest surrogate model.
\end{comment} 

\begin{figure}[!ht] 
    \centering
    \hspace{0.05\textwidth}\textbf{IF} \hspace{0.29\textwidth} \textbf{EIF} \hspace{0.29\textwidth} \textbf{EIF+}
    % First row with vertical caption on the left
    \begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Ad-Hoc}}} % Adjust the parbox width as necessary for your caption text
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
      \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Yaxis/Feature_Selection/08-05-2024_15-45-11_Yaxis_EIF+_IF_EXIFFI_feature_selection_2.pdf}
      \caption{\approach applied to IF}
      \label{fig:Feat-Sel_Yaxis_valEIF+_DIFFI_2}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.30\textwidth}
    \centering
      \includegraphics[trim={0 0 3.5cm 0}, clip,width=\linewidth]{Newfigures/Yaxis/Feature_Selection/08-05-2024_15-44-49_Yaxis_EIF+_EXIFFI_feature_selection_2.pdf}
      \caption{\approach applied to EIF}
      \label{fig:Feat-Sel_Yaxis_valEIF+_EXIFFI_2}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.30\textwidth}
    \centering
      \includegraphics[trim={0 0 3.5cm 0}, clip,width=\linewidth]{Newfigures/Yaxis/Feature_Selection/08-05-2024_15-44-25_Yaxis_EIF+_EXIFFI+_feature_selection_2.pdf}
      \caption{\approach applied to \EIFplus}
      \label{fig:Feat-Sel_Yaxis_valEIF+_EXIFFI+_2}
      \end{subfigure}
    \end{minipage}
\end{minipage}

% Second row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Post-Hoc}}} % Adjust as necessary
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
              \includegraphics[trim={0 0 3.5cm 0}, clip,width=\linewidth]{Newfigures/Yaxis/Feature_Selection/08-05-2024_15-45-33_Yaxis_EIF+_IF_RandomForest_feature_selection_2.pdf}
              \caption{RandomForest fitted to IF}
              \label{fig:Feat-Sel_Yaxis_valEIF+_IF_RandomForest_2}
            \end{subfigure}\hfil % <-- added
            \begin{subfigure}[t]{0.30\textwidth}
            \centering
              \includegraphics[trim={0 0 3.5cm 0}, clip,width=\linewidth]{Newfigures/Yaxis/Feature_Selection/08-05-2024_15-45-55_Yaxis_EIF+_EIF_RandomForest_feature_selection_2.pdf}
              \caption{RandomForest fitted to EIF}
              \label{fig:Feat-Sel_Yaxis_valEIF+_EIF_RandomForest_2}
            \end{subfigure}\hfil % <-- added
            \begin{subfigure}[t]{0.30\textwidth}
            \centering
              \includegraphics[trim={0 0 3.5cm 0}, clip,width=\linewidth]{Newfigures/Yaxis/Feature_Selection/08-05-2024_15-46-17_Yaxis_EIF+_EIF+_RandomForest_feature_selection_2.pdf}
              \caption{RandomForest fitted to \EIFplus}
              \label{fig:Feat-Sel_Yaxis_valEIF+_EIF+_RandomForest_2}
                    \end{subfigure}
            \end{minipage}
        \end{minipage}
      \caption{Feature Selection of the different Ad-Hoc and Post-Hoc methods applied to the 3 Isolation Forest models: IF, EIF and \EIFplus. The blue line is the values of average precision, calculated with the \EIFplus model in the Scenario II, dropping the most important feature at each step, the red line is the values of average precision dropping the least important feature at each step and the green line is the value of the feature selection dropping a random feature at each step.}\label{fig:fs-interpretation-Yaxis}
\end{figure}

\ale{The outcomes just commented after a detailed observation of the Feature Selection plots are reflected on the $AUC_{FS}$ values collected, for all the possible combinations of evaluation and interpretation methods, in Table \ref{tab:fs-tab-Yaxis}. The best values are associated to \approach and \approach+ models which are also the best performing ones in terms of computational efficiency. }




==> sections/sections_world_dataset_results/annthyroid.tex <==
\subsubsection*{{\ttfamily Annthyroid}}

%\modifica{introduzione ad Annthyroid richiamando la sezione \ref{sec:real-world-data}}

The dataset named {\ttfamily Annthyroid}, %which can be found in the UCI Machine Learning Repository and was introduced in Section \ref{datasets}, 
was originally designed for Multi-Class Classification and then adapted to Anomaly Detection % with three distinct classes. However, for the purposes of this study, it underwent modifications to adapt it for Anomaly Detection, 
as described in detail in Appendix \ref{sec:appendix-real-world-data}. 
%This dataset comprises six numerical features, the analysis of which is the focal point of this section. 
%\todo[inline, color=red]{Ho ulteriormente sintetizzato, visto che in appendice abbiamo la descrizione dettagliata di tutti i dataset (Chiara)}
%\modifica{mettere risultati importances nel caso in cui è allenata interamente sul dataset di annthyroid}

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}{0.45\textwidth}
    \centering
      \includegraphics[width=\linewidth]{figures/annthyroid/Feat_bar_plot_annthyroid.pdf}
      \caption{Score Plot {\ttfamily Annthyroid} Scenario I}
      \label{fig:Feat-imp-Annthyroid}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
    \centering
      \includegraphics[width=\linewidth]{figures/annthyroid/Feat_bar_plot_annthyroid_split.pdf}
      \caption{Score Plot {\ttfamily Annthyroid} Scenario II}
      \label{fig:Feat-imp-Annthyroid-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
    \centering
      \includegraphics[width=\linewidth]{figures/annthyroid/GFI_annthyroid_synt.pdf}
      \caption{Bar Plot {\ttfamily Annthyroid} Scenario I}
      \label{fig:GFI-annthyroid}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
    \centering
      \includegraphics[width=\linewidth]{figures/annthyroid/GFI_annthyroid_split_synt.pdf}
      \caption{Bar Plot {\ttfamily Annthyroid} Scenario II}
      \label{fig:GFI-annthyroid-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
    \centering
      \includegraphics[width=\linewidth]{figures/scoremaps_real_world/Local_Scoremap_plot_annthyroid.png}
      \caption{Scoremap {\ttfamily Annthyroid} Scenario I}
      \label{fig:Local-annthyroid}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
    \centering
      \includegraphics[width=\linewidth]{figures/scoremaps_real_world/Local_Scoremap_Plot_annthyroid_split.png}
      \caption{Scoremap {\ttfamily Annthyroid} Scenario II}
      \label{fig:Local-annthyroid-split}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot and Scoremap for {\ttfamily Annthyroid}}\label{fig:interpretation-annthyroid}
\end{figure}

%\modifica{ si vede come non c'è una feature principale su cui si distribuiscono i punti che deviano dal dataset, infatti sia lungo la feature 1 che lungo la 5 ci sono punti che allo stesso livello di anomalia}
We initially train Isolation-based AD models on the entire dataset. The Bar Plot (Figure \ref{fig:GFI-annthyroid}) reveals no single dominant feature; instead, features 1, 5, and 3 hold the top positions, with a slight preference for feature 1. This trend is reinforced by the Scoremap (Figure \ref{fig:Local-annthyroid}), depicting the dataset's distribution along features 1 and 5. It's evident that the dataset deviates equally along both feature 1 and feature 5, despite the labeled anomalies (stars) primarily deviating along feature 1. %These points, represented in the plot as red stars, have similar Anomaly Score values since they are contained in the same contour lines. 

%\modifica{risultato che si può osservare anche dalle precisioni carenti nel saper individuare le specifiche anomalie che vediamo nello scoremaps distribuirsi senza dubbio principalmente lungo la feature 1}
The reason behind this phenomenon is that the algorithm does not pinpoint the specific features responsible for causing the labeled anomalies to deviate. Instead, it tends to focus on the features that align the most with the predicted anomalies. This becomes evident when considering the low Average Precision score in Table \ref{tab:avg-prec-table}. It suggests that the isolation forest models struggle to accurately identify the labeled anomalies, that are, as already said in Section \ref{datasets} just a part of the dataset distribution rather than a deviation from it.
%A possible explanation of the indecision of the \approach model to clearly identify a single anomalous feature, instead  comes from the performance metrics reported on Table \ref{tab:annthyroid-perf-complete}. The reported values are significantly low and thus the model is not able to correctly detect the anomalies clearly distributed along Feature 1 as it can be noticed in the Local Scoremap.

%\modifica{feature che in ogni caso il nostro algoritmo di interpretazione è in grado di riconoscere, probabilmente dovuto alla maggiore deviazione della distribuzione lungo quella feature, senza però adeguata robustezza}

%In any case, Feature 1 is identified as the most important feature, as it can be observed in the Feature Importance Score Plot depicted in Figure \ref{fig:Feat-imp-Annthyroid}, probably because of a higher deviation of the data distribution along that direction, but with a lack of robustness. 

%\modifica{mettere tabella precisioni allenato su tutto}
\begin{comment}
\begin{table}[ht]
\parbox{.45\linewidth}{
\centering
\begin{tabular}{|c|ccc|}
\hline
\multicolumn{4}{|c|}{\textbf{annthyroid} complete training} \\ \hline
\textbf{Metric} & \textbf{IF} & \textbf{EIF} & \textbf{EIF+} \\ \hline
Precision         & 0.34 & 0.27 & 0.27 \\
Recall            & 0.34 & 0.27 & 0.27 \\
f1 score          & 0.34 & 0.27 & 0.27 \\
Accuracy          & 0.90 & 0.89 & 0.89 \\

Average Precision & 0.33 & 0.23 & 0.22 \\
ROC AUC Score     & 0.82 & 0.70 & 0.72 \\ \hline
\end{tabular}
\caption{Performance Report \texttt{annthyroid} Dataset}
\label{tab:annthyroid-perf-complete}}
\end{table}
\end{comment}

%\modifica{allora decidiamo di allenare sui soli inlier per vedere se l'algoritmo è in grado di migliorare la propria robustezza nel caso in cui il modello è maggiormente adattato agli inliers}

After constructing the AD model exclusively on the labeled inlier portion of the dataset, we help the model to recognize that the labeled anomalies deviate from the normal distribution within the dataset. As a result, we can notice a substantial improvement in the Average Precision, as indicated in Table \ref{tab:avg-prec-table}. This improvement signifies a stronger alignment between the labeled anomalies and the predictions of the model.

Consequently, the output generated by the interpretation algorithm \approach, becomes more attuned to the structural characteristics of the labeled anomalies. This enhanced alignment leads to greater robustness in identifying Feature 1 as the primary contributor to the dataset's deviation, it can be seen in Figures \ref{fig:GFI-annthyroid-split} and \ref{fig:Feat-imp-Annthyroid-split}.

%\modifica{far vedere nel caso in cui si splitta il training per capire se va meglio}

%\modifica{in questo caso grazie al fatto che il modello è stato allenato sui soli inliers, e che le anomalie sono effettivamente un cluster specifico dei dati. L'algoritmo di interpretazione di questo modello mostra correttamente risultati più robusti nel riconoscere la feature 1 come la più importante. Inoltre dai contourplots di questo scoremap si vede come il modello si è centrato maggiormente sugli inliers senza inglobare nella distribuzione normale il gruppo di dati labeled come anomalie.}

%As it can be noticed from the Global Feature Importance Bar Plot, reported in Figure \ref{fig:GFI-annthyroid-split}, the strategy of training the model only on the inliers helped in the isolation of Feature 1 as the most important feature with a significant margin on the others as it can be observed in the Feature Importance Score Plot in Figure \ref{fig:Feat-imp-Annthyroid-split}. 

%Moreover, some changes are visible also on the Local Scoremap placed in Figure \ref{fig:Local-annthyroid-split}. The Anomaly Score Contour lines are in fact centered mainly on the main cluster of the data excluding from the normal distribution the group of data labeled as anomalies. 

%\modifica{si vede come nella tabella seguente le precisioni migliorano nettamente, dunque quando l'algoritmo ha score di precisione più alti è anche più robusto e reliable nel riconoscere le feature più importanti}

%The Performance Report Table, contained in Table \ref{tab:annthyroid-perf-split}, confirms the graphical improvements already seen. The metrics values are much higher than the ones reported in Table \ref{tab:annthyroid-perf-complete} meaning that the model increased its robustness and reliability in detecting the most important features. 
%\modifica{inserire tabella precisioni}
\begin{comment}
\begin{table}[ht]
\parbox{.45\linewidth}{
\centering
\begin{tabular}{|c|ccc|}
\hline
\multicolumn{4}{|c|}{\textbf{annthyroid} inlier training} \\ 
\hline
\textbf{Metric} & \textbf{IF} & \textbf{EIF} & 
\textbf{EIF+} \\ \hline
Precision         & 0.51 & 0.44 & 0.45 \\
Recall            & 0.51 & 0.44 & 0.45 \\
f1 score          & 0.51 & 0.44 & 0.45 \\
Accuracy          & 0.93 & 0.92 & 0.92 \\

Average Precision & 0.57 & 0.50 & 0.51 \\
ROC AUC Score     & 0.94 & 0.89 & 0.89 \\ \hline
\end{tabular}
\caption{Performance Report \texttt{annthyroid} Dataset}
\label{tab:annthyroid-perf-split}
}
\end{table}
\end{comment}
%\modifica{la feature selection conferma che la selezione di feature più importanti ha funzionato bene evidenziando come la precisione migliori di tanto una volta che si selezionano poche feature importanti}
%\modifica{mettere feature selection per confermare ipotesi}
\begin{figure}[!ht] 
  \centering
  \includegraphics[width=0.7\linewidth]{figures/feature_selection_plots_final/featsel_annthyroid_final.pdf}
    \caption{Feature Selection Plot {\ttfamily Annthyroid}}
  \label{fig:fs-annthyroid-plus}
\end{figure}%\hfil % <-- added

In Figure \ref{fig:fs-annthyroid-plus}, we present the Feature Selection Plot for the {\ttfamily Annthyroid} dataset. This plot serves as unequivocal confirmation that \approach's assessment of the most important feature is accurate. It's worth noting that even if the interpretation is more robust when the model is trained on the inliers only, in both scenarios Feature 1 emerges as the most significant feature. Moreover, the feature selection is very similar considering the different algorithms and the different training datasets.
%\todo[inline, color=red]{@Alessio: qui consideriamo due scenari va mediamo solo EIF, vero? non mi torna la frase sopra (Chiara)}
%\todo[inline, color=orange]{Non ho capito bene come risolverlo, vedremo poi insieme}

In summary, this dataset proves to be non-trivial for Anomaly Detection, as evidenced by the notably low Average Precision scores. Consequently, it becomes challenging to accurately evaluate the interpretative algorithm's performance in the initial scenario. However, by leveraging the insights gleaned from the Scoremap (see Figure \ref{fig:Local-annthyroid} and Figure \ref{fig:Local-annthyroid-split}), which highlights Feature 1 as the most critical for identifying labeled anomalies, once we enforce the separation of labeled anomalies from the normal distribution of the dataset, the results become both satisfactory and robust. This leads us to confidently conclude that the interpretation algorithm performed effectively on this particular dataset.

%\todo[inline, color=red]{@Alessio ti lascio due note. Detto ciò, mi pare sia ok in generale. Ho due proposte: 1) riusciamo a raggruppare le figure per Scenario I e Scenario II? 2) possiamo mettere come primo caso uno in cui le cose funzionano in modo smooth, se esiste? (Chiara)}



%As it can be noticed all the Feature Ranking Algorithms except for Random Forest and Casual show an increase in Average Precision up to almost 0.9 as the number of features decreases. A similar behavior can be observed for Random Forest which however has a drop in precision values as the number of features is reduced from 2 to 1. Finally, the Casual feature ranking algorithm has much lower values. The reason \chiara{behind} that may be the casual removal of one important feature in the step corresponding to the reduction from 4 to 3 features.  This outcome confirms that the selection of the most important features according to the Isolation Forest-based model's interpretation results worked well since the Average Precision increases as only the most relevant attributes are considered in the input. 

%\modifica{Collegare i risulati ottenuti con il significato della Feature 1, spiegando cosa rappresenta questa feature si può giustificare il fatto che sia stata selezionata come più importante.}

%As described in Appendix \ref{sec:real-world-data} Feature 1 represents the T3 hormone levels. T3 (Triiodothyronine) is one of the two main hormones (T3 and T4) produced by the thyroid. It regulates the metabolism, energy production, and other physiological processes in the body. The results of the Experiments performed on the \approach model outputs just described confirmed the importance of this hormone in the correct functioning of the thyroidal organ. Indeed, anomalous levels of the T3 hormone can cause hypothyroidism or hyperthyroidism.


%\todo[inline, color=red]{In generale, questo mi pare un buon esempio, con tanto di spiegazione "medica". Il tema a mio vedere è semplicemente che le anomalie secondo le etichetto non corrispondono alla definizione di punti facili da isolare, ci sta che nel training con tutto il dataset IF e EIF non le becchino (Chiara)}
%

%\davide{
%For what concerns the feature importance scores of the {\ttfamily Annthyroid} dataset, presented in \ref{sec:real-world-data}, it is very clear that the most important feature is Feature 1. Indeed, it is always considered the most important one in \ref{fig:GFI-annthyroid} and it has an average importance score significantly higher than the ones of the other features as it can be noticed in \ref{fig:Feat-imp-Annthyroid}. On the other hand, the least important feature is Feature 0 which is placed in the last ranking 60\% of the time.

%As described in Section \ref{sec:LFI-output} in the Local Importance Scoremap it is possible to visualize only a pair of features at a time. In this example, in Figure \ref{fig:Local-annthyroid}, Features 1 and 0 were considered. Looking at Figures \ref{fig:GFI-annthyroid} and \ref{fig:Feat-imp-Annthyroid} the comparison under analysis is considering the most and the least important features. Carefully observing the Local Scoremap it is understandable that Feature 1 is a very important feature since all the outliers (represented by the red stars) are spread along its direction. In particular, four inliers on the bottom right area of the feature space are highly separated from all the other samples. These samples can be isolated also with a horizontal cut, this is the reason why the right region of the scoremap anomalies are easily detected trough Feature 0 and thus the region  
%is almost fully colored in red. 

%\davide {
%Table \ref{tab:annthyroid-perf} lists the values of the common Classification performance metrics for the IF,EIF and EIF+ models on the {\ttfamily Annthyroid} dataset. Posing the focus on the two most important metrics, i.e. F1 Score and Average Precision, it is possible to notice how the EIF+ model improves the performances of both the EIF and IF models confirming its superior generalization capabilities. A noteworthy thing to mention are the better performances of the iF model over the EIF one, probably due to the alignment of almost all the outliers along a single feature. Hence, the IF model, in this particular dataset, may be considered a good choice since it is able to easily isolate anomalies using a vertical or horizontal cut along the interested feature. 
%}



==> sections/sections_world_dataset_results/annthyroid_new.tex <==
\subsection*{{\ttfamily Annthyroid}}

\subsubsection{Performance}
\ale{In Figure \ref{fig:Annthyroid_contamination}, we note that the DIF, EIF, and \EIFplus models exhibit similar performance levels, whereas the IF model overall surpasses them on this specific dataset, likely due to its structural characteristics. Interestingly, at a contamination value of $0$, the \EIFplus model slightly outperforms the others, underscoring its superior capability to generalize across unseen anomalies. This is particularly evident in Figure \ref{fig:Annthyroid_contaminationEIFvsEIF+}, where the \EIFplus model starts with negligible differences from EIF at a contamination level of $0.1$, but its advantage becomes more pronounced as the contamination level decreases. This pattern suggests the \EIFplus model's enhanced adaptability and effectiveness in handling datasets with lower contamination rates.}

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.49\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Annthyroid/Contamination/18-03-2024_16-05-16_annthyroid_contamination_full_plot.pdf}
      \caption{Models evaluation, varying the contamination levels}
      \label{fig:Annthyroid_contamination_full}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.44\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Annthyroid/Contamination/19-03-2024_09-16-42_annthyroid_EIF+_minus_EIF_precision_over_contamination.pdf}
      \caption{Difference between \EIFplus and EIF average precision}
      \label{fig:Annthyroid_contaminationEIFvsEIF+}
    \end{subfigure}\hfil % <-- added
\caption{Figure \ref{fig:Annthyroid_contamination_full} illustrates the average precision as the contamination level in the training set increases. Figure \ref{fig:Annthyroid_contaminationEIFvsEIF+} compares the performance graphs of EIF and \EIFplus, using the difference of their scores in various contamination levels.}
\label{fig:Annthyroid_contamination}
\end{figure}

\ale{The Table \ref{tab:Annthyroid_perf}  elaborates on the numerical results depicted in the plots from Figure \ref{fig:Annthyroid_contamination}, detailing the performance improvement from Scenario I to Scenario II. The most notable enhancement is observed with the \EIFplus model, which not only demonstrates significant performance gains but also retains the fastest computational efficiency in model fitting—being 100 times quicker than the DIF model. Additionally, it boasts the second-best timing in prediction speed. This showcases \EIFplus's dual advantage of superior anomaly detection capability across different scenarios and exceptional computational performance, highlighting its practicality for real-world applications.}


\begin{table}[htbp]
\centering
%\caption{{\ttfamily Annthyroid} Precision Report}
\caption{Performances of 5 different Anomaly Detection models over {\ttfamily Annthyroid} are compared using classical Classification metrics. Moreover, the last two columns contain the average time for a fit and predict operation. The highest metric values and the lowest execution times are highlighted in bold}\label{tab:Annthyroid_perf}
\begin{tabular}{|c||ccc|ccc||cc|}
\toprule
\hline
&\multicolumn{3}{c|}{Scenario I}&\multicolumn{3}{c||}{Scenario II}&\multicolumn{2}{c|}{Time}\\
\hline
AD Model & Avg & Prec & ROC & Avg & Prec & ROC & fit & pred \\
& Prec &  & AUC & Prec &  & AUC & fit & pred \\
\hline
IF          & \textbf{0.30} & \textbf{0.32} & \textbf{0.63} & 0.45 & 0.43 & 0.69 & 0.17 & \textbf{0.15} \\
EIF         & 0.19 & 0.24 & 0.59 & 0.45 & 0.41 & 0.68 & 0.09 & 0.43 \\
\EIFplus       & 0.20 & 0.28 & 0.61 & \textbf{0.46} & \textbf{0.46} & \textbf{0.70} & \textbf{0.08} & 0.35 \\
DIF         & 0.21 & 0.26 & 0.6 & 0.39 & 0.39 & 0.67 & 8.85 & 6.9 \\
AE & 0.21 & 0.25 & 0.59 & 0.44 & 0.42 & 0.69 & 16.7 & 0.29 \\
\hline
\end{tabular}
\end{table}


\subsubsection{Importance Plots}

\ale{In Figure \ref{fig:interpretation-annthyroid}, the interpretation plots for both scenarios reveal Feature 1 as the most significant, exhibiting greater robustness in Scenario II, where the model was trained solely on inliers. This robustness likely stems from enhanced precision scores. The scoremaps in Figures \ref{fig:Local-annthyroid} and \ref{fig:Local-annthyroid-split} highlight a unique distribution pattern across Features 1 and 5, suggesting a dependency between them. Notably, anomalies predominantly align along Feature 1, despite some outliers along Feature 5 that appear distanced from the normal distribution, potentially impacting negatively the right prediction of the outliers which has a significant effect on interpretation outcomes. In Scenario II, the local scoremap more clearly demonstrates how anomalies are concentrated in areas where Feature 1 holds greater significance, offering insights into the feature's critical role in anomaly distribution.}

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Annthyroid/Importance_plots/02-03-2024_16-24-07_GFI_Bar_plot_annthyroid_EXIFFI+_1.pdf}
      \caption{Score Plot {\ttfamily Annthyroid} Scenario I}
      \label{fig:Feat-imp-Annthyroid}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.27\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Annthyroid/Importance_plots/02-03-2024_16-24-08_GFI_Score_plot_annthyroid_EXIFFI+_1.pdf}
      \caption{Bar Plot {\ttfamily Annthyroid} Scenario I}
      \label{fig:GFI-annthyroid}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Annthyroid/Local_Scoremap/15-03-2024_11-53-38_importance_map_annthyroid_EXIFFI+_1_feat_1_3.pdf}
      \caption{Scoremap {\ttfamily Annthyroid} Scenario I}
      \label{fig:Local-annthyroid}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Annthyroid/Importance_plots/02-03-2024_14-48-10_GFI_Bar_plot_annthyroid_EXIFFI+_2.pdf}
      \caption{Score Plot {\ttfamily Annthyroid} Scenario II}
      \label{fig:Feat-imp-Annthyroid-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.27\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Annthyroid/Importance_plots/02-03-2024_14-48-10_GFI_Score_plot_annthyroid_EXIFFI+_2.pdf}
      \caption{Bar Plot {\ttfamily Annthyroid} Scenario II}
      \label{fig:GFI-annthyroid-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Annthyroid/Local_Scoremap/21-03-2024_16-16-30_importance_map_annthyroid_EXIFFI+_2_feat_1_3.pdf}
      \caption{Scoremap {\ttfamily Annthyroid} Scenario II}
      \label{fig:Local-annthyroid-split}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot and Scoremap for {\ttfamily Annthyroid} in the two different Scenarios, using the \approach algorithm applied to the \EIFplus model.}\label{fig:interpretation-annthyroid}
\end{figure}


\subsubsection{Feature Selection}

\ale{Figure \ref{fig:interpretation-annthyroid} showcases the Feature Selection plots derived from the feature rankings provided by two distinct interpretation algorithms for each of the three Isolation based model, including one ad-hoc and one post-hoc interpretation via a surrogate Random Forest model. These plots depict the average precision achieved by the \EIFplus model on the dataset, progressively excluding the least important feature as identified by each interpretation algorithm (illustrated by the red line), and excluding the most important feature at every step (shown by the blue line). The similarity in the plots, particularly within the extent of the red areas, indicates that the Feature Selection outcomes are largely equivalent.} 

\begin{figure}[htbp] 
\centering
\hspace{0.05\textwidth}\textbf{IF} \hspace{0.29\textwidth} \textbf{EIF} \hspace{0.29\textwidth} \textbf{EIF+}
% First row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Ad-Hoc}}} % Adjust the parbox width as necessary for your caption text
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Annthyroid/Feature_Selection/06-05-2024_12-36-37_annthyroid_EIF+_IF_EXIFFI_feature_selection_2.pdf}
            \caption{\approach applied to IF}
            \label{fig:Feat-Sel_Annthyroid_valEIF+_DIFFI_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Annthyroid/Feature_Selection/19-03-2024_20-56-49_annthyroid_EIF+_EXIFFI_feature_selection_2.pdf}
            \caption{\approach applied to EIF}
            \label{fig:Feat-Sel_Annthyroid_valEIF+_EXIFFI_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Annthyroid/Feature_Selection/19-03-2024_20-55-10_annthyroid_EIF+_EXIFFI+_feature_selection_2.pdf}
            \caption{\approach applied to \EIFplus}
            \label{fig:Feat-Sel_Annthyroid_valEIF+_EXIFFI+_2}
        \end{subfigure}
    \end{minipage}
\end{minipage}

\vspace{5mm} % Space between rows

% Second row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Post-Hoc}}} % Adjust as necessary
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Annthyroid/Feature_Selection/19-03-2024_21-02-17_annthyroid_EIF+_IF_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to IF}
            \label{fig:Feat-Sel_Annthyroid_valEIF+_IF_RandomForest_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Annthyroid/Feature_Selection/19-03-2024_21-00-45_annthyroid_EIF+_EIF_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to EIF}
            \label{fig:Feat-Sel_Annthyroid_valEIF+_EIF_RandomForest_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Annthyroid/Feature_Selection/19-03-2024_20-59-32_annthyroid_EIF+_EIF+_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to \EIFplus}
            \label{fig:Feat-Sel_Annthyroid_valEIF+_EIF+_RandomForest_2}
        \end{subfigure}
    \end{minipage}
\end{minipage}

\caption{Feature Selection of the different Ad-Hoc and Post-Hoc methods applied to the 3 Isolation Forest models: IF, EIF and \EIFplus. The blue line is the values of average precision, calculated with the \EIFplus model in the Scenario II, dropping the most important feature at each step, the red line is the values of average precision dropping the least important feature at each step and the green line is the value of the feature selection dropping a random feature at each step.}\label{fig:feature_selections-annthyroid}
\end{figure}

\ale{Table \ref{tab:fs-tab-annthyroid}  highlights distinct performance variations between Scenario I and Scenario II, with Scenario I showing reduced effectiveness overall, particularly in post-hoc interpretation methods. This trend suggests that reliance on post-hoc interpretations might be less beneficial when the performance of anomaly detection (AD) models is low. In contrast, ad-hoc interpretation methods exhibit more consistency and slightly improved results in Scenario II, surpassing post-hoc techniques. Among these, the interpretation of the \approach applied to the IF model stands out for its superior efficiency. Moreover, the execution speed of ad-hoc interpretations notably exceeds that of post-hoc methods, emphasizing ad-hoc strategies' effectiveness and speed across different scenarios.}

\begin{table}[htbp]
\centering
\caption{Quantitative evaluation of the effectiveness of 6 different interpretation algorithms on {\ttfamily Annthyroid} through the $AUC_{FS}$ metric, introduced in \ref{sec:interpr_evaluat}. In the last column the average time taken by the different models to produce the importance scores is reported. The highest $AUC_{FS}$ and lowest Importance time values are highlighted in bold.}\label{tab:fs-tab-annthyroid}
\begin{tabular}{|c||c|c|c|c||c|}
\toprule
\hline
&\multicolumn{2}{c|}{Evaluation with EIF}&\multicolumn{2}{c||}{Evaluation with \EIFplus}&\\
\hline
& Scenario I & Scenario II & Scenario I & Scenario II & Time\\

 Algorithm & $AUC_{FS}$  & $AUC_{FS}$ & $AUC_{FS}$  & $AUC_{FS}$ &  \\
\hline
DIFFI         & 0.963      & 2.040& 0.910& 2.000& 0.57 \\
IF\_\approach         & \textbf{1.127}      & \textbf{2.259}& \textbf{1.103}& \textbf{2.238}& 0.93 \\
EIF\_\approach        & 0.985& 2.032& 0.937& 1.922& \textbf{0.55} \\
\EIFplus\_\approach       & 0.983 & 2.180& 0.975& 2.174& 0.59 \\
IF\_RF        & 0.453& 2.055& 0.429& 1.999& 2.82 \\
EIF\_RF       & -0.689& 2.034& -0.672& 1.97& 2.82 \\
EIF+\_RF      & -1.198& 2.094& -1.165& 2.029& 2.82 \\
\hline
\end{tabular}
\end{table}





==> sections/sections_world_dataset_results/breast.tex <==

\subsubsection{{\ttfamily Breast}} 

%\modifica{introduzione a breastw}

The {\ttfamily Breast} dataset is normally used for the Binary Classification.
%task of distinguishing between female patients suffering or not of breast cancer using medical data. 
Following the usual procedure, the dataset was converted into a dataset tailored for the Anomaly Detection task. As explained in Appendix \ref{sec:real-world-data}, the peculiarity of this dataset is that its nine features are categorical. This fact makes the Anomaly Detection and interpretability tasks more challenging. 
%\todo[inline, color=red]{Vista la natura categorica del dataset, sarei per  mandarlo in appendice, a meno che non vogliate sottolineare che ExIFFI funziona anche su feature categoriche (Chiara)}

%\modifica{mettere risultati importances nel caso in cui è allenata interamente}

\begin{figure}[!ht] 
    \centering % <-- added
     \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]
      {figures/breastw/Feat_bar_plot_breastw.pdf}
      \caption{Score Plot {\ttfamily Breast} Scenario I}
      \label{fig:Feat-imp-breast}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]
      {figures/breastw/Feat_bar_plot_breastw_split.pdf}
      \caption{Score Plot {\ttfamily Breast} Scenario II}
      \label{fig:Feat-imp-breast-split}
      \end{subfigure}
      \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/breastw/GFI_breastw_synt.pdf}
      \caption{Bar Plot {\ttfamily Breast} Scenario I}
      \label{fig:GFI-breast}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]
       {figures/breastw/GFI_breastw_split_synt.pdf}
      \caption{Bar Plot {\ttfamily Breast} Scenario II}
      \label{fig:GFI-breast-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]
      {figures/scoremaps_real_world/Local_Scoremap_Plot_breast.png}
      \caption{Scoremap {\ttfamily Breast} Scenario I}
      \label{fig:Local-breast}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/scoremaps_real_world/Local_Scoremap_Plot_breast_split.png}
      \caption{Scoremap {\ttfamily Breast} Scenario II}
      \label{fig:Local-breast-split}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot and Scoremap for breast }
\label{fig:interpretation-breast}
\end{figure}
    


%\modifica{Qua la Feture 8 è dominate nell'importanza in quanto viene sempre selezionata come prima. E' un pò più complicato per questo dataset analizzare la Local Scoremap visto che le variabili sono categoriche. Infatti in questo caso le stelline sono distribuite sia lungo la feature 8 che lungo la feature 2.}

The Bar Plot, in Figure \ref{fig:GFI-breast}, recognized Feature 8 as the most important feature as highlighted also in the Score Plot, represented in Figure \ref{fig:Feat-imp-breast}, where it has a significant margin, in terms of average importance score, towards the other attributes. 

Because of the categorical nature of the features composing the {\ttfamily Breast} dataset analysing the Scoremap (Figure \ref{fig:Local-breast} is not as straightforward as for the other datasets. In fact the grid-like data distribution shows anomalous samples scattered along both Feature 8 and Feature 2 and some pairs of inliers and outliers are even overlapped. 

However, there is a clear separation between deviant and normal points and high differences in terms of Anomaly Score, according to the positions of the contour lines, thus the Average Precision values reported in Table \ref{tab:avg-prec-table} are considerably high. 

%\modifica{mettere tabella precisioni allenato su tutto}

%\begin{table}[ht]
%\parbox{.45\linewidth}{
%\centering
%\begin{tabular}{|c|ccc|}
%\hline
%\multicolumn{4}{|c|}{\textbf{breast} complete training} \\ \hline
%\textbf{Metric} & \textbf{IF} & \textbf{EIF} & \textbf{EIF+} \\ \hline
%Precision         & 0.90 & 0.89 & 0.87 \\
%Recall            & 0.90 & 0.89 & 0.87 \\
%f1 score          & 0.90 & 0.89 & 0.87 \\
%Accuracy          & 0.89 & 0.88 & 0.86 \\
%Average Precision & 0.95 & 0.92 & 0.90 \\
%ROC AUC Score     & 0.96 & 0.94 & 0.93 \\ \hline
%\end{tabular}
%\caption{Performance Report \texttt{Breast} Dataset}
%\label{tab:breast-perf-complete}}
%\end{table}

%\modifica{Qua le prestazioni sono molto buone, lungo tutte le metriche, per tutti i modelli con differenze minime tra i tre. Questo probabilmente è dovuto alla struttura a griglia con cui si distribuiscono i dati come si può chiaramente vedere dalla scoremap. Quindi anche i tagli solo verticali o orrizontali apportati dal modello IF permettono di isolare le anomalie.}




%\modifica{far vedere nel caso in cui si splitta il training per capire se va meglio}

%\modifica{Grazie all'applicazione del training solo sugli inlier la Feature 2 assume maggiore importanza e, come già si intuiva dai risultati spiegati nel caso in cui il modello era stato allenato sull'intero dataset, arriva quasi allo stesso livello di importanza della Feature 8 che comunque rimane sempre al primo posto. Nella Local Scoremap si vede come i contour plot degli Anomaly Score si concentrino di più verso la regione sinistra dello spazio che è quella dove si concentrano gli inlier.}

As a result of the application of the inlier training strategy in the Score Plot (Figure \ref{fig:Feat-imp-breast-split}), Feature 2 assumes higher positions in the ranking of the average importance scores by taking the second place behind Feature 8 that is still considered the most important. 

The Scoremap, in Figure \ref{fig:Local-breast-split}, is composed by Anomaly Scores contour lines focused on the left side portion of the feature space, thus increasing the separation between inliers and outliers. As a consequence, there is a further improvement in the performance metric reported in Table \ref{tab:avg-prec-table}. 

%\modifica{inserire tabella precisioni e vedere di quanto è migliorata e come potrebbe aver influito nell'interpretazione}

%\begin{table}[ht]
%\parbox{.45\linewidth}{
%\centering
%\begin{tabular}{|c|ccc|}
%\hline
%\multicolumn{4}{|c|}{\textbf{breast} inlier training} \\ 
%\hline
%\textbf{Metric} & \textbf{IF} & \textbf{EIF} & 
%\textbf{EIF+} \\ \hline
%Precision         & 0.95 & 0.94 & 0.94 \\
%Recall            & 0.95 & 0.94 & 0.94 \\
%f1 score          & 0.95 & 0.94 & 0.94 \\
%Accuracy          & 0.95 & 0.94 & 0.94 \\
%Average Precision & 0.99 & 0.98 & 0.99 \\
%ROC AUC Score     & 0.99 & 0.98 & 0.99 \\ \hline
%\end{tabular}
%\caption{Performance Report \texttt{breast} Dataset}
%\label{tab:breast-perf-split}
%}
%\end{table}

%\modifica{La conseguenza di quanto osservabile nella Local Scoremap è che aumentano i valori per tutte le metriche arrivando quasi al massimo valore raggiungibile di 1. }


\begin{figure}
  \centering
  \includegraphics[width=0.7\linewidth]{figures/feature_selection_plots_final/featsel_breastw_final.pdf}
  \caption{Feature Selection {\ttfamily Breastw}}
  \label{fig:fs-breastw-plus}
\end{figure}\hfil % <-- added

Figure \ref{fig:fs-breastw-plus} reports the Feature Selection Plot for the {\ttfamily Breast} dataset.
The behavior is similar for all the Feature Ranking Algorithms presented with the Average Precision decreasing as the number of features decreases. The situation depicted in Figure \ref{fig:fs-breastw-plus} confirms the high uncertainty in finding a dominant feature in the {\ttfamily Breastw} dataset and the presence of a shared importance among multiple features. The result is that the decrease in the input features may remove some of the features that are part of the subset carrying all the importance and thus the Average Precision of the model suffers a decrease. 




%\davide {
%The interpretation results obtained for the {\ttfamily Breast} dataset, presented in Section \ref{sec:real-world-data}, are reported in Figure \ref{fig:breast}. 
%For what concerns the feature importance according to \approach the situation is not very clear in fact there are 5 features that were selected as the most important ones (8,6,4,1, and 0) at least in one execution. These features represent respectively Mitoses, Bland Chromatin, Single Epithelial Cell Size, Uniformity of Cell Size, and Clump Thickness. From an intuitive point of view, all these attributes seem to be relevant factors for the determination of the presence of breast cancer. 
%and in \ref{fig:Feat-imp-breast} the average scores are very similar among all the features. 

%Feature 8 and Feature 0 were compared in Figure \ref{fig:Local-breast} in the Local Importance Scoremap. As it can be noticed from the scoremap the anomalies are mainly distributed along Feature 8 thus the main importance is carried by Feature 8 in fact using a 1 dimensional hyperplane on this feature is possible to isolate the outliers easily. Moreover, along Feature 8 it is also possible to detect some inliers far from their main distribution. This means that these samples can be labeled as \textit{model anomalies}. 

%}
%\davide {
%Exceptionally good detection performances can be observed in Table \ref{tab:breast-perf}. Following the outcomes achieved on the benchmark datasets previously described the superior generalization capabilities of the EIF+ confirm it as the top performing model also in the {\ttfamily Breast} dataset, still followed by the EIF and IF models, in this order. 
%}



==> sections/sections_world_dataset_results/breastw_new.tex <==
\subsection*{{\ttfamily Breastw}} \label{sec:Breastw}

\subsubsection{Performance}

\ale{Figure \ref{fig:Breastw_contamination_full} portraits the trend of the Average Precision metric as the contamination of the training set enlarges from 0 to 10 \% on the different AD methods discussed in Section \ref{sec:performance_evaluation}. It can be noticed how all the models perform more or less perfectly (i.e. with a score of 1) independently on the amount of anomalous samples seen at training time except for the DIF model that shows low precision values, around 0.6.}

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.49\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Breastw/Contamination/21-03-2024_15-44-24_breastw_contamination_full_plot.pdf}
      \caption{ }
      \label{fig:Breastw_contamination_full}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.44\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Breastw/Contamination/21-03-2024_15-46-45_breastw_EIF+_minus_EIF_precision_over_contamination.pdf}
      \caption{ }
      \label{fig:Breastw_contaminationEIFvsEIF+}
    \end{subfigure}\hfil % <-- added
\caption{Fig. \ref{fig:Breastw_contamination_full} Represent the average precision the more the level of contamination of the train set is increased. The Fig. \ref{fig:Breastw_contaminationEIFvsEIF+} Give show specifically the graphs of the EIF and EIF+}
\label{fig:Breastw_contamination}
\end{figure}

\ale{In Table \ref{tab:Breastw_perf}  it is possible to compare in detail different typical metrics used to assess the overall performances of AD models. In particular dividing the evaluation between Scenario I and Scenario II it is possible to observe how these two training strategies may or may not affect the model's performances. With regard to the {\ttfamily Breastw} dataset one can discern that there is a clear difference between the two scenarios only for the DIF model (that is in fact the only model not showing a perfectly constant trend in the Contamination Plot of Figure \ref{fig:Breastw_contamination_full}) while the other models manifest only minor changes passing from Scenario I to Scenario II. Finally in the context of time efficiency a significant gap can be observed between isolation-based approaches (i.e. IF, EIF and \EIFplus) and AD methods based on deep learning models (i.e. DIF and Autoencoder).}

\begin{table}[htbp]
\begin{minipage}[t]{0.46\textwidth}
\strut\vspace*{-\baselineskip}\newline
\resizebox{\textwidth}{!}{
%\caption{{\ttfamily Breastw} Precision Report}
\begin{tabular}{|c||ccc|ccc||cc|}
\toprule
\hline
&\multicolumn{3}{c|}{Scenario I}&\multicolumn{3}{c||}{Scenario II}&\multicolumn{2}{c|}{Time}\\
\hline
AD Model & Avg & Prec & ROC & Avg & Prec & ROC & fit & pred \\
& Prec &  & AUC & Prec &  & AUC &  &  \\
\hline
IF          & \textbf{0.96}& \textbf{0.90}& \textbf{0.90}& 0.99& 0.94& 0.94& \textbf{0.11}& 0.005\\
EIF         & 0.91& 0.86& 0.86& 0.98& 0.93& 0.93& 0.12& 0.0007\\
EIF+        & 0.88& 0.85& 0.84& \textbf{0.99}& \textbf{0.95}& \textbf{0.95}& 0.12& \textbf{0.0006}\\
DIF         & 0.44& 0.49& 0.46& 0.60& 0.66& 0.64& 0.74& 0.58\\
AE & 0.61& 0.44& 0.41& 0.98& 0.94& 0.93& 2.56& 0.05\\
\hline
\end{tabular}}
\vspace{0.41cm}
\caption{Performances of 5 different Anomaly Detection models over {\ttfamily Breastw} are compared using classical Classification metrics. Moreover, the last two columns contain the average time for a fit and predict operation. The highest metric values and the lowest execution times are highlighted in bold}\label{tab:Breastw_perf}
\end{minipage}
\hfill
\begin{minipage}[t]{0.46\textwidth}
\strut\vspace*{-\baselineskip}\newline
\resizebox{\textwidth}{!}{
\begin{tabular}{|c||c|c|c|c||c|}
\toprule
\hline
&\multicolumn{2}{c|}{Evaluation with EIF}&\multicolumn{2}{c||}{Evaluation with \EIFplus}&\\
\hline
& Scenario I & Scenario II & Scenario I & Scenario II & Time\\

 Algorithm & $AUC_{FS}$  & $AUC_{FS}$ & $AUC_{FS}$  & $AUC_{FS}$ &  \\
\hline
DIFFI         & 0.11& 0.064& 0.083& 0.067& 0.46\\
IF\_\approach        & \textbf{0.25}& 0.082& \textbf{0.284}& 0.087& 0.10\\
EIF\_\approach        & 0.044& 0.062& 0.026& 0.084& \textbf{0.04}\\
\EIFplus\_\approach       & 0.079& 0.027& 0.084& 0.063& 0.04\\
IF\_RF        & -0.148& 0.091& -0.142& 0.063& 0.19\\
EIF\_RF       & -0.181& \textbf{0.109}& -0.169& \textbf{0.090}& 0.19\\
EIF+\_RF      & -0.164& 0.104& -0.145& 0.079& 0.19\\
\hline
\end{tabular}}
\caption{Quantitative evaluation of the effectiveness of 6 different interpretation algorithms on {\ttfamily Breastw} through the $AUC_{FS}$ metric, introduced in \ref{sec:interpr_evaluat}. In the last column the average time taken by the different models to produce the importance scores is reported. The highest $AUC_{FS}$ and lowest Importance time values are highlighted in bold.}\label{tab:fs-tab-Breastw}
\end{minipage}
\end{table}


\subsubsection{Importance Plots}

\ale{The peculiar grid-like distribution of samples within the {\ttfamily Breastw} dataset, as exhibited in the Figure \ref{fig:Local-Breastw}, generates interpretation results in the Bar and Score plots not aligned with the typical outcomes described in the other real world datasets included in this study. Indeed discerning the distribution of relevance scores between different attributes is easier in Scenario I where Feature 8 clearly emerges as the crucial feature (Figure \ref{fig:Feat-imp-Breastw}  while in Scenario II the latter, still considered the most prominent as shown in Figure \ref{fig:Feat-imp-Breastw-split}, is associated with a lower margin on the other features. Figures \ref{fig:Local-Breastw} and \ref{fig:Local-Breastw-split}  illustrate the Local Scoremap that are not particularly effective in showing the distribution of anomalies as points easy to isolate from others because of the grid-like distribution of samples.}

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Breastw/Importance_plots/02-03-2024_16-21-20_GFI_Bar_plot_breastw_EXIFFI+_1.pdf}
      \caption{Score Plot {\ttfamily Breastw} Scenario I}
      \label{fig:Feat-imp-Breastw}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.27\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Breastw/Importance_plots/02-03-2024_16-21-20_GFI_Score_plot_breastw_EXIFFI+_1.pdf}
      \caption{Bar Plot {\ttfamily Breastw} Scenario I}
      \label{fig:GFI-Breastw}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Breastw/Local_Scoremaps/21-03-2024_16-11-20_importance_map_breastw_EXIFFI+_1_feat_8_2.pdf}
      \caption{Scoremap {\ttfamily Breastw} Scenario I}
      \label{fig:Local-Breastw}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Breastw/Importance_plots/02-03-2024_14-45-18_GFI_Bar_plot_breastw_EXIFFI+_2.pdf}
      \caption{Score Plot {\ttfamily Breastw} Scenario II}
      \label{fig:Feat-imp-Breastw-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.27\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Breastw/Importance_plots/02-03-2024_14-45-19_GFI_Score_plot_breastw_EXIFFI+_2.pdf}
      \caption{Bar Plot {\ttfamily Breastw} Scenario II}
      \label{fig:GFI-Breastw-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Breastw/Local_Scoremaps/21-03-2024_16-11-10_importance_map_breastw_EXIFFI+_2_feat_8_2.pdf}
      \caption{Scoremap {\ttfamily Breastw} Scenario II}
      \label{fig:Local-Breastw-split}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot and Scoremap for {\ttfamily Breastw}  in the two different Scenarios, using the \approach algorithm applied to the \EIFplus model.}\label{fig:interpretation-Breastw}
\end{figure}

\subsubsection{Feature Selection}

\ale{The series of plots contained in Figure \ref{fig:fs-interpretation-Breastw}  confirms the uncertainty in distributing the importance of different features in this particular set of data. In fact for all the interpretation algorithms evaluated there is not a significant difference in applying the Unsupervised Feature Selection proxy task in increasing (red line) or decreasing (blue line) order of feature relevance. Notably also the green line, representing a Feature Selection strategy in which a random feature is removed at each step, is almost overlapped to the other two meaning that there is not a single or a group of features with an importance significantly higher than the others. As a result, the quantitative measures of interpretability efficiency, represented by the $AUC_{FS}$ metric, are all approximately equal to zero. The trend of the Average Precision metric is roughly constant at perfect scores (i.e. close to 1) until the number of features composing the input space is reduced to 3 where the Average Precision starts to decrease its magnitude. The likely implication is that the model needs at least three features to maintain acceptable performances in detecting outliers. It is possible to conclude that the behavior depicted by plots below is very similar to the one observed for the {\ttfamily Bisect6D} synthetic dataset (Section \ref{sec:Bisect6D}), where the anomalies were distributed across all the features.}

\begin{figure}[!ht] 
\centering
\hspace{0.05\textwidth}\textbf{IF} \hspace{0.29\textwidth} \textbf{EIF} \hspace{0.29\textwidth} \textbf{EIF+}
% First row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Ad-Hoc}}} % Adjust the parbox width as necessary for your caption text
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Breastw/Feature_Selection/07-05-2024_14-38-59_breastw_EIF+_IF_EXIFFI_feature_selection_2.pdf}
            \caption{\approach applied to IF}
            \label{fig:Feat-Sel_Breastw_valEIF+_DIFFI_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Breastw/Feature_Selection/21-03-2024_09-06-25_breastw_EIF+_EXIFFI_feature_selection_2.pdf}
            \caption{\approach applied to EIF}
            \label{fig:Feat-Sel_Breastw_valEIF+_EXIFFI_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Breastw/Feature_Selection/21-03-2024_09-03-35_breastw_EIF+_EXIFFI+_feature_selection_2.pdf}
            \caption{\approach applied to \EIFplus}
            \label{fig:Feat-Sel_Breastw_valEIF+_EXIFFI+_2}
        \end{subfigure}
    \end{minipage}
\end{minipage}

\vspace{5mm} % Space between rows

% Second row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Post-Hoc}}} % Adjust as necessary
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Breastw/Feature_Selection/21-03-2024_09-10-01_breastw_EIF+_IF_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to IF}
            \label{fig:Feat-Sel_Breastw_valEIF+_IF_RandomForest_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Breastw/Feature_Selection/21-03-2024_09-09-40_breastw_EIF+_EIF_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to EIF}
            \label{fig:Feat-Sel_Breastw_valEIF+_EIF_RandomForest_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Breastw/Feature_Selection/21-03-2024_09-09-20_breastw_EIF+_EIF+_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to \EIFplus}
            \label{fig:Feat-Sel_Breastw_valEIF+_EIF+_RandomForest_2}
        \end{subfigure}
    \end{minipage}
\end{minipage}

\caption{Feature Selection of the different Ad-Hoc and Post-Hoc methods applied to the 3 Isolation Forest models: IF, EIF and \EIFplus. The blue line is the values of average precision, calculated with the \EIFplus model in the Scenario II, dropping the most important feature at each step, the red line is the values of average precision dropping the least important feature at each step and the green line is the value of the feature selection dropping a random feature at each step.}\label{fig:fs-interpretation-Breastw}
\end{figure}

\ale{As already discussed in previous sections, in the {\ttfamily Breastw} dataset the relevance is evenly shared across most of the features and consequently there it not possible to identify an interpretation method that achieves a better explanation than the others. We can indeed consider the slight differences in the $AUC_{FS}$ values grouped in Table \ref{tab:fs-tab-Breastw} as a result of the stochasticity inherently present in the attribution of importance scores. Finally it is important to note how the interpretations obtained with the proposed approach \approach are an order of magnitude faster with the respect to post-hoc RandomForest based interpretations, making \approach certainly more appealing to be exploited in a practical application.} 


==> sections/sections_world_dataset_results/cardio.tex <==

\subsubsection{{\ttfamily Cardio}}
%\modifica{richiamare introduzione al dataset della sezione \ref{sec:real-world-data}}

The {\ttfamily Cardio} dataset is part of the UCI Machine Learning Repository. It was adapted to be used for the Anomaly Detection task since originally it is used for a three-class Classification Task. It is formed by twenty-one features which will be carefully analyzed, in terms of importance, in this section. Further details on this dataset can be found in Appendix \ref{sec:real-world-data}. 

%\modifica{interpretazioni dataset completo}
\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/cardio/Feat_bar_plot_cardio.pdf}
      \caption{Score Plot {\ttfamily Cardio} Scenario I}
      \label{fig:Feat-imp-cardio}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/cardio/Feat_bar_plot_cardio_split.pdf}
      \caption{Score Plot {\ttfamily Cardio} Scenario II}
      \label{fig:Feat-imp-cardio-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/cardio/GFI_cardio_synt.pdf}
      \caption{Bar Plot {\ttfamily Cardio} Scenario I}
      \label{fig:GFI-cardio}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/cardio/GFI_cardio_split_synt.pdf}
      \caption{Bar Plot {\ttfamily Cardio} Scenario II}
      \label{fig:GFI-cardio-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/scoremaps_real_world/Local_Scoremap_Plot_cardio.png}
      \caption{Scoremap {\ttfamily Cardio} Scenario I}
      \label{fig:Local-cardio}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/scoremaps_real_world/Local_Scoremap_Plot_cardio_split.png}
      \caption{Scoremap {\ttfamily Cardio} Scenario II}
      \label{fig:Local-cardio-split}
    \end{subfigure}\hfil % <-- added
\caption{GFI Bar Plot, Feature Importance Plot and Local Importance Scoremap for {\ttfamily Cardio} }\label{fig:interpretation-cardio}
\end{figure}

%\modifica{L'algoritmo di interpretazione vede la feature 2 e la feature 6 come le più importanti, però non con molta consistenza nel riconoscerle}
%\modifica{dallo scoremap si riesce a vedere come effettivamente siano entrambe direzioni in cui dei punti deviano dalla distribuzione normale del dataset che è maggiormente centrata in (0,0) e che la feature 2 ha anomalie leggermente più distanti dal centro della distribuzione}

The Score Plot, illustrated in Figure \ref{fig:Feat-imp-cardio}, shows how the interpretation algorithm identifies Feature 2 and Feature 6 as the most important but with limited consistency. In fact the Bar Plot, in Figure \ref{fig:GFI-cardio}, depicts how Feature 2 was selected as the top feature 80\% of the time while Feature 6 only 10\% of the time. 

After careful observation of the Scoremap, in Figure \ref{fig:Local-cardio}, it is possible to conclude that, indeed, Feature 2 and 6 are directions along which there is an accumulation of anomalous points deviating from the normal dataset distribution, which is centered in (0,0). Furthermore, it can be noticed that outliers connected to Feature 2 are slightly further from the distribution center than the ones placed along Feature 6. 

\begin{comment}
\begin{table}[ht]
\parbox{.45\linewidth}{
\centering
\begin{tabular}{|c|ccc|}
\hline
\multicolumn{4}{|c|}{\textbf{cardio} complete training} \\ \hline
\textbf{Metric} & \textbf{IF} & \textbf{EIF} & \textbf{EIF+} \\ \hline
Precision         & 0.50 & 0.54 & 0.53 \\
Recall            & 0.50 & 0.54 & 0.53 \\
f1 score          & 0.50 & 0.54 & 0.53 \\
Accuracy          & 0.90 & 0.91 & 0.91 \\

Average Precision & 0.58 & 0.56 & 0.53 \\
ROC AUC Score     & 0.93 & 0.93 & 0.93 \\ \hline
\end{tabular}
\caption{Performance Report \texttt{cardio} Dataset}
\label{tab:cardio-perf-complete}}
\end{table}
\end{comment}

%\modifica{la tabella delle precisioni ci fa vedere che l'algoritmo ha una precisione mediocre proviamo a migliorarla dividendo tra inlier e outliers}

Table \ref{tab:avg-prec-table} reports the Average Precision values for the {\ttfamily Cardio} dataset. The metric values are similar among the three models under analysis with a slight advantage of the \EIFplus model. The metrics values however are not outstandingly good, so they can be improved by adopting the strategy of training the model solely on the inlier data and successively testing it on the complete dataset. 


%\modifica{dall'interpretazione si vede come l'algoritmo sia molto più sicuro nel riconoscere giustamente la feature 6 come la più importante per la distribuzione degli outlier, e lo scoremap in questo caso, siccome il modello è stato trainato solo sugli inliers, è più centrato lungo la verticale, con una zona di score di importanza schiarita e ristretta in verticale, dunque diminuito il peso di quella feature.Inoltre vediamo come i punti anomali di destra escano maggiormente dai contourplots quindi vengono riconosciuti di più come anomalie. Infatti la tabella seguente evidenzia un netto aumento in precisione rispetto al modello precedente, ciò ci da maggiore sicurezza nella reliability dell'interpretazione}

Observing the Bar Plot, in Figure \ref{fig:GFI-cardio-split}, it is possible to notice how the model has increased its level of confidence in recognizing Feature 6 as the most relevant one. Moreover, its Importance Score is significantly higher than the ones of the other features as reported in the Score Plot in Figure \ref{fig:Feat-imp-cardio-split}. One of the consequences of the inlier training can be appreciated in the Scoremap in Figure \ref{fig:Local-cardio-split} where the region of the space colored in red reduced a lot its extension and intensity with respect to Figure \ref{fig:Local-cardio} meaning that the importance of Feature 2 decreased a lot in favor of Feature 6. Moreover, the contour lines, used to highlight the different Anomaly Score values, are shifted towards the inliers making it easier to recognize the samples placed on the right extremes of the plot as anomalies. 

\begin{comment}
\begin{table}[ht]
\parbox{.45\linewidth}{
\centering
\begin{tabular}{|c|ccc|}
\hline
\multicolumn{4}{|c|}{\textbf{cardio} inlier training} \\ \hline
\textbf{Metric} & \textbf{IF} & \textbf{EIF} & \textbf{EIF+} \\ \hline
Precision         & 0.63 & 0.73 & 0.73 \\
Recall            & 0.63 & 0.73 & 0.73 \\
f1 score          & 0.63 & 0.73 & 0.73 \\
Accuracy          & 0.93 & 0.95 & 0.95 \\

Average Precision & 0.71 & 0.74 & 0.78 \\
ROC AUC Score     & 0.96 & 0.97 & 0.97 \\ \hline
\end{tabular}
\caption{Performance Report \texttt{cardio} Dataset}
\label{tab:cardio-perf-split}}
\end{table}
\end{comment}

Encouraging results are encountered also in Table (Table \ref{tab:avg-prec-table}) with an increase of the Average Precision values for all the models meaning that there is higher confidence in the reliability of the interpretation results. 


%\modifica{la feature selection ci da la conferma di aver selezionato la giusta feature vedendo una maggiore performance del modello in caso in cui utilizziamo il precedente ordine di importanza}

\begin{figure}
  \centering
  \includegraphics[width=0.7\linewidth]{figures/feature_selection_plots_final/featsel_cardio_final.pdf}
  \caption{Feature Selection Plot Cardio}
  \label{fig:fs-cardio-plus}
\end{figure}\hfil % <-- added

The outcomes of the application of the Proxy Task of Unsupervised Feature Selection to the {\ttfamily Cardio} dataset can be found in Figure \ref{fig:fs-cardio-plus}. The Casual and Random Forest Feature Ranking algorithms are the worst ones. On the other hand, ExIFFI-plus-split has a similar behavior to the other models until 7 features are reached causing its Average Precision to increase elevating it as the best-performing model by far for multiple steps, confirming the improvements of model performances once the inlier training approach is used. The benefits of the mentioned approach can be noticed also in ExIFFI-split which has a similar behavior to ExIFFI-plus-split providing significantly lower Average Precision scores with respect to the latter solely in the interval between 8 and 4 features. 

The remaining algorithms, on the other hand, show a decreasing trend in the Average Precision values as the number of input features decreases with the exception of DIFFI which presents a sudden increase in its precision values in the passage from 2 to 1 feature. 

%\todo[inline, color=red]{Questo lo possiamo passare in appendice perché la narrazione mi pare simile a quella di annthyroid, o no? (Chiara)}


%\davide {The results provided by the \approach model for the {\ttfamily Cardio} dataset, whose detailed description can be found in Section \ref{sec:real-world-data}, are depicted in Figure \ref{fig:cardio}. 
%Considering the Global Importance Bar Plot, depicted in Figure \ref{figa:GFI-cardio} it is possible to notice a dominance of Feature 6 that is also the most important according to the Feature Importance Score Plot as represented in \ref{fig:Feat-imp-cardio}. The Local Importance Scoremap gives a confirmation of the dominance of Feature 6 in the importance scores for the {\ttfamily Cardio} dataset. In fact, as represented in \ref{fig:Local-cardio}, the anomalies are distributed along Feature 6 in a similar way to what happens in the synthetic datasets {\ttfamily X-xaxis},{\ttfamily X-yaxis} and {\ttfamily X-bisec}. This is the reason why there is a light red portion of the scoremap in correspondence of the inliers distribution while the rest of the scoremap is dominated by the blue color that represents the importance of Feature 6 over Feature 0 also for data points not included in the {\ttfamily Cardio} dataset. 
%According to the list of feature names Feature 6 is coded as DP and it represents the number of prolonged decelerations per second in the hearth beat}

%\davide {
%Table \ref{tab:cardio-perf} reports the Performance Report for the {\ttfamily Cardio} dataset. In this case the results expected from a theoretical point of view are obtained with the EIF+ model being the best one, in terms of F1 Score and Average Precision, followed by the EIF and IF models respectively.
%}


==> sections/sections_world_dataset_results/cardio_new.tex <==
\subsection*{{\ttfamily Cardio}}

\subsubsection{Performance}

\ale{The plot contained in Figure \ref{fig:Cardio_contamination_full} illustrates how the gradual addition of outliers in the training set affects the Average Precision values achieved by various AD models on the {\ttfamily Cardio} dataset. The trend is similar across all the datasets and the difference between the metrics values across the models are minor: passing from 0 to 10 \% of contamination the Average Precision is associated with a decrease of about 3 percentage points. A focus on the proposed method, \EIFplus, and its counterpart,  EIF, is proposed in Figure \ref{fig:Cardio_contaminationEIFvsEIF+} and it shows how\EIFplus starts from higher values for low contamination levels and it is overcomed by EIF as the number of anomalies included in the fitting stage raises. The following behavior aligns with the expectations associated to the inherent structure of these two algorithms, in fact \EIFplus is optimized in settings where there is a lack of anomalous points in the training set.}

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.49\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Cardio/Contamination/21-03-2024_21-28-11_cardio_contamination_full_plot.pdf}
      \caption{Models evaluation, varying the contamination levels}
      \label{fig:Cardio_contamination_full}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.44\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Cardio/Contamination/21-03-2024_21-29-01_cardio_EIF+_minus_EIF_precision_over_contamination.pdf}
      \caption{Difference between \EIFplus and EIF average precision}
      \label{fig:Cardio_contaminationEIFvsEIF+}
    \end{subfigure}\hfil % <-- added
\caption{Figure \ref{fig:Cardio_contamination_full} illustrates the average precision as the contamination level in the training set increases. Figure \ref{fig:Cardio_contaminationEIFvsEIF+} compares the performance graphs of EIF and \EIFplus, using the difference of their scores in various contamination levels.}
\label{fig:Cardio_contamination}
\end{figure}

\ale{In Table \ref{tab:Cardio_perf}  the AD models are evaluated through some well-known classification metrics in Scenario I and Scenario II. The decreasing trend described in Figure \ref{fig:Cardio_contamination_full} is reflected here not only on the Average Precision metrics but also on Precision and ROC AUC score. From an overall analysis of the metrics the DIF model appears as the one with the highest values of Average Precision but at the same time it is affected by notably elevated fit and prediction times. On the other hand, acceptable metric values and execution times are showed by EIF and \EIFplus making them more appropiate models for this task.}

\begin{table}[htbp]
\begin{minipage}[t]{0.46\textwidth}
\strut\vspace*{-\baselineskip}\newline
\resizebox{\textwidth}{!}{
\begin{tabular}{|c||ccc|ccc||cc|}
\toprule
\hline
&\multicolumn{3}{c|}{Scenario I}&\multicolumn{3}{c||}{Scenario II}&\multicolumn{2}{c|}{Time}\\
\hline
AD Model & Avg & Prec & ROC & Avg & Prec & ROC & fit & pred \\
& Prec &  & AUC & Prec &  & AUC &  &  \\
\hline
IF          & 0.53& 0.44& 0.69& 0.68& 0.60& 0.78& \textbf{0.12}& 0.014\\
EIF         & 0.55& 0.59& 0.77& 0.74& 0.72& 0.84& 0.16& \textbf{0.001}\\
EIF+        & 0.50& 0.52& 0.73& 0.76& \textbf{0.73}& \textbf{0.85}& 0.133& 0.05\\
DIF         & 0.58& 0.52& 0.73& \textbf{0.79}& 0.70& 0.83& 2.81& 2.28\\
AE & \textbf{0.62}& \textbf{0.62}& \textbf{0.79}& 0.83& 0.70& 0.76& 6.1& 0.104\\
\hline
\end{tabular}}
\vspace{0.41cm}
\caption{Performances of 5 different Anomaly Detection models over {\ttfamily Cardio} are compared using classical Classification metrics. Moreover, the last two columns contain the average time for a fit and predict operation. The highest metric values and the lowest execution times are highlighted in bold}\label{tab:Cardio_perf}
\end{minipage}
\hfill
\begin{minipage}[t]{0.46\textwidth}
\strut\vspace*{-\baselineskip}\newline
\resizebox{\textwidth}{!}{
\begin{tabular}{|c||c|c|c|c||c|}
\toprule
\hline
&\multicolumn{2}{c|}{Evaluation with EIF}&\multicolumn{2}{c||}{Evaluation with \EIFplus}&\\
\hline
& Scenario I & Scenario II & Scenario I & Scenario II & Time\\

 Algorithm & $AUC_{FS}$  & $AUC_{FS}$ & $AUC_{FS}$  & $AUC_{FS}$ &  \\
\hline
DIFFI                & 4.653& 4.768& 4.398& 4.333& 0.57 \\
IF\_\approach         & 1.933& 3.496& 2.4& 3.433& 0.36\\
EIF\_\approach        & \textbf{5.417}& 8.286& \textbf{5.122}& 8.381& \textbf{0.34}\\
\EIFplus\_\approach   & 4.421& \textbf{8.609}& 4.252& \textbf{8.730}& \textbf{0.30}\\
IF\_RF               & 1.483& 7.696& 1.282& 7.889& 1.80\\
EIF\_RF              & 1.358& 7.781& 1.353& 7.855& 1.80\\
EIF+\_RF             & 0.320& 8.241& 0.360& 8.302& 1.80\\
\hline
\end{tabular}}
\caption{Quantitative evaluation of the effectiveness of 6 different interpretation algorithms on {\ttfamily Cardio} through the $AUC_{FS}$ metric, introduced in \ref{sec:interpr_evaluat}. In the last column the average time taken by the different models to produce the importance scores is reported. The highest $AUC_{FS}$ and lowest Importance time values are highlighted in bold.}\label{tab:fs-tab-Cardio}
\end{minipage}
\end{table}


\subsubsection{Importance Plots}

\ale{Figure \ref{fig:interpretation-Cardio} exploits the Bar Plot, Score Plot and Local Scoremaps to compare the different explanations provided by \approach+ in Scenario I and Scenario II. In both training strategies Feature 6 and Feature 2 stand out as two of the most relevant features to distinguish between a normal and a pathological condition in a Cardiotogram, as explained in Appendix \ref{sec:appendix-real-world-data}. The Local Scoremaps (Figure \ref{fig:Local-Cardio} and \ref{fig:Local-Cardio-split}) provide a visual aid on how anomalies (represented by red stars) are indeed scattered along the directions identified by the previously cited attributes.}

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.38\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Cardio/Importance_plots/02-03-2024_16-18-44_GFI_Bar_plot_cardio_EXIFFI+_1.pdf}
      \caption{Bar Plot {\ttfamily Cardio} Scenario I}
      \label{fig:GFI-Cardio}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.27\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Cardio/Importance_plots/02-03-2024_16-18-44_GFI_Score_plot_cardio_EXIFFI+_1.pdf}
      \caption{Score Plot {\ttfamily Cardio} Scenario I}
      \label{fig:Feat-imp-Cardio}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Cardio/Local_Scoremap/21-03-2024_21-44-41_importance_map_cardio_EXIFFI+_1_feat_6_2.pdf}
      \caption{Scoremap {\ttfamily Cardio} Scenario I}
      \label{fig:Local-Cardio}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.38\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Cardio/Importance_plots/02-03-2024_14-42-41_GFI_Bar_plot_cardio_EXIFFI+_2.pdf}
      \caption{Bar Plot {\ttfamily Cardio} Scenario II}
      \label{fig:GFI-Cardio-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.27\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Cardio/Importance_plots/02-03-2024_14-42-42_GFI_Score_plot_cardio_EXIFFI+_2.pdf}
      \caption{Score Plot {\ttfamily Cardio} Scenario II}
      \label{fig:Feat-imp-Cardio-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Cardio/Local_Scoremap/21-03-2024_21-44-32_importance_map_cardio_EXIFFI+_2_feat_6_2.pdf}
      \caption{Scoremap {\ttfamily Cardio} Scenario II}
      \label{fig:Local-Cardio-split}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot and Scoremap for {\ttfamily Cardio} in the two different Scenarios, using the \approach algorithm applied to the \EIFplus model.}\label{fig:interpretation-Cardio}
\end{figure}

\subsubsection{Feature Selection}

\ale{The Feature Selection plots portrayed in Figure \ref{fig:fs-interpretation-Cardio} represents a clear marker in support of the superiority of the proposed interpretation algorithms \approach and \approach+. As a matter of fact the plots related to the methods just mentioned, contained in Figure \ref{fig:Feat-Sel_Cardio_valEIF+_EXIFFI_2} and \ref{fig:Feat-Sel_Cardio_valEIF+_EXIFFI+_2}, present a symmetric shape. This is the ideal shape we expected to achieve when this kind of plot for the performance evaluation and comparison of interpretation models was firstly designed. In fact, this shape proves that the model is able to correctly rank all the features according to its importance scores. This happens because as features are removed in increasing order of relevance (red line) the Average Precision displays a constantly increasing trend while a constantly decreasing one can be observed as the most important attributes are progressively excluded from the feature space.}
\begin{figure}[!ht] 
\centering
\hspace{0.05\textwidth}\textbf{IF} \hspace{0.29\textwidth} \textbf{EIF} \hspace{0.29\textwidth} \textbf{EIF+}
% First row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Ad-Hoc}}} % Adjust the parbox width as necessary for your caption text
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Cardio/Feature_Selection/07-05-2024_14-57-41_cardio_EIF+_IF_EXIFFI_feature_selection_2.pdf}
            \caption{\approach applied to IF}
            \label{fig:Feat-Sel_Cardio_valEIF+_DIFFI_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Cardio/Feature_Selection/21-03-2024_21-50-25_cardio_EIF+_EXIFFI_feature_selection_2.pdf}
            \caption{\approach applied to EIF}
            \label{fig:Feat-Sel_Cardio_valEIF+_EXIFFI_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Cardio/Feature_Selection/21-03-2024_21-48-58_cardio_EIF+_EXIFFI+_feature_selection_2.pdf}
            \caption{\approach applied to \EIFplus}
            \label{fig:Feat-Sel_Cardio_valEIF+_EXIFFI+_2}
        \end{subfigure}
    \end{minipage}
\end{minipage}

\vspace{5mm} % Space between rows

% Second row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Post-Hoc}}} % Adjust as necessary
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Cardio/Feature_Selection/21-03-2024_21-55-57_cardio_EIF+_IF_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to IF}
            \label{fig:Feat-Sel_Cardio_valEIF+_IF_RandomForest_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Cardio/Feature_Selection/21-03-2024_21-54-35_cardio_EIF+_EIF_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to EIF}
            \label{fig:Feat-Sel_Cardio_valEIF+_EIF_RandomForest_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Cardio/Feature_Selection/21-03-2024_21-53-11_cardio_EIF+_EIF+_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to \EIFplus}
            \label{fig:Feat-Sel_Cardio_valEIF+_EIF+_RandomForest_2}
        \end{subfigure}
    \end{minipage}
\end{minipage}

\caption{Feature Selection of the different Ad-Hoc and Post-Hoc methods applied to the 3 Isolation Forest models: IF, EIF and \EIFplus. The blue line is the values of average precision, calculated with the \EIFplus model in the Scenario II, dropping the most important feature at each step, the red line is the values of average precision dropping the least important feature at each step and the green line is the value of the feature selection dropping a random feature at each step.}\label{fig:fs-interpretation-Cardio}
\end{figure}

\ale{The direct consequence of the optimal behavior of \approach and \approach+ is certified in Table \ref{tab:fs-tab-Cardio} where these two models display the highest $AUC_{FS}$ values, weather they are evaluated with EIF or \EIFplus. The metric values obtained by \approach applied on IF and post-hoc interpretation based on Random Forest are instead inferior because, as it can be observed in Figures, the increasing trend of the red line is not perfectly mirrored by the blue one that displays a oscillating behavior. To conclude, another point in favour to the proposed approaches is the time taken to obtain the importance scores which is substantially reduced with the respect to the ones of the other models considered.}







==> sections/sections_world_dataset_results/diabetes.tex <==
\subsubsection{{\ttfamily Diabetes}}

The {\ttfamily Diabetes} dataset is originally exploited for the Binary Classification task since it contains medical records about patients who may or may not suffer from diabetes disease. As usual, the dataset was modified accordingly to be used for the Anomaly Detection task, details about that are contained in Appendix \ref{sec:real-world-data}. 
%Finally, the dataset is constituted by 4 numerical features, deeply studied in the interpretation analysis that follows. 

%\modifica{mettere risultati importances nel caso in cui è allenata interamente sul dataset di diabetes}

\begin{figure}[!ht] 
    \centering % <-- added

    \begin{subfigure}{0.40\textwidth}
      \includegraphics[width=\linewidth]{figures/diabetes/Feat_bar_plot_diabetes.pdf}
      \caption{Score Plot {\ttfamily Diabetes} Scenario I}
      \label{fig:Feat-imp-diabetes}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.40\textwidth}
      \includegraphics[width=\linewidth]{figures/diabetes/Feat_bar_plot_diabetes_split.pdf}
      \caption{Score Plot {\ttfamily Diabetes} Scenario II}
      \label{fig:Feat-imp-diabetes-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/diabetes/GFI_diabetes_synt.pdf}
      \caption{Bar Plot {\ttfamily Diabetes} Scenario I}
      \label{fig:GFI-diabetes}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/diabetes/GFI_diabetes_split_synt.pdf}
      \caption{Bar Plot {\ttfamily Diabetes} Scenario II}
      \label{fig:GFI-diabetes-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/scoremaps_real_world/Local_Scoremap_Plot_diabetes.png}
      \caption{Scoremap {\ttfamily Diabetes} Scenario I}
      \label{fig:Local-diabetes}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/scoremaps_real_world/Local_Scoremap_Plot_diabetes_split.png}
      \caption{Scoremap {\ttfamily Diabetes} Scenario II}
      \label{fig:Local-diabetes-split}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot and Scoremap for {\ttfamily Diabetes}}
\label{fig:interpretation-diabetes}
\end{figure}

Figure \ref{fig:GFI-diabetes} shows how the importance is divided between Feture 1,2 and 3 while Feature 0 is consistently ranked as the least important attribute. A confirmation of these results can be found in Figure \ref{fig:Feat-imp-diabetes} which reports the Score Plot. Here, in fact, the average importance scores of the first three features display minimal differences and are significantly higher than the ones of Feature 0. 

Similarly to what happens in the {\ttfamily Breastw} dataset the scatter plot of the data, superimposed on the Scoremap (Figure \ref{fig:Local-diabetes}), shows a grid-like structure. It is possible to notice the presence of two rectangular-shaped clusters of points: the one on the bottom left region mainly contains inliers (i.e. blue dots) while the one on the top right portion of the space is formed by outliers (i.e. red stars). There is a small portion of the feature space where the two clusters overlap.

In any case, the difficulty of the model in detecting a single feature as the most important can be noticed from the Local Scoremap. In fact, because of the grid-like shape of the data distribution, the outliers are distributed around both the directions of Feature 2 and 3. 

%\modifica{mettere tabella precisioni allenato su tutto}

%\begin{table}[ht]
%\parbox{.45\linewidth}{
%\centering
%\begin{tabular}{|c|ccc|}
%\hline
%\multicolumn{4}{|c|}{\textbf{diabetes} complete training} \\ \hline
%\textbf{Metric} & \textbf{IF} & \textbf{EIF} & \textbf{EIF+} \\ \hline
%Precision         & 0.47 & 0.49 & 0.48 \\
%Recall            & 0.47 & 0.49 & 0.48 \\
%f1 score          & 0.47 & 0.49 & 0.48 \\
%Accuracy          & 0.90 & 0.90 & 0.90 \\
%Average Precision & 0.46 & 0.44 & 0.42 \\
%ROC AUC Score     & 0.74 & 0.75 & 0.74 \\ \hline
%\end{tabular}
%\caption{Performance Report \texttt{diabetes} Dataset}
%\label{tab:diabetes-perf-complete}}
%\end{table}

For what concerns the anomaly detection performances of the models, reported in Table \ref{tab:avg-prec-table}, the listed values of Average Precision are not too high and not too low if compared with the ones seen in the other benchmark datasets considered in this section. The reason for these not outstanding performances may be found in the overlapping between the inliers and outliers cluster presented in Figure \ref{fig:Local-diabetes} which may create confusion in the process of distinguishing between anomalies and normal samples. 

The inlier training approach was exploited also for the {\ttfamily Diabetes} dataset in order to try to obtain further improvements both in the model's performances and in the reliability of the interpretation results. 

%\modifica{far vedere nel caso in cui si splitta il training per capire se va meglio}


An evident improvement can be noticed in Figure \ref{fig:GFI-diabetes-split} which depicts the Bar Plot where it becomes clear how the feature importance is shared between Feature 2 and 3. These two attributes are in fact always included in the first or second ranking position among the different model executions considered and possess similar average importance score values, as reported in Figure \ref{fig:Feat-imp-diabetes-split}, which are significantly higher than the ones of Feature 0 and 1. 

The most important features, Feature 2 and 3, represent the HbA1c and blood glucose levels respectively as it was described in Appendix \ref{sec:real-world-data}. Thus, the results are highly reliable if matched with the domain knowledge since it is well known that the main consequence of diabetes disease is an excessive level of glucose in the patient's blood.

The Scoremap, in Figure \ref{fig:Local-diabetes}, is similar to the ones obtained using the Scenario I approach with the difference that the colors are lighter in correspondence of the inliers cluster and darker in correspondence with the outliers one, meaning that the model, exploring the better knowledge of the inlier distribution acquired during the training step, has improved its capabilities in the detection of anomalies over normal samples. This is confirmed by the Average Precision, contained in Table \ref{tab:avg-prec-table}, which contains better metric than the ones obtained in Scenario I. An interesting thing to note is how the Average Precision metric increases passing from the Isolation Forest to the newly introduced \EIFplus model. 

%\modifica{inserire tabella precisioni e vedere di quanto è migliorata e come potrebbe aver influito nell'interpretazione}


%\begin{table}[ht]
%\parbox{.45\linewidth}{
%\centering
%\begin{tabular}{|c|ccc|}
%\hline
%\multicolumn{4}{|c|}{\textbf{diabetes} inlier training} \\ 
%\hline
%\textbf{Metric} & \textbf{IF} & \textbf{EIF} & 
%\textbf{EIF+} \\ \hline
%Precision         & 0.29 & 0.54 & 0.56 \\
%Recall            & 0.29 & 0.54 & 0.56 \\
%f1 score          & 0.29 & 0.54 & 0.56 \\
%Accuracy          & 0.86 & 0.91 & 0.91 \\
%Average Precision & 0.21 & 0.49 & 0.58 \\
%ROC AUC Score     & 0.65 & 0.75 & 0.76 \\ \hline
%\end{tabular}
%\caption{Performance Report \texttt{diabetes} Dataset}
%\label{tab:diabetes-perf-split}
%}
%\end{table}


\begin{figure}
  \centering
  \includegraphics[width=0.7\linewidth]{figures/feature_selection_plots_final/featsel_diabetes_final.pdf}
  \caption{Feature Selection Plot Diabetes}
  \label{fig:fs-diabetes-plus}
\end{figure}\hfil % <-- added

Finally, the Feature Selection Plot for the {\ttfamily Diabetes} dataset is reported in Figure \ref{fig:fs-diabetes-plus}. As expected the best performing Feature Ranking Algorithm, in terms of Average Precision, are ExIFFI-plus-split and ExIFFI-split. In ExIFFI-plus-split the Average Precision slightly decreases for input sets with 3 or fewer features but still remaining at high levels. In the case of ExIFFI-split, instead, the precision values are constantly increasing, in particular from 3 features onwards. On the other hand, for all the remaining algorithms considered the Average Precision decreases with the number of features. 

%\todo[inline, color=red]{Questo penso che possa andare in appendice, se nessuno ha niente in contrario (Chiara)}


%\davide{
%. As it can be noticed the E-IFFI,E-IFFI-plus and E-DIFFI models have an almost equal conduct 
%with a constant increase in their Average Precision values up to 2 features to end up with a decrease in the passage from 2 to a single feature. On the other hand, Casual decreases when passing from 3 to 2 features, probably because of the early random removal of one between Feature 2 and Feature 3. Finally, the DIFFI and Random Forest Feature Ranking Algorithms show a constant decrease.  
 
% }


%\davide{
 

%The Local Importance Scoremap (Figure \ref{fig:Local-diabetes} was plotted on the two most important features (Feature 2 and 3). It is worth noting that the data have a grid-like shape. The reason for this distribution is likely the fact that there are multiple HbA1c levels associated to the same value of blood glucose level and vice-versa. Both the inlier's and outlier's distributions possess a rectangular shape. An overlap between the two distributions can be spotted between the top right corner of the inlier distribution and the low left angle of the outlier one.

%As a consequence the inliers are aligned along both the directions considered in this analysis, confirming the shared importance of the HbA1c and blood glucose levels. 
%}

%\davide {

%Table \ref{tab:diabetes-perf} reports the Performance metrics' values for the {\ttfamily Diabetes} dataset. The EIF and EIF+ models outperform by a high amount the IF model which is surely not recommended for this particular dataset considering the low level of its metric values. 

%}





==> sections/sections_world_dataset_results/diabetes_new.tex <==
\subsection*{{\ttfamily Diabetes}}

\subsubsection{Performance}

\ale{The peculiarity of the {\ttfamily Diabetes} dataset, as described in \ref{sec:appendix-real-world-data}, in the context of this study is its low dimensionality: its observations are, in fact, fully described using just four features. As a consequence the behavior of the AD models considered as abnormal samples are progressively included in the training set, displayed in Figure \ref{fig:Diabetes_contamination_full}, is diverse from the ones observed in other benchmark datasets. In particular the IF model possesses an unique increasing Average Precision trend that saturates at a contamination level around 5 \%. On the other hand the DIF model showcases an essentially constant trend at substantially low Average Precision values if compared to the other methods. An explanation of the underperformance of this model could be the presence of overfitting because of the usage of an highly complex approach from a simple task as the ones of separating anomalous points from normal ones on a four dimensional feature space. Finally, the proposed \EIFplus model stands out as the reference model in this study, immediately followed by EIF as highlighted in Figure \ref{fig:Diabetes_contaminationEIFvsEIF+}.} 

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.49\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Diabetes/Contamination/22-03-2024_09-01-43_diabetes_contamination_full_plot.pdf}
      \caption{Models evaluation, varying the contamination levels}
      \label{fig:Diabetes_contamination_full}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.44\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Diabetes/Contamination/22-03-2024_09-03-03_diabetes_EIF+_minus_EIF_precision_over_contamination.pdf}
      \caption{Difference between \EIFplus and EIF average precision}
      \label{fig:Diabetes_contaminationEIFvsEIF+}
    \end{subfigure}\hfil % <-- added
\caption{Figure \ref{fig:Diabetes_contamination_full} illustrates the average precision as the contamination level in the training set increases. Figure \ref{fig:Diabetes_contaminationEIFvsEIF+} compares the performance graphs of EIF and \EIFplus, using the difference of their scores in various contamination levels.}
\label{fig:Diabetes_contamination}
\end{figure}

\ale{Table \ref{tab:Diabetes_perf}  portraits the difference, in terms of the Average Precision, Precision and AUC ROC score metrics, in the two approaches used to train, and successively test, the presented Anomaly Detection approaches: Scenario I and Scenario II. As already made clear in Figure \ref{fig:Diabetes_contamination_full} there are some visible differences in the model performances as anomalies are included in the training process (i.e. in the passage from Scenario II to Scenario I). The most optimal model is the proposed \EIFplus due to its superior metric values and its unparalleled efficiency in both the fitting and prediction stages.}

\begin{table}[htbp]
\begin{minipage}[t]{0.46\textwidth}
\strut\vspace*{-\baselineskip}\newline
\resizebox{\textwidth}{!}{
\begin{tabular}{|c||ccc|ccc||cc|}
\toprule
\hline
&\multicolumn{3}{c|}{Scenario I}&\multicolumn{3}{c||}{Scenario II}&\multicolumn{2}{c|}{Time}\\
\hline
AD Model & Avg & Prec & ROC & Avg & Prec & ROC & fit & pred \\
& Prec &  & AUC & Prec &  & AUC &  &  \\
\hline
IF          & 0.46& 0.46& 0.70& 0.26& 0.31& 0.62& 0.13& 0.069\\
EIF         & \textbf{0.47}& 0.48& 0.71& 0.55& 0.61& 0.78& \textbf{0.10}& \textbf{0.008}\\
EIF+        & 0.44& \textbf{0.49}& \textbf{0.72}& \textbf{0.61}& \textbf{0.56}& \textbf{0.76}& \textbf{0.10}& \textbf{0.008}\\
DIF         & 0.10& 0.90& 0.49& 0.13& 0.17& 0.54& 10.2& 9.05\\
AE          & 0.45& 0.47& 0.70& 0.50& 0.52& 0.73& 17.82& 0.28\\
\hline
\end{tabular}}
\vspace{0.41cm}
\caption{Performances of 5 different Anomaly Detection models over {\ttfamily Diabetes} are compared using classical Classification metrics. Moreover, the last two columns contain the average time for a fit and predict operation. The highest metric values and the lowest execution times are highlighted in bold}\label{tab:Diabetes_perf}
\end{minipage}
\hfill
\begin{minipage}[t]{0.46\textwidth}
\strut\vspace*{-\baselineskip}\newline
\resizebox{\textwidth}{!}{
\begin{tabular}{|c||c|c|c|c||c|}
\toprule
\hline
&\multicolumn{2}{c|}{Evaluation with EIF}&\multicolumn{2}{c||}{Evaluation with \EIFplus}&\\
\hline
& Scenario I & Scenario II & Scenario I & Scenario II& Time\\

 Algorithm & $AUC_{FS}$  & $AUC_{FS}$ & $AUC_{FS}$  & $AUC_{FS}$ &  \\
\hline
DIFFI               & -0.363& -1.455& -0.345& -1.481& 0.63\\
IF\_\approach        & 0.847& -1.013& 0.812& -0.930& 0.73\\
EIF\_\approach       & 0.967& 0.354& \textbf{0.826}& 0.313& \textbf{0.50}\\
\EIFplus\_\approach  & \textbf{1.058}& \textbf{0.822}& 0.747& \textbf{1.171}& 0.52\\
IF\_RF              & -0.303& -0.059& -0.302& -0.123& 2.04\\
EIF\_RF             & 0.491& 0.315& 0.383& 0.355& 2.04\\
EIF+\_RF            & 0.463& 0.332& 0.407& 0.296& 2.04\\
\hline
\end{tabular}}
\caption{Quantitative evaluation of the effectiveness of 6 different interpretation algorithms on {\ttfamily Diabetes} through the $AUC_{FS}$ metric, introduced in \ref{sec:interpr_evaluat}. In the last column the average time taken by the different models to produce the importance scores is reported. The highest $AUC_{FS}$ and lowest Importance time values are highlighted in bold.}\label{tab:fs-tab-Diabetes}
\end{minipage}
\end{table}


\subsubsection{Importance Plots}

\ale{The outcomes of the explanations granted by \approach+ are illustrated in Figure \ref{fig:interpretation-Diabetes}. Analyzing the Score Plots, represented in Figures \ref{fig:Feat-imp-Diabetes} and \ref{fig:Feat-imp-Diabetes-split} and the Bar Plots, represented in Figures \ref{fig:GFI-Diabetes} and \ref{fig:GFI-Diabetes-split}, it is clear how the two most important features are  {\itshape HbA1c\_level} and  {\itshape blood\_glucose\_level}. As elucidated in \ref{sec:appendix-real-world-data} the Hemoglobin A1c Level and the amount of glucose in the bloodstream represent crucial indicators to discriminate between patients affected or not by diabetes.}

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Diabetes/Importance_plots/02-03-2024_17-15-42_GFI_Bar_plot_diabetes_EXIFFI+_1.pdf}
      \caption{Bar Plot {\ttfamily Diabetes} Scenario I}
      \label{fig:GFI-Diabetes}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.29\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Diabetes/Importance_plots/02-03-2024_17-15-42_GFI_Score_plot_diabetes_EXIFFI+_1.pdf}
      \caption{Score Plot {\ttfamily Diabetes} Scenario I}
      \label{fig:Feat-imp-Diabetes}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.26\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Diabetes/Local_Scoremap/22-03-2024_08-22-16_importance_map_diabetes_EXIFFI+_1_feat_2_3.pdf}
      \caption{Scoremap {\ttfamily Diabetes} Scenario I}
      \label{fig:Local-Diabetes}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Diabetes/Importance_plots/02-03-2024_15-07-58_GFI_Bar_plot_diabetes_EXIFFI+_2.pdf}
      \caption{Bar Plot {\ttfamily Diabetes} Scenario II}
      \label{fig:GFI-Diabetes-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.29\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Diabetes/Importance_plots/02-03-2024_15-07-58_GFI_Score_plot_diabetes_EXIFFI+_2.pdf}
      \caption{Score Plot {\ttfamily Diabetes} Scenario II}
      \label{fig:Feat-imp-Diabetes-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.26\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Diabetes/Local_Scoremap/22-03-2024_08-22-06_importance_map_diabetes_EXIFFI+_2_feat_2_3.pdf}
      \caption{Scoremap {\ttfamily Diabetes} Scenario II}
      \label{fig:Local-Diabetes-split}
    \end{subfigure}\hfil % <-- addedDiabetes
\caption{Bar Plot, Score Plot and Scoremap for {\ttfamily Diabetes} in the two different Scenarios, using the \approach algorithm applied to the \EIFplus model.}\label{fig:interpretation-Diabetes}
\end{figure}

\subsubsection{Feature Selection}

\ale{The validity of the interpretation of the \EIFplus model provided by \approach is confirmed once again in the plots represented in Figure \ref{fig:interpretation-Diabetes} where Unsupervised Feature Selection is exploited as a proxy task for the comparison of ad-hoc and post-hoc interpretation algorithms. The plot related to the \approach+ model is the only one associated with a shape that certifies a correct feature ranking for the Anomaly Detection task. Indeed the plot placed in Figure \ref{fig:Feat-Sel_Diabetes_valEIF+_EXIFFI+_2} is the unique graph where the red line always contains superior Average Precision values in comparison to the blue line. Conversely in the plots referred to other interpretation methods the metrics values oscillate without providing any clear sign of weather the feature selection approach associated with the blue or red line is superior.} 

\begin{figure}[!ht] 
\centering
\hspace{0.05\textwidth}\textbf{IF} \hspace{0.29\textwidth} \textbf{EIF} \hspace{0.29\textwidth} \textbf{EIF+}
% First row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Ad-Hoc}}} % Adjust the parbox width as necessary for your caption text
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Diabetes/Feature_Selection/07-05-2024_15-14-00_diabetes_EIF+_IF_EXIFFI_feature_selection_2.pdf}
            \caption{\approach applied to IF}
            \label{fig:Feat-Sel_Diabetes_valEIF+_DIFFI_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Diabetes/Feature_Selection/22-03-2024_07-44-48_diabetes_EIF+_EXIFFI_feature_selection_2.pdf}
            \caption{\approach applied to EIF}
            \label{fig:Feat-Sel_Diabetes_valEIF+_EXIFFI_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Diabetes/Feature_Selection/22-03-2024_07-44-48_diabetes_EIF+_EXIFFI+_feature_selection_2.pdf}
            \caption{\approach applied to \EIFplus}
            \label{fig:Feat-Sel_Diabetes_valEIF+_EXIFFI+_2}
        \end{subfigure}
    \end{minipage}
\end{minipage}

\vspace{5mm} % Space between rows

% Second row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Post-Hoc}}} % Adjust as necessary
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Diabetes/Feature_Selection/22-03-2024_07-44-48_diabetes_EIF+_IF_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to IF}
            \label{fig:Feat-Sel_Diabetes_valEIF+_IF_RandomForest_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Diabetes/Feature_Selection/22-03-2024_07-44-48_diabetes_EIF+_EIF_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to EIF}
            \label{fig:Feat-Sel_Diabetes_valEIF+_EIF_RandomForest_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Diabetes/Feature_Selection/22-03-2024_07-44-49_diabetes_EIF+_EIF+_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to \EIFplus}
            \label{fig:Feat-Sel_Diabetes_valEIF+_EIF+_RandomForest_2}
        \end{subfigure}
    \end{minipage}
\end{minipage}

\caption{Feature Selection of the different Ad-Hoc and Post-Hoc methods applied to the 3 Isolation Forest models: IF, EIF and \EIFplus. The blue line is the values of average precision, calculated with the \EIFplus model in the Scenario II, dropping the most important feature at each step, the red line is the values of average precision dropping the least important feature at each step and the green line is the value of the feature selection dropping a random feature at each step.}\label{fig:fs-interpretation-Diabetes}
\end{figure}

\ale{In Table \ref{tab:fs-tab-Diabetes} the $AUC_{FS}$ values, for a quantitative comparison of the effectiveness of the interpretability provided by the diverse methods analysed in this study are contained. As already observed from a careful analysis of the Feature Selection plots (Figure \ref{fig:fs-interpretation-Diabetes} the explanation better aligned with the ground truth is the one provided by the proposed \approach+ approach. On the other hand the outcomes provided by the other considered models prove to be less satisfactory, in particular the ones produced by \approach on the IF model which are paired with negative $AUC_{FS}$ values, a clear prove of an erroneous ranking of attributes' relevance.} 



==> sections/sections_world_dataset_results/glass.tex <==
\subsubsection*{{\ttfamily Glass}}
%\modifica{introduzione a Glass}

%\todo[inline, color=red]{Questo è un caso interessante perché è un caso estremo del mismatch tra outlier secondo le etichette fornite e punti isolati secondo il concetto di anomalie che ha l'IF. Infatt non migliora neanche togliendo gli outlier. Potrebbe interessante anche tenerlo nel corpo del paper, è esattamente un esempio di "non usare EIF se sei in un caso così" (Chiara)}


The {\ttfamily Glass} dataset is described in details in Appendix \ref{sec:real-world-data}. 

%\modifica{feature importance nel caso no split}

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/glass/Feat_bar_plot_glass.pdf}
      \caption{Score Plot  {\ttfamily Glass} Scenario I}
      \label{fig:Feat-imp-glass}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/glass/Feat_bar_plot_glass_split.pdf}
      \caption{Score Plot {\ttfamily Glass} Scenario II}
      \label{fig:Feat-imp-glass-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/glass/GFI_glass_synt.pdf}
      \caption{Bar Plot  {\ttfamily Glass} Scenario I}
      \label{fig:GFI-Glass}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/glass/GFI_glass_split_synt.pdf}
      \caption{Bar Plot {\ttfamily Glass} Scenario II}
      \label{fig:GFI-glass-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/scoremaps_real_world/Local_Scoremap_Plot_glass.png}
      \caption{Scoremap {\ttfamily Glass} Scenario I}
      \label{fig:Local-glass}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/scoremaps_real_world/Local_Scoremap_Plot_glass_split.png}
      \caption{Scoremap {\ttfamily Glass} Scenario II}
      \label{fig:Local-glass-split}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot and Scoremap for {\ttfamily Glass}}\label{fig:interpretation-glass}
\end{figure}


%\modifica{si vede dalle barre dello score della feature importance che l'algoritmo sta avendo molta fatica nel riconoscere una specifica feature come la più importante, in ogni caso la feature 5 risulta prima e probabilmente è dovuto al fatto che, come vediamo dallo scormap, ci sono dei punti che deviano di molto dalla distribuzione centrale.}

%After careful observation of the Global Feature Importance Bar Plot, depicted in Figure \ref{fig:GFI-Glass}, it is possible to conclude that the interpretation algorithm is struggling to identify a single feature as the dominant one in terms of Importance Score. A confirmation of that comes from the Feature Importance Score Plot in Figure \ref{fig:Feat-imp-glass} where a high similarity can be appreciated in the scores of the first four features in the ranking.  

Upon close examination of the Bar Plot obtained for \EIFplus, illustrated in Figure \ref{fig:GFI-Glass}, it becomes apparent that it is difficult for the interpretation algorithm to single out a predominant feature in terms of Importance Score. This conclusion is reinforced by the Score Plot shown in Figure \ref{fig:Feat-imp-glass}, where the four top ranked features exhibit similar importance scores.


Examining Figure \ref{fig:Local-glass}, we can discern that the points exhibiting the greatest deviations from the dataset's normal distribution are designated as inliers, represented by the blue dots. Interestingly, the outliers, which are labeled as such, are predominantly situated within the main cluster alongside the majority of inliers. This suggests that the model's ability to detect outliers is compromised by the dataset's inherent structure, leading to low Average Precision scores (refer to Table \ref{tab:avg-prec-table}). Consequently, since the model's interpretation aligns with the anomalies it predicts, it does not correspond well to the labeled anomalies.


%\modifica{Inoltre dallo scoremap si può vedere come gli outlier (labels) del dataset siano principalmente all'interno della distribuzione normale, con conseguente bassa precisione del modello evidenziata dalla tabella.Dunque possiamo osservare come effettivamente le feature più importanti non siano comunque relative alle labels date}


%\modifica{tabella precisioni caso no split ancora non ho risultati}
\begin{comment}
\begin{table}[ht]
\parbox{.45\linewidth}{
\centering
\begin{tabular}{|c|ccc|}
\hline
\multicolumn{4}{|c|}{\textbf{glass} complete training} \\ \hline
\textbf{Metric} & \textbf{IF} & \textbf{EIF} & \textbf{EIF+} \\ \hline
Precision         & 0.11 & 0.11 & 0.11 \\
Recall            & 0.11 & 0.11 & 0.11 \\
f1 score          & 0.11 & 0.11 & 0.11 \\
Accuracy          & 0.92 & 0.92 & 0.92 \\

Average Precision & 0.10 & 0.10 & 0.21 \\
ROC AUC Score     & 0.76 & 0.73 & 0.77 \\ \hline
\end{tabular}
\caption{Performance Report \texttt{glass} Dataset}
\label{tab:glass-perf-complete}}
\end{table}
\end{comment}
%\modifica{come nei casi precedenti proviamo a vedere di allenare solo sugli inlier, cercando di isolare gli outlier che sono dati dal dataset quindi migliorare la precisione}

Then, similarly to the metodology used for the \texttt{Annthyroid} dataset, we train the model only on the inliers. This strategy aims to improve the correspondence between predicted and labeled anomalies to simplify the qualitative evaluation of importance scores obtained with \approach.%, as it is expected by the anomaly detection model. We aim this result in order to better highlight the distinctive features that define the labeled anomalies.
%By interpreting models with better classification performance, we expect the feature importance scores to reflect the actual role played by features. In particular,  actually affect the definition of anomalous samples according to the provided labels.




Unfortunately, the outcomes fail to meet our expectations. As evident in Table \ref{tab:avg-prec-table}, the Average Precision scores remain unchanged. This stems from the absence of any deviations in the labeled anomalies within the dataset. In other words, these anomalies do not satisfy the isolation assumption behind unsupervised tree-based AD models. Consequently, we cannot attain better classification performance, even if we train the models exclusively on the inliers.

%\modifica{grafici interpretazione nel caso split}


%\modifica{osserviamo che sostanzialmente non è cambiato nulla sia per lo scoremap sia per quanto riguarda l'interpretazione che per quanto riguarda la precisione, ancora una volta sottolineando quanto effettivamente tali anomalie non riescono ad essere riconosciute da questo tipo di modelli}

Furthermore, the inability to pinpoint the feature that most distinctly characterizes the anomalies is emphasized by the Bar Plot presented in Figure \ref{fig:GFI-glass-split} and the Score Plot in Figure \ref{fig:Feat-imp-glass-split}. These visualizations reveal a striking similarity in the feature importance ranking with the interpretation plots of the model trained with the whole dataset.

\begin{comment}
\begin{table}[ht]
\parbox{.45\linewidth}{
\centering
\begin{tabular}{|c|ccc|}
\hline
\multicolumn{4}{|c|}{\textbf{glass} inlier training} \\ \hline
\textbf{Metric} & \textbf{IF} & \textbf{EIF} & \textbf{EIF+} \\ \hline
Precision         & 0.11 & 0.00 & 0.11 \\
Recall            & 0.11 & 0.00 & 0.11 \\
f1 score          & 0.11 & 0.00 & 0.11 \\
Accuracy          & 0.92 & 0.92 & 0.92 \\

Average Precision & 0.10 & 0.08 & 0.20 \\
ROC AUC Score     & 0.76 & 0.71 & 0.76 \\ \hline
\end{tabular}
\caption{Performance Report \texttt{glass} Dataset}
\label{tab:glass-perf-split}}
\end{table}
\end{comment}
%\modifica{la feature selection non performante conferma quanto detto fino ad adesso}

\begin{figure}[!ht] 
  \centering
  \includegraphics[width=0.7\linewidth]{figures/feature_selection_plots_final/featsel_glass_final.pdf}
  \caption{Feature Selection Plot {\ttfamily Glass}}
  \label{fig:fs-glass-plus}
\end{figure}%\hfil % <-- added

The Feature Selection Plot, shown in Figure \ref{fig:fs-glass-plus}, underscores the subpar results achieved so far in the analysis of the {\ttfamily Glass} dataset. It is evident that all algorithms, including the supervised Random Forest, exhibit poor performance, resembling a random selection of the most critical features.

In conclusion, the unsatisfactory outcomes stemming from the interpretability analysis of the {\ttfamily Glass} dataset serve as an extreme illustration of the challenges associated with employing benchmark datasets originally designed for classification tasks to evaluate isolation-based approaches in the field of anomaly detection.

%\davide{
%Figure \ref{fig:fs-glass-plus} depicts the Feature Importance Plot for the {\ttfamily Glass} dataset. All the models show a very similar behavior with almost constant Average Precisions values up to the step in which 3 features are considered. At this point E-IFFI and E-DIFFI drop significantly. The Casual and Random Forest Feature Ranking algortihms maintain more or less constant values and E-IFFI-plus increases to have a little drop passing from 2 to 1 feature. The DIFFI model possesses an odd behavior since in the passage from 5 to 4 features it experiences a drop in performances that reaches its minimum at 2 features (here the Average Precision is a bit lower than 0.05) and increases up to the levels of Casual and Random Forest with 1 feature. 
%}

%\davide {
%Interpretability results for the {\ttfamily Glass} dataset, introduced in Section \ref{sec:real-world-data}, are reported in Figure \ref{fig:glass}. It is possible to say that there is a shared importance between Feature 4 and 5 representing the Iron (Fe) and Sodium (Na) concentration respectively. These two attributes have very similar average Feature Scores in \ref{fig:Feat-imp-glass} and they are considered the most or second most important feature almost all the time in \ref{fig:GFI-Glass}.

%In the Local Importance Scoremap depicted in Figure \ref{fig:Local-glass} the two most important features, Feature 4 and 5, are compared. The importance of Feature 4 is justified by the fact that the outlier are almost perfectly aligned along its direction. On the contrary, Feature 5 represents a peculiar behavior. In fact, as already mentioned in the Algorithm Output section, in this instance, we are facing an obvious case of \textit{model anomalies} since at least three inlier points, placed along Feature 5, which are clearly isolated from the main cluster of points can be noticed. This is the reason why Feature 5 was assigned with one of the highest Feature Importance scores. 

%}

%\davide {
%As it can be observed from Table \ref{tab:glass-perf}, the {\ttfamily Glass} dataset is by far the one with the worst detection performances over all the Benchmark Datasets considered in this section. Focusing on the metrics' values similarly to the {\ttfamily Cardio} dataset the best model is EIF+, followed by EIF and IF. 
%}


==> sections/sections_world_dataset_results/glass_new.tex <==
\subsection*{{\ttfamily Glass}}\label{sec:glass}

% Additional comment to satisfy comment 7 by reviewer 2 and Comment 11 of reviewer 1 
\davide{Next, the {\ttfamily Glass} dataset is considered. As explained in \ref{sec:appendix-real-world-data} this dataset in a Multi-Class Classification task to distinguish between different glass qualities. In particular this dataset was chosen for the evaluation of the reliability and alignment with human cognition of \approach since it is equipped with a sort of ground truth on what are the most important features to distinguish between anomalous and non anomalous samples, which is provided by studies conducted by domain experts.}

\subsubsection{Performance}
\ale{In Figure \ref{fig:Glass_contamination}, we notice that the performance of all models improves as the contamination level in the training dataset decreases, with the DIF model outperforming the rest, followed by the \EIFplus. Specifically, the plot in Figure \ref{fig:Glass_contaminationEIFvsEIF+} highlights the \EIFplus model's distinct advantage in achieving higher average precision at lower contamination levels, showcasing its enhanced capability to generalize effectively when trained without anomalies. This demonstrates the \EIFplus model's proficiency in adapting to datasets with low contamination, emphasizing its strength in scenarios with unseen anomalies compared to EIF.}

\begin{figure}[htbp] 
    \centering % <-- added
    \begin{subfigure}[t]{0.49\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Glass/Contamination/18-03-2024_16-12-32_glass_DIFFI_contamination_full_plot.pdf}
      \caption{Models evaluation, varying the contamination levels}
      \label{fig:Glass_contamination_full}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.44\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Glass/Contamination/19-03-2024_09-16-39_glass_DIFFI_EIF+_minus_EIF_precision_over_contamination.pdf}
      \caption{Difference between \EIFplus and EIF average precision}
      \label{fig:Glass_contaminationEIFvsEIF+}
    \end{subfigure}\hfil % <-- added
\caption{Figure \ref{fig:Glass_contamination_full} illustrates the average precision as the contamination level in the training set increases. Figure \ref{fig:Glass_contaminationEIFvsEIF+} compares the performance graphs of EIF and \EIFplus, using the difference of their scores in various contamination levels.}
\label{fig:Glass_contamination}
\end{figure}

\ale{Table \ref{tab:glasspr} illustrates that \EIFplus maintains comparable outcomes in Scenario I and, leveraging its enhanced generalization capabilities for unseen anomalies, ranks as the second highest-performing algorithm in Scenario II. Notably, it fits 10 times faster than the DIF and predicts the entire dataset's scores 30 times more swiftly, showcasing its efficiency and efficacy in both model fitting and anomaly detection across scenarios.}

\begin{table}[!ht]
\centering
%\caption{{\ttfamily Glass} Performance Report}
\caption{Performances of 5 different Anomaly Detection models over {\ttfamily Glass} are compared using classical Classification metrics. Moreover, the last two columns contain the average time for a fit and predict operation. The highest metric values and the lowest execution times are highlighted in bold}\label{tab:glasspr}
\begin{tabular}{|c||ccc|ccc||cc|}
\toprule
\hline
& \multicolumn{3}{c|}{Scenario I} & \multicolumn{3}{c||}{Scenario II} & \multicolumn{2}{c|}{Time} \\
\hline
AD Model & Avg & Prec & ROC & Avg & Prec & ROC & fit & pred \\
& Prec &  & AUC & Prec &  & AUC & fit & pred \\
\hline
IF          & 0.36 & 0.34 & 0.62 & 0.65 & 0.68 & 0.82 & \textbf{0.07}& \textbf{0.002}\\
EIF         & 0.35 & 0.27 & 0.58 & 0.57 & 0.68 & 0.82 & \textbf{0.07}& 0.01  \\
\EIFplus        & 0.31 & 0.24 & 0.56 & 0.69& 0.79& 0.88 & \textbf{0.07}& 0.01  \\
DIF         & 0.3 & 0.2& 0.54& \textbf{0.85}& \textbf{0.82}& \textbf{0.9}& 0.67 & 0.29  \\
AE & \textbf{0.41}& \textbf{0.44}& \textbf{0.68}& 0.53 & 0.62& 0.78& 2.25 & 0.04  \\
\hline
\end{tabular}
\end{table}

\subsubsection{Importance Plots} \label{sec:glass-imp-plots}
\ale{In the Figures \ref{fig:Feat-imp-Glass}, which illustrate the importance scores for Scenario I, there's noticeable uncertainty with no clear indication of a single feature standing out as the most important. This ambiguity is highlighted by the data point distribution in Figure \ref{fig:Local-glass}, where we see significant variance in both the dimensions. The model appears to blend a subset of anomalies with inliers, as indicated by a broader contour plot along the feature {\ttfamily Ba} (Barium) compared to its narrower counterpart in Scenario II (Figure \ref{fig:Local-glass-split}). This difference is likely because anomalies are more distinctly clustered in a specific area of the space, suggesting they are more a subset of the data distribution. This concept was further discussed in \ref{sec:appendix-real-world-data}.}

\ale{The dataset comprise objects made of glass, characterized by features like the refractive index (RI) and concentrations of elements. Carletti et al. \cite{carletti2019explainable} pointed out that the outliers are the data belonging to the subclass of headlamp glass. The key difference between headlamp and window glass is the Barium due to its contribution to optical enhancements. Specifically, Barium boosts the refractive index, thus augmenting light transmission and brightness \cite{D3RA08015C} vital for automotive headlamps. Its incorporation into headlamp glass optimizes light focus and directionality, underscoring its significance in improving headlamp functionality.}

\begin{figure}[htbp] 
    \centering % <-- added
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Glass/Importance_plots/07-03-2024_08-57-53_GFI_Bar_plot_glass_DIFFI_EXIFFI+_1.pdf}
      \caption{Score Plot {\ttfamily Glass} Scenario I}
      \label{fig:Feat-imp-Glass}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.27\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Glass/Importance_plots/07-03-2024_08-57-53_GFI_Score_plot_glass_DIFFI_EXIFFI+_1.pdf}
      \caption{Bar Plot {\ttfamily Glass} Scenario I}
      \label{fig:GFI-glass}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Glass/Local_Scoremap/07-03-2024_16-59-33_importance_map_glass_DIFFI_EXIFFI+_1.pdf}
      \caption{Scoremap {\ttfamily Glass} Scenario I}
      \label{fig:Local-glass}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Glass/Importance_plots/07-03-2024_08-56-27_GFI_Bar_plot_glass_DIFFI_EXIFFI+_2.pdf}
      \caption{Score Plot {\ttfamily Glass} Scenario II}
      \label{fig:Feat-imp-Glass-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.27\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Glass/Importance_plots/07-03-2024_08-56-51_GFI_Score_plot_glass_DIFFI_EXIFFI+_2.pdf}
      \caption{Bar Plot {\ttfamily Glass} Scenario II}
      \label{fig:GFI-glass-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Glass/Local_Scoremap/07-03-2024_16-58-14_importance_map_glass_DIFFI_EXIFFI+_2.pdf}
      \caption{Scoremap {\ttfamily Glass} Scenario II}
      \label{fig:Local-glass-split}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot and Scoremap for {\ttfamily Glass}  in the two different Scenarios, using the \approach algorithm applied to the \EIFplus model.}\label{fig:interpretation-glass}
\end{figure}

\ale{In addition, The Potassium (K) it is especially used in glass types requiring increased strength or thermal resistance, such as certain window glasses. But we can observe in the local Scoremap that the deviation from the distribution along the variable K does not coincide with a particular distribution of anomalies.}

\ale{As depicted in Figures \ref{fig:Feat-imp-Glass-split} and \ref{fig:GFI-glass-split}  Scenario II's analysis highlights Barium (Ba) as a pivotal feature, followed by Potassium (K). This results provides an additional confirmation on the correctness of the proposed approach that aligns with the domain knowledge on what is the most relevant attribute for the distinction between window and headlamp glasses.}

\subsubsection{Feature Selection}
\ale{Figure \ref{fig:interpretation-glass} showcases the Feature Selection for the glass dataset, highlighting the superior performance of ad-hoc interpretation algorithms over the surrogate Random Forest's feature importance method. All models succeed in identifying key features because the performance improve the more the less important features are dropped, improving the average precision score as features are shrinked to the most important ones.}

\begin{figure}[htbp] 
\centering
\hspace{0.05\textwidth}\textbf{IF} \hspace{0.29\textwidth} \textbf{EIF} \hspace{0.29\textwidth} \textbf{EIF+}
% First row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Ad-Hoc}}} % Adjust the parbox width as necessary for your caption text
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Glass/Feature_Selection/06-05-2024_12-27-40_glass_EIF+_IF_EXIFFI_feature_selection_2.pdf}
            \caption{\approach applied to IF}
            \label{fig:Feat-Sel_Glass_valEIF+_DIFFI_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Glass/Feature_Selection/19-03-2024_20-36-33_glass_DIFFI_EIF+_EXIFFI_feature_selection_2.pdf}
            \caption{\approach applied to EIF}
            \label{fig:Feat-Sel_Glass_valEIF+_EXIFFI_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Glass/Feature_Selection/19-03-2024_20-35-25_glass_DIFFI_EIF+_EXIFFI+_feature_selection_2.pdf}
            \caption{\approach applied to \EIFplus}
            \label{fig:Feat-Sel_Glass_valEIF+_EXIFFI+_2}
        \end{subfigure}
    \end{minipage}
\end{minipage}

\vspace{5mm} % Space between rows

% Second row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Post-Hoc}}} % Adjust as necessary
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Glass/Feature_Selection/19-03-2024_20-45-20_glass_DIFFI_EIF+_IF_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest applied to IF}
            \label{fig:Feat-Sel_Glass_valEIF+_IF_RandomForest_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Glass/Feature_Selection/19-03-2024_20-43-46_glass_DIFFI_EIF+_EIF_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest applied to EIF}
            \label{fig:Feat-Sel_Glass_valEIF+_EIF_RandomForest_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Glass/Feature_Selection/19-03-2024_20-42-39_glass_DIFFI_EIF+_EIF+_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest applied to \EIFplus}
            \label{fig:Feat-Sel_Glass_valEIF+_EIF+_RandomForest_2}
        \end{subfigure}
    \end{minipage}
\end{minipage}
\caption{Feature Selection of the different Ad-Hoc and Post-Hoc methods applied to the 3 Isolation Forest models: IF, EIF and \EIFplus. The blue line is the values of average precision, calculated with the \EIFplus model in the Scenario II, dropping the most important feature at each step, the red line is the values of average precision dropping the least important feature at each step and the green line is the value of the feature selection dropping a random feature at each step.}\label{fig:feature_selections-Glass}
\end{figure}


\ale{In contrast, the Random Forest feature importance method not only falls short in selecting features that enhance the average precision score—resulting in a decreased score—but also demonstrates a scenario where the blue line surpasses the red line in the post-hoc interpretation of the EIF. This indicates that important features impacting the score were prematurely dropped due to being assigned low importance scores by the model. So the Random Forest not only have bad performances but in the specific case of the EIF it gave wrong scores.}

\ale{Table \ref{tab:fs-tab-glass} reveals the performance of various interpretation algorithms across two scenarios. In Scenario I, the DIFFI interpretation algorithm emerges as the top performer. Conversely, in Scenario II, \approach stand out when applied to the 3 models, in particular when applied to the IF model, demonstrating significantly improved results, whereas the Random Forest model consistently faces challenges in accurately interpreting feature importance. This contrast in performance between scenarios underscores the adaptability of ad-hoc algorithms in understanding feature relevance in complex datasets like {\ttfamily glass}, while highlighting the limitations of conventional methods like Random Forest in nuanced interpretation tasks. Moreover \approach shows an improved time efficiency in the computation of importance scores being almost 20 times faster than post-hoc interpretability methods like Random Forest.}


\begin{table}[htbp]
\centering
%\caption{Feature Selection Scores  {\ttfamily Glass}}
\caption{Quantitative evaluation of the effectiveness of 6 different interpretation algorithms on {\ttfamily Glass} through the $AUC_{FS}$ metric, introduced in \ref{sec:interpr_evaluat}. In the last column the average time taken by the different models to produce the importance scores is reported. The highest $AUC_{FS}$ and lowest Importance time values are highlighted in bold.}\label{tab:fs-tab-glass}
\begin{tabular}{|c||c|c|c|c||c|}
\toprule
\hline
&\multicolumn{2}{c|}{Evaluation with EIF}&\multicolumn{2}{c||}{Evaluation with \EIFplus}&\\
\hline
& Scenario I & Scenario II  & Scenario I & Scenario II & Time\\

 Algorithm & $AUC_{FS}$  & $AUC_{FS}$ & $AUC_{FS}$  & $AUC_{FS}$ &  \\
\hline
DIFFI         & \textbf{1.591}      & 2.117     & \textbf{1.555}    & 2.447     & 0.44 \\
IF\_\approach         & 0.302      & \textbf{3.45}     &  0.483   & \textbf{3.413}     & 0.08 \\
EIF\_\approach        & 0.465      & 2.554    & 0.564     & 2.431     & \textbf{0.01} \\
\EIFplus\_\approach       & 0.403      & 1.769     & 0.527     & 2.263     & \textbf{0.01} \\
IF\_RF        & -1.733      & 2.183       & -1.313     & 2.282     & 0.17 \\
EIF\_RF       & -1.718     & -1.634     & -1.511    & -1.64     & 0.17 \\
\EIFplus\_RF      & -1.464     & 1.944     & -1.308    & 1.632     & 0.17 \\
\hline
\end{tabular}
\end{table}



==> sections/sections_world_dataset_results/ionosphere.tex <==
\subsubsection*{{\ttfamily Ionosphere}}

%\modifica{introduzione ad ionosphere richiamando la sezione \ref{sec:real-world-data} sottolineando che è un dataset molto multidimensionale}

The peculiarity of {\ttfamily Ionosphere} dataset, whose detailed information can be found in Appendix \ref{sec:real-world-data}, is the fact that it is composed of thirty-three features. This poses an additional challenge in evaluating the interpretation results. 

%\modifica{mettere risultati importances nel caso in cui è allenata interamente sul dataset di ionosphere}

\begin{figure}[tbh]
    \centering % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/ionosphere/GFI_ionosphere_synt.pdf}
      \caption{Bar Plot \texttt{Ionosphere} Scenario I}
      \label{fig:GFI-ionosphere}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/ionosphere/GFI_ionosphere_split_synt.pdf}
      \caption{Bar Plot \texttt{Ionosphere} Scenario II}
      \label{fig:GFI-ionosphere-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/ionosphere/Feat_bar_plot_ionosphere.pdf}
      \caption{Score Plot \texttt{Ionosphere} Scenario I}
      \label{fig:Feat-imp-ionosphere}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/ionosphere/Feat_bar_plot_ionosphere_split.pdf}
      \caption{Score Plot \texttt{Ionosphere} Scenario II}
      \label{fig:Feat-imp-ionosphere-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/scoremaps_real_world/Local_Scoremap_Plot_ionosphere.png}
      \caption{Scoremap \texttt{Ionosphere} Scenario I}
      \label{fig:Local-ionosphere}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/scoremaps_real_world/Local_Scoremap_Plot_ionosphere_split.png}
      \caption{Scoremap \texttt{Ionosphere} Scenario II}
      \label{fig:Local-ionosphere-split}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot and Scoremap for \texttt{Ionosphere} }\label{fig:interpretation-ionosphere}
\end{figure}


%\modifica{ si può osservare che la feature importance non evidenzia nessuna feature come più importante dele altre e come vediamo nello scoreplot, i contourplot circondano una distribuzione centrale identificando con una buona precisione le anomalie che si trovano attorno tale distribuzione, precisione evidenziata dai buoni risultati della tabella degli scores.}

The Bar Plot depicted in Figure \ref{fig:GFI-ionosphere} does not provide evidence of the presence of a single prevailing feature. Moreover in the Score Plot in Figure \ref{fig:Feat-imp-ionosphere} the differences between the average Importance Scores reported for the different features are minimal. This distinctive situation is probably due to the extremely high dimensionality of the {\ttfamily Ionosphere} dataset with respect to the other datasets presented in this study. 

On the other hand, the Scoremap plot, reported in Figure \ref{fig:Local-ionosphere} shows how most of the outliers are scattered along Feature 1 which however is not highlighted in Figure \ref{fig:GFI-ionosphere} and \ref{fig:Feat-imp-ionosphere}. The Anomaly Score contour plot clearly surrounds the central inlier distribution isolating the outliers. 

As a consequence the Average Precision values reported in Table \ref{tab:avg-prec-table} are quite satisfactory. 

%\modifica{Inoltre si può osservare che tali anomalie effettivamente si distribuiscano maggiornmente lungo la feature 1 non evidenziata dall'interpretazione}

\begin{comment}
\begin{table}[ht] 
\parbox{.45\linewidth}{
\centering
\begin{tabular}{|c|ccc|}
\hline
\multicolumn{4}{|c|}{\textbf{ionosphere} complete training} \\ \hline
\textbf{Metric} & \textbf{IF} & \textbf{EIF} & \textbf{EIF+} \\ \hline
Precision         & 0.66 & 0.69 & 0.70 \\
Recall            & 0.66 & 0.69 & 0.70 \\
f1 score          & 0.66 & 0.69 & 0.70 \\
Accuracy          & 0.76 & 0.78 & 0.78 \\

Average Precision & 0.82 & 0.83 & 0.84 \\
ROC AUC Score     & 0.86 & 0.87 & 0.88 \\ \hline
\end{tabular}
\caption{Performance Report \texttt{ionosphere} Dataset}
\label{tab:ionosphere-perf-complete}}
\end{table}
\end{comment}

%\modifica{ancora una volta proviamo a replicare }
%\modifica{far vedere nel caso in cui si splitta il training per capire se va meglio}

As usual, at this point, the inlier training approach is adopted in order to see if some improvement in the model's precision and reliability on the interpretation provided can be achieved. 

The Bar Plot (Figure \ref{fig:GFI-ionosphere-split} shows a much more evident confidence of the model in the identification of Feature 1 as the most relevant one for the detection of anomalies. The predominance of Feature 1 is highlighted also in the Score Plot (Figure \ref{fig:Feat-imp-ionosphere-split}) with a significant margin on the importance scores of the remaining features. 

For what concerns the Scoremap (Figure \ref{fig:Local-ionosphere-split}) is very similar to the one obtained with the complete training approach that confirms the high Average Precision values obtained in Table \ref{tab:avg-prec-table}. 

%\modifica{inserire tabella precisioni e vedere di quanto è migliorata e come potrebbe aver influito nell'interpretazione}

\begin{comment}
\begin{table}[ht]
\parbox{.45\linewidth}{
\centering
\begin{tabular}{|c|ccc|}
\hline
\multicolumn{4}{|c|}{\textbf{ionosphere} inlier training} \\ 
\hline
\textbf{Metric} & \textbf{IF} & \textbf{EIF} & 
\textbf{EIF+} \\ \hline
Precision         & 0.79 & 0.86 & 0.90 \\
Recall            & 0.79 & 0.86 & 0.90 \\
f1 score          & 0.79 & 0.86 & 0.90 \\
Accuracy          & 0.85 & 0.90 & 0.93 \\

Average Precision & 0.88 & 0.92 & 0.96 \\
ROC AUC Score     & 0.93 & 0.95 & 0.97 \\ \hline
\end{tabular}
\caption{Performance Report \texttt{ionosphere} Dataset}
\label{tab:ionosphere-perf-split}
}
\end{table}
\end{comment}

\begin{figure}[tbh]
  \centering
  \includegraphics[width=0.7\linewidth]{figures/feature_selection_plots_final/featsel_ionosphere_final.pdf}
  \caption{Feature Selection Plot {\ttfamily Ionosphere}}
  \label{fig:fs-ionosphere-plus}
\end{figure}%\hfil % <-- added

Figure \ref{fig:fs-ionosphere-plus} shows the results of the application of Unsupervised Feature Selection to the {\ttfamily Ionosphere} dataset. Differently from the outcomes obtained in the previously described datasets, in this instance, the Average Precision scores possess an overall decreasing behavior with the progressive removal of the input features. This is probably a consequence of the high-dimensionality of this dataset. 

The behavior of all the Feature Ranking Algorithms is very similar: the precision values stay constant for multiple steps and the decreasing effect starts to be noticed at around 10 features. A peculiar result is the one obtained with the ExIFFI algorithm which shows a huge increase in its Average Precision values passing from 2 (where it is the worst-performing model) to 1 feature where it becomes the best-performing model in terms of Average Precision. 

%\todo[inline, color=red]{Questo è un dataset interessante, ma rispetto ai precedenti mi pare che la cosa "nuova" sia solo il bell'andamento del plot di feature selection, o sbaglio? comunque è un buon dataset, usato anche nel paper originale dell'EIF, ed ha un aspetto "sensato" dal punto di vista della geometria delle anomalie. (Chiara)}


%\davide{

%The high number of features composing the {\ttfamily Ionosphere} dataset, presented in Section \ref{sec:real-world-data}, makes the interpretability task more challenging. The obtained outcomes are graphically summarized in Figure \ref{fig:ionosphere}.

%In any case, from \ref{fig:GFI-ionosphere} it is possible to see that Feature 3 is selected as the most important one 90\% of the time, and its importance is confirmed in \ref{fig:Feat-imp-ionosphere} where it is the feature with the highest average importance score. 

%In the Local Importance Scoremap, represented in \ref{fig:Local-ionosphere}, the comparison is performed on Feature 3 and Feature 26, the most and least important features respectively according to the Feature Importance Score Plot. Observing the scoremap, even though some of the outliers are part of the main cluster of inliers distributed along Feature 26, most of the anomalous data samples are scattered along Feature 3, confirming the high relevance of this feature for the {\ttfamily Ionosphere} dataset. The outliers are mainly contained on the left side of the plot, which is also the region dominated by blue-colored pixels meaning that the importance of Feature 3 is very high in this portion of the space.

%}

%\davide{
%Table \ref{tab:ionosphere-perf} reports the Classification metrics values for the {\ttfamily Ionosphere} dataset. Anomalies are detected with much higher efficiency with respect to the {\ttfamily Glass} dataset and the hierarchy between the three models under analysis remains the same. 
%}




==> sections/sections_world_dataset_results/ionosphere_new.tex <==
\subsection*{{\ttfamily Ionosphere}}

\ale{The {\ttfamily Ionosphere} dataset, as described in \ref{sec:appendix-real-world-data}, stands out as the dataset with the highest dimensionality (i.e. 33 features) inside the list of benchmark datasets used for the performance assessment in this study. This characteristic may have some consequences on the outcomes of the experiments described in the following sections.}

\subsubsection{Performance}

\ale{The results of the evaluation of each Anomaly Detection model across different values of the contamination hyperparameter are portrayed in Figure \ref{fig:Ionosphere_contamination_full}. The entirety of the models show how the gradual addition of anomalies in the dataset does not result in a significant effect on the Average Precision metric that, in fact, shows more or less constant values very close to a perfect score of 1. The proposed approach \EIFplus, together with the DIF model, are the ones showing the best metric values, followed by EIF, as highligthed in the comparison between \EIFplus and EIF displayed in Figure \ref{fig:Ionosphere_contaminationEIFvsEIF+}.}

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.49\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Ionosphere/Contamination/22-03-2024_14-36-31_ionosphere_contamination_full_plot.pdf}
      \caption{Models evaluation, varying the contamination levels}
      \label{fig:Ionosphere_contamination_full}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.44\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Ionosphere/Contamination/22-03-2024_14-38-31_ionosphere_EIF+_minus_EIF_precision_over_contamination.pdf}
      \caption{Difference between \EIFplus and EIF average precision}
      \label{fig:Ionosphere_contaminationEIFvsEIF+}
    \end{subfigure}\hfil % <-- added
\caption{Figure \ref{fig:Ionosphere_contamination_full} illustrates the average precision as the contamination level in the training set increases. Figure \ref{fig:Ionosphere_contaminationEIFvsEIF+} compares the performance graphs of EIF and \EIFplus, using the difference of their scores in various contamination levels.}
\label{fig:Ionosphere_contamination}
\end{figure}

\ale{As a result of a careful observations of Table \ref{tab:Ionosphere_perf}  it is possible to conclude that the optimal models for the Anomaly Detection task on the {\ttfamily Ionosphere} dataset are \EIFplus and DIF. The performances offered by these models are in fact  superior to the ones of all other methods but since \EIFplus demonstrates significantly improved efficiency during both the fitting and prediction phases it is the best choice in this scenario.}

\begin{table}[htbp]
\begin{minipage}[t]{0.46\textwidth}
\strut\vspace*{-\baselineskip}\newline
\resizebox{\textwidth}{!}{
\begin{tabular}{|c||ccc|ccc||cc|}
\toprule
\hline
&\multicolumn{3}{c|}{Scenario I}&\multicolumn{3}{c||}{Scenario II}&\multicolumn{2}{c|}{Time}\\
\hline
AD Model & Avg & Prec & ROC & Avg & Prec & ROC & fit & pred \\
& Prec &  & AUC & Prec &  & AUC &  &  \\
\hline
IF          & 0.79& 0.65& 0.73& 0.89& 0.79& 0.83& \textbf{0.05}& \textbf{0.0026}\\
EIF         & 0.82& 0.69& 0.76& 0.9& 0.82& 0.86& 0.14& 0.02\\
EIF+        & 0.84& 0.72& 0.78& 0.96& 0.87& 0.9& 0.11& 0.02\\
DIF         & \textbf{0.87}& \textbf{0.76}& \textbf{0.81}& \textbf{0.96}& \textbf{0.89}& \textbf{0.9}& 0.72& 0.44\\
AE & 0.76& 0.6& 0.68& 0.87& 0.75& 0.8& 2.26& 0.09\\
\hline
\end{tabular}}
\vspace{0.41cm}
\caption{Performances of 5 different Anomaly Detection models over {\ttfamily Ionosphere} are compared using classical Classification metrics. Moreover, the last two columns contain the average time for a fit and predict operation. The highest metric values and the lowest execution times are highlighted in bold}\label{tab:Ionosphere_perf}
\end{minipage}
\hfill
\begin{minipage}[t]{0.46\textwidth}
\strut\vspace*{-\baselineskip}\newline
\resizebox{\textwidth}{!}{
\begin{tabular}{|c||c|c|c|c||c|}
\toprule
\hline
&\multicolumn{2}{c|}{Evaluation with EIF}&\multicolumn{2}{c||}{Evaluation with \EIFplus}&\\
\hline
& Scenario I & Scenario II & Scenario I & Scenario II & Time\\

 Algorithm & $AUC_{FS}$  & $AUC_{FS}$ & $AUC_{FS}$  & $AUC_{FS}$ &  \\
\hline
DIFFI               & 2.367& -1.336& -1.135& 1.924& 0.31\\
IF\_\approach        & \textbf{3.294}& 0.891& \textbf{2.683}& 0.266& \textbf{0.16}\\
EIF\_\approach       & 1.828& \textbf{4.313}& 1.615& \textbf{2.841}& \textbf{0.16}\\
\EIFplus\_\approach  & 0.619& 2.268& 0.454& 1.410& 0.17\\
IF\_RF              & -1.914& -1.237& 1.762& -1.087& 0.60\\
EIF\_RF             & -1.975& 1.337& -1.857& 0.695& 0.60\\
EIF+\_RF            & -1.871& 3.586& -1.568& 2.171& 0.60\\
\hline
\end{tabular}}
\caption{Quantitative evaluation of the effectiveness of 6 different interpretation algorithms on {\ttfamily Ionosphere} through the $AUC_{FS}$ metric, introduced in \ref{sec:interpr_evaluat}. In the last column the average time taken by the different models to produce the importance scores is reported. The highest $AUC_{FS}$ and lowest Importance time values are highlighted in bold.}\label{tab:fs-tab-Ionosphere}
\end{minipage}
\end{table}


\subsubsection{Importance Plots}

\ale{In Figure \ref{fig:interpretation-Ionosphere} it is possible to see how challenging the task of interpreting the relevance of the features used by and AD model can be in the case of feature spaces of high dimensionality. As it can be in fact concluded observing both the Score Plots (Figures \ref{fig:Feat-imp-Ionosphere}, \ref{fig:Feat-imp-Ionosphere-split}) and the Bar Plots (Figures \ref{fig:GFI-Ionosphere}, \ref{fig:GFI-Ionosphere-split}) the importance is evenly shared across all features and it is daunting to find a single feature or a small subset of features whose relevance is significantly higher than the ones of the remaining attributes.} 

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.35\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Ionosphere/Importance_plots/02-03-2024_16-21-53_GFI_Bar_plot_ionosphere_EXIFFI+_1.pdf}
      \caption{Bar Plot {\ttfamily Ionosphere} Scenario I}
      \label{fig:GFI-Ionosphere}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.25\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Ionosphere/Importance_plots/02-03-2024_16-21-54_GFI_Score_plot_ionosphere_EXIFFI+_1.pdf}
      \caption{Score Plot {\ttfamily Ionosphere} Scenario I}
      \label{fig:Feat-imp-Ionosphere}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Ionosphere/Local_Scoremaps/22-03-2024_10-21-38_importance_map_ionosphere_EXIFFI+_1_feat_1_2.pdf}
      \caption{Scoremap {\ttfamily Ionosphere} Scenario I}
      \label{fig:Local-Ionosphere}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.35\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Ionosphere/Importance_plots/02-03-2024_14-45-53_GFI_Bar_plot_ionosphere_EXIFFI+_2.pdf}
      \caption{Bar Plot {\ttfamily Ionosphere} Scenario II}
      \label{fig:GFI-Ionosphere-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.25\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Ionosphere/Importance_plots/02-03-2024_14-45-53_GFI_Score_plot_ionosphere_EXIFFI+_2.pdf}
      \caption{Score Plot {\ttfamily Ionosphere} Scenario II}
      \label{fig:Feat-imp-Ionosphere-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Ionosphere/Local_Scoremaps/22-03-2024_10-21-29_importance_map_ionosphere_EXIFFI+_2_feat_1_2.pdf}
      \caption{Scoremap {\ttfamily Ionosphere} Scenario II}
      \label{fig:Local-Ionosphere-split}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot and Scoremap for {\ttfamily Ionosphere} in the two different Scenarios, using the \approach algorithm applied to the \EIFplus model.}\label{fig:interpretation-Ionosphere}
\end{figure}

\subsubsection{Feature Selection}

\ale{The phenomenon observable in the Feature Selection plots of the {\ttfamily Ionosphere} (Figure \ref{fig:fs-interpretation-Diabetes}) dataset is similar to the one presented in section \ref{sec:Breastw}  for the {\ttfamily Breastw} dataset. Essentially since the importance is shared across a group of features the Average Precision follows a constant trend and starts to decrease as important features are progressively removed from the group of relevant attributes, as it can be noticed in Figure \ref{fig:Feat-Sel_Ionosphere_valEIF+_EXIFFI+_2}.}

\begin{figure}[!ht] 
\centering
\hspace{0.05\textwidth}\textbf{IF} \hspace{0.29\textwidth} \textbf{EIF} \hspace{0.29\textwidth} \textbf{EIF+}
% First row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Ad-Hoc}}} % Adjust the parbox width as necessary for your caption text
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Ionosphere/Feature_Selection/07-05-2024_15-31-24_ionosphere_EIF+_IF_EXIFFI_feature_selection_2.pdf}
            \caption{\approach applied to IF}
            \label{fig:Feat-Sel_Ionosphere_valEIF+_DIFFI_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Ionosphere/Feature_Selection/22-03-2024_14-48-05_ionosphere_EIF+_EXIFFI_feature_selection_2.pdf}
            \caption{\approach applied to EIF}
            \label{fig:Feat-Sel_Ionosphere_valEIF+_EXIFFI_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Ionosphere/Feature_Selection/22-03-2024_14-51-55_ionosphere_EIF+_EXIFFI+_feature_selection_2.pdf}
            \caption{\approach applied to \EIFplus}
            \label{fig:Feat-Sel_Ionosphere_valEIF+_EXIFFI+_2}
        \end{subfigure}
    \end{minipage}
\end{minipage}

\vspace{5mm} % Space between rows

% Second row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Post-Hoc}}} % Adjust as necessary
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Ionosphere/Feature_Selection/22-03-2024_14-48-05_ionosphere_EIF+_IF_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to IF}
            \label{fig:Feat-Sel_Ionosphere_valEIF+_IF_RandomForest_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Ionosphere/Feature_Selection/22-03-2024_12-32-45_ionosphere_EIF+_EIF_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to EIF}
            \label{fig:Feat-Sel_Ionosphere_valEIF+_EIF_RandomForest_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Ionosphere/Feature_Selection/22-03-2024_14-48-05_ionosphere_EIF+_EIF+_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to \EIFplus}
            \label{fig:Feat-Sel_Ionosphere_valEIF+_EIF+_RandomForest_2}
        \end{subfigure}
    \end{minipage}
\end{minipage}

\caption{Feature Selection of the different Ad-Hoc and Post-Hoc methods applied to the 3 Isolation Forest models: IF, EIF and \EIFplus. The blue line is the values of average precision, calculated with the \EIFplus model in the Scenario II, dropping the most important feature at each step, the red line is the values of average precision dropping the least important feature at each step and the green line is the value of the feature selection dropping a random feature at each step.}\label{fig:fs-interpretation-Ionosphere}
\end{figure}

\ale{Table \ref{tab:fs-tab-Ionosphere} lists the values of the $AUC_{FS}$ metric in Scenario I and Scenario II. The only interpretation models able to provide a feature ranking correctly aligning with the dataset's characteristics are \approach, \approach+ and the post-hoc Random Forest model applied to the \EIFplus AD method. Among these two the most efficient one in terms of computational time is \approach+.} 



==> sections/sections_world_dataset_results/moodify.tex <==
\subsubsection*{{\ttfamily Moodify}}


In Appendix \ref{sec:real-world-data}, we present an overview of the {\ttfamily Moodify} dataset. This dataset consists of eleven numerical features, which will be the primary focus of our analysis in this section. Notably, this dataset is unique because it includes a clearly defined outlier class, corresponding to music labeled as "Calm," in contrast to the inliers, which encompass the categories of "Happy," "Sad," and "Energetic."

Furthermore, it is worth noting that the features in this dataset are labeled in a straightforward manner, obviating the need for specialized expertise to discern their relevance. This accessibility enables us to reasonably evaluate the significance of each feature.

%\modifica{mettere risultati importances nel caso in cui è allenata interamente sul dataset di moodify}

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/moodify/Feat_bar_plot_moodify.pdf}
      \caption{Score Plot \texttt{Moodify} Scenario I}
      \label{fig:Feat-imp-moodify}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/moodify/Feat_bar_plot_moodify_split.pdf}
      \caption{Score Plot \texttt{Moodify} Scenario II}
      \label{fig:Feat-imp-moodify-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/moodify/GFI_moodify_synt.pdf}
      \caption{Bar Plot \texttt{Moodify} Scenario I}
      \label{fig:GFI-moodify}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/moodify/GFI_moodify_split_synt.pdf}
      \caption{Bar Plot \texttt{Moodify} Scenario II}
      \label{fig:GFI-moodify-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/scoremaps_real_world/Local_Scoremap_Plot_moodify.png}
      \caption{Scoremap \texttt{Moodify} Scenario I}
      \label{fig:Local-moodify}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/scoremaps_real_world/Local_Scoremap_Plot_moodify_split.png}
      \caption{Scoremap \texttt{Moodify} Scenario II}
      \label{fig:Local-moodify-split}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot and Scoremap for \texttt{Moodify} }\label{fig:interpretation-moodify}
\end{figure}

Just like we witnessed in the \texttt{Annthyroid} dataset, the model's Average Precision, as depicted in Table \ref{tab:avg-prec-table}, is notably low. This suggests that distinguishing labeled anomalies from the majority of inliers within the dataset is a challenging task due to their limited separation.

Furthermore, as was the case with the \texttt{Annthyroid} dataset, Figures \ref{fig:GFI-moodify} and \ref{fig:Feat-imp-moodify} demonstrate that no single feature stands out as significantly more important than the others. However, a closer examination of Figure \ref{fig:Local-moodify} reveals an interesting pattern: while the anomalies are spread across the dataset, Feature 3 appears to have a higher concentration of labeled anomalies, despite it is possible to observe a greater deviation from the distribution along Feature 7.

In line with our approach in other examples, we opted to exclusively train the model using inliers. This strategy aimed to align the model's predictions with the labeled data, enabling us to discern which features play a pivotal role in characterizing the deviations within the anomalies given by the dataset.

Upon examination of Table \ref{tab:avg-prec-table}, it becomes evident that the Average Precision metric doubled, resulting in more congruent results with the labeled anomalies. This enhancement in performance reinforces the significance of our approach.

Furthermore, when analyzing Figure \ref{fig:GFI-moodify-split} and Figure \ref{fig:Feat-imp-moodify-split}, Feature 3 consistently emerges as the most influential feature. This reaffirms our previous observations from the Scoremap analysis. 

\begin{comment}
\begin{table}[ht]
\parbox{.45\linewidth}{
\centering
\begin{tabular}{|c|ccc|}
\hline
\multicolumn{4}{|c|}{\textbf{moodify} complete training} \\ \hline
\textbf{Metric} & \textbf{IF} & \textbf{EIF} & \textbf{EIF+} \\ \hline
Precision         & 0.35 & 0.35 & 0.35 \\
Recall            & 0.35 & 0.35 & 0.35 \\
f1 score          & 0.35 & 0.35 & 0.35 \\
Accuracy          & 0.80 & 0.80 & 0.80 \\

Average Precision & 0.34 & 0.32 & 0.32 \\
ROC AUC Score     & 0.82 & 0.81 & 0.81 \\ \hline
\end{tabular}
\caption{Performance Report \texttt{moodify} Dataset}
\label{tab:moodify-perf-complete}}
\end{table}
\end{comment}

%\modifica{far vedere nel caso in cui si splitta il training per capire se va meglio}
Feature 3, as explained in Appendix \ref{sec:real-world-data}, quantifies the energy level present in a typical Spotify track. It is reasonable to intuitively assume that the Energy feature plays a crucial role in distinguishing "Calm" songs from those categorized as "Happy," "Energetic," or "Sad." As anticipated, the inlier group indeed exhibits significantly higher energy values (with an average of 0.62) compared to the outlier group (which has an average of 0.18).

%\modifica{inserire tabella precisioni e vedere di quanto è migliorata e come potrebbe aver influito nell'interpretazione}
\begin{comment}
\begin{table}[ht]
\parbox{.45\linewidth}{
\centering
\begin{tabular}{|c|ccc|}
\hline
\multicolumn{4}{|c|}{\textbf{moodify} inlier training} \\ 
\hline
\textbf{Metric} & \textbf{IF} & \textbf{EIF} & 
\textbf{EIF+} \\ \hline
Precision         & 0.75 & 0.72 & 0.75 \\
Recall            & 0.75 & 0.72 & 0.75 \\
f1 score          & 0.75 & 0.72 & 0.75 \\
Accuracy          & 0.92 & 0.92 & 0.92 \\

Average Precision & 0.75 & 0.67 & 0.71 \\
ROC AUC Score     & 0.96 & 0.96 & 0.96 \\ \hline
\end{tabular}
\caption{Performance Report \texttt{moodify} Dataset}
\label{tab:moodify-perf-split}
}
\end{table}
\end{comment}

\begin{figure}[!ht] 
  \centering
  \includegraphics[width=0.7\linewidth]{figures/feature_selection_plots_final/featsel_moodify_final.pdf}
  \caption{Feature Selection Plot {\ttfamily Moodify}}
  \label{fig:fs-moodify-plus}
\end{figure}\hfil % <-- added

Finally, let's delve into the Feature Selection Plot for the {\ttfamily Moodify} dataset, as depicted in Figure \ref{fig:fs-moodify-plus}. This plot provides further validation for the consistency of the model's interpretation when trained exclusively on inliers. Specifically, when utilizing the ExIFFI-plus-split and ExIFFI-split Feature Ranking Algorithms, we observe a consistent improvement in Average Precision values as the number of input features decreases.

In conclusion, this reaffirms the effectiveness of the feature importance evaluation by our approach. It's essential to emphasize that this interpretation remains closely tied to the anomalies detected by the model, even in this context.

%\todo[inline, color=red]{Questo ha il vantaggio che possiamo un po' interpretarlo qualitativamente sapendo cosa sono le features.. ditemi voi se ha senso tenerlo o no nel corpo del paper (Chiara)}


%\davide{
% Up to 2 features, the Average Precision of the E-DIFFI,E-IFFI-plus, and E-IFFI models increases. A precision drop can be observed in the passage from 2 to 1 features. This probably means that the two most important featueres, i.e. Feature 3 and Feature 10, are better considered together than alone. On the other hand DIFFI, Random Forest and Casual start a constant decrease from Feature 8 onwards. 
%}



%\davide{

%As it can be noticed from Figure \ref{fig:GFI-moodify} and \ref{fig:Feat-imp-moodify} The most important feature here is Feature 3 followed by Feature 0 and Feature 10. 

%According to the dataset description, placed in Section \ref{sec:real-world-data}, these features represents respectively the Energy, Duration and Spec-rate of a Spotify track.

%The Energy feature can be considered as a dominant feature since it was placed in the top ranking of the Global Feature Importance Bar Plot in all the model's instances and possesses the highest Average Feature Score with a significant margin over the remaining features. 

%In the Local Importance Scoremap (Figure \ref{fig:Local-moodify}) Features 3 and 10 were compared. An exhaustive analysis of the points distribution along these aforementioned features brings to the conclusion that all the outliers are dispersed along Feature 3. On the contrary a set of \textit{model anomalies} scattered along Feature 10 are likely responsible for the high importance of the spec-rate attribute

%}
%\davide {

%The {\ttfamily Moodify} dataset posseses a pecualiar behavior with the presence of \textit{model anomalies} which sligthly effects the Performance Report placed in Table \ref{tab:moodify-perf}. The three models under analysis, i.e. IF,EIF and EIF+, have very similar values across all the metrics. Differently from other cases the IF model's performance metrics are very close to the ones of the more complex EIF and EIF+ models. 

%}


==> sections/sections_world_dataset_results/moodify_new.tex <==
\subsection*{{\ttfamily Moodify}}

% Additional comment to satisfy comment 7 by reviewer 2 and Comment 11 of reviewer 1 
\davide{The final datasets considered for the evaluation of the quality of the explanations is the {\ttfamily moodify} datasets, introduced in \ref{sec:appendix-real-world-data}. Converting this dataset in order to make it suitable for the Anomaly Detection task corresponds to distinguish \textit{calm} Spotify tracks from the rest. Thus, similarly to the {\ttfamily glass} dataset \ref{sec:glass}, it is possible to compare the conclusions reached by the model (i.e. \approach) with human intuition on what are the most relevent features to perform the previously cited distinction.} 

\subsubsection{Performance}
In the contamination plot \ref{fig:Moodify_contamination_full}, it's evident that all models perform better when there are no anomalies in the training data (contamination=0), with the DIF model showing the most significant improvement. Although the \EIFplus does not consistently yield high performance, it surpasses EIF in scenarios where it is trained exclusively on inliers, as anticipated. This trend is depicted in the plot comparing the performance differences between \EIFplus and EIF in Figure \ref{fig:Moodify_contaminationEIFvsEIF+}, illustrating \EIFplus's enhanced ability to adapt and identify anomalies when trained on a clean dataset.\ref{fig:Moodify_contaminationEIFvsEIF+}.

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.49\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Moodify/Contamination/18-03-2024_18-24-06_moodify_contamination_full_plot.pdf}
      \caption{Models evaluation, varying the contamination levels}
      \label{fig:Moodify_contamination_full}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.44\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Moodify/Contamination/19-03-2024_09-16-46_moodify_EIF+_minus_EIF_precision_over_contamination.pdf}
      \caption{Difference between \EIFplus and EIF average precision}
      \label{fig:Moodify_contaminationEIFvsEIF+}
    \end{subfigure}\hfil % <-- added
\caption{Figure \ref{fig:Moodify_contamination_full} illustrates the average precision as the contamination level in the training set increases. Figure \ref{fig:Moodify_contaminationEIFvsEIF+} compares the performance graphs of EIF and \EIFplus, using the difference of their scores in various contamination levels.}
\label{fig:Moodify_contamination}
\end{figure}

Table \ref{tab:performance_moodify} provides detailed insights into the performance metrics of the models. 

Although both the DIF and the IF model achieves the highest value of Average Precision in Scenario II, as reported in the performance table,  the DIF proves to be significantly slower in the fitting and predicting operations compared to the IF method.

%This indicates that the DIF model fails to identify a significant number of actual anomalies within the dataset. 
\begin{table}[htbp]
\centering
%\caption{{\ttfamily Moodify} Precision Report}
\caption{Performances of 5 different Anomaly Detection models over {\ttfamily Moodify} are compared using classical Classification metrics. Moreover, the last two columns contain the average time for a fit and predict operation. The highest metric values and the lowest execution times are highlighted in bold}\label{tab:performance_moodify}
\begin{tabular}{|c||ccc|ccc||cc|}
\toprule
\hline
& \multicolumn{3}{c|}{Scenario I} & \multicolumn{3}{c||}{Scenario II} & \multicolumn{2}{c|}{Time} \\
\hline
AD Model& Avg & Prec & ROC & Avg & Prec & ROC & fit & pred \\
 & Prec &  & AUC & Prec &  & AUC &  &  \\
\hline
IF          & 0.35 & 0.30 & 0.59 & \textbf{0.72}& \textbf{0.73}& \textbf{0.84}& 0.11 & \textbf{0.05}\\
EIF         & 0.33 & 0.37 & 0.63 & 0.65 & 0.64 & 0.79 & \textbf{0.09}& 0.27  \\
\EIFplus        & 0.28 & 0.27 & 0.57 & 0.66 & 0.66 & 0.80 & \textbf{0.09}& 0.25 \\
DIF         & 0.26& 0.26& 0.56& \textbf{0.72}& \textbf{0.73}& \textbf{0.84}& 7.76 & 7.5  \\
AE & \textbf{0.45}& \textbf{0.53}& \textbf{0.72}& 0.65& 0.68& 0.81& 16.6 & 0.26 \\
\hline
\end{tabular}
\end{table}

Consequently, the consistent results demonstrated by the IF model make it a more reliable choice in this scenario, balancing the ability to detect anomalies with computational efficiency. %fewer misses 

The outcomes for Scenario I significantly diverge from those observed at a contamination level of 0.1, as depicted in plot \ref{fig:Moodify_contamination_full}. In Scenario I, the contamination level inherent to the dataset, 0.1527, is specifically considered. Notably, in this context, the Anomaly Autoencoder exhibits very low sensitivity to changes in the training dataset's contamination level compared to the other models. 


\subsubsection{Importance Plots}

The importance plots in Scenario I, depicted in Figures \ref{fig:Feat-imp-Moodify}, highlight four features that significantly characterize the anomalies of the dataset, in particular the ``speechliness" and the ``duration", suggesting that the dataset includes unique song types. These variations may point to specific genres such as instrumental music or tracks of atypical lengths, like podcasts or classical music, that stand out from standard musical distributions.

In contrast, Scenario II sheds light on the characteristics that set the outlier class separates from the general dataset distribution. Specifically, the 'loudness' feature, which measures a track's overall volume in decibels (dB), as explained in the Appendix \ref{sec:appendix-real-world-data}, is identified as particularly significant in Figure \ref{fig:Feat-imp-Moodify-split}. This observation is consistent with the expectation that 'Calm' music tracks, the ones labelled as outliers, exhibit lower dB levels. The local scoremap presented in Figure \ref{fig:interpretation-Moodify} provides further insight, demonstrating how 'Calm' tracks distinctly deviate based on this feature, thus reinforcing the importance of 'loudness' in distinguishing these outliers within the dataset.

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.38\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Moodify/Importance_plots/02-03-2024_17-19-20_GFI_Bar_plot_moodify_EXIFFI+_1.pdf}
      \caption{Score Plot {\ttfamily Moodify} Scenario I}
      \label{fig:Feat-imp-Moodify}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.32\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Moodify/Importance_plots/02-03-2024_17-19-21_GFI_Score_plot_moodify_EXIFFI+_1.pdf}
      \caption{Bar Plot {\ttfamily Moodify} Scenario I}
      \label{fig:GFI-Moodify}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Moodify/Local_Scoremap/07-03-2024_17-23-57_importance_map_moodify_EXIFFI+_1_feat_3_10.pdf}
      \caption{Scoremap {\ttfamily Moodify} Scenario I}
      \label{fig:Local-Moodify}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.35\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Moodify/Importance_plots/08-05-2024_18-06-54_GFI_Bar_plot_moodify_EXIFFI+_2.pdf}
      \caption{Score Plot {\ttfamily Moodify} Scenario II}
      \label{fig:Feat-imp-Moodify-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.30\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Moodify/Importance_plots/08-05-2024_18-06-54_GFI_Score_plot_moodify_EXIFFI+_2.pdf}
      \caption{Bar Plot {\ttfamily Moodify} Scenario II}
      \label{fig:GFI-Moodify-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Moodify/Local_Scoremap/07-03-2024_17-23-43_importance_map_moodify_EXIFFI+_2_feat_3_10.pdf}
      \caption{Scoremap {\ttfamily Moodify} Scenario II}
      \label{fig:Local-Moodify-split}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot and Scoremap for {\ttfamily Moodify}  in the two different Scenarios, using the \approach algorithm applied to the \EIFplus model.}\label{fig:interpretation-Moodify}
\end{figure}

\subsubsection{Feature Selection}

The Feature Selection plots grouped in \ref{fig:feature_selections-Moodify} outline a similar behavior, all showing positive values of the $AUC_{FS}$ metric. 

Both the EIF and \EIFplus models, when analyzed through ad-hoc and post-hoc interpretation methods, achieve high scores. They demonstrate a similar trend of improved average precision as the dataset is condensed to its most significant dimensions. This indicates that both interpretation algorithms, regardless of the interpretation method applied, are adept at distilling essential information, thereby enhancing their predictive accuracy when focusing on the most important features.

However, the application of \approach to the IF model (Figure \ref{fig:Feat-Sel_Moodify_valIF_EXIFFI_2}) stands out as the best interpretability approach for the {\ttfamily moodify} dataset. The main difference with the respect to the other methods can be observed in the Average Precision trend depicted in the blue curve, representing the approach of removing features in increasing order of relevance, that is associated with a clear decreasing behavior. On the other hand, in the other approaches the aforementioned curve presents an oscillating trend, consequence of a feature importance ranking not perfectly aligned with the ground truth. 

\begin{comment}
During the Feature Selection process, it becomes evident that the DIFFI algorithm struggles to accurately identify the most critical features, leading to bad performance when the feature selection evaluate the model using the most important features according to this interpretation method and , thus, yielding to a negative value of the $AUC_{FS}$ metric. Conversely, utilizing Random Forest as a surrogate model for interpreting the IF model's results yields better performance, showcasing its effectiveness in feature importance evaluation.
\end{comment}


\begin{figure}[!ht] 
\centering
\textbf{IF} \hspace{0.25\textwidth} \textbf{EIF} \hspace{0.25\textwidth} \textbf{\EIFplus}
% First row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Ad-Hoc}}} % Adjust the parbox width as necessary for your caption text
    \begin{minipage}{0.90\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Moodify/Feature_Selection/07-05-2024_09-31-32_moodify_EIF+_IF_EXIFFI_feature_selection_2.pdf}
            \caption{\approach applied to IF}
            \label{fig:Feat-Sel_Moodify_valIF_EXIFFI_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Moodify/Feature_Selection/08-05-2024_16-52-16_moodify_EIF+_EXIFFI_feature_selection_2.pdf}
            \caption{\approach applied to EIF}
            \label{fig:Feat-Sel_Moodify_valEIF+_EXIFFI_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Moodify/Feature_Selection/08-05-2024_18-09-12_moodify_EIF+_EXIFFI+_feature_selection_2.pdf}
            \caption{\approach applied to \EIFplus}
            \label{fig:Feat-Sel_Moodify_valEIF+_EXIFFI+_2}
        \end{subfigure}
    \end{minipage}
\end{minipage}

\vspace{5mm} % Space between rows

% Second row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Post-Hoc}}} % Adjust as necessary
    \begin{minipage}{0.90\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Moodify/Feature_Selection/19-03-2024_21-35-41_moodify_EIF+_IF_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest applied to IF}
            \label{fig:Feat-Sel_Moodify_valEIF+_IF_RandomForest_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Moodify/Feature_Selection/19-03-2024_21-32-15_moodify_EIF+_EIF_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest applied to EIF}
            \label{fig:Feat-Sel_Moodify_valEIF+_EIF_RandomForest_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Moodify/Feature_Selection/19-03-2024_21-26-23_moodify_EIF+_EIF+_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest applied to \EIFplus}
            \label{fig:Feat-Sel_Moodify_valEIF+_EIF+_RandomForest_2}
        \end{subfigure}
    \end{minipage}
\end{minipage}
\caption{Feature Selection of the different Ad-Hoc and Post-Hoc methods applied to the 3 Isolation Forest models: IF, EIF and \EIFplus. The blue line is the values of average precision, calculated with the \EIFplus model in the Scenario II, dropping the most important feature at each step, the red line is the values of average precision dropping the least important feature at each step and the green line is the value of the feature selection dropping a random feature at each step.}\label{fig:feature_selections-Moodify}
\end{figure}

\begin{table}[htbp]
\centering
%\caption{Feature Selection Scores {\ttfamily moodify}}
\caption{Quantitative evaluation of the effectiveness of 6 different interpretation algorithms on {\ttfamily Moodify} through the $AUC_{FS}$ metric, introduced in \ref{sec:interpr_evaluat}. In the last column the average time taken by the different models to produce the importance scores is reported. The highest $AUC_{FS}$ and lowest Importance time values are highlighted in bold.}\label{tab:fs-tab-moodify}
\begin{tabular}{|c||c|c|c|c||c|}
\toprule
\hline
&\multicolumn{2}{c|}{Evaluation with EIF}&\multicolumn{2}{c||}{Evaluation with \EIFplus}&\\
\hline
& Scenario I & Scenario II & Scenario I & Scenario II & Time\\

 Algorithm & $AUC_{FS}$  & $AUC_{FS}$ & $AUC_{FS}$  & $AUC_{FS}$ &  \\
\hline
DIFFI         & -1.484     & -3.66    & -1.118     & -3.368   & \textbf{0.57} \\
IF\_\approach         & -1.681    & \textbf{4.398}    & -1.162     & \textbf{4.231}   & 1.05 \\
EIF\_\approach        & -1.787     & 1.844& -1.37     & 2.049& \textbf{0.94} \\
\EIFplus\_\approach       & -1.51     & 2.331& -0.991     & 2.39& 0.99 \\
IF\_RF        & \textbf{-0.785}     & 2.077     & \textbf{-0.723}     & 2.483     & 8.05 \\
EIF\_RF       & -0.848    & 1.631    & -0.717     & 2.174    & 8.05  \\
\EIFplus\_RF      & -1.882     & 1.476     & -1.433     & 2.086     & 8.05  \\
\hline
\end{tabular}
\end{table}

Table \ref{tab:fs-tab-moodify} showcases the $AUC_{FS}$ scores derived from various interpretation methods. In Scenario I, interpretations appear to fail, likely because the model fails to accurately pinpoint the given anomalies, but rather represent other kinds of deviation from the normal distribution of the dataset. Conversely, when models are trained exclusively with inliers, there's a notable improvement in results. Particularly, the \approach and post-hoc algorithms excel, demonstrating robust performance. This behavior holds for all the considered interpretation apporaches except for DIFFI, where the struggle to accurately identify the most critical features becomes evident for the presence of negative values of the $AUC_{FS}$ metric in both scenarios. 

Finally, a critical observation is the computational efficiency of the \approach, which is 10 times faster than that of post-hoc models. This highlights the \approach's advantage in scenarios with limited computational resources, emphasizing its efficacy and speed in model interpretation tasks.







==> sections/sections_world_dataset_results/pendigits.tex <==
\subsubsection{{\ttfamily Pendigits}}

The {\ttfamily Pendigits} dataset collects data regarding handwritten digits produced by Forty-four human writers. The task is the one of recognizing the correct written digit but the dataset, as usual, was adapted to be used for the evaluation of the Anomaly Detection model considered in this study. The dataset is composed by sixteen features. Additional details can be found in Appendix \ref{sec:real-world-data}. 

%\modifica{mettere risultati importances nel caso in cui è allenata interamente sul dataset di pendigits}

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/pendigits/Feat_bar_plot_pendigits.pdf}
      \caption{Score Plot \texttt{Pendigits} Scenario I}
      \label{fig:Feat-imp-pendigits}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/pendigits/Feat_bar_plot_pendigits_split.pdf}
      \caption{Score Plot \texttt{Pendigits} Scenario II}
      \label{fig:Feat-imp-pendigits-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/pendigits/GFI_pendigits_synt.pdf}
      \caption{Bar Plot \texttt{Pendigits} Scenario I}
      \label{fig:GFI-pendigits}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/pendigits/GFI_pendigits_split_synt.pdf}
      \caption{Bar Plot \texttt{Pendigits} Scenario II}
      \label{fig:GFI-pendigits-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/scoremaps_real_world/Local_Scoremap_Plot_pendigits.png}
      \caption{Scoremap \texttt{Pendigits} Scenario I}
      \label{fig:Local-pendigits}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/scoremaps_real_world/Local_Scoremap_Plot_pendigits_split.png}
      \caption{Scoremap \texttt{Pendigits} Scenario II}
      \label{fig:Local-pendigits-split}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot and Scoremap for \texttt{Pendigits}}
\label{fig:interpretation-pendigits}
\end{figure}

The Bar Plot for the {\ttfamily Pendigits} dataset is displayed in Figure \ref{fig:GFI-pendigits}. There is not a clear dominant feature in terms of importance score. Two features that may be considered significantly relevant are Feature 1 and Feature 3 which were selected respectively 40\% and 30\% of the time as the top feature in the dataset. These two features are also placed in the first two positions in the Score Plot, in Figure \ref{fig:Feat-imp-pendigits} but their average importance score values are not considerably higher than the ones obtained by the other attributes. 

Looking at the Scoremap (Figure \ref{fig:Local-pendigits}) it is possible to notice that, indeed, anomalous samples are distributed along both Feature 3 and 1 although most of them are overlapped with the inliers. Additionally, two small clusters of points, isolated from the main data distribution, can be detected. The first one is a cluster of outliers scattered along Feature 1, the second one is, instead, a group of inliers placed along Feature 3. 

%\modifica{mettere tabella precisioni allenato su tutto}

\begin{comment}
\begin{table}[ht]
\parbox{.45\linewidth}{
\centering
\begin{tabular}{|c|ccc|}
\hline
\multicolumn{4}{|c|}{\textbf{Pendigits} complete training} \\ \hline
\textbf{Metric} & \textbf{IF} & \textbf{EIF} & \textbf{EIF+} \\ \hline
Precision         & 0.37 & 0.37 & 0.35 \\
Recall            & 0.37 & 0.37 & 0.35 \\
f1 score          & 0.37 & 0.37 & 0.35 \\
Accuracy          & 0.97 & 0.97 & 0.97 \\

Average Precision & 0.27 & 0.24 & 0.25 \\
ROC AUC Score     & 0.94 & 0.93 & 0.93 \\ \hline
\end{tabular}
\caption{Performance Report \texttt{Pendigits} Dataset}
\label{tab:pendigits-perf-complete}}
\end{table}
\end{comment}

Probably because of the overlapping nature of most of the outlier points with inliers and because of the presence of a group of deviant points labeled, according to the dataset, as inliers, the Average Precision values (Table \ref{tab:avg-prec-table}) are not satisfactory. 

%\modifica{far vedere nel caso in cui si splitta il training per capire se va meglio}

In order to refine the interpretability and precision results shown up to this point, the strategy of training the model exclusively on the inliers and using the entire dataset to test the model was adopted. 


The results of this new approach are reported on the right column of Figure \ref{fig:interpretation-pendigits}. In particular, Figure \ref{fig:GFI-pendigits-split} shows how also Feature 5 plays a role in helping the model to detect anomalous points, together with the usual Feature 1 and 3. These two features are still considered in pair to evaluate the Scoremap (Figure \ref{fig:Local-pendigits-split}. The latter does not undergo major changes with the ones obtained in Scenario I. Some of these changes include the contour lines which are able to isolate a higher number of outliers. 

As a consequence, the performance metrics for Scenario II reported on Table \ref{tab:avg-prec-table} increase their values with respect to Scenario I. 

%\modifica{inserire tabella precisioni e vedere di quanto è migliorata e come potrebbe aver influito nell'interpretazione}

\begin{comment}
\begin{table}[ht]
\parbox{.45\linewidth}{
\centering
\begin{tabular}{|c|ccc|}
\hline
\multicolumn{4}{|c|}{\textbf{pendigits} inlier training} \\ 
\hline
\textbf{Metric} & \textbf{IF} & \textbf{EIF} & 
\textbf{EIF+} \\ \hline
Precision         & 0.42 & 0.39 & 0.51 \\
Recall            & 0.42 & 0.39 & 0.51 \\
f1 score          & 0.42 & 0.39 & 0.51 \\
Accuracy          & 0.97 & 0.97 & 0.98 \\

Average Precision & 0.36 & 0.30 & 0.44 \\
ROC AUC Score     & 0.97 & 0.96 & 0.97 \\ \hline
\end{tabular}
\caption{Performance Report \texttt{pendigits} Dataset}
\label{tab:pendigits-perf-split}
}
\end{table}
\end{comment}

\begin{figure}
  \centering
  \includegraphics[width=0.7\linewidth]{figures/feature_selection_plots_final/featsel_pendigits_final.pdf}
  \caption{Feature Selection Plot {\ttfamily Pendigits}}
  \label{fig:fs-pendigits-plus}
\end{figure}\hfil % <-- added

In the Feature Selection Plot, in Figure \ref{fig:fs-diabetes-plus}, ExIFFI-plus-split is almost always the best Feature Ranking Algorithm. In particular, its Average Precision is much higher than all the other models in the range between 10 and 4 features. ExIFFI has a significant drop going from 7 to 6 features. The other algorithms considered, on the other hand, are associated with more or less constant Average Precision values with the exception of DIFFI (i.e. the brown line) which shows signs of improvements from 5 features onwards. 

%\todo[inline, color=red]{Questo penso che possa andare in appendice, se nessuno ha niente in contrario (Chiara)}


%\davide{

%The instruments to exploit in order to conduct an interpretability analysis of the {\ttfamily Pendigits} dataset, described in details in Section \ref{sec:real-world-data}, are provided in Figure \ref{fig:pendigits}. 

%As it can be observed by analyzing the Global Feature Importance Bar Plot and the Feature Importance Score Plot, depicted in Figure \ref{fig:GFI-pendigits} and \ref{fig:Feat-imp-pendigits} respectively, features 3 and 5 can be found in the top 2 ranking in more than half of the model instances considered. These attributes also appear as the ones with the two highest Average Feature Importance Scores. As a conclusion, it is possible to assert that the importance in the {\ttfamily Pendigits} dataset is shared between Feature 3 and 5.

%Feature 3 and 5 were compared on the Local Importance Scoremap represented in \ref{fig:Local-pendigits}. After a detailed inspection, a set of inliers aligned along Feature 3 can be highlighted together with another set of anomalies scattered along an oblique line which is parallel to the bisector line of the subspace created by the two attributes under analysis. Finally, a small cluster of inliers separated from the main cluster (i.e. \textit{model anomalies}) can be noted in the left region of the plot. Also, these points are placed along an oblique direction contributing to the importance of both Features 3 and 5. 

%}

%\davide {
%In a similar way to the {\ttfamily Pima} dataset the shared importance between a pair of features hinders the detection capabilities of the considered models also on the {\ttfamily Pendigits} dataset. The F1 Score values are almost equal across the three models while EIF+ outperforms the other two on the Average Precision metrics probably because of its high Recall value of 0.92. 
%}


==> sections/sections_world_dataset_results/pendigits_new.tex <==
\subsection*{{\ttfamily Pendigits}}

\subsubsection{Performance}

\ale{Figure \ref{fig:Pendigits_contamination_full} represents the trend of the Average Precision metrics as anomalies are gradually inserted into the train process of the five Anomaly Detection models used for experimental evaluation. The models presenting the higher precision values in presence of only inliers in the training set (i.e. Scenario II) are DIF, IF and the proposed \EIFplus, whose performances drop as the number of outliers increases and saturate to reach similar values as the other models. For what concerns the comparison between EIF and its improved version, introduced in this study, \EIFplus , depicted in Figure \ref{fig:Pendigits_contaminationEIFvsEIF+}, it is possible to notice how \EIFplus shows better performances than EIF when the number of outliers considers for training is limited and the two models tend to become closer in terms of performances as the contamination factor increases. This behavior is a direct consequence of how the \EIFplus approach is build to optimize the generalizability capabilities of the EIF model.} 

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.49\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Pendigits/Contamination/22-03-2024_15-41-59_pendigits_contamination_full_plot.pdf}
      \caption{Models evaluation, varying the contamination levels}
      \label{fig:Pendigits_contamination_full}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.44\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Pendigits/Contamination/22-03-2024_15-52-17_pendigits_EIF+_minus_EIF_precision_over_contamination.pdf}
      \caption{Difference between \EIFplus and EIF average precision}
      \label{fig:Pendigits_contaminationEIFvsEIF+}
    \end{subfigure}\hfil % <-- added
\caption{Figure \ref{fig:Pendigits_contamination_full} illustrates the average precision as the contamination level in the training set increases. Figure \ref{fig:Pendigits_contaminationEIFvsEIF+} compares the performance graphs of EIF and \EIFplus, using the difference of their scores in various contamination levels.}
\label{fig:Pendigits_contamination}
\end{figure}

Table \ref{tab:Pendigits_perf}  reports a detailed evaluation of the performances of the AD models compared in the Contamination plot, focusing on the comparison between the Scenario I and Scenario II training approaches. The three models highligthed in Figure \ref{fig:Pendigits_contamination_full} (i.e. IF, DIF and \EIFplus) are the unique ones where a significant difference can be noticed switching from Scenario I to Scenario II. The best model in terms of Average Precision is DIF but, at the same time, it is associated with dramatically high computational time, in terms of fit and predict, with the respect to the isolation-based AD models making its usage not ideal, mainly in real world applications. As a consequence \EIFplus can be considered as the optimal choice for the {\ttfamily Pendigits} dataset.

\begin{table}[htbp]
\begin{minipage}[t]{0.46\textwidth}
\strut\vspace*{-\baselineskip}\newline
\resizebox{\textwidth}{!}{
\begin{tabular}{|c||ccc|ccc||cc|}
\toprule
\hline
&\multicolumn{3}{c|}{Scenario I}&\multicolumn{3}{c||}{Scenario II}&\multicolumn{2}{c|}{Time}\\
\hline
AD Model & Avg & Prec & ROC & Avg & Prec & ROC & fit & pred \\
& Prec &  & AUC & Prec &  & AUC &  &  \\
\hline
IF          & 0.28& 0.31& 0.64& 0.37& 0.42& 0.7& \textbf{0.07}& \textbf{0.03}\\
EIF         & 0.23& 0.24 & 0.61& 0.27& 0.36& 0.67& 0.07& 0.44\\
EIF+        & 0.21& 0.41& \textbf{0.69}& 0.36& 0.45& 0.72& 0.07& 0.45\\
DIF         & \textbf{0.34}& \textbf{0.39}& 0.68& \textbf{0.46}& \textbf{0.53}& \textbf{0.76}& 10.2& 8.36\\
AE & 0.22& 0.33& 0.65& 0.24& 0.33& 0.66& 19.0& 0.32  \\
\hline
\end{tabular}}
\vspace{0.41cm}
\caption{Performances of 5 different Anomaly Detection models over {\ttfamily Pendigits} are compared using classical Classification metrics. Moreover, the last two columns contain the average time for a fit and predict operation. The highest metric values and the lowest execution times are highlighted in bold}\label{tab:Pendigits_perf}
\end{minipage}
\hfill
\begin{minipage}[t]{0.46\textwidth}
\strut\vspace*{-\baselineskip}\newline
\resizebox{\textwidth}{!}{
\begin{tabular}{|c||c|c|c|c||c|}
\toprule
\hline
&\multicolumn{2}{c|}{Evaluation with EIF}&\multicolumn{2}{c||}{Evaluation with \EIFplus}&\\
\hline
& Scenario I & Scenario II & Scenario I & Scenario II & Time\\

 Algorithm & $AUC_{FS}$  & $AUC_{FS}$ & $AUC_{FS}$  & $AUC_{FS}$ &  \\
\hline
DIFFI               & 0.118& -0.384& 0.233& -0.766& 0.37\\
IF\_\approach        & \textbf{2.198}& \textbf{2.688}& \textbf{2.172}& \textbf{3.187}& 1.13\\
EIF\_\approach       & 1.588& 1.887& 1.767& 2.232& 1.25\\
EIF+\_\approach      & 1.868& 1.227& 1.921& 1.326& 1.22\\
IF\_RF              & 1.484& 1.281& 1.377& 1.380& 8.90\\
EIF\_RF             & -0.728& -0.842& -0.368& -1.287& 8.90\\
EIF+\_RF            & -1.402& -0.249& -0.971& -0.748& 8.90\\
\hline
\end{tabular}}
\caption{Quantitative evaluation of the effectiveness of 6 different interpretation algorithms on {\ttfamily Pendigits} through the $AUC_{FS}$ metric, introduced in \ref{sec:interpr_evaluat}. In the last column the average time taken by the different models to produce the importance scores is reported. The highest $AUC_{FS}$ and lowest Importance time values are highlighted in bold.}\label{tab:fs-tab-Pendigits}
\end{minipage}
\end{table}


\subsubsection{Importance Plots} \label{sec:Pendigits-imp-plots}

\ale{Similarly to what can be observed in the {\ttfamily Ionosphere} dataset, Figure \ref{fig:interpretation-Pendigits} portraits how it is challenging to identify a single dominant feature in terms of importance. As a consequence it can be concluded the probably there is a small group of features along which anomalies are distributed. Observing the Score Plots (Figures \ref{fig:Feat-imp-Pendigits}, \ref{fig:Feat-imp-Pendigits-split}) and the Bar Plots (Figures \ref{fig:GFI-Pendigits}, \ref{fig:GFI-Pendigits-split}) it can be noticed how Features 1, 3 and 5 appear in the top 3 ranking in both Scenario I and Scenario II and thus may be the variables composing the aforementioned group of important features.} 

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Pendigits/Importance_plots/02-03-2024_16-26-11_GFI_Bar_plot_pendigits_EXIFFI+_1.pdf}
      \caption{Bar Plot {\ttfamily Pendigits} Scenario I}
      \label{fig:GFI-Pendigits}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.27\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Pendigits/Importance_plots/02-03-2024_16-26-12_GFI_Score_plot_pendigits_EXIFFI+_1.pdf}
      \caption{Score Plot {\ttfamily Pendigits} Scenario I}
      \label{fig:Feat-imp-Pendigits}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Pendigits/Local_Scoremaps/22-03-2024_15-38-37_importance_map_pendigits_EXIFFI+_1_feat_3_1.pdf}
      \caption{Scoremap {\ttfamily Pendigits} Scenario I}
      \label{fig:Local-Pendigits}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Pendigits/Importance_plots/02-03-2024_15-03-21_GFI_Bar_plot_pendigits_EXIFFI+_2.pdf}
      \caption{Bar Plot {\ttfamily Pendigits} Scenario II}
      \label{fig:GFI-Pendigits-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.27\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Pendigits/Importance_plots/02-03-2024_15-03-22_GFI_Score_plot_pendigits_EXIFFI+_2.pdf}
      \caption{Score Plot {\ttfamily Pendigits} Scenario II}
      \label{fig:Feat-imp-Pendigits-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Pendigits/Local_Scoremaps/22-03-2024_15-38-24_importance_map_pendigits_EXIFFI+_2_feat_3_1.pdf}
      \caption{Scoremap {\ttfamily Pendigits} Scenario II}
      \label{fig:Local-Pendigits-split}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot and Scoremap for {\ttfamily Pendigits} in the two different Scenarios, using the \approach algorithm applied to the \EIFplus model.}\label{fig:interpretation-Pendigits}
\end{figure}

\subsubsection{Feature Selection}

\ale{A confirmation of the conclusions reached from the analysis conducted in \ref{sec:Pendigits-imp-plots} can be achieved looking at the Feature Selection plots organized in Figure \ref{fig:fs-interpretation-Pendigits}. In particular in Figure \ref{fig:Feat-Sel_Pendigits_valEIF+_EXIFFI+_2}  it is possible to highlight how the Average Precision gradually decreases reducing the number of input features from 3 to 1, meaning that dropping one of features 1,3 or 5 the model loses crucial information for the detection of anomalous points and thus its detecting performance experience a considerable drop. Notably the only model whose explanations are associated to a Feature Selection plot where the red curve is always placed above the blue one is the IF model as depicted in Figures \ref{fig:Feat-Sel_Pendigits_valEIF+_DIFFI_2} and \ref{fig:Feat-Sel_Pendigits_valEIF+_IF_RandomForest_2}.}

\begin{figure}[!ht] 
\centering
\hspace{0.05\textwidth}\textbf{IF} \hspace{0.29\textwidth} \textbf{EIF} \hspace{0.29\textwidth} \textbf{EIF+}
% First row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Ad-Hoc}}} % Adjust the parbox width as necessary for your caption text
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Pendigits/Feature_Selection/07-05-2024_15-57-13_pendigits_EIF+_IF_EXIFFI_feature_selection_2.pdf}
            \caption{\approach applied to IF}
            \label{fig:Feat-Sel_Pendigits_valEIF+_DIFFI_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Pendigits/Feature_Selection/22-03-2024_16-23-48_pendigits_EIF+_EXIFFI_feature_selection_2.pdf}
            \caption{\approach applied to EIF}
            \label{fig:Feat-Sel_Pendigits_valEIF+_EXIFFI_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Pendigits/Feature_Selection/22-03-2024_16-23-48_pendigits_EIF+_EXIFFI+_feature_selection_2.pdf}
            \caption{\approach applied to \EIFplus}
            \label{fig:Feat-Sel_Pendigits_valEIF+_EXIFFI+_2}
        \end{subfigure}
    \end{minipage}
\end{minipage}

\vspace{5mm} % Space between rows

% Second row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Post-Hoc}}} % Adjust as necessary
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Pendigits/Feature_Selection/22-03-2024_16-23-48_pendigits_EIF+_IF_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to IF}
            \label{fig:Feat-Sel_Pendigits_valEIF+_IF_RandomForest_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Pendigits/Feature_Selection/22-03-2024_16-23-49_pendigits_EIF+_EIF_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to EIF}
            \label{fig:Feat-Sel_Pendigits_valEIF+_EIF_RandomForest_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Pendigits/Feature_Selection/22-03-2024_16-23-48_pendigits_EIF+_EXIFFI+_feature_selection_2.pdf}
            \caption{RandomForest fitted to \EIFplus}
            \label{fig:Feat-Sel_Pendigits_valEIF+_EIF+_RandomForest_2}
        \end{subfigure}
    \end{minipage}
\end{minipage}

\caption{Feature Selection of the different Ad-Hoc and Post-Hoc methods applied to the 3 Isolation Forest models: IF, EIF and \EIFplus. The blue line is the values of average precision, calculated with the \EIFplus model in the Scenario II, dropping the most important feature at each step, the red line is the values of average precision dropping the least important feature at each step and the green line is the value of the feature selection dropping a random feature at each step.}\label{fig:fs-interpretation-Pendigits}
\end{figure}

\ale{To conclude the experimental evaluation of the {\ttfamily Pendigits} dataset it is possible to analyse Table \ref{tab:fs-tab-Pendigits}, where a quantitative analysis of the effectiveness of the different interpretation methods proposed is presented. The model that correctly captures the ranking of features according to their relevance is IF\_\approach, followed by \approach+ as it is testified by the high values of the $AUC_{FS}$ metric. On the other hand explanations based on DIFFI and post-hoc methods using Random Forest as a surrogate model prove to wrongly interpret the importance of features and are consequently associated to negative values of $AUC_{FS}$. Finally it is also worth noticing how the interpretation methods deriving from Isolation-based AD methods (i.e. IF\_\approach, \approach and \approach+) showcase much more efficient time performances in the computation of the importance scores with the respect to the post-hoc methods.}  






==> sections/sections_world_dataset_results/pima.tex <==
\subsubsection{{\ttfamily Pima}}

The {\ttfamily Pima} dataset comes from the National Institute of Diabetes, Digestive and Kidney Diseases. As it happens in the {\ttfamily Diabetes} dataset the task at hand is one of identifying whether a patient has diabetes or not. The dataset contains eightfeatures and its details are contained in Appendix \ref{sec:real-world-data}.

%\modifica{mettere risultati importances nel caso in cui è allenata interamente sul dataset di pima}

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/pima/Feat_bar_plot_pima.pdf}
      \caption{Score Plot \texttt{Pima} Scenario I}
      \label{fig:Feat-imp-pima}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/pima/Feat_bar_plot_pima_split.pdf}
      \caption{Score Plot \texttt{Pima} Scenario II}
      \label{fig:Feat-imp-pima-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/pima/GFI_pima_synt.pdf}
      \caption{Bar Plot \texttt{Pima} Scenario I}
      \label{fig:GFI-pima}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/pima/GFI_pima_split_synt.pdf}
      \caption{Bar Plot \texttt{Pima} Scenario II}
      \label{fig:GFI-pima-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/scoremaps_real_world/Local_Scoremap_Plot_pima.png}
      \caption{Scoremap \texttt{Pima} Scenario I}
      \label{fig:Local-pima}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/scoremaps_real_world/Local_Scoremap_Plot_pima_split.png}
      \caption{Scoremap \texttt{Pima} Scenario II}
      \label{fig:Local-pima-split}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot and Scoremap for \texttt{Pima}}
\label{fig:interpretation-pima}
\end{figure}

Figure \ref{fig:GFI-pima} shows the Bar Plot for the {\ttfamily Pima} dataset from which it is possible to conclude that there is a shared importance between Feature 2 and 5. These two attributes are consistently placed in the top 2 rankings both in Figure \ref{fig:GFI-pima} and in Figure \ref{fig:Feat-imp-pima}. However, there is not an evident margin in their average importance scores to consider them as two dominant features over the entire dataset. 

The Scoremap, depicted in Figure \ref{fig:Local-pima}, shows how the two main clusters of inliers and outliers almost perfectly overlap one over the other. Moreover looking at the contour lines also the Anomaly Scores associated to these two groups of points should be similar. Notably, it is also possible to appreciate the presence of two smaller groups of points, isolated from the two main sets, distributed along both Feature 1 and Feature 5 containing both inliers and outliers. 

The Average Precision values, contained in Table \ref{tab:avg-prec-table}, presents almost equal levels across all the three models considered. 

%\modifica{mettere tabella precisioni allenato su tutto}

\begin{comment}    
\begin{table}[ht]
\parbox{.45\linewidth}{
\centering
\begin{tabular}{|c|ccc|}
\hline
\multicolumn{4}{|c|}{\textbf{pima} complete training} \\ \hline
\textbf{Metric} & \textbf{IF} & \textbf{EIF} & \textbf{EIF+} \\ \hline
Precision         & 0.51 & 0.51 & 0.51 \\
Recall            & 0.51 & 0.51 & 0.51 \\
f1 score          & 0.51 & 0.51 & 0.51 \\
Accuracy          & 0.66 & 0.66 & 0.66 \\

Average Precision & 0.51 & 0.49 & 0.49 \\
ROC AUC Score     & 0.68 & 0.68 & 0.67 \\ \hline
\end{tabular}
\caption{Performance Report \texttt{Pima} Dataset}
\label{tab:pima-perf-complete}}
\end{table}
\end{comment}

In the following the results obtained after the application of the Scenario II approach to the {\ttfamily Pima} dataset are shown. 

%\modifica{far vedere nel caso in cui si splitta il training per capire se va meglio}

The Bar Plot (Figure \ref{fig:GFI-pima-split}) is associated with a higher degree of uncertainty in detecting the most decisive features. In fact, as it can also be noticed from an analysis of the Score Plot in Figure \ref{fig:Feat-imp-pima-split}, in this case, the number of features among which the importance is shared is three: Feature 5,1 and 4. 

Moreover, the Scoremap reports also in this case the peculiar situation in which the main cluster of anomalies is overlapped with the cluster representing the normal points distribution. In this case, however, some changes can be observed in the positions of the contour lines which make it easier to separate inliers from outliers. In fact, the Average Precisions reported in Table \ref{tab:avg-prec-table} display a significant increase across all three models that continue to possess very close values. 

%\modifica{inserire tabella precisioni e vedere di quanto è migliorata e come potrebbe aver influito nell'interpretazione}

\begin{comment}
\begin{table}[ht]
\parbox{.45\linewidth}{
\centering
\begin{tabular}{|c|ccc|}
\hline
\multicolumn{4}{|c|}{\textbf{pima} inlier training} \\ 
\hline
\textbf{Metric} & \textbf{IF} & \textbf{EIF} & 
\textbf{EIF+} \\ \hline
Precision         & 0.59 & 0.57 & 0.58 \\
Recall            & 0.59 & 0.57 & 0.58 \\
f1 score          & 0.59 & 0.57 & 0.58 \\
Accuracy          & 0.72 & 0.70 & 0.71 \\

Average Precision & 0.58 & 0.55 & 0.59 \\
ROC AUC Score     & 0.74 & 0.74 & 0.75 \\ \hline
\end{tabular}
\caption{Performance Report \texttt{pima} Dataset}
\label{tab:pima-perf-split}
}
\end{table}
\end{comment}

\begin{figure}
  \centering
  \includegraphics[width=0.7\linewidth]{figures/feature_selection_plots_final/featsel_pima_final.pdf}
  \caption{Feature Selection Plot {\ttfamily Pima}}
  \label{fig:fs-pima-plus}
\end{figure}\hfil % <-- added

The results of the application of Unsupervised Feature Selection to the {\ttfamily Pima} dataset are reported in Figure \ref{fig:fs-pima-plus}. The outcomes are considerably unique with respect to the other datasets. In fact, all the Feature Ranking Algorithms show Average Precision values that tend to decrease as features are removed from the input space. A slight increase in performance can be observed in ExIFFI-plus-split passing from 3 to 2 features to, however, end with a decrease in the next step (i.e. in the passage from 2 to 1 feature). A peculiar situation can instead be observed for the Random Forest model where the Average Precision presents a huge increase in the passage from 2 to 1 feature obtaining a value surpassing by far the ones of all the other ranking approaches considered in this analysis. 
These uncertain behaviors certify the difficulty in the application of the Anomaly Detection task to the {\ttfamily Pima} dataset.

%\todo[inline, color=red]{Questo penso che possa andare in appendice, se nessuno ha niente in contrario (Chiara)}


%\davide{
% All the models show some sort of "zig-zagging" behavior. In particular, Random Forest has a peak in precision going from 2 to 1 feature. E-IFFI-plus has a similar more or less constant precision until and starts to increase when the number of features becomes 4 but it ends with a drop passing from 2 to 1 feature.  
%}

%\davide{

%The plots reporting the results obtained after the application of the \approach model to the {\ttfamily Pima} dataset, illustrated in Section \ref{sec:real-world-data}, can be found in Figure \ref{fig:pima}. 

%From a careful observation of the Feature Importance Score Plot, depicted in Figure \ref{fig:Feat-imp-pima}, the {\ttfamily Pima} there is characterized by shared importance between Feature 2 and 5 (corresponding respectively to Diastolic Blood Pressure and to BMI) which have very similar Average Importance Scores and were placed in the top two rankings of the Global Feature Importance Bar Plot in multiple executions as it can be noticed in Figure \ref{fig:GFI-pima}. 

%Analyzing the Local Importance Scoremap, illustrated in Figure \ref{fig:Local-pima}, it is possible to notice that almost all the inliers are overlapped with the inliers in the main cluster of points. However, there is a significant number of \textit{model anomalies} almost perfectly aligned along both Feature 2 and 5 together with some outliers. This peculiar point distribution confirms the shared importance between the Features representing Diastolic Blood Pressure and BMI which are indeed two key factors in determining the presence or absence of diabetes in a patient. 

%}

%\davide {
%In the {\ttfamily Pima} dataset the Anomaly Detection task is slightly more challenging because of the shared Feature Importance between Feature 2 and 5. This is reflected in Table \ref{tab:pima-perf} where the Performance metric's values are lower than the ones of other datasets described in this section. In particular, the f1 Scores obtained by the IF, EIF and EIF+ models are very similar one to the other. On the other hand, the EIF+ model outperforms the other two in terms of Average Precision where a margin of over 30\% can be noticed. 
%}


==> sections/sections_world_dataset_results/pima_new.tex <==
\subsection*{{\ttfamily Pima}}

\subsubsection{Performance} \label{sec:Pima-Contamination-sec}

\ale{The Contamination plot for the {\ttfamily Pima} dataset is reported in Figure \ref{fig:Pima_contamination_full}. It depicts how the Average Precision metric of the AD models considered is not affected by the amount of outliers included in the training set. The Isolation-based models (i.e. IF, EIF and \EIFplus) emerge as the ones with the better performances, though the margin on the deep learning based methods (i.e. DIF and Autoencoder) is minimal.}

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.49\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Pima/Contamination/21-03-2024_17-08-59_pima_contamination_full_plot.pdf}
      \caption{Models evaluation, varying the contamination levels}
      \label{fig:Pima_contamination_full}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.44\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Pima/Contamination/21-03-2024_17-10-14_pima_EIF+_minus_EIF_precision_over_contamination.pdf}
      \caption{Difference between \EIFplus and EIF average precision}
      \label{fig:Pima_contaminationEIFvsEIF+}
    \end{subfigure}\hfil % <-- added
\caption{Figure \ref{fig:Pima_contamination_full} illustrates the average precision as the contamination level in the training set increases. Figure \ref{fig:Pima_contaminationEIFvsEIF+} compares the performance graphs of EIF and \EIFplus, using the difference of their scores in various contamination levels.}
\label{fig:Pima_contamination}
\end{figure}

\ale{Table \ref{tab:Pima_perf} includes additional metrics other than Average Precision and focuses on the cases in which the training set's contamination is null (i.e. Scenario II) and equal to the total number of outliers in the dataset (i.e. Scenario I). As already described in \ref{sec:Pima-Contamination-sec} the difference between the two previously depicted scenarios is minimal and the proposed \EIFplus once again proves to be the optimal model also on the {\ttfamily Pima} dataset.}

\begin{table}[htbp]
\begin{minipage}[t]{0.46\textwidth}
\strut\vspace*{-\baselineskip}\newline
\resizebox{\textwidth}{!}{
\begin{tabular}{|c||ccc|ccc||cc|}
\toprule
\hline
&\multicolumn{3}{c|}{Scenario I}&\multicolumn{3}{c||}{Scenario II}&\multicolumn{2}{c|}{Time}\\
\hline
AD Model & Avg & Prec & ROC & Avg & Prec & ROC & fit & pred \\
& Prec &  & AUC & Prec &  & AUC &  &  \\
\hline
IF          & \textbf{0.51}& \textbf{0.52}& \textbf{0.63}& 0.58& 0.55& 0.66& 0.11& \textbf{0.008}\\
EIF         & 0.49& 0.49& 0.61& 0.54& 0.57& 0.67& \textbf{0.07}& 0.03\\
EIF+        & 0.49& 0.5& 0.61 & \textbf{0.58}& \textbf{0.57}& \textbf{0.67}& 0.08& 0.03\\
DIF         & 0.41& 0.41& 0.54& 0.49& 0.46& 0.59& 1.17& 1.00\\
AE & 0.43& 0.44& 0.57& 0.5& 0.54& 0.64& 3.11& 0.06\\
\hline
\end{tabular}}
\vspace{0.41cm}
\caption{Performances of 5 different Anomaly Detection models over {\ttfamily Pima} are compared using classical Classification metrics. Moreover, the last two columns contain the average time for a fit and predict operation. The highest metric values and the lowest execution times are highlighted in bold}\label{tab:Pima_perf}
\end{minipage}
\hfill
\begin{minipage}[t]{0.46\textwidth}
\strut\vspace*{-\baselineskip}\newline
\resizebox{\textwidth}{!}{
\begin{tabular}{|c||c|c|c|c||c|}
\toprule
\hline
&\multicolumn{2}{c|}{Evaluation with EIF}&\multicolumn{2}{c||}{Evaluation with \EIFplus}&\\
\hline
& Scenario I & Scenario II & Scenario I & Scenario II & Time\\

 Algorithm & $AUC_{FS}$  & $AUC_{FS}$ & $AUC_{FS}$  & $AUC_{FS}$ &  \\
\hline
DIFFI                    & -0.489& 0.256& -0.497& 0.303& 0.57 \\
IF\_\approach             & -0.310& \textbf{0.373}& \textbf{-0.237}& \textbf{0.367}& 0.14\\
EIF\_\approach            & -0.316& -0.214& -0.324& -0.201& \textbf{0.07}\\
\EIFplus\_\approach       & -0.309& -0.037& -0.272& -0.020& 0.06\\
IF\_RF                   & -0.369& 0.191& -0.301& 0.218& 0.43\\
EIF\_RF                  & -0.443& 0.127& -0.416& 0.178& 0.43\\
EIF+\_RF                 & \textbf{-0.288}& 0.063& -0.286& 0.149& 0.43\\
\hline
\end{tabular}
}
\caption{Quantitative evaluation of the effectiveness of 6 different interpretation algorithms on {\ttfamily Pima} through the $AUC_{FS}$ metric, introduced in \ref{sec:interpr_evaluat}. In the last column the average time taken by the different models to produce the importance scores is reported. The highest $AUC_{FS}$ and lowest Importance time values are highlighted in bold.}\label{tab:fs-tab-Pima}
\end{minipage}
\end{table}


\subsubsection{Importance Plots}

\ale{In Figure \ref{fig:interpretation-Pima} the outcomes produced by the \approach+ model in interpreting the \EIFplus model are reported. Prior to commenting the feature ranking produced by the Score and Bar Plots it is crucial to notice how the outliers are overlapped with the normal points in the {\ttfamily Pima} dataset as it can be realized looking at the Local scoremaps contained in Figures \ref{fig:Local-Pima} and \ref{fig:Local-Pima-split}. This observation is explanatory for the peculiar phenomenon encountered in the Contamination plot, in fact since outliers are mostly overlapped to normal points including them or not into the training set will not affect the Average Precision metric.}

\ale{The superimposition of anomalies and normal observations is verified because, as described in \ref{sec:real-dataset-experiments}, the real world benchmark datasets normally used in the literature to assess the performances of Anomaly Detection models are nothing more than an adaptation of Binary or Multi Class Classification datasets to the task of identifying outliers. As a consequence the data points that are labeled as anomalous (i.e. the data samples beholding to the least represented class) in some cases may not truly deviate from the inliers distributions as they should as anomalous points. As a consequence AD models based on the concept of isolating anomalies from inliers (such as \EIFplus) may not be effective to solve the Anomaly Detection task on this dataset and the interpretations furnished by \approach+ may be misleading and not aligned with the ground truth. 
In any case, according to the Score Plots produced (and represented in Figure \ref{fig:Feat-imp-Pima} and \ref{fig:Feat-imp-Pima-split}) the most important features, both in Scenario I and Scenatio II, are \textit{BloodPressure, BMI} and \textit{Insulin}.}

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Pima/Importance_plots/02-03-2024_16-20-45_GFI_Bar_plot_pima_EXIFFI+_1.pdf}
      \caption{Bar Plot {\ttfamily Pima} Scenario I}
      \label{fig:GFI-Pima}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.27\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Pima/Importance_plots/02-03-2024_16-20-46_GFI_Score_plot_pima_EXIFFI+_1.pdf}
      \caption{Score Plot {\ttfamily Pima} Scenario I}
      \label{fig:Feat-imp-Pima}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Pima/Local_Scoremaps/21-03-2024_17-26-34_importance_map_pima_EXIFFI+_1_feat_5_1.pdf}
      \caption{Scoremap {\ttfamily Pima} Scenario I}
      \label{fig:Local-Pima}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Pima/Importance_plots/02-03-2024_14-44-44_GFI_Bar_plot_pima_EXIFFI+_2.pdf}
      \caption{Bar Plot {\ttfamily Pima} Scenario II}
      \label{fig:GFI-Pima-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.27\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Pima/Importance_plots/02-03-2024_14-44-44_GFI_Score_plot_pima_EXIFFI+_2.pdf}
      \caption{Score Plot {\ttfamily Pima} Scenario II}
      \label{fig:Feat-imp-Pima-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Pima/Local_Scoremaps/21-03-2024_17-26-25_importance_map_pima_EXIFFI+_2_feat_5_1.pdf}
      \caption{Scoremap {\ttfamily Pima} Scenario II}
      \label{fig:Local-Pima-split}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot and Scoremap for {\ttfamily Pima} in the two different Scenarios, using the \approach algorithm applied to the \EIFplus model.}\label{fig:interpretation-Pima}
\end{figure}

\subsubsection{Feature Selection}

\ale{As a consequence of the peculiar distribution of anomalies in the {\ttfamily Pima} dataset, the results produced by the application of the Unsupervised Feature Selection proxy task (Figure \ref{fig:interpretation-Pima} do not show interesting shapes since in most of the cases the Average Precision stays more or less constant, both in the red and blue line, across all the different subset of features considered. A possible exception to this behavior is represented by the IF\_\approach interpretation approach, presented in Figure \ref{fig:Feat-Sel_Pima_valEIF+_DIFFI_2}, which shows a slight advantage in omitting features in increasing order of importance (i.e. red line) with the respect to the decreasing order (i.e. blue line), however it is not as significant as in other datasets.}
 
\begin{figure}[!ht] 
\centering
\hspace{0.05\textwidth}\textbf{IF} \hspace{0.29\textwidth} \textbf{EIF} \hspace{0.29\textwidth} \textbf{EIF+}
% First row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Ad-Hoc}}} % Adjust the parbox width as necessary for your caption text
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Pima/Feature_Selection/07-05-2024_16-16-26_pima_EIF+_IF_EXIFFI_feature_selection_2.pdf}
            \caption{\approach applied to IF}
            \label{fig:Feat-Sel_Pima_valEIF+_DIFFI_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Pima/Feature_Selection/21-03-2024_17-30-36_pima_EIF+_EXIFFI_feature_selection_2.pdf}
            \caption{\approach applied to EIF}
            \label{fig:Feat-Sel_Pima_valEIF+_EXIFFI_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Pima/Feature_Selection/21-03-2024_17-30-13_pima_EIF+_EXIFFI+_feature_selection_2.pdf}
            \caption{\approach applied to \EIFplus}
            \label{fig:Feat-Sel_Pima_valEIF+_EXIFFI+_2}
        \end{subfigure}
    \end{minipage}
\end{minipage}

\vspace{5mm} % Space between rows

% Second row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Post-Hoc}}} % Adjust as necessary
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Pima/Feature_Selection/21-03-2024_17-32-12_pima_EIF+_IF_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to IF}
            \label{fig:Feat-Sel_Pima_valEIF+_IF_RandomForest_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Pima/Feature_Selection/21-03-2024_17-31-47_pima_EIF+_EIF_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to EIF}
            \label{fig:Feat-Sel_Pima_valEIF+_EIF_RandomForest_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Pima/Feature_Selection/21-03-2024_17-31-24_pima_EIF+_EIF+_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to \EIFplus}
            \label{fig:Feat-Sel_Pima_valEIF+_EIF+_RandomForest_2}
        \end{subfigure}
    \end{minipage}
\end{minipage}

\caption{Feature Selection of the different Ad-Hoc and Post-Hoc methods applied to the 3 Isolation Forest models: IF, EIF and \EIFplus. The blue line is the values of average precision, calculated with the \EIFplus model in the Scenario II, dropping the most important feature at each step, the red line is the values of average precision dropping the least important feature at each step and the green line is the value of the feature selection dropping a random feature at each step.}\label{fig:fs-interpretaion-Pima}
\end{figure}

\ale{The values of the $AUC_{FS}$ metric are grouped together in Table \ref{tab:fs-tab-Pima}. As previously explained the best interpretation method in quantitative terms is IF\_\approach although not presenting significant values of the metric. For what concerns the remaining approaches considered their scores are mostly close to zero or negative, as a consequence of the flat shapes observed in the Feature Selection plots.}



==> sections/sections_world_dataset_results/shuttle.tex <==
\subsubsection*{{\ttfamily Shuttle}}

The {\ttfamily Shuttle} dataset is composed by nine attributes describing the radiator positions in a NASA space shuttle. The original task associated to this dataset is a 7-class classification. The name of the classes' labels and other details about the {\ttfamily Shuttle} dataset are contained in Appendix \ref{sec:real-world-data}. 

%\modifica{mettere risultati importances nel caso in cui è allenata interamente sul dataset di shuttle}

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/shuttle/Feat_bar_plot_shuttle.pdf}
      \caption{Score Plot \texttt{Shuttle} Scenario I}
      \label{fig:Feat-imp-shuttle}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/shuttle/Feat_bar_plot_shuttle_split.pdf}
      \caption{Score Plot \texttt{Shuttle} Scenario II}
      \label{fig:Feat-imp-shuttle-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/shuttle/GFI_shuttle_synt.pdf}
      \caption{Bar Plot \texttt{Shuttle} Scenario I}
      \label{fig:GFI-shuttle}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/shuttle/GFI_shuttle_split_synt.pdf}
      \caption{Bar Plot \texttt{Shuttle} Scenario II}
      \label{fig:GFI-shuttle-split}
    \end{subfigure}\hfil % <-- added    
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/scoremaps_real_world/Local_Scoremap_Plot_shuttle.png}
      \caption{Scoremap \texttt{Shuttle} Scenario I}
      \label{fig:Local-shuttle}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/scoremaps_real_world/Local_Scoremap_Plot_shuttle_split.png}
      \caption{Scoremap \texttt{Shuttle} Scenario II}
      \label{fig:Local-shuttle-split}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot and Scoremap for \texttt{Shuttle}}
\label{fig:interpretation-shuttle}
\end{figure}

The outcomes of the Feature Importance analysis for the {\ttfamily Shuttle} dataset are reported in Figure \ref{fig:interpretation-shuttle}. In particular, Figure \ref{fig:GFI-shuttle} displays the Bar Plot which highlights Feature 3 as one of the most decisive for the detection of anomalies since it was ranked in the top position in 70\% of the model execution performed. Figure \ref{fig:Feat-imp-shuttle} depicts, instead, the Score Plot where it is possible to notice that another relevant feature is Feature 0 which has a similar average importance score to the one of Feature 3. However, the remaining features also possess similar scores thus it is possible to conclude that the model is not extremely reliable in isolating a group of features significantly more important than the rest. 

In Figure \ref{fig:Local-shuttle} the Scoremap is reported showing how there are two main groups of outliers clearly scattered along Feature 0, not along Feature 3 as one should expect considering the results derived from Figure \ref{fig:GFI-shuttle} and \ref{fig:Feat-imp-shuttle}. 

However, the clear spatial separation between inliers and outliers and the position of the Anomaly Score contour lines help the model in easily distinguish between the two classes. In fact the Average Precision values reported in Table \ref{tab:avg-prec-table} for the {\ttfamily Shuttle} dataset are excellent, making it as one of the datasets with the best performances in this study. 


%\modifica{mettere tabella precisioni allenato su tutto}

In order to obtain clearer results in the explainability and performance reports the Scenario II approach was exploited. 

\begin{comment}
\begin{table}[ht]
\parbox{.45\linewidth}{
\centering
\begin{tabular}{|c|ccc|}
\hline
\multicolumn{4}{|c|}{\textbf{shuttle} complete training} \\ \hline
\textbf{Metric} & \textbf{IF} & \textbf{EIF} & \textbf{EIF+} \\ \hline
Precision         & 0.97 & 0.91 & 0.78 \\
Recall            & 0.97 & 0.91 & 0.78 \\
f1 score          & 0.97 & 0.91 & 0.78 \\
Accuracy          & 1.00 & 0.99 & 0.97 \\

Average Precision & 0.95 & 0.86 & 0.78 \\
ROC AUC Score     & 1.00 & 0.99 & 0.99 \\ \hline
\end{tabular}
\caption{Performance Report \texttt{shuttle} Dataset}
\label{tab:shuttle-perf-complete}}
\end{table}
\end{comment}

%\modifica{far vedere nel caso in cui si splitta il training per capire se va meglio}


With the application of the Scenario II strategy, the results are further improved. In fact, as reported in Figure \ref{fig:GFI-shuttle-split}, now the model is able to consistently recognize Feature 0 as the one along which most of the anomalies are grouped. Its importance score, as depicted in Figure \ref{fig:Feat-imp-shuttle-split}, is significantly higher than the ones of other features. Moreover in the Local Scoremap (Figure \ref{fig:Local-shuttle-split}), the differences between deviant and normal point are more visible thanks to the higher contrasts in the shapes of the red and blue colors in different regions of the feature space. 

Some slight improvements can also be noticed in the Average Precisions (Table \ref{tab:avg-prec-table}), where the scores are almost reaching the perfect value of 1 across all the models. 

%\modifica{inserire tabella precisioni e vedere di quanto è migliorata e come potrebbe aver influito nell'interpretazione}

\begin{comment}
\begin{table}[ht]
\parbox{.45\linewidth}{
\centering
\begin{tabular}{|c|ccc|}
\hline
\multicolumn{4}{|c|}{\textbf{shuttle} inlier training} \\ 
\hline
\textbf{Metric} & \textbf{IF} & \textbf{EIF} & 
\textbf{EIF+} \\ \hline
Precision         & 0.94 & 0.94 & 0.96 \\
Recall            & 0.94 & 0.94 & 0.96 \\
f1 score          & 0.94 & 0.94 & 0.96 \\
Accuracy          & 0.99 & 0.99 & 0.99 \\

Average Precision & 0.99 & 0.91 & 0.92 \\
ROC AUC Score     & 1.00 & 1.00 & 1.00 \\ \hline
\end{tabular}
\caption{Performance Report \texttt{shuttle} Dataset}
\label{tab:shuttle-perf-split}
}
\end{table}
\end{comment}


\begin{figure}
  \centering
  \includegraphics[width=0.7\linewidth]{figures/feature_selection_plots_final/featsel_shuttle_final.pdf}
  \caption{Feature Selection Shuttle}
  \label{fig:fs-shuttle-plus}
\end{figure}\hfil % <-- added

As it was observed in Table \ref{tab:avg-prec-table} also in the Feature Selection Plot, depicted in Figure \ref{fig:fs-shuttle-plus}, high values of Average Precision (around 0.9) may be observed. The algorithm showing the highest values for this metric is ExIFFI-split, in particular in the range between 6 and 3 features. ExIFFI-plus-split, on the other hand, decreased its Average Precision passing from 6 to 5 features. Original behaviors were noticeable in DIFFI and ExIFFI-plus. The first one drops its Average Precision value from 0.7 to 0.2 passing from 4 to 3 features, the second one suffered a similar effect but in the passage from 3 to 2 and finally to 1 feature. 

%\todo[inline, color=red]{Questo è un altro caso in cui la natura clusterizzata delle anomalie limita l'efficacia delle tecniche isolation-based sul dato intero... togliendo gli outlier nel training diventa semplice per il modello riuscire a separarli in pochi tagli e le performance migliorano notevolmente. Valutiamo se tenerlo o se possa andare in appendice (Chiara)}


%\davide{

%The \approach model was applied also to the {\ttfamily Shuttle}, introduced in Section \ref{sec:real-world-data}, dataset and the obtained outcomes are depicted in Figure \ref{fig:shuttle}.

%Similarly to {\ttfamily Breast} also in the {\ttfamily Shuttle} dataset there are multiple candidates to be considered as the top-ranked feature (Figure \ref{fig:GFI-shuttle}). It is possible however to say that Feature 0 has an edge on the other features since it was considered the most important feature 50\% of the time and has a slightly higher average Importance score than the ones of the other features as it is reported in \ref{fig:Feat-imp-shuttle}. 

%For this dataset the Local Importance Scoremap was used to compare Feature 6 and Feature 0 that can be considered as the most important feature according to \ref{fig:GFI-shuttle} and \ref{fig:Feat-imp-shuttle}. Some of the outliers are overlapped on the inliers distribution while the majority of them is aligned along the Feature 0 axis. That is why, as we move along the horizontal axis, the scoremap colouring gets darker and darker and blue confirming the importance of Feature 0.

%}
%\davide {
%Similarly to the {\ttfamily Breast} dataset very high performance metric values can be noticed in Table \ref{tab:shuttle-perf}. Moreover, in this particular dataset, the metric values are very close among all the three models under analysis. 
%}


==> sections/sections_world_dataset_results/shuttle_new.tex <==
\subsection*{{\ttfamily Shuttle}}

\subsubsection{Performance}

\ale{Figure \ref{fig:Shuttle_contamination_full} displays changes in the Average Precision metric as the contamination level of the training set used for the fitting process of the AD models considered in this study increased from 0 to 10 \%. The \EIFplus and DIF model present a decreasing trend proving once again how these methods, \EIFplus in particular, are more suitable for datasets in which the contamination is limited. As it can be observed in Figure \ref{fig:Shuttle_contaminationEIFvsEIF+} the EIF model achieves sligthly better performances than \EIFplus in this particular dataset.} 

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.49\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Shuttle/Contamination/22-03-2024_17-54-14_shuttle_contamination_full_plot.pdf}
      \caption{Models evaluation, varying the contamination levels}
      \label{fig:Shuttle_contamination_full}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.44\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Shuttle/Contamination/22-03-2024_18-19-29_shuttle_EIF+_minus_EIF_precision_over_contamination.pdf}
      \caption{Difference between \EIFplus and EIF average precision}
      \label{fig:Shuttle_contaminationEIFvsEIF+}
    \end{subfigure}\hfil % <-- added
\caption{Figure \ref{fig:Shuttle_contamination_full} illustrates the average precision as the contamination level in the training set increases. Figure \ref{fig:Shuttle_contaminationEIFvsEIF+} compares the performance graphs of EIF and \EIFplus, using the difference of their scores in various contamination levels.}
\label{fig:Shuttle_contamination}
\end{figure}

\ale{A comparison between Classification reports of the AD models in Scenario I and Scenario II is reported in Table \ref{tab:Shuttle_perf}. The IF model can be considered the best according to the metric values but it is worth noticing the significant improvement of the proposed \EIFplus model passing from Scenario I to Scenario II.} 

\begin{table}[htbp]
\begin{minipage}[t]{0.46\textwidth}
\strut\vspace*{-\baselineskip}\newline
\resizebox{\textwidth}{!}{
\begin{tabular}{|c||ccc|ccc||cc|}
\toprule
\hline
&\multicolumn{3}{c|}{Scenario I}&\multicolumn{3}{c||}{Scenario II}&\multicolumn{2}{c|}{Time}\\
\hline
AD Model & Avg & Prec & ROC & Avg & Prec & ROC & fit & pred \\
& Prec &  & AUC & Prec &  & AUC &  &  \\
\hline
IF          & \textbf{0.98}& \textbf{0.96}& \textbf{0.97}& \textbf{0.98}& \textbf{0.97}& \textbf{0.98}& 0.21& \textbf{0.06}\\
EIF         & 0.90& 0.87& 0.93& 0.97& 0.95& 0.97& \textbf{0.16}& 0.54\\
EIF+        & 0.70& 0.71& 0.84& 0.91& 0.96& 0.97& 0.20& 0.36\\
DIF         & 0.54& 0.60& 0.78& \textbf{0.99}& \textbf{0.97}& \textbf{0.98}& 10.5& 9.02\\
AE & 0.90& 0.95& 0.97& 0.90& 0.94& 0.97& 19.6& 0.25\\
\hline
\end{tabular}}
\vspace{0.41cm}
\caption{Performances of 5 different Anomaly Detection models over {\ttfamily Shuttle} are compared using classical Classification metrics. Moreover, the last two columns contain the average time for a fit and predict operation. The highest metric values and the lowest execution times are highlighted in bold}\label{tab:Shuttle_perf}
\end{minipage}
\hfill
\begin{minipage}[t]{0.46\textwidth}
\strut\vspace*{-\baselineskip}\newline
\resizebox{\textwidth}{!}{
\begin{tabular}{|c||c|c|c|c||c|}
\toprule
\hline
&\multicolumn{2}{c|}{Evaluation with EIF}&\multicolumn{2}{c||}{Evaluation with \EIFplus}&\\
\hline
& Scenario I & Scenario II & Scenario I & Scenario II & Time\\

 Algorithm & $AUC_{FS}$  & $AUC_{FS}$ & $AUC_{FS}$  & $AUC_{FS}$ &  \\
\hline
DIFFI                    & -0.514& -1.487& -0.693& -1.456& 0.95\\
IF\_\approach             & \textbf{2.764}& \textbf{2.881}& \textbf{2.789}& \textbf {3.079}& \textbf{0.89}\\
EIF\_\approach            & -1.432& 0.766& 1.223& 0.315& 1.38\\
\EIFplus\_\approach       & 0.459& 0.019& 0.736& -0.131& 1.39\\
IF\_RF                   & 0.440& 0.904& 0.360& 0.648& 2.33\\
EIF\_RF                  & 1.692& 2.747& 1.733& 2.112& 2.33\\
EIF+\_RF                 & 1.904& 2.138& 1.628& 2.117& 2.33\\
\hline
\end{tabular}}
\caption{Quantitative evaluation of the effectiveness of 6 different interpretation algorithms on {\ttfamily Shuttle} through the $AUC_{FS}$ metric, introduced in \ref{sec:interpr_evaluat}. In the last column the average time taken by the different models to produce the importance scores is reported. The highest $AUC_{FS}$ and lowest Importance time values are highlighted in bold.}\label{tab:fs-tab-Shuttle}
\end{minipage}
\end{table}


\subsubsection{Importance Plots}

\ale{Similarly to the {\ttfamily Pima} dataset also in {\ttfamily Shuttle} anomalies are superimposed to the inliers distribution, as observable in the Local Scoremaps depicted in Figures \ref{fig:Local-Shuttle} and \ref{fig:Local-Shuttle-split} thus also for this dataset the explanations produced should be evaluated with care. Comparing the feature rankings produced in the Score Plots in Figure \ref{fig:Feat-imp-Shuttle} and \ref{fig:Feat-imp-Shuttle-split} a feature that should be considered as relevant is Feature 0 since it is placed in second position in both Scenario I and II. }

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Shuttle/Importance_plots/02-03-2024_17-17-06_GFI_Bar_plot_shuttle_EXIFFI+_1.pdf}
      \caption{Bar Plot {\ttfamily Shuttle} Scenario I}
      \label{fig:GFI-Shuttle}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.27\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Shuttle/Importance_plots/02-03-2024_17-17-07_GFI_Score_plot_shuttle_EXIFFI+_1.pdf}
      \caption{Score Plot {\ttfamily Shuttle} Scenario I}
      \label{fig:Feat-imp-Shuttle}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Shuttle/Local_Scoremaps/22-03-2024_17-45-49_importance_map_shuttle_EXIFFI+_1_feat_3_0.pdf}
      \caption{Scoremap {\ttfamily Shuttle} Scenario I}
      \label{fig:Local-Shuttle}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Shuttle/Importance_plots/02-03-2024_15-09-33_GFI_Bar_plot_shuttle_EXIFFI+_2.pdf}
      \caption{Bar Plot {\ttfamily Shuttle} Scenario II}
      \label{fig:GFI-Shuttle-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.27\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Shuttle/Importance_plots/02-03-2024_15-09-33_GFI_Score_plot_shuttle_EXIFFI+_2.pdf}
      \caption{Score Plot {\ttfamily Shuttle} Scenario II}
      \label{fig:Feat-imp-Shuttle-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Shuttle/Local_Scoremaps/22-03-2024_17-45-40_importance_map_shuttle_EXIFFI+_2_feat_3_0.pdf}
      \caption{Scoremap {\ttfamily Shuttle} Scenario II}
      \label{fig:Local-Shuttle-split}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot and Scoremap for {\ttfamily Shuttle} in the two different Scenarios, using the \approach algorithm applied to the \EIFplus model.}\label{fig:interpretation-Shuttle}
\end{figure}

\subsubsection{Feature Selection} \label{sec:Shuttle-fs}

\ale{Feature Selection plots for the {\ttfamily Shuttle} dataset are grouped together in Figure \ref{fig:fs-interpretation-Shuttle}. The best results are achieved by \approach applied to IF and by the post-hoc interpretability methods exploited to explain the EIF and \EIFplus models. Both these three plots, reported in Figures \ref{fig:Feat-Sel_Shuttle_valEIF+_DIFFI_2}, \ref{fig:Feat-Sel_Shuttle_valEIF+_EIF_RandomForest_2} and \ref{fig:Feat-Sel_Shuttle_valEIF+_EIF+_RandomForest_2}, share a common behavior: as features are removed in increasing order of importance (red line) the Average Precision scores show a constant behavior while in the blue line, representing the approach in which attributes are omitted in decreasing order of importance, a significant drop in the scores can be observed passing from 5 to 4 features. A possible interpretation of this peculiar phenomenon may be related to the removal of all the relevant features leaving only the redundant and uninformative ones leading the Average Precision scores to be reduced under the value of 0.4.
On the other hand in Figures related to the \approach and \approach+ models (Figures \ref{fig:Feat-Sel_Shuttle_valEIF+_EXIFFI_2}, \ref{fig:Feat-Sel_Shuttle_valEIF+_EXIFFI+_2}) the red line presents a decreasing trend leading to small (if not negative) values of the $AUC_{FS}$ metric.}

\begin{comment}
Because of the peculiar distribution of the data points, that violates the typical properties anomalies are intended to have, post-hoc interpretation methods achieve better results than Isolation-based models. In fact in Figures \ref{fig:Feat-Sel_Shuttle_valEIF+_IF_RandomForest_2}, \ref{fig:Feat-Sel_Shuttle_valEIF+_EIF_RandomForest_2}, \ref{fig:Feat-Sel_Shuttle_valEIF+_EIF+_RandomForest_2} are associated with a constant trend in Average Precision as features are removed in increasing order of importance (red line) while precision decreases as features are excluded from the input space in decreasing order or relevance (blue line). 
\end{comment}
 

\begin{figure}[!ht] 
\centering
\hspace{0.05\textwidth}\textbf{IF} \hspace{0.29\textwidth} \textbf{EIF} \hspace{0.29\textwidth} \textbf{EIF+}
% First row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Ad-Hoc}}} % Adjust the parbox width as necessary for your caption text
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Shuttle/Feature_Selection/07-05-2024_16-28-29_shuttle_EIF+_IF_EXIFFI_feature_selection_2.pdf}
            \caption{\approach applied to IF}
            \label{fig:Feat-Sel_Shuttle_valEIF+_DIFFI_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Shuttle/Feature_Selection/22-03-2024_18-23-41_shuttle_EIF+_EXIFFI_feature_selection_2.pdf}
            \caption{\approach applied to EIF}
            \label{fig:Feat-Sel_Shuttle_valEIF+_EXIFFI_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Shuttle/Feature_Selection/22-03-2024_18-23-41_shuttle_EIF+_EXIFFI+_feature_selection_2.pdf}
            \caption{\approach applied to \EIFplus}
            \label{fig:Feat-Sel_Shuttle_valEIF+_EXIFFI+_2}
        \end{subfigure}
    \end{minipage}
\end{minipage}

\vspace{5mm} % Space between rows

% Second row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Post-Hoc}}} % Adjust as necessary
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Shuttle/Feature_Selection/22-03-2024_18-23-42_shuttle_EIF+_IF_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to IF}
            \label{fig:Feat-Sel_Shuttle_valEIF+_IF_RandomForest_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Shuttle/Feature_Selection/22-03-2024_18-23-42_shuttle_EIF+_EIF_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to EIF}
            \label{fig:Feat-Sel_Shuttle_valEIF+_EIF_RandomForest_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Shuttle/Feature_Selection/22-03-2024_18-23-42_shuttle_EIF+_EIF+_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to \EIFplus}
            \label{fig:Feat-Sel_Shuttle_valEIF+_EIF+_RandomForest_2}
        \end{subfigure}
    \end{minipage}
\end{minipage}

\caption{Feature Selection of the different Ad-Hoc and Post-Hoc methods applied to the 3 Isolation Forest models: IF, EIF and \EIFplus. The blue line is the values of average precision, calculated with the \EIFplus model in the Scenario II, dropping the most important feature at each step, the red line is the values of average precision dropping the least important feature at each step and the green line is the value of the feature selection dropping a random feature at each step.}\label{fig:fs-interpretation-Shuttle}
\end{figure}

\ale{Table \ref{tab:fs-tab-Shuttle} contains the $AUC_{FS}$ metrics values for all the combinations of interpretation and evaluation model both for Scenario I and Scenario II. As already discussed in \ref{sec:Shuttle-fs} three models (i.e. IF\_\approach, EIF\_RandomForest and \EIFplus\_RandomForest) showcase superior quantitative outcomes. On the other hand, the $AUC_{FS}$ values of the proposed interpretation algorithms \approach and \approach+, even though faster than post-hoc methods, are lower and in some cases also negative.}  



==> sections/sections_world_dataset_results/wine.tex <==

\subsubsection{{\ttfamily Wine}}

%\modifica{intro al dataset richiamando la sezione \ref{sec:real-world-data}}

Similarly to the {\ttfamily Annthyroid} and {\ttfamily Cardio} dataset, the {\ttfamily Wine} dataset is part of the UCI Machine Learning Repository and it is originally used as a Multi Class Classification dataset for the case of three classes representing three different wine cultivars. Thirteen numerical features describing the chemical properties of wine samples are used in this instance. Further details about the specific semantic meaning of each feature and about the dataset in general are contained in Appendix \ref{sec:real-world-data}. 

%\modifica{mettere grafici di importanza}

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/wine/Feat_bar_plot_wine.pdf}
      \caption{Score Plot \texttt{Wine} Scenario I}
      \label{fig:Feat-imp-Wine}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/wine/Feat_bar_plot_wine_split.pdf}
      \caption{Score Plot \texttt{Wine} Scenario II}
      \label{fig:Feat-imp-Wine-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/wine/GFI_wine_synt.pdf}
      \caption{Bar Plot \texttt{Wine} Scenario I}
      \label{fig:GFI-wine}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/wine/GFI_wine_synt_split.pdf}
      \caption{Bar Plot \texttt{Wine} Scenario II}
      \label{fig:GFI-wine-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/scoremaps_real_world/Local_Scoremap_Plot_wine.png}
      \caption{Scoremap \texttt{Wine} Scenario I}
      \label{fig:Local-wine}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/scoremaps_real_world/Local_Scoremap_Plot_wine_split.png}
      \caption{Scoremap \texttt{Wine} Scenario II}
      \label{fig:Local-wine-split}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot and Scoremap for \texttt{Wine}}
\label{fig:interpretation-wine}
\end{figure}

Looking at the Bar Plot it is possible to notice the presence of a shared importance between Feature 4 and 8. Although the certainty and consistency of the model on the feature ranking is not satisfactory since, as it is represented in Figure \ref{fig:GFI-wine}, Feature 4 is selected as the top feature in half of the executions while Feature 8 only in 30 \% of them. 

%\modifica{sottolineare dallo scoremap 12 vs 4 come le anomalie (stelline) vengano in realtà inglobate nella distribuzione normale grazie all'analisi dei contourplot, richiamare un appendix dove metteremo lo scoremap di tutte le feature contro tutte}

Moreover, the Scoremap (Figure \ref{fig:Local-wine}) depicts how the anomalies (i.e. the red stars) are somehow incorporated in the normal distribution. This effect can be noticed by analyzing the Anomaly Score contour plots. 

%\davide{Non so quanto sia corretta questa frase}

In fact, the two lines covering the lowest area, so the contour plots associated to the lowest Anomaly Scores, contain not only the inliers but also the outliers. 

%\modifica{presentazione dei risultati nel caso del train sul tutto il dataset}

\begin{comment}
\begin{table}[ht]
\parbox{.45\linewidth}{
\centering
\begin{tabular}{|c|ccc|}
\hline
\multicolumn{4}{|c|}{\textbf{wine} complete training} \\ \hline
\textbf{Metric} & \textbf{IF} & \textbf{EIF} & \textbf{EIF+} \\ \hline
Precision         & 0.10 & 0.20 & 0.10 \\
Recall            & 0.10 & 0.20 & 0.10 \\
f1 score          & 0.10 & 0.20 & 0.10 \\
Accuracy          & 0.86 & 0.88 & 0.86 \\

Average Precision & 0.22 & 0.22 & 0.18 \\
ROC AUC Score     & 0.82 & 0.82 & 0.78 \\ \hline
\end{tabular}
\caption{Performance Report \texttt{Wine} Dataset}
\label{tab:wine-perf-complete}}
\end{table}
\end{comment}

%\modifica{far vedere come i risultati della predizione sono bassi ritenendo che gli score più importanti non sono effettivamente legati alla feature che di più devia secondo gli outlier dati dal dataset}

As expected from the graphical results the Average Precision values (Table \ref{tab:avg-prec-table}) of the {\ttfamily Wine} dataset are very low, less than 0.25 for all the models. This suggests that the feature ranking returned by the interpretation algorithm, and shown in Figure \ref{fig:Feat-imp-Wine}, cannot be fully trusted. In fact, observing the Scoremap it is clear how the anomalies are distributed along Feature 12 rather than Feature 8 or 4. 

%\modifica{Introdurre caso in cui trainiamo solo sugli inlier}

A possible solution to improve the performance metrics and the reliability of the interpretability results is the one of training the model exclusively on the inliers and testing it on the entire dataset. 

%\modifica{mettere le interpretazioni di questo caso}


%\modifica{far vedere come le interpretazioni sono più robuste ad identificare la feature 12 corrispondente alla prolina come la più anomala e come effetticamente lo scoremap in questo caso fa vedere contourplot che non si "adattano alle anomalie}

As expected the consistency of the model in selecting the most important feature increases as Feature 12 (which represents Proline) is selected as the most relevant attribute in all the model executions performed to obtain the Bar Plot contained in Figure \ref{fig:GFI-wine-split}. 

Furthermore from the Scoremap, represented in Figure \ref{fig:Local-wine-split}, the contour lines are now excluding the anomalous samples from the inlier distribution. 

The result is that in this instance the model has an easier task in correctly detecting the anomalous points as can be noticed by looking at the Average Precision values (Table \ref{tab:avg-prec-table}). Here it is also possible to notice a significant passing from the IF to the newly introduced EIF+ model which presents an improvement of almost 30\% on the IF model. 

%\modifica{inserire tabelle precisioni}

\begin{comment}
\begin{table}[ht]
\parbox{.45\linewidth}{
\centering
\begin{tabular}{|c|ccc|}
\hline
\multicolumn{4}{|c|}{\textbf{wine} inlier training} \\ 
\hline
\textbf{Metric} & \textbf{IF} & \textbf{EIF} & 
\textbf{EIF+} \\ \hline
Precision         & 0.40 & 0.50 & 0.60 \\
Recall            & 0.40 & 0.50 & 0.60 \\
f1 score          & 0.40 & 0.50 & 0.60 \\
Accuracy          & 0.91 & 0.92 & 0.94 \\

Average Precision & 0.40 & 0.58 & 0.78 \\
ROC AUC Score     & 0.91 & 0.95 & 0.98 \\ \hline
\end{tabular}
\caption{Performance Report \texttt{wine} Dataset}
\label{tab:wine-perf-split}
}
\end{table}
\end{comment}

%\modifica{sottolineare come in questo caso effettivamente il modello performa meglio quindi le interpretazioni sono più reliable}

\begin{comment}
    \modifica{mettere feature selection \textbf{allenando l'intero dataset in ogni modello}, (bisogna fare diffi e RF 
 e casual sul dataset SCALATO) mettendo 
\begin{itemize}
    \item RF
    \item casual
    \item diffi
    \item ExIFFI selection usando la feature importance del caso in cui il modello era allenato su tutto
    \item ExIFFI+ selection usando la feature importance del caso in cui il modello era allenato su tutto
    \item ExIFFI selection usando la feature importance del caso in cui il modello era allenato sul training set
    \item ExIFFI+ selection usando la feature importance del caso in cui il modello era allenato sul training set
\end{itemize}
}
\end{comment}


\begin{figure}
  \centering
  \includegraphics[width=0.7\linewidth]{figures/feature_selection_plots_final/featsel_wine_final.pdf}
  \caption{Feature Selection Plot {\ttfamily Wine}}
  \label{fig:fs-wine-plus}
\end{figure}\hfil % <-- added


%\modifica{evidenziare come effettivamente utilizzando la feature importance del caso in cui il modello è allenato sugli inlier nella feature selection si vede che effettivamente porta a migliorare i risultati, ma tale miglioramento è legato solo alla concezione di quali sono le anomalie definite dal dataset}

The Feature Selection Plot for the {\ttfamily Wine} dataset is reported in Figure \ref{fig:fs-wine-plus}. 
The Average Precision of ExIFFI-plus-split and ExIFFI-split increases up to 1 with the progressive removal of all the input features with ExIFFI-plus-split being the feature selection algorithm performing better in terms of Average Precision. 

For what concerns the other Feature Ranking Algorithms they present more or less constant Average Precision values across all the different sets of input features considered. 

The fact that the Average Precision values of the two algorithms derived from the inlier training show a significant improvement on the others is strictly connected to the performance enhancement obtained with the usage of this novel training approach as shown on the right column of Figure \ref{fig:interpretation-wine} and Table \ref{tab:avg-prec-table}. 

%\todo[inline, color=red]{Questo penso che possa andare in appendice, se nessuno ha niente in contrario (Chiara)}
%\todo[inline, color=green]{Son d'accordo(GAS)}


% PLOT WITH SPLIT 


% PLOT WITHOUT SPLIT 


%The analysis of the feature importances for the {\ttfamily Wine} dataset, described in Section \ref{sec:real-world-data}, are presented in Figure \ref{fig:wine}. 

%In the {\ttfamily Wine} dataset there is a significant importance in detecting anomalies in Feature 12 that is considered the most important 60\% of the time and 30\% of the time as the second most important feature, as depicted in Figure \ref{fig:GFI-wine}. Other relevant features to highlight are Feature 0 and 8 which are considered very important in some executions and have similar average Feature Score values to the ones of Feature 12 as observable from Figure \ref{fig:Feat-imp-Wine}. 

%Figure \ref{fig:Local-wine} represents the comparison between two of the most important features (Feature 12 and 0) on the Local Importance Scoremap. With a detailed observation of the data samples distribution it is possible to see the dissemination of anomalies along Feature 12, in particular these are concentrated in the top right section of the feature space. On the contrary, 
%inliers are mainly distributed along Feature 0. The importance of Feature 0 may be due to the fact that some of the inliers are slightly outside the main cluster and thus can be considered as \textit{model anomalies}. 

%According to the dataset description, that can be found in \ref{sec:real-world-data}, Feature 12 represents the concentration of Proline. This means that wines obtained from the culture associated with the outliers can be easily distinguished from the other two cultures by looking at their Proline values. 




%\davide {
%The Performance Report Table for the {\ttfamily Wine} dataset can be found in Table \ref{tab:wine-perf}. Similarly to the {\ttfamily Annthyroid} dataset, the EIF+ model outperforms the other two on the F1 Score and Average Precision metrics with a significant margin of more than 30\%.
%}













==> sections/sections_world_dataset_results/wine_new.tex <==
\subsection*{{\ttfamily Wine}}

\subsubsection{Performance}

\ale{The Contamination plot, depicted in Figure \ref{fig:Wine_contamination_full}, shows how the Average Precision of all the Anomaly Detection models considered diminishes as outliers are progressively included as part of the training set. \EIFplus is the model with the best metric values for low values of the contamination parameter confirming another time its effectiveness in datasets with a limited number of outliers as {\ttfamily Wine}. Moreover Figure \ref{fig:Wine_contaminationEIFvsEIF+} , that represents the difference in the Average Precision values of the EIF and \EIFplus, enhances the superiority of the proposed model with the respect to its counterpart.} 

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.49\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Wine/Contamination/20-03-2024_13-51-21_wine_contamination_full_plot.pdf}
      \caption{ }
      \label{fig:Wine_contamination_full}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.44\textwidth}
      \includegraphics[width=\linewidth]{Newfigures/Wine/Contamination/20-03-2024_13-54-40_wine_EIF+_minus_EIF_precision_over_contamination.pdf}
      \caption{ }
      \label{fig:Wine_contaminationEIFvsEIF+}
    \end{subfigure}\hfil % <-- added
\caption{Fig. \ref{fig:Wine_contamination_full} Represent the average precision the more the level of contamination of the train set is increased. The Fig. \ref{fig:Wine_contaminationEIFvsEIF+} Give show specifically the graphs of the EIF and EIF+}
\label{fig:Wine_contamination}
\end{figure}

\ale{Table \ref{tab:Wine_perf}  provides a comprehensive comparison of the performances of the different methods analyzed in this study in the two different evaluation scenarios described in \ref{sec:interpr_evaluat} . In Scenario I the performances of Isolation based models (i.e. IF, EIF and \EIFplus) overcome the ones of  deep learning based approaches (i.e. DIF and Autoencoder) while in Scenario II \EIFplus stands out as the best performing model. Referring to the computational efficiency argument there is a clear separation between Isolation based and deep learning based models with the first ones being the fastest in fitting the model and providing predictions on new samples.}

\begin{table}[htbp]
\begin{minipage}[t]{0.46\textwidth}
\strut\vspace*{-\baselineskip}\newline
\resizebox{\textwidth}{!}{
\begin{tabular}{|c||ccc|ccc||cc|}
\toprule
\hline
&\multicolumn{3}{c|}{Scenario I}&\multicolumn{3}{c||}{Scenario II}&\multicolumn{2}{c|}{Time}\\
\hline
AD Model & Avg & Prec & ROC & Avg & Prec & ROC & fit & pred \\
& Prec &  & AUC & Prec &  & AUC &  & pred \\
\hline
IF          & \textbf{0.26}& \textbf{0.20}& \textbf{0.56}& 0.61& 0.50& 0.72& 0.10& \textbf{0.002}\\
EIF         & 0.21& 0.20& 0.56& 0.57& 0.60& 0.78& \textbf{0.09}& 0.005\\
EIF+        & 0.17& 0.00& 0.45& \textbf{0.79}& \textbf{0.70}& \textbf{0.83}& 0.10& \textbf{0.002}\\
DIF         & 0.07& 0.00& 0.45& 0.72& 0.70& 0.83& 0.57& 0.210\\
AE          & 0.14& 0.10& 0.51& 0.45& 0.50& 0.72& 2.13& 0.040\\
\hline
\end{tabular}}
\vspace{0.41cm}
\caption{Performances of 5 different Anomaly Detection models over {\ttfamily Wine} are compared using classical Classification metrics. Moreover the last two columns contain the average time for a fit and predict operation. The highest metric values and the lowest execution times are highlighted in bold}\label{tab:Wine_perf}
\end{minipage}
\hfill
\begin{minipage}[t]{0.46\textwidth}
\strut\vspace*{-\baselineskip}\newline
\resizebox{\textwidth}{!}{
\begin{tabular}{|c||c|c|c|c||c|}
\toprule
\hline
&\multicolumn{2}{c|}{Evaluation with EIF}&\multicolumn{2}{c||}{Evaluation with \EIFplus}&\\
\hline
& Scenario I & Scenario II & Scenario I & Scenario II & Time\\

 Algorithm & $AUC_{FS}$  & $AUC_{FS}$ & $AUC_{FS}$  & $AUC_{FS}$ &  \\
\hline
DIFFI                & 0.176& -3.799& 0.437& -3.491& 0.33\\
IF\_\approach        & \textbf{0.682}& 8.076& \textbf{0.628}& \textbf{9.401}& 0.07\\
EIF\_\approach       & 0.451& 7.122& 0.459& 8.120& \textbf{0.01}\\
\EIFplus\_\approach  & 0.127& \textbf{9.000}& 0.180& 9.25& 0.01\\
IF\_RF               & -3.093& 4.413& -2.339& 4.539& 0.18\\
EIF\_RF              & -2.415& 3.946& -1.570& 4.369& 0.18\\
EIF+\_RF             & -2.816& 4.873& -2.056& 5.642& 0.18\\
\hline
\end{tabular}
}
\caption{Quantitative evaluation of the effectiveness of 6 different interpretation algorithms on {\ttfamily Wine} through the $AUC_{FS}$ metric, introduced in \ref{sec:interpr_evaluat}. In the last column the average time taken by the different models to produce the importance scores is reported. The highest $AUC_{FS}$ and lowest Importance time values are highlighted in bold.}\label{tab:fs-tab-Wine}
\end{minipage}
\end{table}


\subsubsection{Importance Plots}

\ale{Figure \ref{fig:interpretation-Wine} provides a qualitative and quantitative evaluation of the proposed interpretation algorithm on the {\ttfamily Wine} dataset. In Scenario I \approach+ is not able to identify, as shown in \ref{fig:GFI-Wine}, an attribute dominating the others in terms of relevance for pursuing the Anomaly Detection task. On the other hand, exploiting the characteristics of \EIFplus when the training set is composed of solely inliers, feature Proline is indicated as the most relevant one in Scenario II as depicted in \ref{fig:Feat-imp-Wine-split}. The relevance of the Proline variable can be assesed observing the Local Scoremap reported in Figure \ref{fig:Local-Wine-split}.}

\begin{figure}[!ht] 
    \centering % <-- added
    \begin{subfigure}[t]{0.36\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Wine/Importance_plots/02-03-2024_15-44-55_GFI_Bar_plot_wine_EXIFFI+_1.pdf}
      \caption{Bar Plot {\ttfamily Wine} Scenario I}
      \label{fig:GFI-Wine}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.31\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Wine/Importance_plots/02-03-2024_15-44-56_GFI_Score_plot_wine_EXIFFI+_1.pdf}
      \caption{Score Plot {\ttfamily Wine} Scenario I}
      \label{fig:Feat-imp-Wine}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.23\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Wine/Local_Scoremap/20-03-2024_16-41-04_importance_map_wine_EXIFFI+_1_feat_12_4.pdf}
      \caption{Scoremap {\ttfamily Wine} Scenario I}
      \label{fig:Local-Wine}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.36\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Wine/Importance_plots/02-03-2024_14-41-24_GFI_Bar_plot_wine_EXIFFI+_2.pdf}
      \caption{Bar Plot {\ttfamily Wine} Scenario II}
      \label{fig:GFI-Wine-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.31\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Wine/Importance_plots/02-03-2024_14-41-25_GFI_Score_plot_wine_EXIFFI+_2.pdf}
      \caption{Score Plot {\ttfamily Wine} Scenario II}
      \label{fig:Feat-imp-Wine-split}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}[t]{0.23\textwidth}
    \centering
      \includegraphics[width=\linewidth]{Newfigures/Wine/Local_Scoremap/20-03-2024_16-39-55_importance_map_wine_EXIFFI+_2_feat_12_4.pdf}
      \caption{Scoremap {\ttfamily Wine} Scenario II}
      \label{fig:Local-Wine-split}
    \end{subfigure}\hfil % <-- added
\caption{Bar Plot, Score Plot and Scoremap for {\ttfamily Wine} in the two different Scenarios, using the \approach algorithm applied to the \EIFplus model.}\label{fig:interpretation-Wine}
\end{figure}

\subsubsection{Feature Selection}

\ale{Figure \ref{fig:fs-interpretation-Wine} shows the superiority of the \approach interpretation algorithm when applied to IF, EIF and the proposed \EIFplus as illustrated in Figures \ref{fig:Feat-Sel_Wine_valEIF+_DIFFI_2}, \ref{fig:Feat-Sel_Wine_valEIF+_EXIFFI_2} and \ref{fig:Feat-Sel_Wine_valEIF+_EXIFFI+_2}. Using the feature ranking derived from the importance scores generated by \approach, in fact, guarantees an increasing Average Precision as non relevant attributes are progressively removed from the feature space (red line) reaching almost perfect scores of 1. On the other hand following the blue line it is possible to notice an instantaneous drop in performance as the most important features are removed from the training set. Conversely the application of the RandomForest based post-hoc method produces sligthly inferior results mainly bacause of the oscillating trend observable in the blue line which demonstrates a non perfect alignment of the feature ranking with the ground truth.}

\begin{figure}[!ht] 
\centering
\hspace{0.05\textwidth}\textbf{IF} \hspace{0.29\textwidth} \textbf{EIF} \hspace{0.29\textwidth} \textbf{EIF+}
% First row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Ad-Hoc}}} % Adjust the parbox width as necessary for your caption text
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Wine/Feature_Selection/07-05-2024_18-22-49_wine_EIF+_IF_EXIFFI_feature_selection_2.pdf}
            \caption{\approach applied to IF}
            \label{fig:Feat-Sel_Wine_valEIF+_DIFFI_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Wine/Feature_Selection/20-03-2024_09-43-38_wine_EIF+_EXIFFI_feature_selection_2.pdf}
            \caption{\approach applied to EIF}
            \label{fig:Feat-Sel_Wine_valEIF+_EXIFFI_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Wine/Feature_Selection/20-03-2024_09-40-08_wine_EIF+_EXIFFI+_feature_selection_2.pdf}
            \caption{\approach applied to \EIFplus}
            \label{fig:Feat-Sel_Wine_valEIF+_EXIFFI+_2}
        \end{subfigure}
    \end{minipage}
\end{minipage}

\vspace{5mm} % Space between rows

% Second row with vertical caption on the left
\begin{minipage}{\textwidth}
    \rotatebox{90}{\parbox{15mm}{\centering \textbf{Post-Hoc}}} % Adjust as necessary
    \begin{minipage}{0.95\textwidth}
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Wine/Feature_Selection/20-03-2024_09-44-54_wine_EIF+_IF_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to IF}
            \label{fig:Feat-Sel_Wine_valEIF+_IF_RandomForest_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Wine/Feature_Selection/20-03-2024_09-44-29_wine_EIF+_EIF_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to EIF}
            \label{fig:Feat-Sel_Wine_valEIF+_EIF_RandomForest_2}
        \end{subfigure}\hfill
        \begin{subfigure}[t]{0.30\textwidth}
            \centering
            \includegraphics[trim={0 0 3.5cm 0}, clip, width=\linewidth]{Newfigures/Wine/Feature_Selection/20-03-2024_09-42-04_wine_EIF+_EIF+_RandomForest_feature_selection_2.pdf}
            \caption{RandomForest fitted to \EIFplus}
            \label{fig:Feat-Sel_Wine_valEIF+_EIF+_RandomForest_2}
        \end{subfigure}
    \end{minipage}
\end{minipage}

\caption{Feature Selection of the different Ad-Hoc and Post-Hoc methods applied to the 3 Isolation Forest models: IF, EIF and \EIFplus. The blue line is the values of average precision, calculated with the \EIFplus model in the Scenario II, dropping the most important feature at each step, the red line is the values of average precision dropping the least important feature at each step and the green line is the value of the feature selection dropping a random feature at each step.}\label{fig:fs-interpretation-Wine}
\end{figure}

\ale{The summary reported in \ref{tab:fs-tab-Wine} confirm the effectiveness of the proposed approach in providing explainability to the EIF and \EIFplus AD methods surpassing DIFFI and post-hoc interpretability approaches such as Random Forest. In particular, the DIFFI interpretation algorithm is the only one producing negative $AUC_{FS}$ values in Scenario II proving its inability in producing correct feature rankings in presence of solely inliers in the training set. Moreover the ineffectiveness of this method is additionally demonstrated by the metric values associated to Scenario I (i.e. 0.176 and 0.437) that, being close to 0, represent a situation is which there is not a significant advantage in removing features in increasing or decreasing order.}




==> sections/toy_examples.tex <==
\subsubsection{Global Feature Importance}
In order to analyze the effectiveness of the global feature importance, we decided to use the synthetic dataset setup shown in the DIFFI paper \cite{diffi} introduced in the Section \ref{datasets}. In this way we will have a previously validated proxy to show how much and to what extent \approach works.
The three examples have a central ball with inliers and  some anomalies distributed along specific directions: the first example has the anomalies along feature 0, the second example along feature 1, and the third along a combination of the previous directions.

Figure \ref{xaxis_yaxis} shows the global feature importance of \approach in the case of the first and the second synthetic example. 
We can observe in Figure \ref{fig:GFI DEIFFI xaxis} that the model detects the correct feature consistently, this means that it detects with strong belief that feature $0$ is the most important one to determine an outlier.
In the case of Figure \ref{fig:GFI DEIFFI yaxis}, the feature $1$ is correctly identified as the most important one. 
%\ale{CONCORDO, AVEVO AGGIUNTO QUESTO PARAGRAFO PERCHE' AVEVO NOTATO DELLE STRANEZZE DEL DATASET} \tom{SECONDO ME POTREMMO RIMUOVERE QUESTO PASSAGGIO, COMUNQUE CERCO DI RIMANEGGIARLO Moreover, we can observe that the second most important feature highlighted by \approach is not random but is feature 1 in the first barplot and feature 0 in the second barplot in Figure \ref{fig:GFI DEIFFI}. This is due to a particular design choice made by \cite{carletti2019explainable} and visible in Figure \ref{fig:synt bisec pairplot} that adds some random points on the first two features.}
%\tomdel{Moreover, we can observe that in the second position in the first barplot there is the feature 1 and in the second the feature 0. If you observe how inliers are distributed, the blue point showed in Figure } \ref{fig:synt bisec pairplot} \tomdel{, that are the same for both the datasets to every example, \jacopo{frase un pò contorta con doppia proposizione incidentale} we can easily observe that in the synthetic dataset used in the DIFFI paper there are few points in blue very far from the distribution along the feature 0 and 1. Then even if some outliers lay along the feature 0 there are some also in the feature 1 and vice-versa.} 
%\todo[color=purple]{concordo con Jacopo sulla necessità di semplificare qui sopra}
\begin{figure}[t]
    \centering % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/diffi_comparison/ExIFFI_Synt_xaxis.pdf}
      \caption{Importance barplot of the dataset of anomalies distributed along the feature 0}
      \label{fig:GFI DEIFFI xaxis}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/diffi_comparison/ExIFFI_Synt_yaxis.pdf}
      \caption{Importance barplot of the dataset of anomalies distributed along the feature 1}
      \label{fig:GFI DEIFFI yaxis}
    \end{subfigure}\hfil % <-- added
\caption{ Feature importance obtained on datasets \texttt{synt xaxis} and \texttt{synt yaxis} explained in Section \ref{toy} where anomalies lie respectively on feature 0 and feature 1.}\label{fig:GFI DEIFFI}
\label{xaxis_yaxis}
\end{figure}
Finally, as Carletti et al. did in \cite{diffi}, we want to analyse what happens when the anomalous points are distributed along the bisector line of the feature 0 and feature 1 as shown in Figure \ref{fig:synt bisec pairplot}. 

\begin{figure}[t]
\centering % <-- added
  \includegraphics[width=0.8\textwidth]{figures/diffi_comparison/pairplot_synth_bisec.pdf}
  \caption{  Synthetic dataset  \texttt{synt bisec} with anomalies in orange distributed along the bisection line of the feature 0 and 1. Training data are depicted in blue, while testing data are depicted in orange.}
  \label{fig:synt bisec pairplot}
\end{figure}

Since the EIF model is stochastic and both of the first two features are important, we expect that computing the model multiple times the feature ranking changes: sometimes the first one is feature 0, and sometimes feature 1, meaning that both of them are important in Figure \ref{fig:GFI DEIFFI bisec}.  The histogram depicted in the Figure \ref{fig:importance scores} illustrates the mean importance scores for each feature in the case of the three 6-dimensional synthetic datasets. In the \texttt{synt xaxis} and \texttt{synt yaxis} datasets, the importance scores for feature 0 and feature 1 are not equal, with one score being greater than the other. In contrast, in the \texttt{synt bisec} dataset, both feature 0 and feature 1 have very high and nearly identical importance scores.
\begin{figure}[t]
    \centering % <-- added
    \begin{subfigure}{0.49\textwidth}
      \includegraphics[width=\linewidth]{figures/diffi_comparison/ExIFFI_Synt_bisec.pdf}
      \caption{Importance barplot of the dataset of anomalies distributed along the feature 1}
      \label{fig:GFI DEIFFI bisec}
    \end{subfigure}\hfil % % <-- added
    \hspace{0.04\textwidth}
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/diffi_comparison/score_barplot.pdf}
      \caption{Importance barplot of the dataset of anomalies distributed along the feature 1}
      \label{fig:importance scores}
    \end{subfigure}\hfil
\caption{ Feature importance obtained on datasets \texttt{synt bisec} explained in Section \ref{toy} where anomalies lie on feature 0 and feature 1.}
\label{bisec}
\end{figure}


\subsubsection{Local Feature Importance}\label{lfi}
It is crucial to know which features are most important for identifying whether a single sample is an outlier. For example, in an industrial process where an AD model detects an outlier, understanding the most relevant features can facilitate root cause analysis and allow for fast and effective corrective actions.

In the paper made by Hariri et al. in \cite{8888179}, they demonstrated that Extended IF  is able to address the bias limitations of IF through the use of a comparative approach. They presented the anomaly score maps of both algorithms, highlighting the ability of EIF to more accurately generalize the score map.

Similarly to that analysis, here we present a scoremap of the Local feature importance score originated from the DIFFI and \approach algorithms, where the corresponding IF and EIF models were trained on a dataset named \texttt{bimodal} introduced in Section \ref{datasets}, mainly made up of points distributed into two separate balls along the bisector line.
Then the scoremap is made by taking in consideration the whole space around the distribution, demonstrating how the \approach is able to generalize better the importance scores related to the anomalies.


\begin{figure}[!ht]
      \includegraphics[width=\linewidth]{figures/diffi_comparison/bimodal.pdf}
\caption{Feature importance scoremap of DIFFI and \approach along the first two features of dataset \texttt{bimodal}.}
\label{scoremap}
\end{figure} 


%\ale{QUA SPIEGO I COLORI DEGLI GLI SCOREMAPS!! E DA QUA IN POI QUANDO MI RIFERISCO A LORO NON RISPIEGO DA CAPO COME LEGGERLI MA SEMPLICEMENTE LI LEGGO!!}\tom{oro} 
In Figure \ref{scoremap}, the scoremaps display the relative importance of two features using red and blue colors. Red regions indicate higher importance of feature 1, while blue regions indicate higher importance of feature 0. The intensity of the color reflects the magnitude of the feature importance at each point. Lighter colors correspond to lower importance values, and thus points in these regions are less likely to be considered outliers with respect to the features under analysis. Additionally, the score map includes contour plots, represented by grey lines surrounding the data points. These contour plots depict different levels of the combined importance of the features.

Similar to IF, the score map of the DIFFI algorithm exhibits a strong bias along the direction orthogonal to the features. This bias can negatively impact the model's comprehension of the feature, as it limits the ability of the DIFFI model to generalize well beyond the region of the feature space where the original distribution is concentrated. As a result, the model may struggle to accurately identify the features that have the greatest influence on determining whether a sample is an outlier in various regions of the feature space.

In a real-world scenario, it is possible that the interpretation algorithm is required to provide accurate interpretations for points that are located far from the distribution of the training dataset. If the DIFFI algorithm exhibits this bias, evidenced with the scoremap, it may struggle to accurately interpret such points, potentially leading to the provision of incorrect information.

To illustrate this point let's consider the scoremap presented in the image on the left of Figure \ref{scoremap}.  The bundles crossing the dataset orthogonally with respect to the principal directions exhibit lighter colors, indicating that data samples located in these regions are less anomalous compared to darker regions. However, it is not clear whether points located within the bundles but farther from the dataset are necessarily less anomalous than points that are at a similar distance but not within the bundles. 
Additionally, the top-left and bottom-right corners of the image appear to have a plain dark  color, without distinguishing the region by intensity or feature colour.


==> tables/BigTable.tex <==

\begin{sidewaystable}
   \scalebox{0.7}{
   \centering
    \begin{tabular}{| *{17}{c|}}
        \hline 
        dataset & sample&df& out& 
        \multicolumn{2}{c|}{E-DIFFI} & 
        \multicolumn{2}{c|}{ACME} & 
        \multicolumn{2}{c|}{DIFFI} & 
        \multicolumn{2}{c|}{\thead{E-DIFFI\\ vs ACME}} & 
        \multicolumn{2}{c|}{\thead{DIFFI vs\\ E-DIFFI}} & 
        \multicolumn{2}{c|}{\thead{ACME \\vs DIFFI}} & 
        \thead{prec \\ EIF} \\ 
         &  &  &  & 
        cos & ken &
        cos & ken &
        cos & ken &
        cos & ken &
        cos & ken &
        cos & ken &
        \\ 
        \hline
annthyroid  &   2500 &   6 &  189 &          0.811 &           0.766 &        0.893 &         0.884 &         0.857 &          0.585 &               0.657 &               -0.283 &                0.893 &                 0.557 &              0.581 &              -0.568 &     0.241 \\
breastw     &    449 &   9 &  236 &          0.725 &           0.501 &        0.737 &         0.627 &         0.924 &          0.685 &               0.717 &               -0.039 &                0.921 &                 0.511 &              0.706 &               0.012 &     0.858 \\
ionosphere  &    350 &  33 &  125 &          0.256 &          -0.019 &        0.818 &         0.602 &         0.623 &          0.252 &               0.778 &                0.020 &                0.768 &                 0.020 &              0.680 &              -0.280 &     0.759 \\
mammography &   2500 &   6 &   81 &          0.864 &           0.787 &        0.968 &         0.884 &         0.776 &          0.766 &               0.554 &               -0.667 &                0.921 &                 0.541 &              0.551 &              -0.723 &     0.262 \\
cardio      &   1822 &  21 &  175 &          0.725 &           0.374 &        0.546 &         0.388 &         0.886 &          0.600 &               0.759 &                0.015 &                0.910 &                 0.425 &              0.739 &              -0.022 &     0.519 \\
lympho      &    148 &  18 &    6 &          0.586 &           0.203 &        0.960 &         0.790 &         0.971 &          0.812 &               0.802 &               -0.037 &                0.854 &                 0.272 &              0.756 &               0.074 &     0.533 \\
pendigits   &   2500 &  16 &   57 &          0.711 &           0.372 &        0.913 &         0.726 &         0.784 &          0.574 &               0.694 &               -0.270 &                0.892 &                 0.405 &              0.692 &              -0.275 &     0.304 \\
pima        &    768 &   8 &  268 &          0.838 &           0.611 &        0.977 &         0.911 &         0.689 &          0.592 &               0.752 &               -0.013 &                0.814 &                 0.369 &              0.752 &               0.033 &     0.522 \\
wine        &    129 &  13 &   10 &          0.508 &           0.154 &        0.968 &         0.774 &         0.687 &          0.433 &               0.828 &                0.055 &                0.739 &                -0.058 &              0.813 &               0.129 &     0.610 \\
shuttle     &   2500 &   9 &  179 &          0.772 &           0.465 &        0.977 &         0.888 &         0.854 &          0.641 &               0.887 &                0.263 &                0.777 &                 0.074 &              0.709 &              -0.160 &     0.854 \\
thyroid     &   2500 &   6 &   64 &          0.661 &           0.588 &        0.961 &         0.926 &         0.906 &          0.710 &               0.661 &               -0.176 &                0.862 &                 0.400 &              0.678 &              -0.160 &     0.286 \\
vowels      &   1452 &  12 &   46 &          0.660 &           0.411 &        0.549 &         0.314 &         0.527 &          0.326 &               0.758 &                0.038 &                0.833 &                 0.285 &              0.783 &               0.118 &     0.263 \\
        \hline
    \end{tabular}
}
  \caption{Blabla}
  \label{tab:1}
\end{sidewaystable}


==> tables/average_precision_table.tex <==
\begin{comment}
\begin{table}[ht]
\centering
\footnotesize
\begin{tabular}{|c|ccc|ccc|}
\hline
\multicolumn{1}{|l|}{} & \multicolumn{3}{c|}{\textbf{Scenario I}}                                      & \multicolumn{3}{c|}{\textbf{Scenario II}}                                        \\ \hline
\textbf{Dataset}       & \multicolumn{1}{c|}{\textbf{IF}} & \multicolumn{1}{c|}{\textbf{EIF}} & \textbf{EIF+} & \multicolumn{1}{c|}{\textbf{IF}} & \multicolumn{1}{c|}{\textbf{EIF}} & \textbf{EIF+} \\ \hline
\texttt{Xaxis}         & \multicolumn{1}{c}{0.15}        & \multicolumn{1}{c}{0.98}         & 0.98          & \multicolumn{1}{c}{0.11}        & \multicolumn{1}{c}{1}            & 1             \\ 
\texttt{Yaxis}         & \multicolumn{1}{c}{0.11}        & \multicolumn{1}{c}{1}            & 1             & \multicolumn{1}{c}{0.11}        & \multicolumn{1}{c}{1}            & 1             \\ 
\texttt{bisect}        & \multicolumn{1}{c}{0.79}        & \multicolumn{1}{c}{1}            & 0.98          & \multicolumn{1}{c}{1}           & \multicolumn{1}{c}{1}            & 1             \\ 
\texttt{bisect 3d}     & \multicolumn{1}{c}{0.98}        & \multicolumn{1}{c}{1}            & 0.99          & \multicolumn{1}{c}{1}           & \multicolumn{1}{c}{1}            & 1             \\ 
\texttt{bisect 6d}     & \multicolumn{1}{c}{1}           & \multicolumn{1}{c}{0.99}         & 0.99          & \multicolumn{1}{c}{1}           & \multicolumn{1}{c}{1}            & 1             \\ 
\texttt{annthyroid}    & \multicolumn{1}{c}{0.33}        & \multicolumn{1}{c}{0.23}         & 0.22          & \multicolumn{1}{c}{0.57}        & \multicolumn{1}{c}{0.50}         & 0.51          \\ 
\texttt{breast}        & \multicolumn{1}{c}{0.95}        & \multicolumn{1}{c}{0.92}         & 0.90          & \multicolumn{1}{c}{0.99}        & \multicolumn{1}{c}{0.98}         & 0.99          \\
\texttt{cardio}        & \multicolumn{1}{c}{0.58}        & \multicolumn{1}{c}{0.56}         & 0.53          & \multicolumn{1}{c}{0.71}        & \multicolumn{1}{c}{0.74}         & 0.78          \\ 
\texttt{glass}         & \multicolumn{1}{c}{0.10}        & \multicolumn{1}{c}{0.10}         & 0.21          & \multicolumn{1}{c}{0.10}        & \multicolumn{1}{c}{0.08}         & 0.20          \\
\texttt{ionosphere}    & \multicolumn{1}{c}{0.82}        & \multicolumn{1}{c}{0.83}         & 0.84          & \multicolumn{1}{c}{0.88}        & \multicolumn{1}{c}{0.92}         & 0.96          \\ 
\texttt{pendigits}     & \multicolumn{1}{c}{0.27}        & \multicolumn{1}{c}{0.24}         & 0.25          & \multicolumn{1}{c}{0.36}        & \multicolumn{1}{c}{0.30}         & 0.44          \\ 
\texttt{pima}          & \multicolumn{1}{c}{0.51}        & \multicolumn{1}{c}{0.49}         & 0.49          & \multicolumn{1}{c}{0.58}        & \multicolumn{1}{c}{0.55}         & 0.59          \\ 
\texttt{shuttle}       & \multicolumn{1}{c}{0.95}        & \multicolumn{1}{c}{0.86}         & 0.78          & \multicolumn{1}{c}{0.99}        & \multicolumn{1}{c}{0.91}         & 0.92          \\ 
\texttt{wine}          & \multicolumn{1}{c}{0.22}        & \multicolumn{1}{c}{0.22}         & 0.18          & \multicolumn{1}{c}{0.40}        & \multicolumn{1}{c}{0.58}         & 0.78          \\
\texttt{diabetes}      & \multicolumn{1}{c}{0.46}        & \multicolumn{1}{c}{0.44}         & 0.42          & \multicolumn{1}{c}{0.21}        & \multicolumn{1}{c}{0.49}         & 0.58          \\ 
\texttt{moodify}       & \multicolumn{1}{c}{0.34}        & \multicolumn{1}{c}{0.32}         & 0.32          & \multicolumn{1}{c}{0.75}        & \multicolumn{1}{c}{0.67}         & 0.71          \\ \hline
\end{tabular}
\caption{Average Precision for the IF, EIF, \EIFplus models in the complete and inlier training scenarios. The Average Precision are obtained as the average value over 10 executions}
\label{tab:avg-prec-table}
\end{table}
\end{comment}

% ACM VERSION 

\begin{comment}
\begin{table}[ht]
\centering
\caption{Average Precision for the IF, EIF, \EIFplus models in the complete and inlier training scenarios. The Average Precision are obtained as the average value over 10 executions}
\label{tab:avg-prec-table}
\footnotesize
\begin{tabular}{ccccccc}
\toprule
\multicolumn{1}{l}{} & \multicolumn{3}{c}{\textbf{Scenario I}}                                      & \multicolumn{3}{c}{\textbf{Scenario II}}                                        \\ \midrule
\textbf{Dataset}       & \multicolumn{1}{c}{\textbf{IF}} & \multicolumn{1}{c}{\textbf{EIF}} & \textbf{EIF+} & \multicolumn{1}{c}{\textbf{IF}} & \multicolumn{1}{c}{\textbf{EIF}} & \textbf{EIF+} \\ \midrule
\texttt{Xaxis}         & \multicolumn{1}{c}{0.15}        & \multicolumn{1}{c}{0.98}         & 0.98          & \multicolumn{1}{c}{0.11}        & \multicolumn{1}{c}{1}            & 1             \\ 
\texttt{Yaxis}         & \multicolumn{1}{c}{0.11}        & \multicolumn{1}{c}{1}            & 1             & \multicolumn{1}{c}{0.11}        & \multicolumn{1}{c}{1}            & 1             \\ 
\texttt{bisect}        & \multicolumn{1}{c}{0.79}        & \multicolumn{1}{c}{1}            & 0.98          & \multicolumn{1}{c}{1}           & \multicolumn{1}{c}{1}            & 1             \\ 
\texttt{bisect 3d}     & \multicolumn{1}{c}{0.98}        & \multicolumn{1}{c}{1}            & 0.99          & \multicolumn{1}{c}{1}           & \multicolumn{1}{c}{1}            & 1             \\ 
\texttt{bisect 6d}     & \multicolumn{1}{c}{1}           & \multicolumn{1}{c}{0.99}         & 0.99          & \multicolumn{1}{c}{1}           & \multicolumn{1}{c}{1}            & 1             \\ 
\texttt{annthyroid}    & \multicolumn{1}{c}{0.33}        & \multicolumn{1}{c}{0.23}         & 0.22          & \multicolumn{1}{c}{0.57}        & \multicolumn{1}{c}{0.50}         & 0.51          \\ 
\texttt{breast}        & \multicolumn{1}{c}{0.95}        & \multicolumn{1}{c}{0.92}         & 0.90          & \multicolumn{1}{c}{0.99}        & \multicolumn{1}{c}{0.98}         & 0.99          \\
\texttt{cardio}        & \multicolumn{1}{c}{0.58}        & \multicolumn{1}{c}{0.56}         & 0.53          & \multicolumn{1}{c}{0.71}        & \multicolumn{1}{c}{0.74}         & 0.78          \\ 
\texttt{glass}         & \multicolumn{1}{c}{0.10}        & \multicolumn{1}{c}{0.10}         & 0.21          & \multicolumn{1}{c}{0.10}        & \multicolumn{1}{c}{0.08}         & 0.20          \\
\texttt{ionosphere}    & \multicolumn{1}{c}{0.82}        & \multicolumn{1}{c}{0.83}         & 0.84          & \multicolumn{1}{c}{0.88}        & \multicolumn{1}{c}{0.92}         & 0.96          \\ 
\texttt{pendigits}     & \multicolumn{1}{c}{0.27}        & \multicolumn{1}{c}{0.24}         & 0.25          & \multicolumn{1}{c}{0.36}        & \multicolumn{1}{c}{0.30}         & 0.44          \\ 
\texttt{pima}          & \multicolumn{1}{c}{0.51}        & \multicolumn{1}{c}{0.49}         & 0.49          & \multicolumn{1}{c}{0.58}        & \multicolumn{1}{c}{0.55}         & 0.59          \\ 
\texttt{shuttle}       & \multicolumn{1}{c}{0.95}        & \multicolumn{1}{c}{0.86}         & 0.78          & \multicolumn{1}{c}{0.99}        & \multicolumn{1}{c}{0.91}         & 0.92          \\ 
\texttt{wine}          & \multicolumn{1}{c}{0.22}        & \multicolumn{1}{c}{0.22}         & 0.18          & \multicolumn{1}{c}{0.40}        & \multicolumn{1}{c}{0.58}         & 0.78          \\
\texttt{diabetes}      & \multicolumn{1}{c}{0.46}        & \multicolumn{1}{c}{0.44}         & 0.42          & \multicolumn{1}{c}{0.21}        & \multicolumn{1}{c}{0.49}         & 0.58          \\ 
\texttt{moodify}       & \multicolumn{1}{c}{0.34}        & \multicolumn{1}{c}{0.32}         & 0.32          & \multicolumn{1}{c}{0.75}        & \multicolumn{1}{c}{0.67}         & 0.71          \\ \bottomrule
\end{tabular}
\end{table}
\end{comment}



==> tables/table.tex <==
\begin{table*}
\begin{tabularx}{\textwidth}{|l|l|rrrrr|}
\toprule
\textbf{name} & \textbf{algorithm} &      \textbf{full} &       \textbf{75\%} &       \textbf{50\%} &       \textbf{25\%} &  \textbf{one} \\
\midrule
annthyroid & E-diffi &  0.24 &  0.28 &  0.31 &  0.43 &         0.95 \\
       & ACME &  0.24 &  0.21 &  0.21 &  0.23 &         0.00 \\
       & diffi &  0.24 &  0.29 &  0.36 &  0.57 &         0.95 \\
       & var &  0.24 &  0.24 &  0.21 &  0.22 &         0.00 \\
       & random\_forest &  0.24 &  0.29 &  0.32 &  0.43 &         0.95 \\
       & casual &  0.25 &  0.24 &  0.23 &  0.28 &         0.33 \\
       \hline
breastw & E-diffi &  0.86 &  0.87 &  0.86 &  0.89 &         0.71 \\
       & ACME &  0.86 &  0.86 &  0.82 &  0.80 &         0.67 \\
       & diffi &  0.86 &  0.86 &  0.86 &  0.81 &         0.71 \\
       & var &  0.86 &  0.86 &  0.87 &  0.82 &         0.78 \\
       & random\_forest &  0.86 &  0.85 &  0.83 &  0.78 &         0.88 \\
       & casual &  0.86 &  0.86 &  0.84 &  0.78 &         0.74 \\
        \hline
ionosphere & E-diffi &  0.76 &  0.74 &  0.76 &  0.79 &         0.21 \\
       & ACME &  0.75 &  0.74 &  0.73 &  0.70 &         0.26 \\
       & diffi &  0.75 &  0.77 &  0.77 &  0.82 &         1.00 \\
       & var &  0.76 &  0.75 &  0.75 &  0.69 &         0.25 \\
       & random\_forest &  0.76 &  0.77 &  0.79 &  0.79 &         0.29 \\
       & casual &  0.76 &  0.75 &  0.75 &  0.72 &         0.22 \\
        \hline
mammography & E-diffi &  0.26 &  0.28 &  0.24 &  0.10 &         0.16 \\
       & ACME &  0.25 &  0.30 &  0.12 &  0.00 &         0.13 \\
       & diffi &  0.26 &  0.26 &  0.24 &  0.10 &         0.16 \\
       & var &  0.26 &  0.26 &  0.25 &  0.00 &         0.00 \\
       & random\_forest &  0.26 &  0.30 &  0.56 &  0.57 &         0.69 \\
       & casual &  0.26 &  0.28 &  0.26 &  0.15 &         0.22 \\
        \hline
cardio & E-diffi &  0.52 &  0.57 &  0.59 &  0.54 &         0.20 \\
       & ACME &  0.53 &  0.59 &  0.63 &  0.55 &         0.00 \\
       & diffi &  0.53 &  0.51 &  0.59 &  0.68 &          NaN \\
       & var &  0.52 &  0.49 &  0.52 &  0.50 &          NaN \\
       & random\_forest &  0.52 &  0.55 &  0.64 &  0.75 &         0.42 \\
       & casual &  0.52 &  0.55 &  0.51 &  0.41 &          NaN \\
        \hline

pendigits & E-diffi &  0.30 &  0.38 &  0.43 &  0.31 &         0.02 \\
       & ACME &  0.28 &  0.34 &  0.30 &  0.49 &         0.09 \\
       & diffi &  0.33 &  0.38 &  0.31 &  0.27 &         0.38 \\
       & var &  0.31 &  0.13 &  0.16 &  0.31 &         0.05 \\
       & random\_forest &  0.27 &  0.38 &  0.45 &  0.61 &         0.05 \\
       & casual &  0.29 &  0.35 &  0.36 &  0.20 &         0.07 \\
        \hline
pima & E-diffi &  0.52 &  0.52 &  0.49 &  0.47 &         0.48 \\
       & ACME &  0.52 &  0.52 &  0.48 &  0.51 &         0.42 \\
       & diffi &  0.52 &  0.52 &  0.40 &  0.35 &         0.29 \\
       & var &  0.52 &  0.52 &  0.51 &  0.51 &         0.42 \\
       & random\_forest &  0.52 &  0.47 &  0.48 &  0.48 &         0.48 \\
       & casual &  0.52 &  0.45 &  0.46 &  0.43 &         0.48 \\
        \hline
wine & E-diffi &  0.61 &  0.62 &  0.78 &  0.79 &         0.83 \\
       & ACME &  0.61 &  0.60 &  0.62 &  0.60 &         0.83 \\
       & diffi &  0.60 &  0.60 &  0.63 &  0.00 &         0.00 \\
       & var &  0.60 &  0.60 &  0.60 &  0.60 &         0.82 \\
       & random\_forest &  0.60 &  0.60 &  0.61 &  0.79 &         0.80 \\
       & casual &  0.60 &  0.54 &  0.20 &  0.19 &         0.00 \\
        \hline
shuttle & E-diffi &  0.85 &  0.88 &  0.81 &  0.82 &         0.50 \\
       & ACME &  0.85 &  0.86 &  0.91 &  0.86 &         0.50 \\
       & diffi &  0.86 &  0.85 &  0.84 &  0.71 &         0.33 \\
       & var &  0.86 &  0.86 &  0.84 &  0.78 &         0.44 \\
       & random\_forest &  0.85 &  0.92 &  0.91 &  0.89 &         0.75 \\
       & casual &  0.86 &  0.86 &  0.84 &  0.70 &         0.59 \\
\bottomrule
\end{tabularx}
\caption{Set of data used in the experimental phase. The first column gives the name of the dataset; the second column describes the number of instances contained in each set; the third column defines the total amount of features; the fourth column gives the number of outliers; the last column presents the contamination rates. }
\label{tab:featsel}
\end{table*}
